Nitrogen-containing Anions and Tholin Growth in Titan's Ionosphere: Implications for Cassini CAPS-ELS Observations

The Cassini Plasma Spectrometer (CAPS) Electron Spectrometer (ELS) instrument onboard Cassini revealed an unexpected abundance of negative ions above 950 km in Titan's ionosphere. \textit{In situ} measurements indicated the presence of negatively charged particles with mass-over-charge ratios up to 13,800 \textit{u/q}. At present, only a handful of anions have been characterized by photochemical models, consisting mainly of C$_n$H$^-$ carbon chain and C$_{n-1}$N$^-$ cyano compounds ($n=2-6$); their formation occurring essentially through proton abstraction from their parent neutral molecules. However, numerous other species have yet to be detected and identified. Considering the efficient anion growth leading to compounds of thousands of \textit{u/q}, it is necessary to better characterize the first light species. Here, we present new negative ion measurements with masses up to 200 \textit{u/q} obtained in an \ce{N2}:\ce{CH4} dusty plasma discharge reproducing analogous conditions to Titan's ionosphere. We perform a comparison with high altitude CAPS-ELS measurements near the top of Titan's ionosphere from the T18 encounter. The main observed peaks are in agreement with the observations. However, a number of other species (\textit{e.g.} \ce{CNN-}, \ce{CHNN-}) previously not considered suggests an abundance of N-bearing compounds, containing two or three nitrogen atoms, consistent with certain adjacent doubly-bonded nitrogen atoms found in tholins. These results suggest that an N-rich incorporation into tholins may follow mechanisms including anion chemistry, further highlighting the important role of negative ions in Titan's aerosol growth.

==> Oct_2018 <==
@article{Alcaraz2004,
    title = {{15N+ + CD4 and O+ + 13CO2 State-Selected Ion-Molecule Reactions Relevant to the Chemistry of Planetary Ionospheres}},
    year = {2004},
    journal = {J. Phys. Chem. A},
    author = {Alcaraz, C. and Nicolas, C. and Thissen, R. and Zabka, J. and Dutuit, O.},
    pages = {9998},
    volume = {108},
    doi = {10.1021/jp0477755},
    issn = {10895639}
}

@article{Dobrijevic2016,
    title = {{1D-coupled photochemical model of neutrals, cations and anions in the atmosphere of Titan}},
    year = {2016},
    journal = {Icarus},
    author = {Dobrijevic, M. and Loison, J. C. and Hickson, K. M. and Gronoff, G.},
    pages = {313--339},
    volume = {268},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.12.045},
    doi = {10.1016/j.icarus.2015.12.045},
    issn = {10902643},
    keywords = {Atmospheres, chemistry, Atmospheres, composition, Ionospheres, Photochemistry, Titan}
}

@article{Lavvasetal2013,
    title = {{2013 Aerosol Growth Supporting Information}},
    year = {2013},
    author = {{Lavvas et al}},
    pages = {1--7},
    doi = {10.1073/pnas.0913556107}
}

@article{Salge2010,
    title = {{41st Lunar and Planetary Science Conference (2010) 1751.pdf}},
    year = {2010},
    author = {Salge, T and Nelson, M J and Spilde, M N and Sciences, Planetary},
    pages = {2--3},
    isbn = {2431244571},
    doi = {10.1016/geomorph.2007.04.017.}
}

@article{Salge2010a,
    title = {{41st Lunar and Planetary Science Conference (2010) 1751.pdf}},
    year = {2010},
    author = {Salge, T and Nelson, M J and Spilde, M N and Sciences, Planetary},
    pages = {2--3},
    isbn = {2431244571},
    doi = {10.1016/geomorph.2007.04.017.}
}

@article{Bagenal2012,
    title = {{43rd Lunar and Planetary Science Conference (2012) 1714.pdf}},
    year = {2012},
    journal = {Applied Physics},
    author = {Bagenal, F and Bills, B G and Blaney, D L and Blankenship, D D and Brinckerhoff, W and Connerney, J E P and Hand, K and Hoehler, T and Kurth, W and Mcgrath, M and Mellon, M and Moore, J M and Prockter, L M and Senske, D A and Shock, E and Smith, D E and Gavin, T and Garner, G and Magner, T and Cooke, B C and Crum, R and Mallder, V and Adams, L and Klaasen, K and Patterson, G W and Vance, S D and City, Iowa}
}

@article{Klaus2013,
    title = {{44th Lunar and Planetary Science Conference}},
    year = {2013},
    journal = {44th Lunar and Planetary Science Conference},
    author = {Klaus, K and Lsperman, M S and Rogers, F},
    pages = {2013--1486},
    isbn = {2037720386},
    doi = {10.1029/2005JE002544.},
    arxivId = {arXiv:1209.47682012}
}

@article{Mahaffy2014,
    title = {{45th Lunar and Planetary Science Conference ( 2014 ) and Planetary Science Conference}},
    year = {2014},
    author = {Mahaffy, P R and Atreya, S and Pavlov, a a and Trainer, M and Wong, M and Science, Exploration and Arbor, Ann},
    pages = {4--5},
    volume = {20723},
    isbn = {1129645568},
    doi = {10.1002/jgre.20118.},
    arxivId = {arXiv:1307.0515}
}

@article{Singh2015a,
    title = {{46th Lunar and Planetary Science Conference ( 2015 ) 46th Lunar and Planetary Science Conference ( 2015 )}},
    year = {2015},
    author = {Singh, Sandeep and Rodriguez, S and Cornet, T and Chevrier, V F and Maltagliati, L and Sci-, Planetary},
    pages = {4--5},
    volume = {72701}
}

@article{Asphaug2016c,
    title = {{47th Lunar and Planetary Science Conference ( 2016 ) 47th Lunar and Planetary Science Conference ( 2016 )}},
    year = {2016},
    author = {Asphaug, E and Spitale, J N and Hemingway, D and Rhoden, A R and Henning, W G and Bills, B G and Kattenhorn, S A and Walker, M and Exploration, Space and Sci-, Planetary and Cruz, Santa and Sciences, Planetary and Cruz, Santa and Hopkins, Johns and Physics, Applied and Com-, Conoco Phillips and Technology, Geological and Angeles, Los and Sciences, Space and Angeles, Los and Stress, Tidal},
    pages = {9--10},
    isbn = {1189985144},
    doi = {10.1016/j.icarus.2007.12.027.}
}

@article{Singh2016,
    title = {{47th Lunar and Planetary Science Conference ( 2016 ) 47th Lunar and Planetary Science Conference ( 2016 )}},
    year = {2016},
    author = {Singh, Sandeep and Rodriguez, S and Cornet, T and Clark, R N and Maltaglia, L and Chevrier, V F and Science, Planetary},
    pages = {6--7},
    volume = {98862}
}

@article{Marchi2004a,
    title = {{A 0.4-2.5 ??m spectroscopic investigation of Triton's two faces}},
    year = {2004},
    journal = {Icarus},
    author = {Marchi, S. and Barbieri, C. and Lazzarin, M. and Owen, T. C. and Corsini, E. M.},
    number = {2},
    pages = {367--373},
    volume = {168},
    doi = {10.1016/j.icarus.2003.12.015},
    issn = {00191035},
    keywords = {Infrared observations, Satellites, Spectroscopy, Surfaces, Triton}
}

@article{Bertaux1972,
    title = {{A calculated hydrogen distribution in the exosphere}},
    year = {1972},
    author = {Vidal-Madjar, A and Bertaux, J L},
    pages = {1147--1162},
    volume = {20}
}

@article{Angelo2017,
    title = {{A Case for an Atmosphere on Super-Earth 55 Cancri e}},
    year = {2017},
    journal = {The Astronomical Journal},
    author = {Angelo, Isabel and Hu, Renyu},
    number = {6},
    pages = {232},
    volume = {154},
    publisher = {IOP Publishing},
    url = {http://arxiv.org/abs/1710.03342},
    doi = {10.3847/1538-3881/aa9278},
    issn = {1538-3881},
    arxivId = {1710.03342},
    keywords = {55 cnc e, atmospheres, individual, occultations, occultations,planets and satellites: atmospheres,p, photometric, planets and satellites, techniques, terrestrial planets}
}

@article{Iyer2016,
    title = {{A CHARACTERISTIC TRANSMISSION SPECTRUM DOMINATED BY H <sub>2</sub> O APPLIES TO THE MAJORITY OF <i>HST</i> /WFC3 EXOPLANET OBSERVATIONS}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Iyer, Aishwarya R. and Swain, Mark R. and Zellem, Robert T. and Line, Michael R. and Roudier, Gael and Rocha, Graça and Livingston, John H.},
    number = {2},
    pages = {109},
    volume = {823},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/823/i=2/a=109?key=crossref.0ac7056c7182912902a28d39ed2ae6e3},
    doi = {10.3847/0004-637X/823/2/109},
    issn = {1538-4357},
    keywords = {atmospheres, data analysis, general, methods, methods: data analysis, planets and satellites, planets and satellites: atmospheres, planets and satellites: general, radiative transfer}
}

@article{Maynard-Casely2016,
    title = {{A co-crystal between benzene and ethane: A potential evaporite material for Saturn's moon Titan}},
    year = {2016},
    journal = {IUCrJ},
    author = {Maynard-Casely, Helen E. and Hodyss, Robert and Cable, Morgan L. and Vu, Tuan Hoang and Rahm, Martin},
    pages = {192--199},
    volume = {3},
    doi = {10.1107/S2052252516002815},
    issn = {20522525},
    keywords = {Titan, co-crystals, evaporite, molecular crystallography, synchrotron powder diffraction}
}

@article{Achilleos2014,
    title = {{A combined model of pressure variations in Titan's plasma environment}},
    year = {2014},
    journal = {Geophysical Research Letters},
    author = {Achilleos, N. and Arridge, C. S. and Bertucci, C. and Guio, P. and Romanelli, N. and Sergis, N.},
    number = {24},
    pages = {8730--8735},
    volume = {41},
    doi = {10.1002/2014GL061747},
    issn = {19448007},
    keywords = {Saturn, Titan, magnetosphere, plasma sheet}
}

@article{Barr2014,
    title = {{A Common Origin for Ridge-and-Trough Terrain on Icy Satellites by Sluggish Lid Convection}},
    year = {2014},
    author = {Barr, Amy C. and Hammond, Noah P.},
    url = {http://arxiv.org/abs/1405.6708 http://dx.doi.org/10.1016/j.pepi.2015.09.009},
    doi = {10.1016/j.pepi.2015.09.009},
    arxivId = {1405.6708}
}

@article{Porco2017,
    title = {{A Community Grows around the Geysering World of Enceladus}},
    year = {2017},
    journal = {Astrobiology},
    author = {Porco, Carolyn C.},
    number = {9},
    pages = {ast.2017.1711},
    volume = {17},
    url = {http://online.liebertpub.com/doi/10.1089/ast.2017.1711},
    doi = {10.1089/ast.2017.1711},
    issn = {1531-1074},
    keywords = {astrobiology 17, enceladus, enceladus focus group, ocean world, search for biosignatures}
}

@article{He2014a,
    title = {{A comprehensive NMR structural study of Titan aerosol analogs: Implications for Titan's atmospheric chemistry}},
    year = {2014},
    journal = {Icarus},
    author = {He, Chao and Smith, Mark A.},
    pages = {31--38},
    volume = {243},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.09.021},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.09.021},
    issn = {10902643},
    keywords = {Organic chemistry, Prebiotic chemistry, Titan, atmosphere}
}

@article{Rannou2004,
    title = {{A coupled dynamics-microphysics model of Titan's atmosphere}},
    year = {2004},
    journal = {Icarus},
    author = {Rannou, P. and Hourdin, F. and McKay, C. P. and Luz, D.},
    number = {2},
    pages = {443--462},
    volume = {170},
    doi = {10.1016/j.icarus.2004.03.007},
    issn = {00191035},
    keywords = {Dynamics, Haze, Photometry, Titan}
}

@article{Zhang2009,
    title = {{A crossed beams and ab initio investigation on the formation of cyanodiacetylene in the reaction of cyano radicals with diacetylene}},
    year = {2009},
    journal = {Journal of Chemical Physics},
    author = {Zhang, Fangtong and Kim, Seol and Kaiser, Ralf I. and Jamal, Adeel and Mebel, Alexander M.},
    number = {23},
    pages = {1--9},
    volume = {130},
    isbn = {doi:10.1063/1.3152714},
    doi = {10.1063/1.3152714},
    issn = {00219606},
    pmid = {19548728}
}

@article{Singh2017a,
    title = {{A Demonstration of a Versatile Low-order Wavefront Sensor Tested on Multiple Coronographs}},
    year = {2017},
    journal = {Publications of the Astronomical Society of the Pacific},
    author = {Singh, Garima and Lozi, Julien and Jovanovic, Nemanja and Guyon, Olivier and Baudoz, Pierre and Martinache, Frantz and Kudo, Tomoyuki},
    number = {979},
    pages = {095002},
    volume = {129},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/1538-3873/129/i=979/a=095002?key=crossref.ee2b12fd2965dc688fb01e81483a87d0},
    doi = {10.1088/1538-3873/aa76c1},
    issn = {0004-6280},
    keywords = {instrumentation: adaptive optics}
}

@article{Carvalho2009,
    title = {{A fast Bayesian approach to discrete object detection in astronomical data sets - PowellSnakes i}},
    year = {2009},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Carvalho, Pedro and Rocha, Graça and Hobson, M. P.},
    number = {3},
    pages = {681--702},
    volume = {393},
    doi = {10.1111/j.1365-2966.2008.14016.x},
    issn = {00358711},
    arxivId = {astro-ph/0204457},
    keywords = {Cosmic microwave background, Cosmology: observations, Methods: data analysis}
}

@article{Xing2016,
    title = {{A Feathered Dinosaur Tail with Primitive Plumage Trapped in Mid-Cretaceous Amber}},
    year = {2016},
    journal = {Current Biology Gang Li Ming Bai},
    author = {Xing, Lida and Mckellar, Ryan C and Xu, Xing and Tseng, Kuowei and Ran, Hao and Currie, Philip J and Benton, Michael J and Zhang, Jianping and Wolfe, Alexander P and Yi, Qiru},
    number = {8},
    pages = {1--913},
    volume = {2641314},
    publisher = {Elsevier Ltd.},
    url = {http://dx.doi.org/10.1016/j.cub.2016.10.008},
    doi = {10.1016/j.cub.2016.10.008},
    issn = {09609822},
    keywords = {Burmese amber, Cenomanian, Coelurosauria, feather evolution}
}

@article{Richards1981,
    title = {{A formula for calculating theoretical photoelectron fluxes resulting from the He + 304 {\AA} solar spectral line}},
    year = {1981},
    journal = {Geophysical Research Letters},
    author = {Richards, P. G. and Torr, D. G.},
    number = {9},
    month = {9},
    pages = {995--998},
    volume = {8},
    url = {http://doi.wiley.com/10.1029/GL008i009p00995},
    doi = {10.1029/GL008i009p00995},
    issn = {00948276}
}

@article{Patterson2007,
    title = {{A global geologic map of Ganymede}},
    year = {2007},
    journal = {Lunar and Planetary Science XXXVIII},
    author = {Patterson, G Wesley and Head, James W and Collins, Geoffrey C and Pappalardo, Robert T and Prockter, Louise M and Lucchitta, Baerbel K},
    pages = {abstract no. 1098},
    volume = {02912}
}

@article{Lorenz2013,
    title = {{A global topographic map of Titan}},
    year = {2013},
    journal = {Icarus},
    author = {Lorenz, Ralph D. and Stiles, Bryan W. and Aharonson, Oded and Lucas, Antoine and Hayes, Alexander G. and Kirk, Randolph L. and Zebker, Howard A. and Turtle, Elizabeth P. and Neish, Catherine D. and Stofan, Ellen R. and Barnes, Jason W.},
    number = {1},
    pages = {367--377},
    volume = {225},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.04.002},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2013.04.002},
    issn = {00191035},
    keywords = {Geological processes, Titan}
}

@article{Wiktorowicz2015,
    title = {{A GROUND-BASED ALBEDO UPPER LIMIT FOR HD 189733b FROM POLARIMETRY}},
    year = {2015},
    journal = {The Astrophysical Journal},
    author = {Wiktorowicz, Sloane J. and Nofi, Larissa A. and Jontof-Hutter, Daniel and Kopparla, Pushkar and Laughlin, Gregory P. and Hermis, Ninos and Yung, Yuk L. and Swain, Mark R.},
    number = {1},
    pages = {48},
    volume = {813},
    url = {http://arxiv.org/abs/1507.03588},
    doi = {10.1088/0004-637X/813/1/48},
    issn = {1538-4357},
    arxivId = {1507.03588},
    keywords = {atmospheres, dust, extinction, hd 189733b, individual, planetary systems, planets and satellites, polarimetric, polarization, techniques}
}

@article{Swain2010,
    title = {{A ground-based near-infrared emission spectrum of the exoplanet HD 189733b.}},
    year = {2010},
    journal = {Nature},
    author = {Swain, Mark R and Deroo, Pieter and Griffith, Caitlin a and Tinetti, Giovanna and Thatte, Azam and Vasisht, Gautam and Chen, Pin and Bouwman, Jeroen and Crossfield, Ian J. M. and Angerhausen, Daniel and Afonso, Cristina and Henning, Thomas},
    number = {1},
    pages = {637--639},
    volume = {463},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/nature08775},
    isbn = {0028-0836},
    doi = {10.1038/nature08775},
    issn = {0028-0836},
    pmid = {20130645},
    arxivId = {1002.2453}
}

@article{Harris2008,
    title = {{A H13CN/HN13C linelist, model atmospheres and synthetic spectra for carbon stars}},
    year = {2008},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Harris, G. J. and Larner, F. C. and Tennyson, J. and Kaminsky, B. M. and Pavlenko, Ya V. and Jones, H. R A},
    number = {1},
    pages = {143--148},
    volume = {390},
    doi = {10.1111/j.1365-2966.2008.13642.x},
    issn = {00358711},
    arxivId = {0807.0717},
    keywords = {Infrared: stars, Molecular data, Stars: AGB and post-AGB, Stars: atmospheres, Stars: carbon}
}

@article{Hui2015,
    title = {{A Hausdorff Distance Based Image Registration Algorithm}},
    year = {2015},
    author = {Hui, Liu and Zhichun, Zhang and Dong, Wei},
    number = {1},
    pages = {125--134},
    volume = {8},
    keywords = {hausdorff distance, image features, image registration}
}

@article{Kollmann2017,
    title = {{A Heavy Ion and Proton Radiation Belt Inside of Jupiter's Rings}},
    year = {2017},
    journal = {Geophysical Research Letters},
    author = {Kollmann, P. and Paranicas, C. and Clark, G. and Mauk, B. H. and Haggerty, D. K. and Rymer, A. M. and Santos-Costa, D. and Connerney, J. E. P. and Allegrini, F. and Valek, P. and Kurth, W. S. and Gladstone, G. R. and Levin, S. and Bolton, S.},
    url = {http://doi.wiley.com/10.1002/2017GL073730},
    doi = {10.1002/2017GL073730},
    issn = {00948276}
}

@article{Preusse2006,
    title = {{A magnetic communication scenario for hot Jupiters}},
    year = {2006},
    journal = {Astronomy and Astrophysics},
    author = {Preusse, S and Kopp, A and Motschmann, U},
    pages = {317--322},
    volume = {460},
    doi = {10.1051/0004-6361},
    issn = {00046361},
    keywords = {activity, general, magnetic fields, outflows, planets and satellites, stars, winds}
}

@book{Turabian1996,
    title = {{A manual for writers of term papers, theses, and dissertations}},
    year = {1996},
    booktitle = {Journal of the American Statistical Association},
    author = {Turabian, Kate L},
    number = {277},
    pages = {108},
    volume = {52},
    url = {http://www.jstor.org/stable/2281411?origin=crossref},
    isbn = {0226816273},
    doi = {10.2307/2281411},
    issn = {01621459},
    pmid = {1813},
    arxivId = {arXiv:1011.1669v3}
}

@article{Knutson2007,
    title = {{A map of the day-night contrast of the extrasolar planet HD 189733b.}},
    year = {2007},
    journal = {Nature},
    author = {Knutson, Heather a and Charbonneau, David and Allen, Lori E and Fortney, Jonathan J and Agol, Eric and Cowan, Nicolas B and Showman, Adam P and Cooper, Curtis S and Megeath, S Thomas},
    number = {7141},
    pages = {183--186},
    volume = {447},
    isbn = {1476-4687 (Electronic){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/nature05782},
    issn = {0028-0836},
    pmid = {17495920},
    arxivId = {0705.0993}
}

@article{Tigrine2016,
    title = {{A microwave plasma source for VUV atmospheric photochemistry}},
    year = {2016},
    journal = {Journal of Physics D: Applied Physics},
    author = {Tigrine, S and Carrasco, N and Vettier, L and Cernogora, G},
    number = {39},
    pages = {395202},
    volume = {49},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0022-3727/49/i=39/a=395202?key=crossref.c271bf76ea98ba3609296eb0d3cdb355},
    doi = {10.1088/0022-3727/49/39/395202},
    issn = {0022-3727}
}

@article{Corby,
    title = {{A Microwave View of Nitriles in Sagittarius B2 ( N ) Nitriles The most diverse family known in the ISM}},
    author = {Corby, Joanna and Steber, Amanda and Seifert, Nathan and Niell, Justin and Remijan, Anthony},
    volume = {2}
}

@article{Mukundan2018,
    title = {{A Model for Negative Ion Chemistry in Titan’s Ionosphere}},
    year = {2018},
    journal = {The Astrophysical Journal},
    author = {Mukundan, Vrinda and Bhardwaj, Anil},
    number = {2},
    pages = {168},
    volume = {856},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/856/i=2/a=168?key=crossref.b14d1b74b2ca76356a92ed40f24250fa},
    doi = {10.3847/1538-4357/aab1f5},
    issn = {1538-4357},
    keywords = {astrochemistry, atmospheres, individual, planets and sa, planets and satellites, planets and satellites: atmospheres, titan}
}

@article{Luhmann2006,
    title = {{A model of the ionosphere of Saturn's rings and its implications}},
    year = {2006},
    journal = {Icarus},
    author = {Luhmann, J. G. and Johnson, R. E. and Tokar, R. L. and Ledvina, S. A. and Cravens, T. E.},
    number = {2},
    pages = {465--474},
    volume = {181},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2005.11.022},
    issn = {00191035},
    keywords = {Atmospheres, dynamics, Ices, Planetary rings, Saturn, Saturn, magnetosphere}
}

@article{Keller1992,
    title = {{A model of the ionosphere of Titan}},
    year = {1992},
    journal = {Journal of Geophysical Research, [Space Physics]},
    author = {Keller, C N and Cravens, T E and Gan, L},
    number = {A8},
    pages = {12117--12135},
    volume = {97},
    keywords = {Planets (Saturn, Titan satellite, http://dx.doi.org/10.1029/92JA00231, doi:10.1029/9, ionosphere of, photochem. model of) planet Saturn Titan satellit}
}

@article{Tomasko2008,
    title = {{A model of Titan's aerosols based on measurements made inside the atmosphere}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Tomasko, M. G. and Doose, L. and Engel, S. and Dafoe, L. E. and West, R. and Lemmon, M. and Karkoschka, E. and See, C.},
    number = {5},
    pages = {669--707},
    volume = {56},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2007.11.019},
    issn = {00320633},
    keywords = {Aerosols, Atmosphere, Huygens, Titan}
}

@article{Tomasko2008b,
    title = {{A model of Titan's aerosols based on measurements made inside the atmosphere}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Tomasko, M. G. and Doose, L. and Engel, S. and Dafoe, L. E. and West, R. and Lemmon, M. and Karkoschka, E. and See, C.},
    number = {5},
    pages = {669--707},
    volume = {56},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2007.11.019},
    issn = {00320633},
    keywords = {Aerosols, Atmosphere, Huygens, Titan}
}

@article{Raymond2018,
    title = {{A Model of Titan-like Chemistry to Connect Experiments and <i>Cassini</i> Observations}},
    year = {2018},
    journal = {The Astrophysical Journal},
    author = {Raymond, Alexander W. and Sciamma-O’Brien, Ella and Salama, Farid and Mazur, Eric},
    number = {2},
    pages = {107},
    volume = {853},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/853/i=2/a=107?key=crossref.609aec5c635c4779ec04096821209f92},
    doi = {10.3847/1538-4357/aaa12c},
    issn = {1538-4357},
    keywords = {astrochemistry, astrochemistry,methods: laboratory: molecular,mole, atmospheres, individual, laboratory, methods, molecular, molecular processes, planets and satellites, plasmas, titan}
}

@article{Osamura1999,
    title = {{A Molecular Orbital Study of the HC3NH+ + e- Dissociative Recombination and its Role in the Production of Cyanoacetylene Isomers in Interstellar Clouds}},
    year = {1999},
    journal = {The Astrophysical Journal},
    author = {Osamura, Yoshihiro and Fukuzawa, Kaori and Terzieva, R. and Herbst, Eric},
    number = {3},
    pages = {697--704},
    volume = {519},
    issn = {15384357}
}

@article{Kopparla2015,
    title = {{A Multiple Scattering Polarized Radiative Transfer Model: Application to HD 189733b}},
    year = {2015},
    journal = {The Astrophysical Journal},
    author = {Kopparla, Pushkar and Natraj, Vijay and Zhang, Xi and Swain, Mark R. and Wiktorowicz, Sloane J. and Yung, Yuk L.},
    number = {1},
    pages = {32},
    volume = {817},
    url = {http://arxiv.org/abs/1512.02308%5Cnhttp://dx.doi.org/10.3847/0004-637X/817/1/32%5Cnhttp://stacks.iop.org/0004-637X/817/i=1/a=32?key=crossref.c5dba1a403076218d54c58408ab4b332},
    doi = {10.3847/0004-637X/817/1/32},
    issn = {1538-4357},
    arxivId = {1512.02308},
    keywords = {2015, ft version december 9}
}

@article{Levi,
    title = {{A New Desalination Pump Help Define the pH of Ocean Worlds}},
    author = {Levi, A and Sasselov, D},
    url = {https://arxiv.org/pdf/1803.08937.pdf},
    arxivId = {1803.08937}
}

@article{Fallis2013a,
    title = {{A New Enceladus Base map and Global Control Network in Support of Geologic Mapping}},
    year = {2013},
    journal = {LPCS},
    author = {Fallis, A.G},
    number = {9},
    pages = {1689--1699},
    volume = {53},
    isbn = {9788578110796},
    doi = {10.1017/CBO9781107415324.004},
    issn = {1098-6596},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {icle}
}

@article{Morello2014,
    title = {{A NEW LOOK AT <i>SPITZER</i> PRIMARY TRANSIT OBSERVATIONS OF THE EXOPLANET HD 189733b}},
    year = {2014},
    journal = {The Astrophysical Journal},
    author = {Morello, G. and Waldmann, I. P. and Tinetti, G. and Peres, G. and Micela, G. and Howarth, I. D.},
    number = {1},
    pages = {22},
    volume = {786},
    url = {http://stacks.iop.org/0004-637X/786/i=1/a=22?key=crossref.1097575620c6e072ce1f033b51e22f18},
    doi = {10.1088/0004-637X/786/1/22},
    issn = {0004-637X},
    keywords = {atmospheres, color figures, data analysis, hd 189733b, individual, methods, online-only material, photometric, planets and satellites, techniques}
}

@article{Grundy1991,
    title = {{A new spectrum of Triton near the time of the Voyager encounter}},
    year = {1991},
    journal = {Icarus},
    author = {Grundy, William M. and Fink, Uwe},
    number = {2},
    pages = {379--385},
    volume = {93},
    doi = {10.1016/0019-1035(91)90220-N},
    issn = {10902643}
}

@article{Coates2015,
    title = {{A new upper limit to the field-aligned potential near Titan}},
    year = {2015},
    journal = {Geophysical Research Letters},
    author = {Coates, Andrew J. and Wellbrock, Anne and Waite, J. Hunter and Jones, Geraint H.},
    number = {12},
    pages = {4676--4684},
    volume = {42},
    isbn = {0094-8276},
    doi = {10.1002/2015GL064474},
    issn = {19448007},
    keywords = {Titan, ambipolar field, escape, ionosphere}
}

@article{Judge2017,
    title = {{A novel strategy to seek bio-signatures at Enceladus and Europa}},
    year = {2017},
    journal = {Astrobiology},
    author = {Judge, Philip},
    number = {9},
    pages = {852--862},
    volume = {17},
    url = {http://arxiv.org/abs/1707.07230},
    doi = {10.1089/ast.2017.1667},
    issn = {1531-1074},
    arxivId = {1707.07230}
}

@article{Hu2017,
    title = {{A numerical method for reorientation of rotating tidally deformed viscoelastic bodies}},
    year = {2017},
    journal = {Journal of Geophysical Research: Planets},
    author = {Hu, H. and van der Wal, W. and Vermeersen, L. L.A.},
    number = {1},
    pages = {228--248},
    volume = {122},
    doi = {10.1002/2016JE005114},
    issn = {21699100},
    keywords = {Linear true polar wander theory, Quasi-fluid approximation, Tidally deformed, True polar wander}
}

@article{Krasnopolsky2009,
    title = {{A photochemical model of Titan's atmosphere and ionosphere}},
    year = {2009},
    journal = {Icarus},
    author = {Krasnopolsky, Vladimir A.},
    number = {1},
    month = {5},
    pages = {226--256},
    volume = {201},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103509000062},
    doi = {10.1016/j.icarus.2008.12.038},
    issn = {00191035},
    keywords = {Atmospheres, Ionospheres, Photochemistry, Titan, chemistry, composition}
}

@article{Toon1992,
    title = {{A Physical Model of Titan's Aerosols}},
    year = {1992},
    author = {Toon, O B and Mckay, C P},
    pages = {24--53},
    volume = {53}
}

@article{Domenico,
    title = {{A portrait of Christiaan Huygens Who recognizes this picture ?}},
    author = {Domenico, Giovanni}
}

@article{Madhusudhan2012,
    title = {{A POSSIBLE CARBON-RICH INTERIOR IN SUPER-EARTH 55 Cancri e}},
    year = {2012},
    author = {Madhusudhan, Nikku and Lee, Kanani K M and Mousis, Olivier},
    volume = {40},
    doi = {10.1088/2041-8205/759/2/L40},
    issn = {2041-8205},
    arxivId = {arXiv:1210.2720v1},
    keywords = {2011a, 55 cancri e, 55 cancri e may, and radius of, be explained by a, carbon-rich interior, general, if the observed mass, in the, individual, madhusudhan 2012, motivated by these studies, planetary systems, planets and satellites, present work we investigate}
}

@article{Huang2008,
    title = {{A procedure for computing accurate ab initio quartic force fields: Application to HO 2+ and H2 O}},
    year = {2008},
    journal = {Journal of Chemical Physics},
    author = {Huang, Xinchuan and Lee, Timothy J.},
    number = {4},
    pages = {1--14},
    volume = {129},
    doi = {10.1063/1.2957488},
    issn = {00219606}
}

@article{Miller1953,
    title = {{A Production of Amino Acids under Possible Primitive Earth Conditions}},
    year = {1953},
    author = {Miller, Stanley L.},
    number = {3046},
    pages = {528--529},
    volume = {117}
}

@article{Kerber2012,
    title = {{A progression of induration in Medusae Fossae Formation transverse aeolian ridges: Evidence for ancient aeolian bedforms and extensive reworking}},
    year = {2012},
    journal = {Earth Surface Processes and Landforms},
    author = {Kerber, Laura and Head, James W.},
    number = {4},
    pages = {422--433},
    volume = {37},
    isbn = {0197-9337},
    doi = {10.1002/esp.2259},
    issn = {01979337},
    keywords = {Aeolian, Ancient, Mars, Medusae Fossae Formation, Transverse aeolian ridge}
}

@article{Agundez2014,
    title = {{A pseudo 2D chemical model of hot Jupiter atmospheres: application to HD 209458b and HD 189733b}},
    year = {2014},
    journal = {arXiv preprint arXiv: {\ldots}},
    author = {Ag{\'{u}}ndez, Marcelino and Parmentier, Vivien and Venot, Olivia},
    pages = {1--22},
    volume = {564},
    url = {http://www.aanda.org/10.1051/0004-6361/201322895%5Cnhttp://arxiv.org/abs/1403.0121},
    doi = {10.1051/0004-6361/201322895},
    issn = {0004-6361},
    arxivId = {arXiv:1403.0121v2},
    keywords = {atmospheres, composition, hd 189733b, hd 209458b, individual, planets and satellites}
}

@article{Schworer2017,
    title = {{A Resolved and Asymmetric Ring of PAHs within the Young Circumstellar Disk of IRS 48}},
    year = {2017},
    journal = {The Astrophysical Journal},
    author = {Schworer, Guillaume and Lacour, Sylvestre and Hu?lamo, Nuria and Pinte, Christophe and Chauvin, Ga?l and du Foresto, Vincent Coud? and Ehrenreich, David and Girard, Julien and Tuthill, Peter},
    number = {2},
    pages = {77},
    volume = {842},
    url = {http://stacks.iop.org/0004-637X/842/i=2/a=77?key=crossref.06e2559028209cc032ceb6136de44c6a},
    doi = {10.3847/1538-4357/aa74b7},
    issn = {1538-4357},
    arxivId = {1706.06678},
    keywords = {planetary systems, protoplanetary disks, radiative transfer, stars: individual: IRS-48, stars: pre-main sequence}
}

@article{Marshall2005,
    title = {{A revised model for cycloid growth mechanics on Europa: Evidence from surface morphologies and geometries}},
    year = {2005},
    journal = {Icarus},
    author = {Marshall, Scott T. and Kattenhorn, Simon A.},
    number = {2},
    pages = {341--366},
    volume = {177},
    isbn = {0527286400},
    doi = {10.1016/j.icarus.2005.02.022},
    issn = {00191035},
    keywords = {Europa, Geological processes, Surfaces, Satellite}
}

@article{Tang2017,
    title = {{A revolution is brewing : observations of TRAPPIST-1 exoplanetary system fosters a new biomarker}},
    year = {2017},
    journal = {Arxiv},
    author = {Tang, B R and Habeertable, Z and Chou, M C and Exquisit, B},
    number = {October 1814},
    arxivId = {arXiv:submit/1849202},
    archivePrefix = {arXiv},
    eprint = {1849202},
    primaryClass = {submit}
}

@article{Hemingway2013,
    title = {{A rigid and weathered ice shell on Titan.}},
    year = {2013},
    journal = {Nature},
    author = {Hemingway, D and Nimmo, F and Zebker, H and Iess, L},
    number = {7464},
    pages = {550--2},
    volume = {500},
    publisher = {Nature Publishing Group},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/23985871},
    isbn = {0028-0836},
    doi = {10.1038/nature12400},
    issn = {1476-4687},
    pmid = {23985871}
}

@article{Caudal1986,
    title = {{A Self-Consistent Model of Jupiter's Magnetodic Including The Effects of Centrifugal Force and Pressure}},
    year = {1986},
    journal = {Journal of Geophysical Research},
    author = {Caudal, G.},
    number = {5},
    pages = {4201--4221},
    volume = {91}
}

@article{Prockter2005,
    title = {{A shear heating origin for ridges on Triton}},
    year = {2005},
    journal = {Geophysical Research Letters},
    author = {Prockter, Louise M. and Nimmo, Francis and Pappalardo, Roberto T.},
    number = {14},
    pages = {1--4},
    volume = {32},
    doi = {10.1029/2005GL022832},
    issn = {00948276},
    keywords = {http://dx.doi.org/10.1029/2005GL022832, doi:10.102}
}

@article{Cowley2005,
    title = {{A simple axisymmetric model of magnetosphere-ionosphere coupling currents in Jupiter's polar ionosphere}},
    year = {2005},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Cowley, S. W H and Alexeev, I. I. and Belenkaya, E. S. and Bunce, E. J. and Cottis, C. E. and Kalegaev, V. V. and Nichols, J. D. and Prang{\'{e}}, R. and Wilson, F. J.},
    number = {A11},
    pages = {1--18},
    volume = {110},
    doi = {10.1029/2005JA011237},
    issn = {21699402}
}

@article{Manifacier2001,
    title = {{A simple method for the determination of the optical constants n, k and the thickness of a weakly absorbing thin film}},
    year = {2001},
    journal = {Journal of Physics E: Scientific Instruments},
    author = {Manifacier, J C and Gasiot, J and Fillard, J P},
    number = {11},
    pages = {1002--1004},
    volume = {9},
    isbn = {0022-3735},
    doi = {10.1088/0022-3735/9/11/032},
    issn = {0022-3735},
    pmid = {20072543}
}

@article{Omidi2017,
    title = {{A Single Deformed Bow Shock for Titan-Saturn System}},
    year = {2017},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Omidi, N. and Sulaiman, A. H. and Kurth, W. and Madanian, H. and Cravens, T. and Sergis, N. and Dougherty, M. K. and Edberg, N. J.T.},
    number = {11},
    pages = {058--11},
    volume = {122},
    doi = {10.1002/2017JA024672},
    issn = {21699402},
    keywords = {Saturn, Titan, bow shock, foreshock}
}

@article{Grillmair2007,
    title = {{A Spitzer Spectrum of the Exoplanet HD 189733b}},
    year = {2007},
    journal = {The Astronomical Journal},
    author = {Grillmair, Carl J and Charbonneau, D. and Burrows, A. and Armus, L. and Stauffer, J. and Meadows, V. and van Cleve, J. and Levine, D.},
    pages = {111--114}
}

@article{Liu2017,
    title = {{A study of woodpecker's pecking process and the impact response of its brain}},
    year = {2017},
    journal = {International Journal of Impact Engineering},
    author = {Liu, Yu Zhe and Qiu, Xin Ming and Ma, Hong Lei and Fu, Wen Wen and Yu, T. X.},
    pages = {263--271},
    volume = {108},
    doi = {10.1016/j.ijimpeng.2017.05.016},
    issn = {0734743X}
}

@article{Bergner2018,
    title = {{A survey of ch3cn and hc3n in protoplanetary disks 3}},
    year = {2018},
    author = {Bergner, J. B. and Guzman, V. G. and Oberg, K. I. and Loomis, R. A. and Pegues, J.},
    pages = {1--27},
    arxivId = {arXiv:1803.04986v1},
    keywords = {astrochemistry, ism, molecules, protoplanetary disks}
}

@article{Raghavan2010,
    title = {{a Survey of Stellar Families: Multiplicity of Solar-Type Stars}},
    year = {2010},
    journal = {The Astrophysical Journal Supplement Series},
    author = {Raghavan, Deepak and McAlister, Harold A. and Henry, Todd J. and Latham, David W. and Marcy, Geoffrey W. and Mason, Brian D. and Gies, Douglas R. and White, Russel J. and ten Brummelaar, Theo A.},
    number = {1},
    pages = {1--42},
    volume = {190},
    url = {http://stacks.iop.org/0067-0049/190/i=1/a=1?key=crossref.da29cd9937113d2f29e2e9f0440ae68d},
    doi = {10.1088/0067-0049/190/1/1},
    issn = {0067-0049},
    keywords = {catalogs, individual, infrared, laboratory, machine-readable tables, methods, online-only material, planetary systems, planets and satellites, spectroscopic, techniques, titan}
}

@article{Hansen1992,
    title = {{A thermal model for the seasonal nitrogen cycle on Triton}},
    year = {1992},
    journal = {Icarus},
    author = {Hansen, Candice J. and Paige, David A.},
    number = {2},
    pages = {273--288},
    volume = {99},
    doi = {10.1016/0019-1035(92)90146-X},
    issn = {10902643}
}

@article{Walterscheid2006,
    title = {{A tidal explanation for the Titan haze layers}},
    year = {2006},
    journal = {Icarus},
    author = {Walterscheid, Richard L. and Schubert, Gerald},
    number = {2},
    pages = {471--478},
    volume = {183},
    doi = {10.1016/j.icarus.2006.03.001},
    issn = {00191035},
    keywords = {Atmospheres, Satellites of Saturn, Tides, Titan, atmospheric, dynamics}
}

@article{Lara2014,
    title = {{A time-dependent photochemical model for Titan’s atmosphere and the origin of H 2 O}},
    year = {2014},
    journal = {Astronomy {\&} Astrophysics},
    author = {Lara, L. M. and Lellouch, E. and Gonz{\'{a}}lez, M. and Moreno, R. and Rengel, M.},
    number = {November 2016},
    pages = {A143},
    volume = {566},
    url = {http://adsabs.harvard.edu/abs/2014A%26A...566A.143L},
    doi = {10.1051/0004-6361/201323085},
    issn = {0004-6361},
    keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: individual: Titan}
}

@article{Schulze-Makuch2011,
    title = {{A Two-Tiered Approach to Assessing the Habitability of Exoplanets}},
    year = {2011},
    journal = {Astrobiology},
    author = {Schulze-Makuch, Dirk and M{\'{e}}ndez, Abel and Fair{\'{e}}n, Alberto G. and von Paris, Philip and Turse, Carol and Boyer, Grayson and Davila, Alfonso F. and Ant{\'{o}}nio, Marina Resendes de Sousa and Catling, David and Irwin, Louis N.},
    number = {10},
    pages = {1041--1052},
    volume = {11},
    url = {http://www.liebertonline.com/doi/abs/10.1089/ast.2010.0592%5Cnhttp://online.liebertpub.com/doi/10.1089/ast.2010.0592},
    isbn = {1531-1074},
    doi = {10.1089/ast.2010.0592},
    issn = {1531-1074},
    pmid = {22017274},
    keywords = {Complexity, Earth similarity, Exoplanets, Habitability, Index, Life}
}

@article{Glein2017,
    title = {{A whiff of nebular gas in Titan’s atmosphere – Potential implications for the conditions and timing of Titan ’ s formation}},
    year = {2017},
    journal = {Icarus},
    author = {Glein, Christopher R},
    pages = {1--12},
    volume = {0},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2017.02.026},
    doi = {10.1016/j.icarus.2017.02.026},
    issn = {0019-1035},
    keywords = {"Atmospheres, "Satellites, "Titan, Solar nebula, Titan, atmosphere", evolution", formation"}
}

@article{Btoschwina1997,
    title = {{Ab initio anharmonic force fields and spectroscopic properties for HC5N and HC5NH+, molecules of interest to astrochemistry}},
    year = {1997},
    journal = {Spectrochimica Acta - Part A: Molecular and Biomolecular Spectroscopy},
    author = {Botschwina, P. and Heyl, A. and Oswald, M. and Hirano, T.},
    number = {8},
    pages = {1079--1090},
    volume = {53},
    doi = {10.1016/S1386-1425(97)00018-8},
    issn = {13861425},
    keywords = {Anharmonic force fields, Astrochemistry, Cyanopolynes}
}

@article{P.1977,
    title = {{Ab initio calculations of the stability of the NH5+ ion}},
    year = {1977},
    journal = {Chemical Physics Letters},
    author = {P., Bugaets O. and A., Zhogolev D.},
    number = {3},
    pages = {3--6},
    volume = {45}
}

@article{Steel2017,
    title = {{Abiotic and biotic formation of amino acids in the Enceladus ocean}},
    year = {2017},
    journal = {Astrobiology},
    author = {Steel, E L and Davila, Alfonso and McKay, Christopher P},
    number = {9},
    pages = {doi:10.1089/ast.2017.1673},
    volume = {17},
    doi = {10.1089/ast.2017.1673},
    issn = {1531-1074}
}

@article{English1996,
    title = {{Ablation and chemistry of meteoric materials in the atmosphere of Titan}},
    year = {1996},
    journal = {Advances in Space Research},
    author = {English, M. A. and Lara, L. M. and Lorenz, R. D. and Ratcliff, P. R. and Rodrigo, R.},
    number = {12},
    pages = {157--160},
    volume = {17},
    doi = {10.1016/0273-1177(95)00774-9},
    issn = {02731177}
}

@article{Khlifi1995,
    title = {{Absolute ir band intensities of diacetylene in the 250-4300 cm-1region: Implications for titan′s atmosphere}},
    year = {1995},
    journal = {Journal of Molecular Spectroscopy},
    author = {Khlifi, M. and Paillous, P. and Delpech, C. and Nishio, M. and Bruston, P. and Raulin, F.},
    number = {1},
    pages = {116--122},
    volume = {174},
    doi = {10.1006/jmsp.1995.1273},
    issn = {1096083X}
}

@article{Horst1990,
    title = {{Absorption Coefficients for the 6190-A OH 4 Band between 290 and 100 {${}^\circ$} K with Application to Uranus ' Atmosphere}},
    year = {1990},
    journal = {Icaurs},
    author = {Hayden Smith, W.M. and Conner, C. P.},
    pages = {58--64},
    volume = {64}
}

@article{Alrefae2014,
    title = {{Absorption cross-section measurements of methane, ethane, ethylene and methanol at high temperatures}},
    year = {2014},
    journal = {Journal of Molecular Spectroscopy},
    author = {Alrefae, Majed and Es-Sebbar, Et Touhami and Farooq, Aamir},
    pages = {8--14},
    volume = {303},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.jms.2014.06.007},
    isbn = {9661280827},
    doi = {10.1016/j.jms.2014.06.007},
    issn = {1096083X},
    keywords = {Absorption cross-section, Ethane, Ethylene, FTIR, HeNe laser, Methane, Methanol}
}

@article{Masterson1990,
    title = {{Absorption intensities and complex refractive indices of crystalline HCN, HC3N, and C4N2 in the infrared region}},
    year = {1990},
    journal = {Icarus},
    author = {Masterson, C. M. and Khanna, R. K.},
    number = {1},
    pages = {83--92},
    volume = {83},
    doi = {10.1016/0019-1035(90)90007-V},
    issn = {10902643}
}

@article{Wood2006,
    title = {{Accretion of the Earth and segregation of its core.}},
    year = {2006},
    journal = {Nature},
    author = {Wood, Bernard J and Walter, Michael J and Wade, Jonathan},
    number = {7095},
    pages = {825--833},
    volume = {441},
    isbn = {0028-0836},
    doi = {10.1038/nature04763},
    issn = {0028-0836},
    pmid = {16778882}
}

@article{Huang2009,
    title = {{Accurate ab initio quartic force fields for NH2- and CCH- and rovibrational spectroscopic constants for their isotopologs}},
    year = {2009},
    journal = {Journal of Chemical Physics},
    author = {Huang, Xinchuan and Lee, Timothy J.},
    number = {10},
    pages = {1--15},
    volume = {131},
    isbn = {0021-9606},
    doi = {10.1063/1.3212560},
    issn = {00219606}
}

@article{Charnley2004,
    title = {{Acetaldehyde in star-forming regions}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Charnley, S. B.},
    number = {1},
    pages = {23--30},
    volume = {33},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2003.08.005},
    issn = {02731177},
    keywords = {ISM: abundances, ISM: clouds, ISM: molecules, Stars: formation}
}

@article{Dodonova1966,
    title = {{Activation of nitrogen by vacuum ultraviolet radiation}},
    year = {1966},
    journal = {Russian Journal of Physical Chemistry},
    author = {Dodonova, N. Y.}
}

@article{Sparks2017,
    title = {{Active Cryovolcanism on Europa?}},
    year = {2017},
    journal = {The Astrophysical Journal Letters},
    author = {Sparks, W B and Schmidt, B E and Mcgrath, M A and Hand, K P and Spencer, J R and Cracraft, M and Deustua, S E},
    number = {2},
    pages = {L18},
    volume = {839},
    publisher = {IOP Publishing},
    url = {http://iopscience.iop.org/article/10.3847/2041-8213/aa67f8/pdf},
    doi = {10.3847/2041-8213/aa67f8},
    issn = {2041-8213},
    arxivId = {1704.04283},
    keywords = {planets and satellites: general}
}

@article{Wall2010,
    title = {{Active shoreline of Ontario Lacus, Titan: A morphological study of the lake and its surroundings}},
    year = {2010},
    journal = {Geophysical Research Letters},
    author = {Wall, S. and Hayes, A. and Bristow, C. and Lorenz, R. and Stofan, E. and Lunine, J. and Le Gall, A. and Janssen, M. and Lopes, R. and Wye, L. and Soderblom, L. and Paillou, P. and Aharonson, O. and Zebker, H. and Farr, T. and Mitri, G. and Kirk, R. and Mitchell, K. and Notarnicola, C. and Casarano, D. and Ventura, B.},
    number = {5},
    pages = {1--5},
    volume = {37},
    isbn = {0094-8276},
    doi = {10.1029/2009GL041821},
    issn = {00948276},
    pmid = {275303000003},
    keywords = {http://dx.doi.org/10.1029/2009GL041821, doi:10.102}
}

@article{Teanby2012,
    title = {{Active upper-atmosphere chemistry and dynamics from polar circulation reversal on Titan}},
    year = {2012},
    journal = {Nature},
    author = {Teanby, N. and Irwin, Patrick G J and Nixon, Conor A. and De Kok, Remco and Vinatier, Sandrine and Coustenis, Athena and Sefton-Nash, Elliot and Calcutt, Simon B. and Flasar, F. Michael},
    number = {7426},
    pages = {732--735},
    volume = {491},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/nature11611},
    isbn = {1476-4687 (Electronic){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/nature11611},
    issn = {00280836},
    pmid = {23192150}
}

@article{Helfenstein1982,
    title = {{Active venting of Europa?: Analysis of a Transient bright surface feature}},
    year = {1982},
    journal = {Lunar Planet. Sci. Conf.},
    author = {Helfenstein, P. and Cook II, A. F.},
    number = {rock 10003},
    pages = {1205--1207},
    volume = {9}
}

@article{DeOliveira2016a,
    title = {{Adsorption of diclofenac onto organoclays: Effects of surfactant and environmental (pH and temperature) conditions}},
    year = {2016},
    journal = {Journal of Hazardous Materials},
    author = {De Oliveira, Tiago and Gu{\'{e}}gan, Régis and Thiebault, Thomas and Milbeau, Claude Le and Muller, Fabrice and Teixeira, Vinicius and Giovanela, Marcelo and Boussafir, Mohammed},
    pages = {558--566},
    volume = {323},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.jhazmat.2016.05.001},
    doi = {10.1016/j.jhazmat.2016.05.001},
    issn = {18733336},
    pmid = {27180207},
    keywords = {Adsorption, Cationic surfactant, Diclofenac, Organoclay, Pharmaceutical}
}

@article{Grimbergen2004,
    title = {{Advancement of Time Measurements Museum van het Nederlandse Uurwerk}},
    year = {2004},
    author = {Grimbergen, Kees}
}

@article{Lavvas2013,
    title = {{Aerosol growth in Titan's ionosphere}},
    year = {2013},
    journal = {Proceedings of the National Academy of Sciences},
    author = {Lavvas, P. and Yelle, R. V. and Koskinen, T. and Bazin, A. and Vuitton, V. and Vigren, E. and Galand, M. and Wellbrock, A. and Coates, A. J. and Wahlund, J.-E. and Crary, F. J. and Snowden, D.},
    number = {8},
    pages = {2729--2734},
    volume = {110},
    url = {http://www.pnas.org/cgi/doi/10.1073/pnas.1217059110},
    isbn = {0027-8424},
    issn = {0027-8424},
    pmid = {23382231}
}

@article{Mukai2006,
    title = {{Aerosol properties and air pollutants over an urban area}},
    year = {2006},
    journal = {Atmospheric Research},
    author = {Mukai, Sonoyo and Sano, Itaru and Satoh, Mutsumi and Holben, Brent N.},
    number = {3-4},
    pages = {643--651},
    volume = {82},
    doi = {10.1016/j.atmosres.2006.02.020},
    issn = {01698095},
    keywords = {Air pollutants, Atmospheric aerosols, OBC, PM2.5, SPM}
}

@article{Lavvas2017EPSC,
    title = {{Aerosols and clouds in the atmosphere of HD 189733 b}},
    year = {2017},
    journal = {EPSC 2017},
    author = {Lavvas, P. and Koskinen, T.},
    pages = {1--2},
    volume = {11}
}

@article{Tomasko2009,
    title = {{Aerosols in Titan’s Atmosphere}},
    year = {2009},
    author = {Tomasko, Martin G and West, Robert A},
    pages = {297--322}
}

@article{Rannou2017,
    title = {{Aerosols optical properties in Titan’s detached haze layer before the equinox}},
    year = {2017},
    journal = {Icarus},
    author = {Seignovert, Benoit and Rannou, Pascal and Lavvas, Panayotis and Cours, Thibaud and West, Robert A},
    doi = {10.5281/ZENODO.165084},
    issn = {00191035},
    arxivId = {arXiv:1704.00842v1},
    keywords = {Aerosols, Atmosphere, Titan}
}

@article{Ramanathan2001,
    title = {{Aerosols, Climate, and the Hydrological Cycle}},
    year = {2001},
    journal = {Science},
    author = {Ramanathan, V.},
    number = {5549},
    pages = {2119--2124},
    volume = {294},
    url = {http://www.sciencemag.org/cgi/doi/10.1126/science.1064034},
    isbn = {00368075},
    doi = {10.1126/science.1064034},
    issn = {00368075},
    pmid = {11739947}
}

@article{Birch2016,
    title = {{Alluvial Fan Morphology, distribution and formation on Titan}},
    year = {2016},
    journal = {Icarus},
    author = {Birch, S. P D and Hayes, A. G. and Howard, A. D. and Moore, J. M. and Radebaugh, J.},
    pages = {238--247},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.02.013},
    doi = {10.1016/j.icarus.2016.02.013},
    issn = {10902643},
    keywords = {Geological processes, Titan, Titan, hydrology, surface}
}

@article{Palmer2017,
    title = {{ALMA detection and astrobiological potential of vinyl cyanide on Titan}},
    year = {2017},
    author = {Palmer, Maureen Y and Cordiner, Martin A and Nixon, Conor A and Charnley, Steven B and Teanby, Nicholas A and Kisiel, Zbigniew and Irwin, Patrick G J and Mumma, Michael J},
    number = {July},
    pages = {1--7}
}

@article{Cordiner2014a,
    title = {{ALMA measurements of the HNC and HC{\_}3N distributions in Titan's atmosphere}},
    year = {2014},
    author = {Cordiner, M. A. and Nixon, C. A. and Teanby, N. A. and Serigano, J. and Charnley, S. B. and Milam, S. N. and Mumma, M. J. and Irwin, P. G. J. and Lis, D. C. and Villanueva, G. and Paganini, L. and Kuan, Y. -J. and Remijan, A. J.},
    number = {2012},
    pages = {2--7},
    url = {http://arxiv.org/abs/1408.6461%0Ahttp://dx.doi.org/10.1088/2041-8205/795/2/L30},
    isbn = {2041-8205},
    doi = {10.1088/2041-8205/795/2/L30},
    issn = {2041-8213},
    arxivId = {1408.6461}
}

@article{Molter2016,
    title = {{ALMA Observations of HCN and its Isotopologues on Titan}},
    year = {2016},
    author = {Molter, Edward M. and Nixon, Conor A. and Cordiner, Martin A. and Serigano, Joseph and Irwin, Patrick G. J. and Teanby, Nicholas A. and Charnley, Steven B. and Lindberg, Johan E.},
    pages = {1--14},
    url = {http://arxiv.org/abs/1606.00348},
    arxivId = {1606.00348}
}

@article{Molter2016a,
    title = {{ALMA Observations of HCN and its Isotopologues on Titan}},
    year = {2016},
    journal = {The Astronomical Journal},
    author = {Molter, Edward M. and Nixon, Conor A. and Cordiner, Martin A. and Serigano, Joseph and Irwin, Patrick G. J. and Teanby, Nicholas A. and Charnley, Steven B. and Lindberg, Johan E.},
    number = {2},
    pages = {1--7},
    volume = {152},
    publisher = {IOP Publishing},
    url = {http://arxiv.org/abs/1606.00348%0Ahttp://dx.doi.org/10.3847/0004-6256/152/2/42},
    doi = {10.3847/0004-6256/152/2/42},
    issn = {1538-3881},
    arxivId = {1606.00348},
    keywords = {atmospheres, individual, planets and satellites, planets and satellites: atmospheres, planets and satellites: individual (Titan), titan}
}

@article{Moreno2015,
    title = {{ALMA observations of Titan : Vertical and spatial distribution of nitriles}},
    year = {2015},
    journal = {EPSC 2015},
    author = {Moreno, R. and Lellouch, E. and Vinatier, S. and Gurwell, M. and Moullet, A. and Lara, L. M. and Hidayat, T},
    pages = {2015},
    volume = {10}
}

@article{Trumbo2017,
    title = {{ALMA Thermal Observations of a Proposed Plume Source Region on Europa}},
    year = {2017},
    author = {Trumbo, Samantha K. and Brown, Michael E. and Butler, Bryan J.},
    pages = {1--7},
    url = {http://arxiv.org/abs/1708.07922},
    arxivId = {1708.07922},
    keywords = {and satellites, europa, general, individual, planets, planets and satellites, surfaces}
}

@article{Fabian2018,
    title = {{Ammonia Clathrate Hydrate As Seen from Grand Canonical Monte Carlo Simulations}},
    year = {2018},
    journal = {ACS Earth and Space Chemistry},
    author = {F{\'{a}}bi{\'{a}}n, Balázs and Picaud, Sylvain and Jedlovszky, Pál and Guilbert-Lepoutre, Aurélie and Mousis, Olivier},
    pages = {acsearthspacechem.7b00133},
    url = {http://pubs.acs.org/doi/10.1021/acsearthspacechem.7b00133},
    doi = {10.1021/acsearthspacechem.7b00133},
    issn = {2472-3452},
    keywords = {ammonia, clathrate, grand canonical monte carlo, planetary science, simulations}
}

@article{Fortes2007,
    title = {{Ammonium sulfate on Titan: Possible origin and role in cryovolcanism}},
    year = {2007},
    journal = {Icarus},
    author = {Fortes, A. D. and Grindrod, P. M. and Trickett, S. K. and Vo{\v{c}}adlo, L.},
    number = {1},
    pages = {139--153},
    volume = {188},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2006.11.002},
    issn = {00191035},
    keywords = {Ices, Interiors, Titan, Volcanism}
}

@article{Martinez2015,
    title = {{An accurate molecular structure of phenyl, the simplest aryl radical}},
    year = {2015},
    journal = {Angewandte Chemie - International Edition},
    author = {Martinez, Oscar and Crabtree, Kyle N. and Gottlieb, Carl A. and Stanton, John F. and McCarthy, Michael C.},
    number = {6},
    pages = {1808--1811},
    volume = {54},
    doi = {10.1002/anie.201409896},
    issn = {15213773},
    pmid = {25521111},
    keywords = {Ab initio calculations, Molecular structure, Rotational spectroscopy}
}

@article{Rule,
    title = {{AN ANALYTICAL SOLUTION FOR SIGNAL , BACKGROUND AND SIGNAL TO BACKGROUND RATIO FOR A LOW FREQUENCY ACTIVE SONAR IN A PEKERIS WAVEGUIDE SATISFYING}},
    author = {Rule, Lambert S},
    number = {April 2010},
    pages = {491--498},
    keywords = {analytical solution, low frequency active sonar, pekeris waveguide, rain noise, reverberation, sonar performance modelling, target echo}
}

@article{Richard2015a,
    title = {{An empirical approach to modeling ion production rates in Titan's ionosphere I: Ion production rates on the dayside and globally}},
    year = {2015},
    author = {Richard, M S and Cravens, T E and Wylie, C and Webb, D and Chediak, Q and Perryman, R and Mandt, K and Westlake, J and Waite, J H and Robertson, I and Magee, B A and Edberg, N J T},
    pages = {1--17},
    doi = {10.1002/2014JA020343.An},
    keywords = {10.1002/2013JA019706 and Titan, empirical, global, ion production, ionosphere}
}

@article{Richard2015b,
    title = {{An empirical approach to modeling ion production rates in Titan's ionosphere II: Ion production rates on the nightside}},
    year = {2015},
    author = {Richard, M S and Cravens, T E and Wylie, C and Webb, D and Chediak, Q and Mandt, K and Waite, J H and Rymer, A and Bertucci, C and Wellbrock, A and Windsor, A and Coates, A J},
    number = {Mimi},
    pages = {1--18},
    doi = {10.1002/2013JA019706.An},
    keywords = {10.1002/2014JA020343 and Titan, electron precipitation, ionization, ionosphere, magnetosphere}
}

@article{Cordier2009,
    title = {{An estimate of the chemical composition of titan's lakes}},
    year = {2009},
    journal = {Astrophysical Journal},
    author = {Cordier, Daniel and Mousis, Olivier and Lunine, Jonathan I. and Lavvas, Panayotis and Vuitton, Véronique},
    number = {2 PART 2},
    volume = {707},
    doi = {10.1088/0004-637X/707/2/L128},
    issn = {15384357},
    arxivId = {0911.1860},
    keywords = {Planets and satellites: general, Planets and satellites: individual (Titan), Solar system: general}
}

@article{Sagan1967,
    title = {{An Estimate of the Surface Temperature of Venus Independent of Passive Microwave Radiometry}},
    year = {1967},
    journal = {The Astrophysical Journal},
    author = {Sagan, Carl},
    volume = {149}
}

@article{Nutanong2011,
    title = {{An incremental Hausdorff distance calculation algorithm}},
    year = {2011},
    journal = {Proceedings of the VLDB Endowment},
    author = {Nutanong, Sarana and Jacox, Edwin H. and Samet, Hanan},
    number = {8},
    pages = {506--517},
    volume = {4},
    url = {http://dl.acm.org/citation.cfm?doid=2002974.2002978},
    doi = {10.14778/2002974.2002978},
    issn = {21508097}
}

@article{Danielson1973,
    title = {{An inversion in the atmosphere of Titan}},
    year = {1973},
    journal = {Icarus},
    author = {Danielson, R. E. and Caldwell, John J. and Larach, D. R.},
    number = {4},
    pages = {437--443},
    volume = {20},
    doi = {10.1016/0019-1035(73)90016-X},
    issn = {10902643}
}

@article{DelGenio2016,
    title = {{An objective classification of Saturn cloud features from Cassini ISS images}},
    year = {2016},
    journal = {Icarus},
    author = {Del Genio, Anthony D. and Barbara, John M.},
    pages = {222--236},
    volume = {271},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.02.011},
    doi = {10.1016/j.icarus.2016.02.011},
    issn = {10902643},
    keywords = {Atmospheres, dynamics, Image processing, Saturn, Saturn, atmosphere}
}

@article{Galopeau2016,
    title = {{An oblate beaming cone for Io-controlled Jovian decameter emission}},
    year = {2016},
    journal = {AGU Publications},
    author = {Galopeau, P H M and Boudjada, M Y},
    pages = {3120--3138},
    doi = {10.1002/2015JA021038.Received},
    keywords = {10.1002/2015JA021038 and Jovian decameter emission}
}

@article{Peale1978,
    title = {{An observational test for the origin of the Titan-Hyperion orbital resonance}},
    year = {1978},
    journal = {Icarus},
    author = {Peale, S. J.},
    number = {2},
    pages = {240--244},
    volume = {36},
    doi = {10.1016/0019-1035(78)90108-2},
    issn = {10902643}
}

@article{Lebreton1992,
    title = {{An overview of the Cassini mission}},
    year = {1992},
    journal = {Il Nuovo Cimento C},
    author = {Lebreton, J. P. and Matson, D. L.},
    number = {6},
    pages = {1137--1147},
    volume = {15},
    doi = {10.1007/BF02506708},
    issn = {03905551},
    keywords = {Saturn}
}

@article{Lebreton2002,
    title = {{An overview of the descent and landing of the Huygens probe on Titan}},
    year = {2005},
    author = {Lebreton, Jean-pierre and Witasse, Olivier and Sollazzo, Claudio and Blancquaert, Thierry and Couzin, Patrice and Schipper, Anne-marie and Jones, Jeremy B and Matson, Dennis L and Gurvits, Leonid I and Atkinson, David H and Kazeminejad, Bobby and Pe, Miguel},
    number = {December},
    volume = {438},
    doi = {10.1038/nature04347}
}

@article{Yung1987,
    title = {{An update of nitrile photochemistry on Titan}},
    year = {1987},
    journal = {Icarus},
    author = {Yung, Yuk L.},
    number = {2},
    pages = {468--472},
    volume = {72},
    doi = {10.1016/0019-1035(87)90186-2},
    issn = {10902643},
    pmid = {11542216}
}

@article{Vinatier2009,
    title = {{Analysis of Cassini/CIRS limb spectra of Titan acquired during the nominal mission I: Hydrocarbons, nitriles and CO2 vertical mixing ratio profiles}},
    year = {2009},
    journal = {Icarus},
    author = {Vinatier, Sandrine and B{\'{e}}zard, Bruno and de Kok, Remco and Anderson, Carrie M. and Samuelson, Robert E. and Nixon, Conor A. and Mamoutkine, Andrei and Carlson, Ronald C. and Jennings, Donald E. and Guandique, Ever A. and Bjoraker, Gordon L. and Michael Flasar, F. and Kunde, Virgil G.},
    number = {2},
    pages = {852--866},
    volume = {210},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.08.013},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2010.06.024},
    issn = {00191035},
    keywords = {Abundances, Atmospheres, Infrared observations, Titan}
}

@article{Vinatier2010,
    title = {{Analysis of Cassini/CIRS limb spectra of Titan acquired during the nominal mission II: Aerosol extinction profiles in the 600-1420cm-1 spectral range}},
    year = {2010},
    journal = {Icarus},
    author = {Vinatier, Sandrine and B{\'{e}}zard, Bruno and de Kok, Remco and Anderson, Carrie M. and Samuelson, Robert E. and Nixon, Conor A. and Mamoutkine, Andrei and Carlson, Ronald C. and Jennings, Donald E. and Guandique, Ever A. and Bjoraker, Gordon L. and Michael Flasar, F. and Kunde, Virgil G.},
    number = {2},
    pages = {852--866},
    volume = {210},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.06.024},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2010.06.024},
    issn = {00191035},
    keywords = {Abundances, Atmospheres, Infrared observations, Titan}
}

@article{Vinatier2010b,
    title = {{Analysis of Cassini/CIRS limb spectra of Titan acquired during the nominal missionI. Hydrocarbons, nitriles and CO2 vertical mixing ratio profiles}},
    year = {2010},
    journal = {Icarus},
    author = {Vinatier, Sandrine and B{\'{e}}zard, Bruno and Nixon, Conor a. and Mamoutkine, Andrei and Carlson, Ronald C. and Jennings, Donald E. and Guandique, Ever a. and Teanby, Nick a. and Bjoraker, Gordon L. and Michael Flasar, F.},
    number = {2},
    pages = {559--570},
    volume = {205},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103509003558},
    doi = {10.1016/j.icarus.2009.08.013},
    issn = {00191035}
}

@article{Liu2006,
    title = {{Analysis of electron impact ionization properties of methane}},
    year = {2006},
    journal = {Journal of Geophysical Research},
    author = {Liu, Xianming and Shemansky, Donald E.},
    number = {A4},
    pages = {A04303},
    volume = {111},
    url = {http://doi.wiley.com/10.1029/2005JA011454},
    doi = {10.1029/2005JA011454},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/2005JA011454, doi:10.102, impact excitation function, ionization oscillator}
}

@article{Cui2009b,
    title = {{Analysis of Titan's neutral upper atmosphere from Cassini Ion Neutral Mass Spectrometer measurements}},
    year = {2009},
    journal = {Icarus},
    author = {Cui, J. and Yelle, R. V. and Vuitton, V. and Waite, J. H. and Kasprzak, W. T. and Gell, D. A. and Niemann, H. B. and M{\"{u}}ller-Wodarg, I. C F and Borggren, N. and Fletcher, G. G. and Patrick, E. L. and Raaen, E. and Magee, B. A.},
    number = {2},
    pages = {581--615},
    volume = {200},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2008.12.005},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2008.12.005},
    issn = {00191035},
    keywords = {Atmospheres, Titan, composition, structure}
}

@article{Beghin2012,
    title = {{Analytic theory of Titan's Schumann resonance: Constraints on ionospheric conductivity and buried water ocean}},
    year = {2012},
    journal = {Icarus},
    author = {B{\'{e}}ghin, C. and Randriamboarison, Orélien and Hamelin, Michel and Karkoschka, Erich and Sotin, Christophe and Whitten, Robert C. and Berthelier, Jean Jacques and Grard, R??jean and Sim??es, Fernando},
    number = {2},
    pages = {1028--1042},
    volume = {218},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2012.02.005},
    issn = {00191035},
    keywords = {Interiors, Lightning, Saturn, Titan, atmosphere, interior, magnetosphere}
}

@article{Zabka2012,
    title = {{Anion chemistry on Titan: A possible route to large N-bearing hydrocarbons}},
    year = {2012},
    journal = {Icarus},
    author = {{\v{Z}}abka, Ján and Romanzin, Claire and Alcaraz, Christian and Pol{\'{a}}{\v{s}}ek, Miroslav},
    number = {1},
    pages = {161--167},
    volume = {219},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2012.02.031},
    issn = {00191035},
    keywords = {Chemistry, Ionospheres, Titan, atmosphere}
}

@article{Hurford2014,
    title = {{Antarctic analog for dilational bands on Europa}},
    year = {2014},
    journal = {Earth and Planetary Science Letters},
    author = {Hurford, T. A. and Brunt, K. M.},
    pages = {275--283},
    volume = {401},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.epsl.2014.05.015},
    doi = {10.1016/j.epsl.2014.05.015},
    issn = {0012821X},
    keywords = {Antarctica, Earth analog, Europa, Tectonics}
}

@article{Head1992,
    title = {{Associations , and Global Distribution from Magellan Data}},
    year = {1992},
    author = {Head, James W and Crumpler, L S and Aubele, Jayne C and Saunders, R Stephen},
    number = {9},
    volume = {97}
}

@article{Raulin2008,
    title = {{Astrobiology and habitability of Titan}},
    year = {2008},
    journal = {Space Science Reviews},
    author = {Raulin, Francois},
    number = {1-4},
    pages = {37--48},
    volume = {135},
    isbn = {0038-6308{\textbackslash}r1572-9672},
    doi = {10.1007/s11214-006-9133-7},
    issn = {00386308},
    pmid = {18668096},
    keywords = {Astrobiology, Cassini-Huygens, Prebiotic chemistry, Primitive Earth, Tholins, Titan}
}

@article{Raulin2008a,
    title = {{Astrobiology and habitability of Titan}},
    year = {2008},
    journal = {Space Science Reviews},
    author = {Raulin, Francois},
    number = {1-4},
    pages = {37--48},
    volume = {135},
    isbn = {0038-6308{\textbackslash}r1572-9672},
    doi = {10.1007/s11214-006-9133-7},
    issn = {00386308},
    pmid = {18668096},
    keywords = {Astrobiology, Cassini-Huygens, Prebiotic chemistry, Primitive Earth, Tholins, Titan}
}

@article{Nicolaidis1932,
    title = {{ASTRONOMY AND POLITICS IN RUSSIA IN THE EARLY}},
    year = {1932},
    author = {Nicolaidis, E.}
}

@article{Fihtengolts1969,
    title = {{Atlas of UV absorption spectra of substances used in synthetic rubber manufacture}},
    year = {1969},
    author = {Fihtengolts, V. S.},
    editor = {{NIST Chemistry WebBook}}
}

@article{Atreya1986,
    title = {{Atmospheres and Ionospheres of the Outer Planets and their satellites}},
    year = {1986},
    author = {Atreya, S. K.},
    volume = {15},
    isbn = {9783642713965}
}

@article{Lunine1984,
    title = {{Atmospheres of Uranus and Neptune}},
    year = {1984},
    journal = {Annual Review of Astronomy and Astrophysics},
    author = {Lunine, Jonathan I},
    number = {1},
    pages = {217--263},
    volume = {31},
    url = {http://adsabs.harvard.edu/full/1993ARA&A..31..217L},
    doi = {10.1038/272403a0},
    issn = {01917811},
    keywords = {composition, outer planets}
}

@article{Plane1995,
    title = {{Atmospheric Chemistry of meteoric metals}},
    year = {1995},
    author = {Plane, John M.C.},
    number = {1},
    pages = {247--250},
    volume = {29}
}

@article{Komacek2016a,
    title = {{Atmospheric Circulation of Hot Jupiters: Dayside-Nightside Temperature Differences}},
    year = {2016},
    author = {Komacek, Thaddeus D. and Showman, Adam P.},
    number = {2013},
    pages = {23},
    url = {http://arxiv.org/abs/1601.00069},
    doi = {10.3847/0004-637X/821/1/16},
    issn = {15384357},
    arxivId = {1601.00069}
}

@article{Lora2017,
    title = {{Atmospheric circulation, chemistry, and infrared spectra of Titan-like exoplanets around different stellar types}},
    year = {2017},
    journal = {The Astrophysical Journal},
    author = {Lora, Juan M. and Kataria, Tiffany and Gao, Peter},
    url = {http://arxiv.org/abs/1712.04069},
    arxivId = {1712.04069},
    keywords = {atmospheres, atmospheric effects, composition, corresponding author, detection, juan m, lora, methods, numerical, planets and satellites}
}

@article{Aplin2006,
    title = {{Atmospheric electrification in the solar system}},
    year = {2006},
    journal = {Surveys in Geophysics},
    author = {Aplin, Karen L.},
    number = {1},
    pages = {63--108},
    volume = {27},
    isbn = {0169-3298},
    doi = {10.1007/s10712-005-0642-9},
    issn = {01693298},
    arxivId = {physics/0505123},
    keywords = {Atmospheric aerosol, Atmospheric electricity, Climate, Cosmic rays, Global electric circuit, Ion-induced nucleation, Ionisation, Lightning, Planetary atmospheres}
}

@article{Torokova2015,
    title = {{Atmospheric pressure glow discharge generated in nitrogen-methane gas mixture: PTR-MS analyzes of the exhaust gas}},
    year = {2015},
    journal = {EPJ Applied Physics},
    author = {Torokova, L. and Mazankova, V. and Krcma, F. and Mason, N.J. and Matejcik, S.},
    number = {2},
    volume = {71},
    isbn = {2015150072},
    doi = {10.1051/epjap/2015150072},
    issn = {12860050 12860042}
}

@article{Lebonnois2003,
    title = {{Atomic and molecular hydrogen budget in Titan's atmosphere}},
    year = {2003},
    journal = {Icarus},
    author = {Lebonnois, Sébastien and Bakes, E. L.O. and McKay, Christopher P.},
    number = {2},
    pages = {474--485},
    volume = {161},
    doi = {10.1016/S0019-1035(02)00039-8},
    issn = {00191035},
    keywords = {Atmospheres, Photochemistry, Titan, composition}
}

@article{Sreejith2016,
    title = {{Balloon UV Experiments for Astronomical and Atmospheric Observations}},
    year = {2016},
    author = {Sreejith, A. G. and Mathew, Joice and Sarpotdar, Mayuresh and Nirmal, K. and Ambily, S. and Prakash, Ajin and Safonova, Margarita and Murthy, Jayant},
    pages = {1--7},
    volume = {9908},
    url = {http://arxiv.org/abs/1608.06385%0Ahttp://dx.doi.org/10.1117/12.2232246},
    isbn = {9781510601956},
    doi = {10.1117/12.2232246},
    issn = {1996756X},
    arxivId = {1608.06385},
    keywords = {balloon, spectrograph, uv}
}

@article{Howell2018,
    title = {{Band formation and ocean-surface interaction on Europa and Ganymede}},
    year = {2018},
    journal = {Geophysical Research Letters},
    author = {Howell, S. M. and Pappalardo, R. T.},
    doi = {10.1029/2018GL077594}
}

@article{Terada2017,
    title = {{Biogenic oxygen from Earth transported to the Moon by a wind of magnetospheric ions}},
    year = {2017},
    journal = {Nature Astronomy},
    author = {Terada, Kentaro and Yokota, Shoichiro and Saito, Yoshifumi and Kitamura, Naritoshi and Asamura, Kazushi and Nishino, Masaki N.},
    number = {2},
    pages = {0026},
    volume = {1},
    url = {http://www.nature.com/articles/s41550-016-0026},
    isbn = {2397-3366},
    doi = {10.1038/s41550-016-0026},
    issn = {2397-3366}
}

@article{Hazen2015,
    title = {{Blue whales (Balaenoptera musculus) optimize foraging efficiency by balancing oxygen use and energy gain as a function of prey density}},
    year = {2015},
    journal = {Science Advances},
    author = {Hazen, E. L. and Friedlaender, Ari S. and Goldbogen, Jeremy A.},
    number = {9},
    pages = {e1500469-e1500469},
    volume = {1},
    url = {http://advances.sciencemag.org/cgi/doi/10.1126/sciadv.1500469},
    isbn = {2375-2548},
    doi = {10.1126/sciadv.1500469},
    issn = {2375-2548},
    pmid = {26601290}
}

@article{Politzer1986,
    title = {{Bond-order-bond-energy correlations}},
    year = {1986},
    journal = {Chemical Physics Letters},
    author = {Politzer, P. and Ranganathan, S.},
    number = {6},
    pages = {527--530},
    volume = {124}
}

@article{Izidoro2017,
    title = {{Breaking the Chains : Hot Super-Earth systems from migration and disruption of compact resonant chains}},
    year = {2017},
    author = {Izidoro, Andre and Ogihara, Masahiro and Raymond, Sean N and Morbidelli, Alessandro and Bitsch, Bertram and Cossou, Christophe and Hersant, Franck},
    number = {March},
    pages = {1--21},
    volume = {21},
    arxivId = {arXiv:1703.03634v1},
    keywords = {disks, hot super-earths, migration}
}

@article{Cordier2017,
    title = {{Bubble streams in Titan's seas as product of liquid N2-CH4-C2H6 cryogenic mixture}},
    year = {2017},
    author = {Cordier, Daniel and Garcia-Sanchez, Fernando and Justo-Garcia, Daimler N. and Liger-Belair, Gerard},
    number = {April},
    pages = {6--9},
    volume = {0102},
    url = {http://arxiv.org/abs/1704.07345%0Ahttp://dx.doi.org/10.1038/s41550-017-0102},
    doi = {10.1038/s41550-017-0102},
    issn = {2397-3366},
    arxivId = {1704.07345}
}

@article{Selvans2005,
    title = {{By KARL JOSEPH FEIERABEND B . S ., Furman University , 2001 A thesis submitted to the Faculty of the Graduate School of the University of Colorado in partial fulfillment of the requirements for the degree of Doctor of Philosophy Department of Chemistry an}},
    year = {2005},
    author = {Selvans, Zane A.}
}

@article{Brewer2016,
    title = {{C/O and O/H Ratios Suggest Some Hot Jupiters Originate Beyond the Snow Line}},
    year = {2016},
    author = {Brewer, John M. and Fischer, Debra A. and Madhusudhan, Nikku},
    url = {http://arxiv.org/abs/1612.04372},
    arxivId = {1612.04372}
}

@article{Maguire1981,
    title = {{C3H8 and C3H4 in Titan's atmosphere}},
    year = {1981},
    journal = {Nature},
    author = {Maguire, W. C. and Hanel, R. A. and Jennings, D. E. and Kunde, V. G. and Samuelson, R. E.},
    number = {5825},
    month = {8},
    pages = {683--686},
    volume = {292},
    url = {http://www.nature.com/doifinder/10.1038/292683a0},
    doi = {10.1038/292683a0},
    issn = {0028-0836}
}

@article{Kunde1981,
    title = {{C4H2, HC3N and C2N2 in Titan's atmosphere}},
    year = {1981},
    journal = {Nature},
    author = {Kunde, V. G. and Aikin, A. C. and Hanel, R. A. and Jennings, D. E. and Maguire, W. C. and Samuelson, R. E.},
    number = {5825},
    month = {8},
    pages = {686--688},
    volume = {292},
    url = {http://www.nature.com/doifinder/10.1038/292686a0},
    doi = {10.1038/292686a0},
    issn = {0028-0836}
}

@article{Samuelson1997,
    title = {{C4N2 ice in Titan's north polar stratosphere}},
    year = {1997},
    journal = {Planet. Space Sci},
    author = {Samuelson, R E and Mayo, L A and Knuckles3, M A and Khanna4, R J},
    number = {8},
    pages = {941--948},
    volume = {45},
    doi = {http://dx.doi.org/10.1016/S0032-0633(97)00088-3},
    issn = {0032-0633}
}

@article{H1993,
    title = {{CALCULATION OF THE BOND DISSOCIATION ENERGY AND OTHER PARAMETERS OF THE ANHARMONIC POTENTIAL OVERTONE SPECTRA}},
    year = {1993},
    author = {H, Function O F and Their, H C O Molecules B Y and Diihtxixjxnxz, E},
    pages = {275--281},
    volume = {58}
}

@article{Alcouffe2010,
    title = {{Capacitively coupled plasma used to simulate Titan's atmospheric chemistry}},
    year = {2010},
    journal = {Plasma Sources Science and Technology},
    author = {Alcouffe, G. and Cavarroc, M. and Cernogora, G. and Ouni, F. and Jolly, A. and Boufendi, L. and Szopa, C.},
    number = {1},
    pages = {15008},
    volume = {19},
    url = {http://stacks.iop.org/0963-0252/19/i=1/a=015008},
    isbn = {0963-0252},
    doi = {10.1088/0963-0252/19/1/015008},
    issn = {0963-0252}
}

@article{Alves2012,
    title = {{Capacitively coupled radio-frequency discharges in nitrogen at low pressures}},
    year = {2012},
    journal = {Plasma Sources Science and Technology},
    author = {Alves, L. L. and Marques, L and Pintassilgo, C D and Wattieaux, G and Es-sebbar, Et and Berndt, J and Kovacevi{\'{c}}, E and Carrasco, N and Boufendi, L and Cernogora, G},
    number = {4},
    pages = {045008},
    volume = {21},
    doi = {10.1088/0963-0252/21/4/045008},
    issn = {0963-0252}
}

@article{Desai2017,
    title = {{Carbon chain anions and the growth of complex organic molecules in Titan's ionosphere}},
    year = {2017},
    journal = {The Astrophysical Journal Letters},
    author = {Desai, R. T. and Coates, A. J. and Wellbrock, A. and Vuitton, V. and Crary, F. J. and Gonz{\'{a}}lez-Caniulef, D. and Shebanits, O. and Jones, G. H. and Lewis, G. R. and Waite, J. H. and Taylor, S. A. and Kataria, D. O. and Wahlund, J. -E. and Edberg, N. J. T. and Sittler, E. C.},
    number = {2},
    pages = {1--8},
    volume = {844},
    publisher = {IOP Publishing},
    url = {http://arxiv.org/abs/1706.01610},
    doi = {10.3847/2041-8213/aa7851},
    issn = {2041-8213},
    arxivId = {1706.01610},
    keywords = {- planets and satellites, and satellites, astrobiology - ism, atmospheres - planets, composition - astrochemistry -, individual, molecules, planets and satellites, titan}
}

@article{He,
    title = {{Carbon Monoxide Affecting Planetary Atmospheric Chemistry}},
    author = {He, Chao and H{\"{o}}rst, Sarah M and Riemer, Sydney and Sebree, Joshua A and Vuitton, Véronique},
    pages = {1--17}
}

@article{Cassini2004,
    title = {{Cassini and saturn}},
    year = {2004},
    journal = {European Space Agency, (Special Publication) ESA SP},
    author = {Cassini, Anna},
    number = {1278},
    pages = {31--41},
    isbn = {92-9092-997-9},
    issn = {03796566}
}

@article{Wellbrock2013,
    title = {{Cassini CAPS-ELS observations of negative ions in Titan's ionosphere: Trends of density with altitude}},
    year = {2013},
    journal = {Geophysical Research Letters},
    author = {Wellbrock, A. and Coates, A. J. and Jones, G. H. and Lewis, G. R. and Waite, J. H.},
    number = {17},
    pages = {4481--4485},
    volume = {40},
    doi = {10.1002/grl.50751},
    issn = {00948276},
    keywords = {Titan, aerosol, atmosphere, electron attachment, ionosphere, negative ions}
}

@article{Samuelson2007,
    title = {{Cassini CIRS update on stratospheric ices at Titan's winter pole}},
    year = {2007},
    journal = {Icarus},
    author = {Samuelson, Robert E. and Smith, Michael D. and Achterberg, R. K. and Pearl, John C.},
    number = {1},
    pages = {63--71},
    volume = {189},
    doi = {10.1016/j.icarus.2007.02.005},
    issn = {00191035},
    keywords = {Atmospheres, IR spectroscopy, Ices, Titan, composition}
}

@article{Waite2017,
    title = {{Cassini finds molecular hydrogen in the Enceladus plume: Evidence for hydrothermal processes}},
    year = {2017},
    journal = {Science},
    author = {Waite, J Hunter and Glein, Christopher R and Perryman, Rebecca S and Teolis, Ben D and Magee, Brian A and Miller, Greg and Grimes, Jacob and Perry, Mark E and Miller, Kelly E and Bouquet, Alexis and Lunine, Jonathan I and Brockwell, Tim and Bolton, Scott J},
    number = {6334},
    pages = {155--159},
    volume = {356}
}

@article{West2016,
    title = {{Cassini Imaging Science Subsystem observations of Titan's south polar cloud}},
    year = {2016},
    journal = {Icarus},
    author = {West, R. A. and Del Genio, A. D. and Barbara, J. M. and Toledo, D. and Lavvas, P. and Rannou, P. and Turtle, E. P. and Perry, J.},
    pages = {399--408},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.11.038},
    doi = {10.1016/j.icarus.2014.11.038},
    issn = {10902643},
    keywords = {Titan, Titan, atmosphere, Titan, clouds}
}

@article{Porco2005a,
    title = {{Cassini imaging science: Instrument characteristics and anticipated scientific investigations at Saturn}},
    year = {2005},
    journal = {Space Science Reviews},
    author = {Porco, Carolyn C. and West, Robert A. and Squyres, Steven and McEwen, Alfred and Thomas, Peter and Murray, Carl D. and Delgenio, Anthony and Ingersoll, Andrew P. and Johnson, Torrence V. and Neukum, Gerhard and Veverka, Joseph and Dones, Luke and Brahic, Andre and Burns, Joseph A. and Haemmerle, Vance and Knowles, Benjamin and Dawson, Douglas and Roatsch, Thomas and Beurle, Kevin and Owen, William},
    number = {1-4},
    pages = {363--497},
    volume = {115},
    isbn = {978-1-4020-3147-2},
    doi = {10.1007/s11214-004-1456-7},
    issn = {00386308},
    keywords = {Cassini, Imaging, Moons, Rings, Saturn}
}

@article{Porco2005b,
    title = {{Cassini imaging science: Instrument characteristics and anticipated scientific investigations at Saturn}},
    year = {2005},
    journal = {Space Science Reviews},
    author = {Porco, Carolyn C. and West, Robert A. and Squyres, Steven and McEwen, Alfred and Thomas, Peter and Murray, Carl D. and Delgenio, Anthony and Ingersoll, Andrew P. and Johnson, Torrence V. and Neukum, Gerhard and Veverka, Joseph and Dones, Luke and Brahic, Andre and Burns, Joseph A. and Haemmerle, Vance and Knowles, Benjamin and Dawson, Douglas and Roatsch, Thomas and Beurle, Kevin and Owen, William},
    number = {1-4},
    pages = {363--497},
    volume = {115},
    isbn = {978-1-4020-3147-2},
    doi = {10.1007/s11214-004-1456-7},
    issn = {00386308},
    keywords = {Cassini, Imaging, Moons, Rings, Saturn}
}

@article{Porco2004,
    title = {{Cassini Imaging Science: Instrument Characteristics And Anticipated Scientific Investigations At Saturn}},
    year = {2004},
    journal = {Space Science Reviews},
    author = {Porco, C.C. Carolyn C and West, Robert A R.A. and Squyres, Steven and McEwen, Alfred and Thomas, Peter and Murray, Carl D C.D. and Delgenio, A. and Ingersoll, Andrew P A.P. and Johnson, T.V. Torrence V and Neukum, Gerhard and Veverka, Joseph and Dones, Luke and Brahic, Andre and Burns, J.A. Joseph A and Haemmerle, Vance and Knowles, Benjamin and Dawson, Douglas and Roatsch, Thomas and Beurle, Kevin and Owen, William and Del Genio, Anthony and Ingersoll, Andrew P A.P. and Johnson, T.V. Torrence V and Neukum, Gerhard and Veverka, Joseph and Dones, Luke and Brahic, Andre and Burns, J.A. Joseph A and Haemmerle, Vance and Knowles, Benjamin and Dawson, Douglas and Roatsch, Thomas and Beurle, Kevin and Owen, William},
    number = {1-4},
    pages = {363},
    volume = {115},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-data_query?bibcode=2004SSRv..115..363P&link_type=ABSTRACT%0Apapers3://publication/doi/10.1007/s11214-004-1456-7},
    doi = {10.1007/s11214-004-1456-7},
    issn = {00386308},
    keywords = {Cassini, Imaging, Moons, Rings, Saturn}
}

@article{Kunde1996,
    title = {{Cassini infrared Fourier spectroscopic investigation}},
    year = {1996},
    journal = {Proceedings of SPIE},
    author = {Kunde, Virgil G. and Ade, Peter A. R. and Barney, Richard D. and Bergman, D. and Bonnal, Jean-Francois and Borelli, R. and Boyd, David and Brasunas, John C. and Brown, Gregory V. and Calcutt, Simon B. and Carroll, F. and Courtin, R. and Cretolle, Jacky B. and Crooke, Julie A. and Davis, Martin A. and Edberg, S. and Fettig, Rainer K. and Flasar, M. and Glenar, David A. and Graham, S. and Hagopian, John G. and Hakun, Claef F. and Hayes, Patricia A. and Herath, L. and Spilker, Linda and Jennings, Donald E. and Karpati, Gabriel and Kellebenz, C. and Lakew, Brook and Lindsay, J. and Lohr, J. and Lyons III, James J. and Martineau, Robert J. and Martino, Anthony J. and Matsumura, Mack and McCloskey, J. and Melak, T. and Michel, Guy and Morrell, Armando and Mosier, C. and Pack, LaTunia G. and Plants, M. and Robinson, D. and Rodriguez, Louis and Romani, Paul and Schaefer, Bill and Schmidt, Stephen M. and Trujillo, Carlos and Vellacott, Tim and Wagner, K. and Yun, D.},
    number = {October},
    pages = {162--177},
    url = {http://proceedings.spiedigitallibrary.org/proceeding.aspx?articleid=1020839},
    doi = {10.1117/12.253416}
}

@article{Perry2015,
    title = {{Cassini INMS measurements of Enceladus plume density}},
    year = {2015},
    journal = {Icarus},
    author = {Perry, M.E. and Teolis, B.D. and Hurley, D.M. and Magee, B.A. and Waite, J.H. and Brockwell, T.G. and Perryman, R.S. and McNutt, R.L.},
    pages = {139--162},
    volume = {257},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103515001803},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2015.04.037},
    issn = {00191035}
}

@article{Wahlund2005,
    title = {{Cassini Measurements of Cold Plasma in the Ionosphere of Titan}},
    year = {2005},
    journal = {Science},
    author = {Wahlund, J.-E.},
    number = {5724},
    pages = {986--989},
    volume = {308},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/15894529%5Cnhttp://www.sciencemag.org/cgi/doi/10.1126/science.1109807},
    isbn = {1095-9203 (Electronic){\textbackslash}r0036-8075 (Linking)},
    doi = {10.1126/science.1109807},
    issn = {0036-8075},
    pmid = {15894529},
    keywords = {Atmosphere, Extraterrestrial Environment, Ions, Magnetics, Saturn, Spacecraft, Temperature}
}

@article{Porco2006,
    title = {{Cassini observes the active south pole of enceladus}},
    year = {2006},
    journal = {Science},
    author = {Porco, C. C. and Helfenstein, P. and Thomas, P. C. and Ingersoll, A. P. and Wisdom, J. and West, R. and Neukum, G. and Denk, T. and Wagner, R. and Roatsch, T. and Kieffer, S. and Turtle, E. and McEwen, A. and Johnson, T. V. and Rathbun, J. and Veverka, J. and Wilson, D. and Perry, J. and Spitale, J. and Brahic, A. and Burns, J. A. and DelGenio, A. D. and Dones, L. and Murray, C. D. and Squyres, S.},
    number = {5766},
    pages = {1393--1401},
    volume = {311},
    isbn = {0036-8075},
    doi = {10.1126/science.1123013},
    issn = {00368075},
    pmid = {16527964}
}

@article{Young2004,
    title = {{Cassini Plasma Spectrometer Investigation}},
    year = {2004},
    journal = {Space Science Reviews},
    author = {Young, D. T.},
    pages = {1--112}
}

@article{PhaseAreport1988,
    title = {{CASSINI. Report on the Phase A study: Saturn Orbiter and Titan probe}},
    year = {1988},
    author = {Aeronaut, National},
    url = {https://ntrs.nasa.gov/search.jsp?R=19910008874}
}

@book{Rodriguez2006,
    title = {{Cassini/VIMS hyperspectral observations of the HUYGENS landing site on Titan}},
    year = {2006},
    booktitle = {Planetary and Space Science},
    author = {Rodriguez, S. and Le Mou{\'{e}}lic, S. and Sotin, C. and Cl{\'{e}}net, H. and Clark, R. N. and Buratti, B. and Brown, R. H. and McCord, T. B. and Nicholson, P. D. and Baines, K. H.},
    number = {15},
    pages = {1510--1523},
    volume = {54},
    isbn = {1481624032},
    doi = {10.1016/j.pss.2006.06.016},
    issn = {00320633},
    arxivId = {0906.5476},
    keywords = {Near-infrared, Satellites, Spectro-imaging, Titan, VIMS}
}

@article{Coradini2004,
    title = {{CASSINI/VIMS-V at Jupiter: Radiometric calibration test and data results}},
    year = {2004},
    journal = {Planetary and Space Science},
    author = {Coradini, A. and Filacchione, G. and Capaccioni, F. and Cerroni, P. and Adriani, A. and Brown, R. H. and Langevin, Y. and Gondet, B.},
    number = {7},
    pages = {661--670},
    volume = {52},
    doi = {10.1016/j.pss.2003.11.005},
    issn = {00320633}
}

@article{Dubois2017,
    title = {{Cation Chemistry in Titan’s Upper Atmosphere and its Influence on Tholin Formation}},
    year = {2017},
    journal = {EPSC 2017},
    author = {Dubois, D. and Carrasco, N. and Jovanovic, L. and Vettier, L},
    pages = {1--2},
    volume = {11}
}

@article{Nimmo2002,
    title = {{Causes, characteristics and consequences of convective diapirism on Europa}},
    year = {2002},
    journal = {Geophysical Research Letters},
    author = {Nimmo, Francis and Manga, Michael},
    number = {23},
    pages = {24},
    volume = {29 VN - r},
    url = {/Users/erinleonard/Desktop/Europa/Papers/Nimmo and Manga 2002.pdf%5Cnhttp://dx.doi.org/10.1029/2002GL015754},
    doi = {10.1029/2002GL015754},
    issn = {1944-8007},
    keywords = {doi:10.102, http://dx.doi.org/10.1029/2002GL015754}
}

@article{Romanini2007,
    title = {{Cavity ringdown overtone spectroscopy of HCN , H13CN and HC15N Cavity ring-down overtone spectroscopy of HCN , H 13 CN and HC 15 N}},
    year = {2007},
    author = {Romanini, Daniele and Lehmann, Kevin K and Romanini, Daniele and Lehmann, Kevin K},
    number = {1995},
    volume = {633},
    doi = {10.1063/1.469462}
}

@article{Stevenson1999,
    title = {{ch17: Tidal Dissipation and Evolution}},
    year = {1999},
    author = {Stevenson, D. J.},
    pages = {187--199}
}

@article{Hoppa,
    title = {{Change detection on Europa and Io from Voyager and Galileo images}},
    author = {Hoppa, G V and Geissler, P E and Pappalardo, R and Greeley, R and Klemaszewski, J and Simonelli, D P and Sullivan, R and Uni-, Brown}
}

@article{Rannou2000,
    title = {{Characterization of Aerosols in the Detached Haze Layer of Titan}},
    year = {2000},
    journal = {Icarus},
    author = {Rannou, P and Ferrari, C and Rages, K and Roos-Serote, M and Cabane, M},
    pages = {267--281},
    volume = {147},
    doi = {10.1006/icar.2000.6416},
    issn = {00191035}
}

@article{Mahjoub2016,
    title = {{Characterization of aromaticity in analogues of Titan’s atmospheric aerosols with Two‐ Step Laser Desorption Ionization Mass Spectrometry}},
    author = {Mahjoub, Ahmed and Schwell, Martin and Carrasco, Nathalie and Benilan, Yves and Cernogora, Guy},
    pages = {1--41},
    keywords = {aerosols, aromatics, l2di-, ms, s atmosphere, titan}
}

@article{Olah2016,
    title = {{Chemical Aspects of Astrophysically Observed Extraterrestrial Methanol, Hydrocarbon Derivatives, and Ions}},
    year = {2016},
    journal = {Journal of the American Chemical Society},
    author = {Olah, George A. and Mathew, Thomas and Prakash, G. K.Surya and Rasul, Golam},
    number = {5},
    pages = {1717--1722},
    volume = {138},
    isbn = {0002-7863},
    doi = {10.1021/jacs.6b00343},
    issn = {15205126}
}

@article{Carrasco2009,
    title = {{Chemical characterization of titan's tholins: Solubility, morphology and molecular structure revisited}},
    year = {2009},
    journal = {Journal of Physical Chemistry A},
    author = {Carrasco, N. and Schmitz-Afonso, I. and Bonnet, J. Y. and Quirico, E. and Thissen, R. and Dutuit, Odile and Bagag, A. and Lapr{\'{e}}vote, O. and Buch, A. and Giulani, A. and Adand{\'{e}}, Gilles and Ouni, F. and Hadamcik, E. and Szopa, C. and Cernogora, G.},
    number = {42},
    pages = {11195--11203},
    volume = {113},
    isbn = {1089-5639},
    doi = {10.1021/jp904735q},
    issn = {10895639},
    pmid = {19827851}
}

@article{Krasnopolsky2014,
    title = {{Chemical composition of Titan’s atmosphere and ionosphere: Observations and the photochemical model}},
    year = {2014},
    journal = {Icarus},
    author = {Krasnopolsky, Vladimir a.},
    pages = {83--91},
    volume = {236},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.03.041},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2006.04.019},
    issn = {00320633},
    keywords = {Atmosphere, Chemical composition, Clouds, Spectroscopy, Venus}
}

@article{McDonald1994a,
    title = {{Chemical investigation of Titan and Triton Tholins}},
    year = {1994},
    journal = {Icarus},
    author = {McDonald, G D and Thompson, W. R. and Heinrich, M. and Khare, Bishun N. and Sagan, Carl},
    pages = {137--145},
    volume = {108},
    publisher = {Icarus}
}

@article{McDonald1994,
    title = {{Chemical Investigation of Titan and Triton Tholins}},
    year = {1994},
    journal = {Icarus},
    author = {McDonald, G D and Reid Thompson, W. and Heinrich, M. and Khare, B. N. and Sagan, C.},
    pages = {137--145},
    volume = {108}
}

@article{Chau2011,
    title = {{Chemical processes in the deep interior of Uranus.}},
    year = {2011},
    journal = {Nature communications},
    author = {Chau, Ricky and Hamel, Sebastien and Nellis, William J},
    pages = {203},
    volume = {2},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/ncomms1198},
    doi = {10.1038/ncomms1198},
    issn = {2041-1723},
    pmid = {21343921}
}

@article{Kovacs2010,
    title = {{Chemical reactions in the Titan's troposphere during lightning}},
    year = {2010},
    journal = {Icarus},
    author = {Kov{\'{a}}cs, Tamás and Tur{\'{a}}nyi, Tamás},
    number = {2},
    pages = {938--947},
    volume = {207},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.01.001},
    doi = {10.1016/j.icarus.2010.01.001},
    issn = {00191035},
    keywords = {Lightning, Titan}
}

@article{Wilson2003,
    title = {{Chemical sources of haze formation in Titan's atmosphere}},
    year = {2003},
    journal = {Planetary and Space Science},
    author = {Wilson, E. H. and Atreya, S. K.},
    number = {14-15},
    pages = {1017--1033},
    volume = {51},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2003.06.003},
    issn = {00320633},
    keywords = {Atmospheric composition, Organic chemistry, Photochemistry, Titan}
}

@article{Strobel1982,
    title = {{Chemistry and evolution of Titan's atmosphere}},
    year = {1982},
    journal = {Planetary and Space Science},
    author = {Strobel, D. F.},
    number = {8},
    pages = {839--848},
    volume = {30},
    isbn = {0032063318},
    doi = {10.1016/0032-0633(82)90116-7},
    issn = {00320633}
}

@book{Rehder2010,
    title = {{Chemistry in Space: From Interstellar Matter to the Origin of Life}},
    year = {2010},
    booktitle = {Chemistry in Space: From Interstellar Matter to the Origin of Life},
    author = {Rehder, Dieter},
    isbn = {9783527326891},
    doi = {10.1002/9783527631605}
}

@article{Molina-Cuberos1999,
    title = {{Chemistry of the galactic cosmic ray induced ionosphere of Titan}},
    year = {1999},
    journal = {Journal of Geophysical Research},
    author = {Molina-Cuberos, G.J. and Lopez-Moreno, J. J. and Rodrigo, R.},
    volume = {104}
}

@article{Gordon1995,
    title = {{CHN2-: A biradical anion and a potentially new type of reactive intermediate}},
    year = {1995},
    journal = {Journal of Physical Chemistry},
    author = {Gordon, Mark S. and Kass, Steven R.},
    number = {17},
    pages = {6548--6550},
    volume = {99},
    doi = {10.1021/j100017a040},
    issn = {00223654}
}

@article{Louwman2004,
    title = {{Christiaan Huygens and his telescopes}},
    year = {2004},
    journal = {Proceedings of the International Conference "Titan - from discovery to encounter"},
    author = {Louwman, Peter}
}

@article{Cohen2004,
    title = {{Christiaan Huygens and the Scientific Revolution}},
    year = {2004},
    author = {Cohen, H Floris},
    number = {April},
    pages = {1--11},
    volume = {1}
}

@article{Carlson2016,
    title = {{Chromophores from Photolyzed Ammonia Reacting with Acetylene: Application to Jupiter{\{}{\textbackslash}rsquo{\}}s Great Red Spot}},
    year = {2016},
    journal = {AAS/Division for Planetary Sciences Meeting Abstracts},
    author = {Carlson, R.~W. and Baines, K.~H. and Anderson, M.~S. and Filacchione, G},
    pages = {{\#}205.01},
    volume = {44},
    publisher = {Elsevier Inc.},
    doi = {10.1016/j.icarus.2016.03.008},
    issn = {00191035},
    keywords = {"Atmospheres, "Jupiter, Organic chemistry, Photochemistry, atmosphere", chemistry", composition"}
}

@article{Nna-Mvondo2018,
    title = {{CIRS-Observed Titan’s Stratospheric Ice Clouds Studied in the Laboratory}},
    year = {2018},
    journal = {American Astronomical Society, AAS Meeting {\#}232, id.{\#}313.03},
    author = {Nna-Mvondo, Delphine and Anderson, Carrie; and Samuelson, Robert E.}
}

@article{Uk2007,
    title = {{Climate Models and Their Evaluation}},
    year = {2007},
    journal = {Evaluation},
    author = {Uk, Richard A Wood},
    pages = {589--662},
    volume = {323},
    url = {http://scholar.google.com/scholar?hl=en&btnG=Search&q=intitle:Climate+Models+and+Their+Evaluation#0},
    isbn = {book pdf},
    doi = {10.1016/j.cub.2007.06.045},
    issn = {09609822},
    pmid = {17629484}
}

@article{Brown2010,
    title = {{Clouds on Titan during the Cassini prime mission: A complete analysis of the VIMS data}},
    year = {2010},
    journal = {Icarus},
    author = {Brown, Michael E. and Roberts, Jessica E. and Schaller, Emily L.},
    number = {2},
    pages = {571--580},
    volume = {205},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.08.024},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.08.024},
    issn = {00191035},
    pmid = {274599400019},
    keywords = {Atmospheres, dynamics, Satellites, atmospheres, Titan}
}

@article{Kim2005,
    title = {{Clouds, haze, and CH4, CH3D, HCN, and C2 H2 in the atmosphere of Titan probed via 3 µm spectroscopy}},
    year = {2005},
    journal = {Icarus},
    author = {Kim, Sang J. and Geballe, T. R. and Noll, Keith S. and Courtin, Regis},
    number = {2},
    pages = {522--532},
    volume = {173},
    doi = {10.1016/j.icarus.2004.09.006},
    issn = {00191035},
    keywords = {Atmosphere, Clouds, Infrared, Molecules, Titan}
}

@article{Takeya2003,
    title = {{Coexistence of structure I and II hydrates formed from a mixture of methane and ethane gases}},
    year = {2003},
    journal = {Canadian Journal of Physics},
    author = {Takeya, S and Kamata, Y and Uchida, T and Nagao, J and Ebinuma, T and Narita, H and Hori, A and Hondoh, T},
    number = {1-2},
    pages = {479--484},
    volume = {81},
    url = {http://www.nrcresearchpress.com/doi/10.1139/p03-038},
    doi = {10.1139/p03-038},
    issn = {0008-4204},
    pmid = {607}
}

@article{Romanzin2010,
    title = {{Combined experimental and theoretical studies on methane photolysis at 121.6 and 248nm—implications on a program of laboratory simulations of Titan’s atmosphere}},
    year = {2010},
    journal = {Planetary and Space Science},
    author = {Romanzin, C. and Arzoumanian, E. and Es-sebbar, Et. and Jolly, A. and Perrier, S. and Gazeau, M.-C. and B{\'{e}}nilan, Y.},
    number = {13},
    month = {11},
    pages = {1748--1757},
    volume = {58},
    url = {http://www.sciencedirect.com/science/article/pii/S0032063310002035},
    doi = {10.1016/j.pss.2010.07.001},
    issn = {00320633},
    keywords = {Experimental simulations, Hydrocarbons, Methane, Photochemical model, Titan, UV photolysis}
}

@article{Oro1961,
    title = {{Comets and the Formation of Biochemical Compounds on the Primitive Earth}},
    year = {1961},
    journal = {Nature},
    author = {Or{\'{o}}, J.},
    pages = {775--776},
    volume = {189}
}

@article{Hamelin2009,
    title = {{Comment on "Evidence of electrical activity on Titan drawn from the Schumann resonances sent by Huygens probe" by J.A. Morente, J.A. Port{\'{i}}, A. Salinas, E.A. Navarro [2008, Icarus, 195, 802-811]}},
    year = {2009},
    journal = {Icarus},
    author = {Hamelin, M. and Grard, R. and L{\'{o}}pez-Moreno, J. J. and Schwingenschuh, K. and B{\'{e}}ghin, C. and Berthelier, J. J. and Simões, F.},
    number = {1},
    pages = {349--351},
    volume = {204},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.01.031},
    doi = {10.1016/j.icarus.2009.01.031},
    issn = {00191035},
    keywords = {Instrumentation, Ionospheres, Lightning, Titan}
}

@misc{Huttenlocher1993,
    title = {{Comparing images using the Hausdorff distance}},
    year = {1993},
    author = {Huttenlocher, D. P. and Kanderman, G. A. and Rucklidge, W. J.}
}

@misc{Bouts1993,
    title = {{Comparing images using the Hausdorff distance}},
    year = {1993},
    author = {Bouts, M.}
}

@article{Wordsworth2015,
    title = {{Comparison of "warm and wet" and "cold and icy" scenarios for early Mars in a 3-D climate model}},
    year = {2015},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Wordsworth, Robin D. and Kerber, Laura and Pierrehumbert, Raymond T. and Forget, Francois and Head, James W.},
    number = {6},
    pages = {1201--1219},
    volume = {120},
    doi = {10.1002/2015JE004787},
    issn = {21699100},
    arxivId = {1506.04817},
    keywords = {astrobiology, atmospheres, early Mars, hydrology, paleoclimate, valley networks}
}

@article{Hoppaa,
    title = {{Comparison of Global Stress Models with Geographical Features on Europa}},
    author = {Hoppa, Gregory and Greenberg, Richard and Geissler, Paul and Tufts, B R and Phillips, C B and Durda, Daniel}
}

@article{Maillard2018,
    title = {{Comparison of soluble and insoluble organic matter in analogues of Titan ’ s aerosols}},
    year = {2018},
    journal = {Earth and Planetary Science Letters},
    author = {Maillard, Julien and Carrasco, Nathalie and Schmitz-afonso, Isabelle and Gautier, Thomas and Afonso, Carlos},
    pages = {185--191},
    volume = {495},
    url = {https://doi.org/10.1016/j.epsl.2018.05.014},
    doi = {10.1016/j.epsl.2018.05.014},
    issn = {0012-821X}
}

@article{Abplanalp2016,
    title = {{Complex Hydrocarbon Chemistry in Interstellar and Solar System Ices Revealed: a Combined Infrared Spectroscopy and Reflectron Time-of-Flight Mass Spectrometry Analysis of Ethane (C 2 H 6 ) and D6-Ethane (C 2 D 6 ) Ices Exposed To Ionizing Radiation}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Abplanalp, Matthew J. and Kaiser, Ralf I.},
    number = {2},
    pages = {132},
    volume = {827},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/827/i=2/a=132?key=crossref.e36fa002a65aa56bb2485664e68cf69e},
    doi = {10.3847/0004-637X/827/2/132},
    issn = {1538-4357},
    keywords = {ISM: molecules, astrochemistry, cosmic rays, general, infrared, infrared: general, ism, laboratory, methods, methods: laboratory: solid state, molecules, non-thermal, radiation mechanisms, radiation mechanisms: non-thermal, solid state}
}

@article{Israel2005,
    title = {{Complex organic matter in Titan's atmospheric aerosols from in situ pyrolysis and analysis.}},
    year = {2005},
    journal = {Nature},
    author = {Israel, G. L. and Szopa, C. and Raulin, F and Cabane, M. and Niemann, Hasso B. and Atreya, Sushil K. and Bauer, S. J. and Brun, J-F and Chassefi{\`{e}}re, Eric and Coll, P. and Cond{\'{e}}, E and Coscia, D. and Hauchecorne, a and Millian, P and Nguyen, M.-J. and Owen, Tobias and Riedler, W and Samuelson, R E and Siguier, J-M and Steller, M and Sternberg, R and Vidal-Madjar, C},
    number = {7069},
    pages = {796--799},
    volume = {438},
    isbn = {1476-4687 (Electronic)},
    doi = {10.1038/nature04349},
    issn = {0028-0836},
    pmid = {16319825}
}

@article{Biemann2006,
    title = {{Complex organic matter in Titan’s aerosols?}},
    year = {2006},
    journal = {Nature},
    author = {Biemann, K},
    number = {November},
    pages = {E6},
    volume = {444},
    doi = {10.038/nature05417}
}

@article{Ramirez2002,
    title = {{Complex Refractive Index of Titan's Aerosol Analogues in the 200–900 nm Domain}},
    year = {2002},
    journal = {Icarus},
    author = {Ramirez, S and Coll, P and da Silva, A and Navarro-Gonz{\'{a}}lez, R and Lafait, J and Raulin, F},
    number = {2},
    pages = {515--529},
    volume = {156},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103501967831},
    isbn = {00191035},
    doi = {10.1006/icar.2001.6783},
    issn = {00191035},
    keywords = {complex refractive, s aerosols, tholins, titan}
}

@article{Bezard2009,
    title = {{Composition and chemistry of Titan's stratosphere.}},
    year = {2009},
    journal = {Philosophical transactions. Series A, Mathematical, physical, and engineering sciences},
    author = {B{\'{e}}zard, B.},
    number = {1889},
    pages = {683--695},
    volume = {367},
    doi = {10.1098/rsta.2008.0233},
    issn = {1364-503X},
    pmid = {19019784},
    keywords = {chemistry, composition, haze, stratosphere, titan}
}

@article{Vuitton2009,
    title = {{Composition and chemistry of Titan's thermosphere and ionosphere}},
    year = {2009},
    journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
    author = {Vuitton, V and Yelle, R.V and Lavvas, P},
    number = {1889},
    pages = {729--741},
    volume = {367},
    url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.2008.0233},
    isbn = {1364-503X},
    doi = {10.1098/rsta.2008.0233},
    issn = {1364-503X},
    pmid = {19019784},
    keywords = {atmospheres, composition, ionospheres, titan}
}

@article{Cravens2006,
    title = {{Composition of Titan's ionosphere}},
    year = {2006},
    journal = {Geophysical Research Letters},
    author = {Cravens, T. E. and Robertson, I. P. and Waite, Jr H. and Yelle, R. V. and Kasprzak, W. T. and Keller, C. N. and Ledvina, S. A. and Niemann, H. B. and Luhmann, J. G. and McNutt, R. L. and Ip, W. H. and De La Haye, V. and Mueller-Wodarg, I. and Wahlund, J. E. and Anicich, V. G. and Vuitton, V.},
    number = {7},
    pages = {8--11},
    volume = {33},
    doi = {10.1029/2005GL025575},
    issn = {00948276}
}

@article{LeGall2016,
    title = {{Composition, seasonal change, and bathymetry of Ligeia Mare, Titan, derived from its microwave thermal emission}},
    year = {2016},
    journal = {AGU Publications},
    author = {Le Gall, A. and Malaska, M. J. and Lorenz, R.D and Janssen, M. A. and Tokano, T. and Hayes, A. G. and Mastrogiuseppe, M. and Lunine, J. I. and Veyssiere, G. and Encrenaz, P. J. and Karatekin, O.},
    pages = {1--29},
    doi = {10.1002/2014JE004627.Received},
    issn = {2169-9100},
    keywords = {10.1002/2014JE004627 and CRISM, MICA, Mars, mineral, spectral parameter, summary product}
}

@article{Bonnefoy2016,
    title = {{Compositional and spatial variations in Titan dune and interdune regions from Cassini VIMS and RADAR}},
    year = {2016},
    journal = {Icarus},
    author = {Bonnefoy, Léa E. and Hayes, Alexander G. and Hayne, Paul O. and Malaska, Michael J. and Le Gall, Alice and Solomonidou, Anezina and Lucas, Antoine},
    pages = {222--237},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.09.014},
    doi = {10.1016/j.icarus.2015.09.014},
    issn = {10902643},
    keywords = {Infrared observations, Radar observations, Surface, Titan}
}

@article{Osegovic2005,
    title = {{Compound clathrate hydrate on Titan's surface}},
    year = {2005},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Osegovic, John P. and Max, Michael D.},
    number = {8},
    pages = {1--6},
    volume = {110},
    isbn = {0148-0227},
    doi = {10.1029/2005JE002435},
    issn = {01480227},
    keywords = {http://dx.doi.org/10.1029/2005JE002435, doi:10.102}
}

@article{Maurice1996,
    title = {{Comprehensive analysis of electron observations at Saturn: Voyager 1 and 2}},
    year = {1996},
    journal = {Journal of Geophysical Research},
    author = {Maurice, S. and Sittler, E. C. and Cooper, J. F. and Mauk, B. H. and Blanc, M and Selesnick, R. S.},
    volume = {101},
    keywords = {doi:10.1029/9, http://dx.doi.org/10.1029/96JA00765}
}

@article{Marin2017,
    title = {{Computation of the transmitted and polarized scattered fluxes by the exoplanet HD 189733b in X-rays}},
    year = {2017},
    author = {Marin, F. and Grosso, N.},
    number = {2013},
    url = {http://arxiv.org/abs/1701.00990},
    arxivId = {1701.00990},
    keywords = {hd 189733, individual, planetary systems, polarimetric, radiative transfer, stars, techniques, x-rays}
}

@article{Gudipati2000,
    title = {{Concentration dependence of the spectroscopic and photochemical properties of atomic and molecular oxygen in argon matrices}},
    year = {2000},
    journal = {Spectrochimica Acta - Part A: Molecular and Biomolecular Spectroscopy},
    author = {Gudipati, Murthy S. and Schouren, Frank and Kalb, Martin and Wagner, Robert},
    number = {13},
    pages = {2581--2588},
    volume = {56},
    doi = {10.1016/S1386-1425(00)00366-8},
    issn = {13861425},
    keywords = {atomic oxygen, matrix isolation, molecular oxygen clusters, vacuum uv spectroscopy}
}

@article{Lavvas2011c,
    title = {{Condensation in Titan's atmosphere at the Huygens landing site}},
    year = {2011},
    journal = {Icarus},
    author = {Lavvas, P. and Griffith, C. A. and Yelle, R. V.},
    number = {2},
    pages = {732--750},
    volume = {215},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.06.040},
    doi = {10.1016/j.icarus.2011.06.040},
    issn = {00191035},
    keywords = {Titan}
}

@article{Sanchez1966,
    title = {{Conditions for Purine Synthesis: Did Prebiotic Synthesis Occur at Low Temperatures?}},
    year = {1966},
    journal = {Science},
    author = {Sanchez, R. and Ferris, J. P. and Orgel, L. E.},
    number = {4},
    pages = {677--686},
    volume = {36},
    isbn = {0506006905},
    doi = {10.1007/sl0869-007-9037-x},
    issn = {0506006905},
    pmid = {15869632}
}

@article{Ledvina2012,
    title = {{Consequences of negative ions for Titan's plasma interaction}},
    year = {2012},
    journal = {Geophysical Research Letters},
    author = {Ledvina, Stephen A. and Brecht, Stephen H.},
    number = {20},
    pages = {1--5},
    volume = {39},
    doi = {10.1029/2012GL053835},
    issn = {00948276},
    keywords = {Titan, ionosphere, negative ions, plasma interaction}
}

@article{Fagents2003,
    title = {{Considerations for effusive cryovolcanism on Europa: The post-Galileo perspective}},
    year = {2003},
    journal = {Journal of Geophysical Research},
    author = {Fagents, Sarah a.},
    number = {E12},
    pages = {5139},
    volume = {108},
    url = {http://doi.wiley.com/10.1029/2003JE002128},
    doi = {10.1029/2003JE002128},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/2003JE002128, doi:10.102}
}

@article{Rocha2015,
    title = {{Constraining Fundamental Physics with Planck Gra{\c{c}}a Rocha JPL / Caltech}},
    year = {2015},
    author = {Rocha, G.},
    number = {January}
}

@article{Michaelides2016,
    title = {{Constraining the physical properties of Titan's empty lake basins using nadir and off-nadir Cassini RADAR backscatter}},
    year = {2016},
    journal = {Icarus},
    author = {Michaelides, R. J. and Hayes, A. G. and Mastrogiuseppe, M. and Zebker, H. A. and Farr, T. G. and Malaska, M. J. and Poggiali, V. and Mullen, J. P.},
    pages = {57--66},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.09.043},
    doi = {10.1016/j.icarus.2015.09.043},
    issn = {10902643},
    keywords = {Radar observations, Titan, Titan, hydrology, Titan, surface}
}

@article{Pearce,
    title = {{Constraining the Time Interval for the Origin of Life on Earth}},
    journal = {Astrobiology},
    author = {Pearce, Ben K D and Tupper, Andrew S and Pudritz, Ralph E and Higgs, Paul G},
    pages = {1--43},
    keywords = {astrobiology, biosignatures, early earth, geochemistry, habitability, origin of life}
}

@article{Rhoden2010,
    title = {{Constraints on Europa's rotational dynamics from modeling of tidally-driven fractures}},
    year = {2010},
    journal = {Icarus},
    author = {Rhoden, Alyssa Rose and Militzer, Burkhard and Huff, Eric M. and Hurford, Terry A. and Manga, Michael and Richards, Mark A.},
    number = {2},
    pages = {770--784},
    volume = {210},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.07.018},
    doi = {10.1016/j.icarus.2010.07.018},
    issn = {00191035},
    keywords = {Europa, Rotational dynamics, Tectonics}
}

@article{Gao2016,
    title = {{Constraints on the microphysics of Pluto's photochemical haze from New Horizons observations}},
    year = {2016},
    journal = {Icarus},
    author = {Gao, Peter and Fan, Siteng and Wong, Michael L. and Liang, Mao Chang and Shia, Run Lie and Kammer, Joshua A. and Yung, Yuk L. and Summers, Michael E. and Gladstone, G. Randall and Young, Leslie A. and Olkin, Catherine B. and Ennico, Kimberly and Weaver, Harold A. and Stern, S. Alan},
    pages = {1--30},
    doi = {10.1016/j.icarus.2016.09.030},
    issn = {10902643},
    keywords = {Abundances, atmospheres, Atmospheres, chemistry, Atmospheres, composition, Pluto, Pluto, atmosphere}
}

@article{Cuk2005,
    title = {{Constraints on the Orbital Evolution of Triton}},
    year = {2005},
    journal = {The Astrophysical Journal},
    author = {{\'{C}}uk, Matija and Gladman, Brett J.},
    number = {2},
    pages = {L113-L116},
    volume = {626},
    url = {http://stacks.iop.org/1538-4357/626/i=2/a=L113},
    doi = {10.1086/431743},
    issn = {0004-637X}
}

@article{Teanby2013,
    title = {{Constraints on Titan's middle atmosphere ammonia abundance from Herschel/SPIRE sub-millimetre spectra}},
    year = {2013},
    journal = {Planetary and Space Science},
    author = {Teanby, N. A. and Irwin, P. G J and Nixon, C. A. and Courtin, R. and Swinyard, B. M. and Moreno, R. and Lellouch, E. and Rengel, M. and Hartogh, P.},
    number = {1},
    pages = {136--147},
    volume = {75},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2012.11.008},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2012.11.008},
    issn = {00320633},
    keywords = {Atmosphere, Composition, Herschel, Photochemistry, Sub-millimetre, Titan}
}

@article{Peale1978a,
    title = {{Contribution of tidal dissipation to lunar thermal history}},
    year = {1978},
    journal = {Icarus},
    author = {Peale, S. J. and Cassen, P.},
    number = {2},
    pages = {245--269},
    volume = {36},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(78)90109-4},
    issn = {10902643}
}

@article{McKinnon1999,
    title = {{Convective instability in Europa's floating ice shell}},
    year = {1999},
    journal = {Geophysical Research Letters},
    author = {McKinnon, William B.},
    number = {7},
    pages = {951--954},
    volume = {26},
    doi = {10.1029/1999GL900125},
    issn = {00948276},
    keywords = {http://dx.doi.org/10.1029/1999GL900125, doi:10.102}
}

@article{FloresMartinez2015,
    title = {{Convergent evolution and the search for biosignatures within the solar system and beyond}},
    year = {2015},
    journal = {Acta Astronautica},
    author = {Flores Martinez, Claudio L.},
    pages = {394--402},
    volume = {116},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.actaastro.2014.11.013},
    doi = {10.1016/j.actaastro.2014.11.013},
    issn = {00945765},
    keywords = {Astrobiology, Biosignatures, Convergent evolution, Europa, SETI, in situ exploration}
}

@article{Horvath2009a,
    title = {{Corona discharge experiments in admixtures of N <sub>2</sub> and CH <sub>4</sub> : a laboratory simulation of Titan's atmosphere}},
    year = {2009},
    journal = {Plasma Sources Science and Technology},
    author = {Horvath, G and Skalny, J D and Mason, N J and Klas, M and Zahoran, M and Vladoiu, R and Manole, M},
    number = {3},
    pages = {034016},
    volume = {18},
    url = {http://stacks.iop.org/0963-0252/18/i=3/a=034016?key=crossref.aec74dd080909c7c624f2f8038952f49},
    doi = {10.1088/0963-0252/18/3/034016},
    issn = {0963-0252}
}

@article{Navarro1997,
    title = {{Corona discharge of Titan's troposphere}},
    year = {1997},
    journal = {Advances in Space Research},
    author = {Navarro-Gonz{\'{a}}lez, Rafael and Ram{\'{i}}rez, Sandra I.},
    number = {7},
    pages = {1121--1133},
    volume = {19},
    isbn = {0273-1177{\textbackslash}r0-08-043108-9},
    doi = {10.1016/S0273-1177(97)00361-X},
    issn = {02731177},
    pmid = {11541341}
}

@article{Chang1991,
    title = {{Corona Discharge Processes}},
    year = {1991},
    journal = {IEEE Transactions on Plasma Science},
    author = {Chang, Jen Shih and Lawless, Phil A. and Yamamoto, Toshiaki},
    number = {6},
    pages = {1152--1166},
    volume = {19},
    isbn = {0093-3813},
    doi = {10.1109/27.125038},
    issn = {19399375}
}

@article{Plane2012,
    title = {{Cosmic dust in the earth's atmosphere}},
    year = {2012},
    journal = {Chemical Society Reviews},
    author = {Plane, John M. C.},
    number = {19},
    pages = {6507},
    volume = {41},
    url = {http://xlink.rsc.org/?DOI=c2cs35132c},
    isbn = {10.1039/C2CS35132C},
    doi = {10.1039/c2cs35132c},
    issn = {0306-0012},
    pmid = {22678029}
}

@article{Zhou2010,
    title = {{Cosmic-ray-mediated formation of benzene on the surface of Saturn's moon Titan}},
    year = {2010},
    journal = {Astrophysical Journal},
    author = {Zhou, Li and Zheng, Weijun and Kaiser, Ralf I. and Landera, Alexander and Mebel, Alexander M. and Liang, Mao Chang and Yung, Yuk L.},
    number = {2},
    pages = {1243--1251},
    volume = {718},
    doi = {10.1088/0004-637X/718/2/1243},
    issn = {15384357},
    keywords = {Astrochemistry, Comets: general, Methods: laboratory, Molecular processes, Planets and satellites: individual (Titan)}
}

@article{Porco2017a,
    title = {{Could It Be Snowing Microbes on Enceladus? Assessing Conditions in Its Plume and Implications for Future Missions}},
    year = {2017},
    journal = {Astrobiology},
    author = {Porco, Carolyn C. and Dones, Luke and Mitchell, Colin},
    number = {9},
    pages = {ast.2017.1665},
    volume = {17},
    url = {http://online.liebertpub.com/doi/10.1089/ast.2017.1665},
    isbn = {1531-1074},
    doi = {10.1089/ast.2017.1665},
    issn = {1531-1074}
}

@article{DeOliveira2016,
    title = {{Coupled Organoclay/Micelle Action for the Adsorption of Diclofenac}},
    year = {2016},
    journal = {Environmental Science and Technology},
    author = {De Oliveira, Tiago and Gu{\'{e}}gan, Régis},
    number = {18},
    pages = {10209--10215},
    volume = {50},
    doi = {10.1021/acs.est.6b03393},
    issn = {15205851}
}

@article{Dobrijevic2014,
    title = {{Coupling of oxygen, nitrogen, and hydrocarbon species in the photochemistry of titan's atmosphere}},
    year = {2014},
    journal = {Icarus},
    author = {Dobrijevic, M. and H??brard, E. and Loison, J. C. and Hickson, K. M.},
    pages = {324--346},
    volume = {228},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.10.015},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2013.10.015},
    issn = {00191035},
    keywords = {Atmospheres, chemistry, Atmospheres, composition, Photochemistry, Titan, atmosphere}
}

@article{Lavvas2008,
    title = {{Coupling photochemistry with haze formation in Titan's atmosphere, Part I: Model description}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Lavvas, P. P. and Coustenis, A. and Vardavas, I. M.},
    number = {1},
    pages = {67--99},
    volume = {56},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2007.05.027},
    issn = {00320633},
    keywords = {Atmosphere structure and composition, Haze, Temperature, Titan}
}

@article{Lavvas2008a,
    title = {{Coupling photochemistry with haze formation in Titan's atmosphere, Part II: Results and validation with Cassini/Huygens data}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Lavvas, P. P. and Coustenis, A. and Vardavas, I. M.},
    number = {1},
    pages = {67--99},
    volume = {56},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2007.05.027},
    issn = {00320633},
    keywords = {Atmosphere structure and composition, Haze, Temperature, Titan}
}

@article{Dutuit2013a,
    title = {{CRITICAL REVIEW OF N , N + , N + 2 , N , And N 2 MAIN PRODUCTION PROCESSES AND REACTIONS OF RELEVANCE TO TITAN ’ S ATMOSPHERE}},
    year = {2013},
    author = {Dutuit, Odile and Carrasco, Nathalie and Thissen, Roland and Alcaraz, Christian and Picard, Le and Loison, Jean-christophe and Herman, Zdenek and Zabka, Jan and Ascenzi, Daniela and Tosi, Paolo},
    volume = {20},
    doi = {10.1088/0067-0049/204/2/20},
    keywords = {atmospheres, atomic data, atomic processes, individual, molecular data, molecular processes, planets and satellites, titan}
}

@article{Dutuit2013,
    title = {{CRITICAL REVIEW OF N, N+ , N2+, N++ , And N++2 MAIN PRODUCTION PROCESSES AND REACTIONS OF RELEVANCE TO TITAN'S ATMOSPHERE}},
    year = {2013},
    journal = {The Astrophysical Journal Supplement Series},
    author = {Dutuit, Odile and Carrasco, Nathalie and Thissen, Roland and Vuitton, Véronique and Alcaraz, Christian and Pernot, Pascal and Balucani, Nadia and Casavecchia, Piergiorgio and Canosa, André and Picard, Sébastien Le and Loison, Jean-Christophe and Herman, Zdenek and Zabka, Jan and Ascenzi, Daniela and Tosi, Paolo and Franceschi, Pietro and Price, Stephen D. and Lavvas, Panayotis},
    number = {2},
    pages = {20},
    volume = {204},
    url = {http://stacks.iop.org/0067-0049/204/i=2/a=20?key=crossref.23de8c3395d21023ed686fde089380fb},
    doi = {10.1088/0067-0049/204/2/20},
    issn = {0067-0049},
    keywords = {atmospheres, atomic data, atomic processes, individual, molecular data, molecular processes, planets and satellites, titan}
}

@article{Beuthe2016,
    title = {{Crustal control of dissipative ocean tides in Enceladus and other icy moons}},
    year = {2016},
    journal = {Icarus},
    author = {Beuthe, Mikael},
    pages = {278--299},
    volume = {280},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103516304730},
    doi = {10.1016/j.icarus.2016.08.009},
    issn = {00191035},
    arxivId = {1608.08488},
    keywords = {Enceladus, Rotational dynamics, Satellites, Tides, dynamics, solid body}
}

@article{Lopes2007,
    title = {{Cryovolcanic features on Titan's surface as revealed by the Cassini Titan Radar Mapper}},
    year = {2007},
    journal = {Icarus},
    author = {Lopes, R. M C and Mitchell, K. L. and Stofan, E. R. and Lunine, J. I. and Lorenz, R. and Paganelli, F. and Kirk, R. L. and Wood, C. A. and Wall, S. D. and Robshaw, L. E. and Fortes, A. D. and Neish, C. D. and Radebaugh, J. and Reffet, E. and Ostro, S. J. and Elachi, C. and Allison, M. D. and Anderson, Y. and Boehmer, R. and Boubin, G. and Callahan, P. and Encrenaz, P. and Flamini, E. and Francescetti, G. and Gim, Y. and Hamilton, G. and Hensley, S. and Janssen, M. A. and Johnson, W. T K and Kelleher, K. and Muhleman, D. O. and Ori, G. and Orosei, R. and Picardi, G. and Posa, F. and Roth, L. E. and Seu, R. and Shaffer, S. and Soderblom, L. A. and Stiles, B. and Vetrella, S. and West, R. D. and Wye, L. and Zebker, H. A.},
    number = {2},
    pages = {395--412},
    volume = {186},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2006.09.006},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2006.09.006},
    issn = {00191035},
    keywords = {Satellites of Saturn, Titan, Volcanism}
}

@article{Sherman,
    title = {{Cryovolcanism on Europa: Evidence for the emplacement of flows and related deposits in the E4 Region and interpreted eruption conditions}},
    author = {Sherman, N D and Pappalardo, R T and Thomas, C and Greeley, R and State, Arizona},
    pages = {13--14}
}

@article{Lopes2013,
    title = {{Cryovolcanism on Titan: New results from Cassini RADAR and VIMS}},
    year = {2013},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Lopes, R. M C and Kirk, R. L. and Mitchell, K. L. and Legall, A. and Barnes, J. W. and Hayes, A. and Kargel, J. and Wye, L. and Radebaugh, J. and Stofan, E. R. and Janssen, M. A. and Neish, C. D. and Wall, S. D. and Wood, C. A. and Lunine, J. I. and Malaska, M. J.},
    number = {3},
    pages = {416--435},
    volume = {118},
    isbn = {0148-0227},
    doi = {10.1002/jgre.20062},
    issn = {01480227},
    keywords = {Titan, volcanism}
}

@article{Wilson2004,
    title = {{Current state of modeling the photochemistry of Titan's mutually dependent atmosphere and ionosphere}},
    year = {2004},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Wilson, E. H. and Atreya, S. K.},
    number = {6},
    volume = {109},
    isbn = {0148-0227},
    doi = {10.1029/2003JE002181},
    issn = {01480227},
    keywords = {Composition, Haze, Ion chemistry, Photochemistry, Planetary atmospheres, Titan}
}

@article{Ray2013,
    title = {{Current-voltage relation for the Saturnian system}},
    year = {2013},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Ray, L. C. and Galand, M. and Delamere, P. A. and Fleshman, B. L.},
    number = {6},
    pages = {3214--3222},
    volume = {118},
    doi = {10.1002/jgra.50330},
    issn = {21699402},
    keywords = {Saturn, auroral acceleration, field-aligned currents, magnetosphere-ionosphere coupling}
}

@book{Hartung1994,
    title = {{Cyanides and nitriles}},
    year = {1994},
    booktitle = {In Patty's Industrial Hygiene and Toxicology},
    author = {Hartung, R.},
    edition = {4th ed. vo},
    pages = {3119–3172},
    publisher = {John Wiley {\&} Sons}
}

@article{Sanchez1966b,
    title = {{Cyanoacetylene in Prebiotic Synthesis}},
    year = {1966},
    journal = {Science},
    author = {Sanchez, R. A. and Ferris, J. P. and Orgel, L. E.},
    number = {3750},
    pages = {785--786},
    volume = {154},
    doi = {10.1126/science.154.3750.785},
    issn = {00368075},
    pmid = {5919448}
}

@article{Khare1975,
    title = {{Cyclic Octatomic Sulfur: A Possible Infrared and Visible Chromophore}},
    year = {1975},
    author = {Khare, B. N. and Sagan, C.},
    pages = {10--11},
    volume = {189}
}

@article{Groenleer2008,
    title = {{Cycloid crack sequences on Europa: Relationship to stress history and constraints on growth mechanics based on cusp angles}},
    year = {2008},
    journal = {Icarus},
    author = {Groenleer, Julie M. and Kattenhorn, Simon A.},
    number = {1},
    pages = {158--181},
    volume = {193},
    doi = {10.1016/j.icarus.2007.08.032},
    issn = {00191035},
    keywords = {Europa, Ices, Satellites, Tectonics, Tides, mechanical properties, solid body, surfaces}
}

@article{Asphaug2016b,
    title = {{Cycloidal and Wavy Lineaments on Europa from Diurnal, Obliquity, and Nonsynchronous rotation stresses in a visco-elastic ice shell}},
    year = {2016},
    author = {Pappalardo, Robert T. and Patthoff, D. A. and Li, J. B. and Ayton, B. J. and Dubois, D.},
    pages = {9--10},
    isbn = {1189985144},
    doi = {10.1016/j.icarus.2007.12.027.}
}

@article{Hurford2007a,
    title = {{Cycloidal cracks on Europa : Improved modeling and non-synchronous rotation implications}},
    year = {2007},
    journal = {Icarus},
    author = {Hurford, T A and Sarid, A R and Greenberg, R},
    pages = {218--233},
    volume = {186},
    doi = {10.1016/j.icarus.2006.08.026},
    keywords = {1, europa, greenberg and weidenschilling, introduction and background, non-synchronous rotation may occur, on europa according, tectonics, tidal torques, to the theory of}
}

@article{Ali2013,
    title = {{Cyclopropenyl cation - the simplest Huckel's aromatic molecule - and its cyclic methyl derivatives inTitan's upper atmosphere}},
    year = {2013},
    journal = {Planetary and Space Science},
    author = {Ali, A. and Sittler, E. C. and Chornay, D. and Rowe, B. R. and Puzzarini, C.},
    pages = {96--105},
    volume = {87},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2013.07.007},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2013.07.007},
    issn = {00320633},
    keywords = {Carbocations, Molecular structures, Organic chemistry, Spectroscopic observations, Titan, Upper atmosphere}
}

@article{Murray2013,
    title = {{Definitions of terms relating to mass spectrometry (IUPAC Recommendations 2013)*}},
    year = {2013},
    journal = {Pure Appl. Chem},
    author = {Murray, Kermit K and Boyd, Robert K and Eberlin, Marcos N and Langley, G John and Li, Liang and Naito, Yasuhide},
    number = {7},
    pages = {1515--1609},
    volume = {85},
    url = {http://dx.doi.org/10.1351/%5Cn%7B%3C%7DGo%5Cnto%5CnISI%7B%3E%7D://WOS:000321547000019%5Cnhttp://www.degruyter.com/dg/viewarticle.fullcontentlink:pdfeventlink/%7B$%7D002fj%7B$%7D002fpac.2013.85.issue-7%7B$%7D002fpac-rec-06-04-06%7B$%7D002fpac-rec-06-04-06.},
    isbn = {1044-0305},
    doi = {10.1351/PAC-REC-06-04-06},
    issn = {1044-0305},
    keywords = {IUPAC Analytical Chemistry Division, atmospheric-pressure photoionization, capillary-zone-electrophoresis, collision-induced dissociation, definitions, fast-atom-bombardment, glossary, hydrogen-deuterium exchange, infrared multiphoton dissociation, ion-cyclotron resonance, iupac analytical chemistry division, liquid-chromatography, mass spectrometry, of-the-art, proton bound dimers, terms}
}

@article{deOliveira2001,
    title = {{Definitive Heat of Formation of Methylenimine, CH2=NH, and of Methylenimmonium Ion, CH2NH2+, by Means of W2 Theory}},
    year = {2001},
    journal = {Technology},
    author = {Oliveira, Glênisson D E and Martin, J A N M L and Silwal, Indira K C and Liebman, Joel F},
    number = {13},
    pages = {1297--1305},
    volume = {22},
    keywords = {anharmonic force field, ch 2 nh 2, comartin, correspondence to, e-mail, j, l, m, martin, methylenimine, w2 theory, wicc}
}

@article{Mutsukura2001,
    title = {{Deposition of Diamondlike Carbon Film and Mass Spectrometry Measurement in CH 4 / N 2 RF Plasma}},
    year = {2001},
    author = {Mutsukura, Nobuki},
    number = {2},
    pages = {265--277},
    volume = {21}
}

@article{Alibay2014,
    title = {{Design of a low cost mission to the Neptunian system}},
    year = {2014},
    journal = {IEEE Aerospace Conference Proceedings},
    author = {Alibay, Farah and Fernandes, Philip and McGranaghan, Ryan and Leonard, Jason and Clegg, Ryan and Craig, Patricia and Day, Mackenzie and Fougere, Nicolas and Girazian, Zachary and Hosseini, Sona and Hutchins, Michael and Scully, Jennifer and Uckert, Kyle and Malaska, Michael and Patthoff, Alex and Ries, Paul and Budney, Charles and Mitchell, Karl},
    number = {March},
    isbn = {9781479916221},
    doi = {10.1109/AERO.2014.6836294},
    issn = {1095323X}
}

@article{Lorenz2016,
    title = {{Detecting volcanism on Titan and Venus with microwave radiometry}},
    year = {2016},
    journal = {Icarus},
    author = {Lorenz, Ralph D. and Le Gall, Alice and Janssen, Michael A.},
    pages = {30--36},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.07.023},
    doi = {10.1016/j.icarus.2015.07.023},
    issn = {10902643},
    keywords = {Radiative transfer, Radio observations, Titan, Venus, Volcanism}
}

@article{Clark2010,
    title = {{Detection and mapping of hydrocarbon deposits on Titan}},
    year = {2010},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Clark, Roger N. and Curchin, John M. and Barnes, Jason W. and Jaumann, Ralf and Soderblom, Larry and Cruikshank, Dale P. and Brown, Robert H. and Rodriguez, Sébastien and Lunine, Jonathan and Stephan, Katrin and Hoefen, Todd M. and Le Mou{\'{e}}lic, Stéphane and Sotin, Christophe and Baines, Kevin H. and Buratti, Bonnie J. and Nicholson, Philip D.},
    number = {10},
    volume = {115},
    isbn = {0148-0227},
    doi = {10.1029/2009JE003369},
    issn = {01480227}
}

@article{Kawaguchi1994,
    title = {{Detection of a new molecular ion HC3NH(+) in TMC-1}},
    year = {1994},
    journal = {The Astrophysical Journal},
    author = {Kawaguchi, Kentarou and Kasai, Yasuko and Ishikawa, Shin-Ichi and Ohishi, Masatoshi and Kaifu, Norio and Amano, Takayoshi},
    number = {April 2017},
    pages = {L95},
    volume = {420},
    doi = {10.1086/187171},
    issn = {0004-637X}
}

@article{Demory2011,
    title = {{Detection of a transit of the super-Earth 55 Cancri e with warm Spitzer}},
    year = {2011},
    journal = {Astronomy and Astrophysics},
    author = {Demory, B and Gillon, M and Deming, D and Valencia, D and Seager, S and Benneke, B and Lovis, C and Cubillos, P and Harrington, J and Stevenson, K B and Mayor, M and Pepe, F and Queloz, D and S{\'{e}}gransan, D and Udry, S},
    pages = {A114},
    volume = {533},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-data_query?bibcode=2011A%2526A...533A.114D&link_type=ABSTRACT%5Cnpapers://0be24a46-325a-4116-a3c6-fd8a3b614472/Paper/p14524},
    doi = {10.1051/0004-6361/201117178},
    issn = {1432-0746},
    arxivId = {1105.0415},
    keywords = {binaries: eclipsing, planetary systems, stars: individual: 55 Cnc, techniques: photometric}
}

@misc{Bezard1993,
    title = {{Detection of acetonitrile on Titan}},
    year = {1993},
    author = {Bezard, B. and Paubert, G.},
    pages = {1100},
    publisher = {Bull. Am. Astron. Soc.}
}

@article{Tsiaras2016,
    title = {{Detection of an Atmosphere Around the Super-Earth 55 Cancri E}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Tsiaras, A. and Rocchetto, M. and Waldmann, I. P. and Venot, O. and Varley, R. and Morello, G. and Damiano, M. and Tinetti, G. and Barton, E. J. and Yurchenko, S. N. and Tennyson, J.},
    number = {2},
    pages = {99},
    volume = {820},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/820/i=2/a=99?key=crossref.3e98c04dcba480b5d7b36b11f5380a07},
    doi = {10.3847/0004-637X/820/2/99},
    issn = {1538-4357},
    keywords = {55 cancri e, atmospheres, data analysis, individual, methods, methods: data analysis, methods: statistical, planets and, planets and satellites, planets and satellites: atmospheres, planets and satellites: individual (55 Cancri e), satellites, spectroscopic, statistical, techniques, techniques: spectroscopic}
}

@article{Pont2008,
    title = {{Detection of atmospheric haze on an extrasolar planet: The 0.55-1.05 ??m transmission spectrum of HD 189733b with the Hubble Space Telescope}},
    year = {2008},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Pont, F. and Knutson, H. and Gilliland, R. L. and Moutou, C. and Charbonneau, D.},
    number = {1},
    pages = {109--118},
    volume = {385},
    doi = {10.1111/j.1365-2966.2008.12852.x},
    issn = {00358711},
    arxivId = {0712.1374},
    keywords = {Methods: data analysis, Planetary systems, Techniques: spectroscopic}
}

@article{Lellouch2016,
    title = {{Detection of CO and HCN in Pluto's atmosphere with ALMA}},
    year = {2016},
    author = {Lellouch, E. and Gurwell, M. and Butler, B. and Fouchet, T. and Lavvas, P. and Strobel, D. F. and Sicardy, B. and Moullet, A. and Moreno, R. and Bockel{\'{e}}e-Morvan, D. and Biver, N. and Young, L. and Lis, D. and Stansberry, J. and Stern, A. and Weaver, H. and Young, E. and Zhu, X. and Boissier, J.},
    number = {i},
    url = {http://arxiv.org/abs/1606.03293},
    doi = {10.1016/j.icarus.2016.10.013},
    issn = {10902643},
    arxivId = {1606.03293}
}

@article{Lellouch2016a,
    title = {{Detection of CO and HCN in Pluto's atmosphere with ALMA}},
    year = {2016},
    author = {Lellouch, E. and Gurwell, M. and Butler, B. and Fouchet, T. and Lavvas, P. and Strobel, D. F. and Sicardy, B. and Moullet, A. and Moreno, R. and Bockel{\'{e}}e-Morvan, D. and Biver, N. and Young, L. and Lis, D. and Stansberry, J. and Stern, A. and Weaver, H. and Young, E. and Zhu, X. and Boissier, J.},
    number = {i},
    url = {http://arxiv.org/abs/1606.03293},
    doi = {10.1016/j.icarus.2016.10.013},
    issn = {10902643},
    arxivId = {1606.03293}
}

@article{Agren2012,
    title = {{Detection of negative ions in the deep ionosphere of Titan during the Cassini T70 flyby}},
    year = {2012},
    journal = {Geophysical Research Letters},
    author = {{\AA}gren, K. and Edberg, N. J T and Wahlund, J. E.},
    number = {10},
    pages = {1--5},
    volume = {39},
    doi = {10.1029/2012GL051714},
    issn = {00948276},
    keywords = {T70, Titan, ionosphere, negative ions}
}

@article{Southworth2017,
    title = {{Detection of the Atmosphere of the 1.6 <i>M</i> <sub>⊕</sub> Exoplanet GJ 1132 b}},
    year = {2017},
    journal = {The Astronomical Journal},
    author = {Southworth, John and Mancini, Luigi and Madhusudhan, Nikku and Molli{\`{e}}re, Paul and Ciceri, Simona and Henning, Thomas},
    number = {4},
    pages = {191},
    volume = {153},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/1538-3881/153/i=4/a=191?key=crossref.f1eba309ebf4172d51db3143399477d3},
    doi = {10.3847/1538-3881/aa6477},
    issn = {1538-3881},
    keywords = {fundamental parameters, gj 1132, individual, planetary systems, planetary systems,stars: fundamental parameters,st, stars}
}

@article{Yamada1981,
    title = {{Detection of the Infrared Spectrum of Cyanobutadiyne, HC5N}},
    year = {1981},
    author = {Yamada, Koichi and Winnewisser, Gisbert},
    pages = {1052--1056},
    volume = {1056}
}

@article{Bird1997,
    title = {{Detection of Titan's Ionosphere from Voyager 1 Radio Occultation Observations}},
    year = {1997},
    journal = {Icarus},
    author = {Bird, M.~K. and Dutta-Roy, R and Asmar, S.~W. and Rebold, T.~A.},
    number = {2},
    pages = {426--436},
    volume = {130},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103597958310},
    doi = {10.1006/icar.1997.5831},
    issn = {00191035},
    keywords = {bauer 1985, during the voyager 1, flyby, imposed from other data, mcnutt and rich-, planetary ionospheres, radio observations, recorded, titan, well as from constraints}
}

@article{Bird1997a,
    title = {{Detection of Titan's Ionosphere from Voyager 1 Radio Occultation Observations}},
    year = {1997},
    journal = {Icarus},
    author = {Bird, M.~K. and Dutta-Roy, R and Asmar, S.~W. and Rebold, T.~A.},
    number = {2},
    pages = {426--436},
    volume = {130},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103597958310},
    doi = {10.1006/icar.1997.5831},
    issn = {00191035},
    keywords = {bauer 1985, during the voyager 1, flyby, imposed from other data, mcnutt and rich-, planetary ionospheres, radio observations, recorded, titan, well as from constraints}
}

@article{Mathe2018,
    title = {{Detection Opportunity for Aromatic Signature in Titan’s Aerosols in the 4.1–5.3 <i>{$\mu$}</i> m Range}},
    year = {2018},
    journal = {The Astrophysical Journal},
    author = {Math{\'{e}}, Christophe and Gautier, Thomas and Trainer, Melissa G. and Carrasco, Nathalie},
    number = {2},
    pages = {L25},
    volume = {861},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/2041-8205/861/i=2/a=L25?key=crossref.7a8901973736de5a89f8c977e0348472},
    doi = {10.3847/2041-8213/aacf88},
    issn = {2041-8213},
    keywords = {astrochemistry, astrochemistry,infrared: planetary systems,methods, atmospheres, infrared, laboratory, methods, planetary systems, planets and satellites, refractory, solid state}
}

@article{Davis1968,
    title = {{Determination of Bond Dissociation Energies in Hydrogen Cyanide. Cyanogen and Cyanogen Halides by the Photodissociation Method}},
    year = {1968},
    journal = {The Journal of Chemical Physics},
    author = {Davis, Douglas D. and Okabe, H.},
    number = {12},
    pages = {5526},
    volume = {49},
    url = {http://scitation.aip.org/content/aip/journal/jcp/49/12/10.1063/1.1670082},
    doi = {10.1063/1.1670082},
    issn = {00219606}
}

@article{Shebanits2010,
    title = {{Determination of Ion Number Density from Langmuir Probe Measurements in the Ionosphere of Titan}},
    year = {2010},
    author = {Shebanits, Oleg}
}

@article{Francisco2000,
    title = {{Determination of the CC bond dissociation energy in C3N radical}},
    year = {2000},
    journal = {Chemical Physics Letters},
    author = {Francisco, Joseph S.},
    number = {4},
    pages = {307--310},
    volume = {324},
    doi = {10.1016/S0009-2614(00)00568-6},
    issn = {00092614}
}

@article{Swanepoel1983,
    title = {{Determination of the thickness and optical constants of amorphous silicon}},
    year = {1983},
    author = {Swanepoel, R.},
    volume = {1214}
}

@article{Mahjoub2016b,
    title = {{Development of a new Experimental Platform to Constrain the Chemical Composition of Titan's Lakes}},
    year = {2016},
    journal = {Lunar and Planetary Science Conference XLVII},
    author = {Mahjoub, A. and Choukroun, M. and Sotin, C. and Hodyss, Robert and Barmatz, Martin},
    number = {2787},
    pages = {46--47},
    isbn = {1315313197},
    doi = {10.1038/ngeo2474.},
    issn = {19453027}
}

@article{Schenk1993,
    title = {{Diapirism on Triton: a record of crustal layering and instability}},
    year = {1993},
    journal = {Geology},
    author = {Schenk, P. and Jackson, M. P A},
    number = {4},
    pages = {299--302},
    volume = {21},
    isbn = {0091-7613},
    doi = {10.1130/0091-7613(1993)021<0299:DOTARO>2.3.CO;2},
    issn = {00917613}
}

@article{Aitken1897,
    title = {{Dimensions of the Planets and Satellites}},
    year = {1897},
    journal = {Publications of the Astronomical Society of the Pacific},
    author = {Aitken, R. G.},
    number = {350},
    pages = {253--256},
    volume = {59}
}

@article{Iguchi1956,
    title = {{Dipole Moment of the HCN Molecule}},
    year = {1956},
    journal = {The Journal of Chemical Physics},
    author = {Iguchi, Kaoru},
    number = {2},
    pages = {217--219},
    volume = {25},
    url = {http://aip.scitation.org/doi/10.1063/1.1742857},
    doi = {10.1063/1.1742857},
    issn = {0021-9606}
}

@article{Stiles2003,
    title = {{Dipole Moments of Molecules Solvated in Helium Nanodroplets}},
    year = {2003},
    journal = {Physical Review Letters},
    author = {Stiles, Paul L. and Nauta, Klaas and Miller, Roger E.},
    number = {13},
    pages = {4},
    volume = {90},
    isbn = {0031-9007},
    doi = {10.1103/PhysRevLett.90.135301},
    issn = {10797114}
}

@article{Brown2002,
    title = {{Direct detection of variable tropospheric clouds near Titan's south pole.}},
    year = {2002},
    journal = {Nature},
    author = {Brown, M. and Bouchez, A. H. and Griffith, C. A.},
    number = {6917},
    pages = {795--797},
    volume = {420},
    isbn = {0028-0836},
    doi = {10.1038/nature01302},
    issn = {0028-0836},
    pmid = {12490943}
}

@article{Cheetham2017,
    title = {{Direct imaging of an ultracool substellar companion to the exoplanet host star HD 4113A}},
    year = {2017},
    author = {Cheetham, A. and S{\'{e}}gransan, D. and Peretti, S. and Delisle, J. -B. and Hagelberg, J. and Beuzit, J-L. and Forveille, T. and Marmier, M. and Udry, S. and Wildi, F.},
    url = {http://arxiv.org/abs/1712.05217},
    arxivId = {1712.05217},
    keywords = {brown dwarfs, detection, planet-star interactions, planets and satellites, stars}
}

@article{Yu2017,
    title = {{Direct Measurement of Interparticle Forces of Titan Aerosol Analogs ('Tholin') Using Atomic Force Microscopy}},
    year = {2017},
    author = {Yu, Xinting and H{\"{o}}rst, Sarah M and He, Chao and Mcguiggan, Patricia and Bridges, Nathan T},
    pages = {1--36},
    url = {https://arxiv.org/pdf/1710.06400.pdf},
    arxivId = {arXiv:1710.06400v1}
}

@article{C.D.,
    title = {{Discovering Huygens}},
    author = {C. D., Andriesse}
}

@article{Kiss2017,
    title = {{Discovery of a satellite of the large trans-Neptunian object (225088) 2007OR10}},
    year = {2017},
    journal = {The Astrophysical Journal Letters},
    author = {Kiss, Csaba and Marton, Gábor and Farkas-Tak{\'{a}}cs, Anikó and Stansberry, John and M{\"{u}}ller, Thomas and Vink{\'{o}}, József and Balog, Zoltán and Ortiz, Jose-Luis and P{\'{a}}l, András},
    number = {1},
    pages = {L1},
    volume = {838},
    publisher = {IOP Publishing},
    url = {http://arxiv.org/abs/1703.01407},
    doi = {10.3847/2041-8213/aa6484},
    issn = {2041-8213},
    arxivId = {1703.01407},
    keywords = {2007or10, asteroids, astrometry, astrometry,Kuiper belt objects: individual (2007OR, general, individual, kuiper belt objects, methods, minor planets, observational, photometric, techniques}
}

@article{Holman2004,
    title = {{Discovery of five irregular moons of Neptune}},
    year = {2004},
    journal = {Nature},
    author = {Holman, M J and Kavelaars, J J and Grav, T and Gladman, B J and Fraser, W C and Milisavljevic, D and Nicholson, P D and Burns, J A and Carruba, V and Petit, J P and Rousselot, P and Moussis, O and Marsden, B G and Jacobson, R A},
    number = {August 2001},
    pages = {865},
    volume = {430},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-data_query?bibcode=2004Natur.430..865H&link_type=ABSTRACT%5Cnpapers://fedb1a86-f693-4042-a040-86e952d868c2/Paper/p236},
    isbn = {1476-4687 (Electronic){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/nature02832},
    issn = {1476-4679},
    pmid = {15318214}
}

@article{Brown2009fog,
    title = {{Discovery of fog at the south pole of Titan}},
    year = {2009},
    journal = {The Astrophysical Journal},
    author = {Brown, M E and Smith, A L and Chen, C and Ad, M},
    pages = {2004--2007},
    doi = {10.1088/0004-637X/706/1/L110},
    keywords = {1 {$\mu$} m and, 5 {$\mu$} m, coupled with several strong, individual, infrared, methane ab-, planets and satellites, s atmosphere throughout this, simultaneous images in up, solar system, sorption features in titan, spectral, this capability, titan, to 256 channels between}
}

@article{Coates2007,
    title = {{Discovery of heavy negative ions in Titan's ionosphere}},
    year = {2007},
    journal = {Geophysical Research Letters},
    author = {Coates, A. J. and Crary, F. J. and Lewis, G. R. and Young, D. T. and Waite, Jr H. and Sittler, Jr C.},
    number = {22},
    pages = {6--11},
    volume = {34},
    isbn = {0094-8276},
    doi = {10.1029/2007GL030978},
    issn = {00948276},
    keywords = {doi:10.102, http://dx.doi.org/10.1029/2007GL030978}
}

@article{Godfrey1973,
    title = {{Discovery of Interstellar Methanimine (Formaldimine)}},
    year = {1973},
    journal = {Astrophysical Letters},
    author = {Godfrey, P. D. and Brown, R. D. and Robinson, B. J. and Sinclair, M. W.},
    pages = {119},
    volume = {13},
    url = {http://adsabs.harvard.edu/abs/1973ApL....13..119G},
    issn = {0004-6388}
}

@article{Meyer1991,
    title = {{Discovery of interstellar NH}},
    year = {1991},
    author = {Meyer, D. and Roth, K.}
}

@article{Rymer2009,
    title = {{Discrete classification and electron energy spectra of Titan's varied magnetospheric environment}},
    year = {2009},
    journal = {Geophysical Research Letters},
    author = {Rymer, A. M. and Smith, H. T. and Wellbrock, A. and Coates, A. J. and Young, D. T.},
    number = {15},
    pages = {1--6},
    volume = {36},
    isbn = {0094-8276},
    doi = {10.1029/2009GL039427},
    issn = {00948276},
    keywords = {Titan, doi:10.1029/2009GL039427, electron, http://dx.doi.org/10.1029/2009GL039427, magnetosphere}
}

@article{Branscomb,
    title = {{Disequilibria and Escapements}},
    author = {Branscomb, Elbert and Biancalani, T. and Russell, Michael J.},
    number = {0},
    pages = {450261},
    volume = {0}
}

@article{Karkoschka2007,
    title = {{DISR imaging and the geometry of the descent of the Huygens probe within Titan's atmosphere}},
    year = {2007},
    journal = {Planetary and Space Science},
    author = {Karkoschka, Erich and Tomasko, Martin G. and Doose, Lyn R. and See, Chuck and McFarlane, Elisabeth A. and Schr{\"{o}}der, Stefan E. and Rizk, Bashar},
    number = {13},
    pages = {1896--1935},
    volume = {55},
    doi = {10.1016/j.pss.2007.04.019},
    issn = {00320633},
    keywords = {Titan}
}

@article{Cornet2015,
    title = {{Dissolution on Titan and on Earth: Toward the age of Titan's karstic landscapes}},
    year = {2015},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Cornet, Thomas and Cordier, Daniel and Bahers, Tangui Le and Bourgeois, Olivier and Fleurant, Cyril and Mou{\'{e}}lic, Stéphane Le and Altobelli, Nicolas},
    number = {6},
    pages = {1044--1074},
    volume = {120},
    doi = {10.1002/2014JE004738},
    issn = {21699100},
    arxivId = {arXiv:1505.08109v1},
    keywords = {Earth, surface, Titan, surface, dissolution, geological processes, karst, thermodynamics}
}

@article{Grundy2006,
    title = {{Distributions of H2O and CO2 ices on Ariel, Umbriel, Titania, and Oberon from IRTF/SpeX observations}},
    year = {2006},
    journal = {Icarus},
    author = {Grundy, W. M. and Young, L. A. and Spencer, J. R. and Johnson, R. E. and Young, E. F. and Buie, M. W.},
    number = {2},
    pages = {543--555},
    volume = {184},
    doi = {10.1016/j.icarus.2006.04.016},
    issn = {00191035},
    keywords = {Ices, Infrared observations, Satellite, Spectroscopy, Uranus, satellites, surfaces}
}

@article{Cui2009,
    title = {{Diurnal variations of Titan’s ionosphere}},
    year = {2009},
    journal = {Journal of Geophysical Research},
    author = {Cui, J. and Galand, M and Yelle, R V and Vuitton, V and Wahlund, J and Lavvas, P P},
    pages = {1--20},
    volume = {114},
    doi = {10.1029/2009JA014228},
    keywords = {Titan, doi:10.1029/2009JA014228, http://dx.doi.org/10.1029/2009JA014228, ionosphere}
}

@article{Dubois2017c,
    title = {{Diurnal, Nonsynchronous Rotation and Obliquity Tidal Effects on Triton using a Viscoelastic Model: SatStressGUI. Implications for Ridge and Cycloid Formation}},
    year = {2017},
    journal = {LPSC 2017},
    author = {Dubois, D. and Patthoff, D. A. and Pappalardo, R. T.},
    pages = {1--2}
}

@article{Pilling2009,
    title = {{DNA nucleobase synthesis at Titan atmosphere analog by soft X-rays}},
    year = {2009},
    journal = {Journal of Physical Chemistry A},
    author = {Pilling, S. and Andrade, D. P.P. and Neto, Á. C. and Rittner, R. and De Brito, A. N.},
    number = {42},
    pages = {11161--11166},
    volume = {113},
    isbn = {1089-5639},
    doi = {10.1021/jp902824v},
    issn = {10895639},
    pmid = {19534497},
    arxivId = {0906.3675}
}

@article{Pappalardo1999,
    title = {{Does Europa have a subsurface ocean? Evaluation of the geological evidence}},
    year = {1999},
    journal = {Journal of Geophysical Research},
    author = {Pappalardo, R. T. and Belton, M. J. S. and Breneman, H. H. and Carr, M. H. and Chapman, C. R. and Collins, G. C. and Denk, T. and Fagents, S. and Geissler, P. E. and Giese, B. and Greeley, R. and Greenberg, R. and Head, J. W. and Helfenstein, P. and Hoppa, G. and Kadel, S. D. and Klaasen, K. P. and Klemaszewski, J. E. and Magee, K. and McEwen, a. S. and Moore, J. M. and Moore, W. B. and Neukum, G. and Phillips, C. B. and Prockter, L. M. and Schubert, G. and Senske, D. a. and Sullivan, R. J. and Tufts, B. R. and Turtle, E. P. and Wagner, R. and Williams, K. K.},
    number = {E10},
    pages = {15--55},
    volume = {104},
    doi = {10.1029/1998JE000628},
    issn = {0148-0227},
    keywords = {doi:10.102, http://dx.doi.org/10.1029/1998JE000628}
}

@article{Buratti1999,
    title = {{Does global warming make Triton blush?}},
    year = {1999},
    journal = {Nature},
    author = {Buratti, B.J. and Hicks, M.D. and Newburn Jr, R.L.},
    number = {6716},
    pages = {219},
    volume = {397},
    url = {http://scholar.google.com/scholar?hl=en&btnG=Search&q=intitle:Does+global+warming+make+Triton+blush?#0},
    issn = {00280836}
}

@article{Thissen2011,
    title = {{Doubly-charged ions in the planetary ionospheres: a review}},
    year = {2011},
    journal = {Physical Chemistry Chemical Physics},
    author = {Thissen, Roland and Witasse, Olivier and Dutuit, Odile and Wedlund, Cyril Simon and Gronoff, Guillaume and Lilensten, Jean},
    number = {41},
    pages = {18264},
    volume = {13},
    url = {http://xlink.rsc.org/?DOI=c1cp21957j},
    isbn = {1463-9084 (Electronic){\textbackslash}r1463-9076 (Linking)},
    doi = {10.1039/c1cp21957j},
    issn = {1463-9076},
    pmid = {21931881}
}

@article{Radebaugh2008,
    title = {{Dunes on Titan observed by Cassini Radar}},
    year = {2008},
    journal = {Icarus},
    author = {Radebaugh, J. and Lorenz, R. D. and Lunine, J. I. and Wall, S. D. and Boubin, G. and Reffet, E. and Kirk, R. L. and Lopes, R. M. and Stofan, E. R. and Soderblom, L. and Allison, M. and Janssen, M. and Paillou, P. and Callahan, P. and Spencer, C. and {the Cassini Radar Team}},
    number = {2},
    pages = {690--703},
    volume = {194},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2007.10.015},
    issn = {00191035},
    keywords = {Satellites, Saturn, Titan, satellites, surfaces}
}

@article{Oza2018,
    title = {{Dusk/dawn atmospheric asymmetries on tidally-locked satellites: O 2 at Europa}},
    year = {2018},
    journal = {Icarus},
    author = {Oza, Apurva V. and Johnson, Robert E. and Leblanc, François},
    pages = {50--55},
    volume = {305},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103517306498},
    doi = {10.1016/j.icarus.2017.12.032},
    issn = {00191035}
}

@article{Lee2016,
    title = {{Dynamic mineral clouds on HD 189733b I. 3D RHD with kinetic, non-equilibrium cloud formation}},
    year = {2016},
    author = {Lee, G. and Dobbs-Dixon, I. and Helling, Ch. and Bognar, K. and Woitke, P.},
    pages = {23},
    volume = {48},
    url = {http://arxiv.org/abs/1603.09098},
    doi = {10.1051/0004-6361/201628606},
    issn = {14320746},
    arxivId = {1603.09098},
    keywords = {atmospheres, hd 189733b, hydrodynamics, individual, methods, numerical, planets and satellites, radiative transfer}
}

@article{Lee2017,
    title = {{Dynamic mineral clouds on HD 189733b II. Monte Carlo radiative transfer for 3D cloudy exoplanet atmospheres: combining scattering and emission spectra}},
    year = {2017},
    author = {Lee, Graham and Wood, Kenneth and Dobbs-Dixon, Ian and Rice, Anna and Helling, Christiane},
    url = {http://arxiv.org/abs/1701.00983},
    arxivId = {1701.00983},
    keywords = {atmospheres, hd 189733b, individual, methods, planets and satellites, radiative transfer}
}

@article{Teanby2009a,
    title = {{Dynamical implications of seasonal and spatial variations in Titan's stratospheric composition.}},
    year = {2009},
    journal = {Philosophical transactions. Series A, Mathematical, physical, and engineering sciences},
    author = {Teanby, N. and Irwin, Patrick G J and de Kok, Remco and Nixon, Conor a},
    number = {1889},
    pages = {697--711},
    volume = {367},
    doi = {10.1098/rsta.2008.0164},
    issn = {1364-503X},
    pmid = {19019781},
    keywords = {atmosphere, cassini, titan}
}

@article{Antonelli2014,
    title = {{Early inner solar system origin for anomalous sulfur isotopes in differentiated protoplanets.}},
    year = {2014},
    journal = {Proceedings of the National Academy of Sciences of the United States of America},
    author = {Antonelli, Michael A and Kim, Sang-Tae and Peters, Marc and Labidi, Jabrane and Cartigny, Pierre and Walker, Richard J. and Lyons, James R and Hoek, Joost and Farquhar, James},
    number = {50},
    pages = {17749--54},
    volume = {111},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/25453079},
    isbn = {1418907111},
    doi = {10.1073/pnas.1418907111},
    issn = {1091-6490},
    pmid = {25453079}
}

@article{Beuthe2010,
    title = {{East-west faults due to planetary contraction}},
    year = {2010},
    journal = {Icarus},
    author = {Beuthe, Mikael},
    number = {2},
    pages = {795--817},
    volume = {209},
    doi = {10.1016/j.icarus.2010.04.019},
    issn = {00191035},
    arxivId = {1006.5818},
    keywords = {Iapetus, Mercury, Planetary dynamics, Satellites, Surfaces, Tectonics}
}

@article{Struve1907,
    title = {{ECLIPSES AND TRANSITS OF THE SATELLITES OF SATURN OCCURRING IN THE YEAR 1907}},
    year = {1907},
    journal = {Publications of the Astronomical Society of the Pacific},
    author = {Struve, Hermann},
    number = {114},
    pages = {125--135},
    volume = {19}
}

@article{Mahjoub2014,
    title = {{Effect of the synthesis temperature on the optical indices of organic materials produced by N2-CH4 RF plasma}},
    year = {2014},
    journal = {Plasma Processes and Polymers},
    author = {Mahjoub, Ahmed and Carrasco, Nathalie and Dahoo, Pierre Richard and Fleury, Benjamin and Gautier, Thomas and Cernogora, Guy},
    number = {5},
    pages = {409--417},
    volume = {11},
    isbn = {1612-8869},
    doi = {10.1002/ppap.201300150},
    issn = {16128869},
    keywords = {ATR/FTIR, HF discharges, cold plasma, ellipsometry, organic substances, refractive index}
}

@article{Jara-Orue2011,
    title = {{Effects of low-viscous layers and a non-zero obliquity on surface stresses induced by diurnal tides and non-synchronous rotation: The case of Europa}},
    year = {2011},
    journal = {Icarus},
    author = {Jara-Oru{\'{e}}, Hermes M. and Vermeersen, Bert L A},
    number = {1},
    pages = {417--438},
    volume = {215},
    doi = {10.1016/j.icarus.2011.05.034},
    issn = {00191035},
    keywords = {Europa, Geophysics, Interiors, Tides, solid body}
}

@article{Showman2005,
    title = {{Effects of plasticity on convection in an ice shell: Implications for Europa}},
    year = {2005},
    journal = {Icarus},
    author = {Showman, Adam P. and Han, Lijie},
    number = {2},
    pages = {425--437},
    volume = {177},
    doi = {10.1016/j.icarus.2005.02.020},
    issn = {00191035},
    keywords = {Europa, Ices, Satellite, Satellites of Jupiter, Surfaces, Tectonics}
}

@article{Goldreich2010,
    title = {{Elastic ice shells of synchronous moons: Implications for cracks on Europa and non-synchronous rotation of Titan}},
    year = {2010},
    journal = {Icarus},
    author = {Goldreich, Peter M. and Mitchell, J. L.},
    number = {2},
    pages = {631--638},
    volume = {209},
    doi = {10.1016/j.icarus.2010.04.013},
    issn = {00191035},
    arxivId = {0910.0032},
    keywords = {Europa, Resonances, Spin-orbit, Titan}
}

@article{Hess2009,
    title = {{Electric potential jumps in the Io-Jupiter flux tube}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Hess, S. and Zarka, P. and Mottez, F. and Ryabov, V. B.},
    number = {1},
    pages = {23--33},
    volume = {57},
    doi = {10.1016/j.pss.2008.10.006},
    issn = {00320633},
    keywords = {Electrons acceleration, Jupiter-Io interaction, Potential drops, Radio emissions, S-bursts}
}

@article{Lethuillier2018,
    title = {{Electrical Properties of Tholins and Derived Constraints on the Huygens Landing Site Composition at the Surface of Titan}},
    year = {2018},
    journal = {Journal of Geophysical Research: Planets},
    author = {Lethuillier, A and Le Gall, A. and Hamelin, M. and Caujolle-Bert, S. and Schreiber, F. and Carrasco, N. and Cernogora, G. and Szopa, C. and Brouet, Y. and Simoes, F. and Correia, J.-J. and Ruffie, G.},
    number = {2016},
    pages = {1--16}
}

@article{Edberg2010,
    title = {{Electron density and temperature measurements in the cold plasma environment of Titan: Implications for atmospheric escape}},
    year = {2010},
    journal = {Geophysical Research Letters},
    author = {Edberg, N. J T and Wahlund, J. E. and {\AA}gren, K. and Morooka, M. W. and Modolo, R. and Bertucci, C. and Dougherty, M. K.},
    number = {20},
    pages = {3--7},
    volume = {37},
    doi = {10.1029/2010GL044544},
    issn = {00948276}
}

@article{Chakrabarty2013,
    title = {{Electronic absorption spectrum of triacetylene cation for astronomical considerations}},
    year = {2013},
    journal = {Journal of Physical Chemistry A},
    author = {Chakrabarty, S. and Rice, C. A. and Mazzotti, F. J. and Dietsche, R. and Maier, J. P.},
    number = {39},
    pages = {9574--9577},
    volume = {117},
    doi = {10.1021/jp312294f},
    issn = {10895639},
    pmid = {23461383}
}

@article{Gudipati2001,
    title = {{Electronic spectrum of atomic sulfur in argon matrices in the vacuum ultraviolet region}},
    year = {2001},
    journal = {Chemical Physics Letters},
    author = {Gudipati, Murthy S. and Klein, Andreas},
    number = {5-6},
    pages = {479--487},
    volume = {344},
    doi = {10.1016/S0009-2614(01)00803-X},
    issn = {00092614}
}

@article{Fischer2003,
    title = {{Electronic spectrum of dicyanoacetylene. 1. Calculations of the geometries and vibrations of ground and excited states of diacetylene, cyanoacetylene, cyanogen, triacetylene, cyanodiacetylene, and dicyanoacetylene}},
    year = {2003},
    journal = {Journal of Physical Chemistry A},
    author = {Fischer, Gad and Ross, I. G.},
    number = {49},
    pages = {10631--10636},
    volume = {107},
    doi = {10.1021/jp034966j},
    issn = {10895639}
}

@article{Berkeley2011,
    title = {{Electronic Thesis and Dissertations The rotation and fracture history of Europa from modeling of tidal-tectonic processes By Alyssa Rose Rhoden A dissertation submitted in partial satisfaction of the requirements for the degree of Doctor of Philosophy in }},
    year = {2011},
    author = {Berkeley, U C and Rose, Alyssa}
}

@article{Gan1992,
    title = {{Electrons in the Ionosphere of Titan}},
    year = {1992},
    journal = {Journal of Geophysical Research},
    author = {Gan, L and Keller, C N and Cravens, T E},
    number = {9},
    volume = {97},
    keywords = {doi:10.1029/92JA00300, http://dx.doi.org/10.1029/92JA00300}
}

@article{McKay1996,
    title = {{Elemental composition, solubility, and optical properties of Titan's organic haze}},
    year = {1996},
    journal = {Planetary and Space Science},
    author = {McKay, Christopher P.},
    number = {8},
    pages = {741--747},
    volume = {44},
    isbn = {0032-0633},
    doi = {10.1016/0032-0633(96)00009-8},
    issn = {00320633}
}

@article{Bourgalais2016,
    title = {{Elusive anion growth in Titan's atmosphere: Low temperature kinetics of the C3N-+ HC3N reaction}},
    year = {2016},
    journal = {Icarus},
    author = {Bourgalais, J. and Jamal-Eddine, Nour and Joalland, Baptiste and Capron, Michael and Balaganesh, Muthiah and Guillemin, Jean Claude and Le Picard, Sébastien D. and Faure, Alexandre and Carles, Sophie and Biennier, Ludovic},
    pages = {194--201},
    volume = {271},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2016.02.003},
    issn = {10902643},
    keywords = {Atmospheres, Chemistry, Ionospheres, Titan, atmosphere}
}

@article{Bland2013,
    title = {{Enceladus' extreme heat flux as revealed by its relaxed craters}},
    year = {2013},
    journal = {Geophysical Research Letters},
    author = {Bland, Michael T. and Singer, Kelsi N. and Mckinnon, William B. and Schenk, Paul M.},
    number = {17},
    pages = {1--5},
    volume = {39},
    isbn = {1944-8007},
    doi = {10.1029/2012GL052736},
    issn = {00948276},
    keywords = {Crater relaxation, Enceladus, Thermal history}
}

@article{Thomas2016,
    title = {{Enceladus's measured physical libration requires a global subsurface ocean}},
    year = {2016},
    journal = {Icarus},
    author = {Thomas, P. C. and Tajeddine, R. and Tiscareno, M. S. and Burns, J. A. and Joseph, J. and Loredo, T. J. and Helfenstein, P. and Porco, C.},
    pages = {37--47},
    volume = {264},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.08.037},
    isbn = {00191035},
    doi = {10.1016/j.icarus.2015.08.037},
    issn = {10902643},
    arxivId = {1509.07555},
    keywords = {Enceladus, Geophysics, Satellites, dynamics, Saturn, satellites}
}

@article{Giese2008,
    title = {{Enceladus: An estimate of heat flux and lithospheric thickness from flexurally supported topography}},
    year = {2008},
    journal = {Geophysical Research Letters},
    author = {Giese, Bernd and Wagner, Roland and Hussmann, Hauke and Neukum, Gerhard and Perry, Jason and Helfenstein, Paul and Thomas, Peter C.},
    number = {24},
    pages = {1--5},
    volume = {35},
    doi = {10.1029/2008GL036149},
    issn = {00948276},
    keywords = {http://dx.doi.org/10.1029/2008GL036149, doi:10.102}
}

@article{Beuthe2016a,
    title = {{Enceladus’ and Dione’s floating ice shells supported by minimum stress isostasy}},
    year = {2016},
    author = {Beuthe, Mikael and Rivoldini, Attilio and Trinh, Antony},
    doi = {10.1002/2016GL070650},
    keywords = {10.1002/2016GL070650 and Enceladus, Dione, crust, gravity, isostasy, subsurface ocean}
}

@article{Cravens2008,
    title = {{Energetic ion precipitation at Titan}},
    year = {2008},
    journal = {Geophysical Research Letters},
    author = {Cravens, T. E. and Robertson, I. P. and Ledvina, S. A. and Mitchell, D. and Krimigis, S. M. and Waite, J. H.},
    number = {3},
    pages = {2--5},
    volume = {35},
    doi = {10.1029/2007GL032451},
    issn = {00948276},
    keywords = {http://dx.doi.org/10.1029/2007GL032451, doi:10.102, s ionosphere, energetic particle precipitation at}
}

@article{Mitchell2005,
    title = {{Energetic Neutral Atom Emissions from Titan Interaction with Saturn's Magnetosphere}},
    year = {2005},
    journal = {Science},
    author = {Mitchell, D. G.},
    number = {5724},
    pages = {989--992},
    volume = {308},
    url = {http://www.sciencemag.org/cgi/doi/10.1126/science.1109805},
    doi = {10.1126/science.1109805},
    issn = {0036-8075}
}

@article{Patel1978,
    title = {{Energetics and Mechanism of the Solid-State Polymerization of Diacetylenes}},
    year = {1978},
    journal = {Journal of the American Chemical Society},
    author = {Patel, G. N. and Chance, R. R. and Turi, E. A. and Khanna, Y. P.},
    number = {21},
    pages = {6644--6649},
    volume = {100},
    doi = {10.1021/ja00489a015},
    issn = {15205126}
}

@article{Eckhardt1983,
    title = {{Energetics of Diacetylene Photopolymerization: A Calorimetric Study}},
    year = {1983},
    journal = {Macromolecules},
    author = {Eckhardt, Helmut and Prusik, Thaddeus and Chance, Ronald R},
    pages = {732--736},
    isbn = {8312216073}
}

@article{Lavvas2011a,
    title = {{Energy deposition and primary chemical products in Titan's upper atmosphere}},
    year = {2011},
    journal = {Icarus},
    author = {Lavvas, P. and Galand, M. and Yelle, R. V. and Heays, A. N. and Lewis, B. R. and Lewis, G. R. and Coates, A. J.},
    number = {1},
    pages = {233--251},
    volume = {213},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.03.001},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2011.03.001},
    issn = {00191035},
    keywords = {Photochemistry, Titan}
}

@article{Fischer2004,
    title = {{Energy dissipation of possible Titan lightning strokes}},
    year = {2004},
    journal = {Planetary and Space Science},
    author = {Fischer, G. and Tokano, T. and Macher, W. and Lammer, H. and Rucker, H. O.},
    number = {5-6},
    pages = {447--458},
    volume = {52},
    doi = {10.1016/j.pss.2003.05.011},
    issn = {00320633},
    keywords = {Lightning, Titan}
}

@article{Hendrix2017,
    title = {{Energy Options for Future Humans on Titan}},
    year = {2017},
    journal = {Journal of Astrobiology {\&} Outreach},
    author = {Hendrix, Amanda R. and Yung, Yuk L.},
    number = {2},
    pages = {2--5},
    volume = {5},
    url = {http://arxiv.org/abs/1707.00365%5Cnhttp://dx.doi.org/10.4172/2332-2519.1000157},
    doi = {10.4172/2332-2519.1000157},
    arxivId = {1707.00365},
    keywords = {isru, planetary environments, titan}
}

@article{Yelle1997,
    title = {{Engineering models for Titan's atmosphere}},
    year = {1997},
    journal = {Esa Sp},
    author = {Yelle, RV and Strobel, DF and Lellouch, E and Gautier, D},
    url = {http://pagesperso.lcp.u-psud.fr/pernot/ISSI_1D/Biblio/Yelle97.pdf}
}

@article{Mousis2014a,
    title = {{Equilibrium composition between liquid and clathrate reservoirs on Titan}},
    year = {2014},
    journal = {Icarus},
    author = {Mousis, Olivier and Choukroun, Mathieu and Lunine, Jonathan I. and Sotin, Christophe},
    number = {May},
    pages = {39--45},
    volume = {239},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.05.032},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.05.032},
    issn = {10902643},
    arxivId = {arXiv:1405.6588v1},
    keywords = {Titan, Titan, atmosphere, Titan, hydrology, Titan, surface}
}

@article{Ruiz2010,
    title = {{Equilibrium Convection on a Tidally Heated and Stressed Icy Shell of Europa for a Composite Water Ice Rheology}},
    year = {2010},
    journal = {Earth, Moon and Planets},
    author = {Ruiz, Javier},
    number = {2-4},
    pages = {157--167},
    volume = {107},
    doi = {10.1007/s11038-010-9357-0},
    issn = {01679295},
    keywords = {Europa, Heat flow, Ice rheology, Ice shell thickness, Satellites of Jupiter, Thermal convection}
}

@article{Hurford2007,
    title = {{Eruptions arising from tidally controlled periodic openings of rifts on Enceladus.}},
    year = {2007},
    journal = {Nature},
    author = {Hurford, T a and Helfenstein, Paul and Hoppa, Gregory V. and Greenberg, Richard and Bills, Bruce G},
    number = {7142},
    pages = {292--294},
    volume = {447},
    isbn = {0028-0836},
    doi = {10.1038/nature05821},
    issn = {0028-0836},
    pmid = {17507977}
}

@article{Nimmo2003,
    title = {{Estimates of Europa's ice shell thickness from elastically-supported topography}},
    year = {2003},
    journal = {Geophysical Research Letters},
    author = {Nimmo, F.},
    number = {5},
    pages = {1--4},
    volume = {30},
    doi = {10.1029/2002GL016660},
    issn = {0094-8276},
    keywords = {http://dx.doi.org/10.1029/2002GL016660, doi:10.102}
}

@article{Cordiner2014b,
    title = {{Ethyl cyanide on Titan: Spectroscopic detection and mapping using ALMA}},
    year = {2014},
    author = {Cordiner, M. A. and Palmer, M. Y. and Nixon, C. A. and Irwin, P. G. J. and Teanby, N. A. and Charnley, S. B. and Mumma, M. J. and Kisiel, Z. and Serigano, J. and Kuan, Y. -J. and Chuang, Y. -L. and Wang, K. -S.},
    pages = {3--8},
    url = {http://arxiv.org/abs/1410.5325%0Ahttp://dx.doi.org/10.1088/2041-8205/800/1/L14},
    doi = {10.1088/2041-8205/800/1/L14},
    issn = {2041-8213},
    arxivId = {1410.5325}
}

@article{Aguilera2013,
    title = {{Eukaryotic organisms in extreme acidic environments, the r{\'{i}}o tinto case.}},
    year = {2013},
    journal = {Life (Basel, Switzerland)},
    author = {Aguilera, A.},
    number = {3},
    pages = {363--74},
    volume = {3},
    url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=4187173&tool=pmcentrez&rendertype=abstract},
    doi = {10.3390/life3030363},
    issn = {2075-1729},
    pmid = {25369810},
    keywords = {acidophiles, eukaryots, extreme environments, extremophiles, photosynthesis}
}

@article{Phillips2014,
    title = {{Europa clipper mission concept: Exploring Jupiter's ocean moon}},
    year = {2014},
    journal = {Eos},
    author = {Phillips, Cynthia B. and Pappalardo, Robert T.},
    number = {20},
    pages = {165--167},
    volume = {95},
    doi = {10.1002/2014EO200002},
    issn = {23249250},
    keywords = {Europa, Jupiter, mission}
}

@article{Hendrix2011,
    title = {{Europa's disk-resolved ultraviolet spectra: Relationships with plasma flux and surface terrains}},
    year = {2011},
    journal = {Icarus},
    author = {Hendrix, Amanda R. and Cassidy, Timothy A. and Johnson, Robert E. and Paranicas, Chris and Carlson, Robert W.},
    number = {2},
    pages = {736--743},
    volume = {212},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.01.023},
    doi = {10.1016/j.icarus.2011.01.023},
    issn = {00191035},
    keywords = {Europa, Ices, UV spectroscopy, Jupiter, Satellites, Satellites, Composition, Ultraviolet observations}
}

@article{Dalton2012,
    title = {{Europa's icy bright plains and dark linea: Exogenic and endogenic contributions to composition and surface properties}},
    year = {2012},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Dalton, J. B. and Shirley, J. H. and Kamp, L. W.},
    number = {3},
    volume = {117},
    doi = {10.1029/2011JE003909},
    issn = {01480227},
    keywords = {Europa, composition, hydrates, infrared}
}

@article{Nimmo2005,
    title = {{Europa's icy shell: Past and present state, and future exploration}},
    year = {2005},
    journal = {Icarus},
    author = {Nimmo, Francis and Prockter, Louise and Schenk, Paul},
    number = {2},
    pages = {293--296},
    volume = {177},
    doi = {10.1016/j.icarus.2005.08.002},
    issn = {00191035}
}

@article{Sotin2002,
    title = {{Europa: Tidal heating of upwelling thermal plumes and the origin of lenticulae and chaos melting}},
    year = {2002},
    journal = {Geophysical Research Letters},
    author = {Sotin, Christophe},
    number = {8},
    pages = {2--5},
    volume = {29},
    doi = {10.1029/2001GL013844},
    issn = {0094-8276}
}

@article{Sotin2002a,
    title = {{Europa: Tidal heating of upwelling thermal plumes and the origin of lenticulae and chaos melting}},
    year = {2002},
    journal = {Geophysical Research Letters},
    author = {Sotin, Christophe},
    number = {8},
    pages = {2--5},
    volume = {29},
    isbn = {0094-8276},
    doi = {10.1029/2001GL013844},
    issn = {0094-8276},
    keywords = {http://dx.doi.org/10.1029/2001GL013844, doi:10.102}
}

@article{Kargel2000,
    title = {{Europa’s Crust and Ocean : Origin, Composition, and the Prospects for Life}},
    year = {2000},
    journal = {Icarus},
    author = {Kargel, Jeffrey S and Kaye, Jonathan Z and Head, James W and Marion, Giles M and Sassen, Roger and Crowley, James K and Grant, Steven A and Hogenboom, David L},
    pages = {226--265},
    volume = {265},
    doi = {10.1006/icar.2000.6471},
    keywords = {cryovolcanism, europa, ocean, prebiotic chemistry, spec-, troscopy}
}

@article{Imanaka2009,
    title = {{EUV photochemical production of unsaturated hydrocarbons: Implications to EUV photochemistry in Titan and Jovian planets}},
    year = {2009},
    journal = {Journal of Physical Chemistry A},
    author = {Imanaka, Hiroshi and Smith, Mark A.},
    number = {42},
    pages = {11187--11194},
    volume = {113},
    doi = {10.1021/jp9041952},
    issn = {10895639},
    pmid = {19673465}
}

@article{Griffith2006,
    title = {{Evidence for a polar ethane cloud on Titan}},
    year = {2006},
    journal = {Science},
    author = {Griffith, C. A. and Penteado, P. and Rannou, P. and Brown, R. and Boudon, V. and Baines, K. H. and Clark, R. and Drossart, P. and Buratti, B. and Nicholson, P. and McKay, C. P. and Coustenis, A. and Negrao, A. and Jaumann, R.},
    number = {5793},
    pages = {1620--1622},
    volume = {313},
    isbn = {1095-9203 (Electronic){\textbackslash}r0036-8075 (Linking)},
    doi = {10.1126/science.1128245},
    issn = {00368075},
    pmid = {16973876}
}

@article{Kristjansdottir,
    title = {{Evidence for a subsurface ocean on Europa}},
    author = {Kristj{\'{a}}nsd{\'{o}}ttir, Sigríður}
}

@article{West1991,
    title = {{Evidence for aggregate particles in the atmospheres of Titan and Jupiter}},
    year = {1991},
    journal = {Icarus},
    author = {West, Robert A. and Smith, Peter H.},
    number = {2},
    pages = {330--333},
    volume = {90},
    doi = {10.1016/0019-1035(91)90113-8},
    issn = {10902643}
}

@article{Kre2010,
    title = {{Evidence for Diacetylene Cation as the Carrier of a Diffuse Interstellar Band}},
    year = {2010},
    journal = {The Astrophysical Journal},
    author = {Kre{\l}, J and Beletsky, Y and Galazutdinov, G A and Ko{\l}os, R and Gronowski, M. and LoCurto, G.},
    pages = {64--67},
    volume = {1},
    doi = {10.1088/2041-8205/714/1/L64},
    keywords = {ism, molecules}
}

@article{Wang2010,
    title = {{Evidence for layered methane clouds in Titan's troposphere}},
    year = {2010},
    journal = {Icarus},
    author = {Wang, Chia C. and Atreya, Sushil K. and Signorell, Ruth},
    number = {2},
    pages = {787--790},
    volume = {206},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.11.022},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.11.022},
    issn = {00191035},
    keywords = {Atmospheres, Structure, Structure, Titan}
}

@article{Kattenhorn2014,
    title = {{Evidence for subduction in the ice shell of Europa}},
    year = {2014},
    journal = {Nature Geoscience},
    author = {Kattenhorn, Simon A. and Prockter, Louise M.},
    number = {10},
    pages = {762--767},
    volume = {7},
    url = {http://www.nature.com/doifinder/10.1038/ngeo2245},
    isbn = {1752-0908},
    doi = {10.1038/ngeo2245},
    issn = {1752-0894}
}

@article{Griffith2003,
    title = {{Evidence for the Exposure of Water Ice on Titan’s Surface}},
    year = {2003},
    journal = {Science},
    author = {Griffith, Caitlin A and Owen, Tobias and Geballe, Thomas R and Rayner, John and Rannou, Pascal},
    number = {April},
    pages = {628--630},
    volume = {300},
    doi = {10.1126/science.1081897},
    issn = {00368075}
}

@article{Morente2008,
    title = {{Evidence of electrical activity on Titan drawn from the Schumann resonances sent by Huygens probe}},
    year = {2008},
    journal = {Icarus},
    author = {Morente, Juan A. and Port??, Jorge A. and Salinas, Alfonso and Navarro, Enrique A.},
    number = {2},
    pages = {802--811},
    volume = {195},
    doi = {10.1016/j.icarus.2008.02.004},
    issn = {00191035},
    keywords = {Ionospheres, Lightning, Titan}
}

@misc{Atreya1978,
    title = {{Evolution of a nitrogen atmosphere on Titan}},
    year = {1978},
    booktitle = {Science},
    author = {Atreya, SK and Donahue, TM and Kuhn, WR},
    number = {4356},
    pages = {611--613},
    volume = {201},
    url = {http://www-personal.umich.edu/~atreya/Articles/1978_Evolution_Nitrogen.pdf},
    issn = {00368075}
}

@article{Johnson2016,
    title = {{Evolution of an early Titan atmosphere}},
    year = {2016},
    journal = {Icarus},
    author = {Johnson, R E and Tucker, O J and Volkov, A N},
    pages = {202--206},
    volume = {271},
    publisher = {Elsevier Inc.},
    doi = {10.1016/j.icarus.2016.01.014},
    keywords = {"Atmospheres, Atmosphere, Titan, atmospheres, evolution, evolution"}
}

@article{Johnson2013,
    title = {{Evolution of an Early Titan Atmosphere: Comment}},
    year = {2013},
    journal = {Journal of Chemical Information and Modeling},
    author = {Johnson, R.E. and Tucker, O J and Volkov, A. N.},
    number = {9},
    pages = {1689--1699},
    volume = {53},
    isbn = {9788578110796},
    doi = {10.1017/CBO9781107415324.004},
    issn = {1098-6596},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {icle}
}

@article{Gebauer2009,
    title = {{Evolution of Earth-like Extrasolar Planetary Atmospheres: Assessing the Atmospheres and Biospheres of Early Earth Analog Planets with a Coupled Atmosphere Biogeochemical Model}},
    year = {2009},
    journal = {Astrobiology},
    author = {Gebauer, S. and Grenfell, J.L. and Stock, J.W. and Lehmann, R. and Godolt, M. and von Paris, P. and Rauer, H.},
    number = {1},
    pages = {27--54},
    volume = {17},
    url = {http://online.liebertpub.com/doi/10.1089/ast.2015.1384},
    isbn = {1531-1074},
    doi = {10.1089/ast.2015.1384},
    issn = {1531-1074},
    pmid = {28103105}
}

@article{Geissler1998,
    title = {{Evolution of Lineaments on Europa : Clues from Galileo Multispectral Imaging Observations}},
    year = {1998},
    journal = {Icarus},
    author = {Geissler, P E and Greenberg, R and Hoppa, G and Mcewen, a and Tufts, R and Phillips, C and Sullivan, R and Greeley, R and Clark, B and Ockert-Bell, M and Helfenstein, P and Burns, J a and Veverka, J and Pappalardo, R T and Head, J W and Belton, M J S and Denk, T},
    pages = {107--126},
    volume = {135},
    doi = {10.1006/icar.1998.5980},
    issn = {00191035}
}

@article{Gilliam2014a,
    title = {{Evolution of Titan's major atmospheric gases and cooling since accretion}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Gilliam, Ashley E. and Lerman, Abraham},
    pages = {41--53},
    volume = {93-94},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2014.02.001},
    doi = {10.1016/j.pss.2014.02.001},
    issn = {00320633},
    keywords = {Atmosphere, Cooling, Kinetic model, Methane and ammonia, Thermal escape, Titan}
}

@article{Gilliam2014,
    title = {{Evolution of Titan's major atmospheric gases and cooling since accretion}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Gilliam, Ashley E. and Lerman, Abraham},
    pages = {41--53},
    volume = {93-94},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2014.07.005},
    doi = {10.1016/j.pss.2014.02.001},
    issn = {00320633},
    keywords = {Atmosphere, Cooling, Kinetic model, Methane and ammonia, Thermal escape, Titan}
}

@article{Gudipati1994,
    title = {{Exciton, exchange, and through-bond interactions in multichromophoric molecules: An analysis of the electronic excited states}},
    year = {1994},
    journal = {Journal of Physical Chemistry},
    author = {Gudipati, Murthy S.},
    number = {39},
    pages = {9750--9763},
    volume = {98},
    isbn = {0022365419},
    doi = {10.1021/j100090a007},
    issn = {00223654}
}

@article{Raulin1995,
    title = {{Exobiology on Titan}},
    year = {1995},
    journal = {Journal of Biological Physics},
    author = {Raulin, F. and Bruston, P. and Coll, P. and Coscia, D. and Gazeau, M.-C. and Guez, L and de Vanssay, E.},
    pages = {39--53}
}

@article{Yurchenko2018,
    title = {{ExoCross: A general program for generating spectra from molecular line lists}},
    year = {2017},
    journal = {Astronomy {\&} Astrophysics},
    author = {Yurchenko, Sergei N and Al-Refaie, Ahmed F and Tennyson, Jonathan},
    arxivId = {1801.09803}
}

@article{Oza2018a,
    title = {{Exogenic Volatiles in the Extended Exospheres of Extrasolar Giant Planets}},
    year = {2018},
    journal = {EPSC2018},
    author = {Oza, A. and Johnson, R. E. and Arras, P. and Thomas, N. and Schmidt, C. and Demory, B. O. and Mordasini, C. and Wyttenbach, A. and Schneider, N. and Bourrier, V. and Ehrenreich, D. and Allart, R. and Dubois, D. and Saxena, P.},
    number = {2015},
    pages = {189733},
    volume = {12}
}

@article{Khalafinejad2016,
    title = {{Exoplanetary atmospheric sodium revealed by the orbital motion. Narrow-band transmission spectroscopy of HD 189733b with UVES}},
    year = {2016},
    author = {Khalafinejad, S. and von Essen, C. and Hoeijmakers, H. J. and Zhou, G. and Klocova, T. and Schmitt, J. H. M. M. and Dreizler, S. and Lopez-Morales, M. and Husser, T. -O. and Schmidt, T. O. B. and Collet, R.},
    url = {http://arxiv.org/abs/1610.01610},
    arxivId = {1610.01610},
    keywords = {activity, atmospheres, hd 189733b, individual, instru-, mentation, methods, observational - stars, planetary systems, planets and satellites, spectrographs, spectroscopic, techniques}
}

@article{Agarwal2016,
    title = {{Exoplanetary Detection By Multifractal Spectral Analysis}},
    year = {2016},
    journal = {The Astronomical Journal},
    author = {Agarwal, Sahil and Sordo, Fabio Del and Wettlaufer, John S.},
    number = {1},
    pages = {12},
    volume = {153},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/1538-3881/153/i=1/a=12?key=crossref.4f1595fe3e84007e0c6aa4b577419d4c},
    doi = {10.3847/1538-3881/153/1/12},
    issn = {1538-3881},
    keywords = {analytical, data analysis, detection, methods, methods: analytical, methods: data analysis, methods: observational, methods: statistical, observational, planets and satellites, planets and satellites: detection, spectroscopic, statistical, techniques, techniques: spectroscopic}
}

@article{Berthelier2016,
    title = {{Exosphere Ionization Europa EGM}},
    year = {2016},
    author = {Berthelier, Jean-jacques}
}

@article{Verma2018,
    title = {{Expected Precision of Europa Clipper Gravity Measurements}},
    year = {2018},
    author = {Verma, Ashok K. and Margot, Jean-Luc},
    pages = {1--26},
    url = {http://arxiv.org/abs/1801.08946},
    arxivId = {1801.08946}
}

@article{Desrier2016,
    title = {{Experimental and ab initio characterization of HC3N+ vibronic structure. I. Synchrotron-based threshold photo-electron spectroscopy}},
    year = {2016},
    journal = {The Journal of Chemical Physics},
    author = {Desrier, Antoine and Romanzin, Claire and Lamarre, Nicolas and Alcaraz, Christian and Gans, Bérenger and Gauyacq, Dolores and Li{\'{e}}vin, Jacques and Boy{\'{e}}-P{\'{e}}ronne, Séverine},
    number = {23},
    pages = {234310},
    volume = {145},
    url = {http://scitation.aip.org/content/aip/journal/jcp/145/23/10.1063/1.4972019},
    doi = {10.1063/1.4972019},
    issn = {0021-9606},
    pmid = {28010106}
}

@article{Vuitton2006,
    title = {{Experimental and theoretical study of hydrocarbon photochemistry applied to Titan stratosphere}},
    year = {2006},
    journal = {Icarus},
    author = {Vuitton, V. and Doussin, J. F. and B{\'{e}}nilan, Y. and Raulin, F. and Gazeau, M. C.},
    number = {1},
    pages = {287--300},
    volume = {185},
    doi = {10.1016/j.icarus.2006.06.002},
    issn = {00191035},
    keywords = {Atmospheres, Experimental techniques, Photochemistry, Titan, composition}
}

@article{Luspay-Kuti2015,
    title = {{Experimental constraints on the composition and dynamics of Titan's polar lakes}},
    year = {2015},
    journal = {Earth and Planetary Science Letters},
    author = {Luspay-Kuti, A. and Chevrier, V. F. and Cordier, D. and Rivera-Valentin, E. G. and Singh, S. and Wagner, A. and Wasiak, F. C.},
    pages = {75--83},
    volume = {410},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.epsl.2014.11.023},
    isbn = {0012-821X},
    doi = {10.1016/j.epsl.2014.11.023},
    issn = {0012821X},
    keywords = {Evaporation rate, Experimental, Hydrocarbon lakes, Lake composition, Titan}
}

@article{SinghS2017,
    title = {{Experimental determination of acetylene and ethylene solubility in liquid methane and ethane: Implications to Titan's surface}},
    year = {2017},
    journal = {Geochimica et Cosmochimica Acta},
    author = {Singh, S. and Combe, J. P. and Cordier, D. and Wagner, A. and Chevrier, V. F. and McMahon, Z.},
    pages = {86--101},
    volume = {208},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.gca.2017.03.007},
    doi = {10.1016/j.gca.2017.03.007},
    issn = {00167037},
    keywords = {Acetylene, Atmosphere, Ethylene, Infrared spectroscopy, Planetary surfaces, Solubility, Titan}
}

@article{Danger2011,
    title = {{Experimental investigation of aminoacetonitrile formation through the Strecker synthesis in astrophysical-like conditions: reactivity of methanimine (CH2NH), ammonia (NH3), and hydrogen cyanide (HCN)}},
    year = {2011},
    journal = {Astronomy {\&} Astrophysics},
    author = {Danger, G and Borget, F and Chomat, M and Duvernay, F and Theul{\'{e}}, P and Guillemin, J C and Le Sergeant d'Hendecourt, L and Chiavassa, T},
    pages = {A47},
    volume = {535},
    isbn = {0004-6361},
    doi = {10.1051/0004-6361/201117602},
    issn = {0004-6361},
    keywords = {astrochemistry, ism, laboratory, methods, molecules}
}

@article{Sagan1971,
    title = {{Experimental Jovian Photochemistry: Initial Results}},
    year = {1971},
    journal = {The Astrophysical Journal},
    author = {Sagan, C. and Khare, B. N.},
    number = {c},
    pages = {563--569},
    volume = {15}
}

@article{Coll1999,
    title = {{Experimental laboratory simulation of Titan’s atmosphere: aerosols and gas phase}},
    year = {1999},
    journal = {Planetary and Space Science},
    author = {Coll, P. and Coscia, D. and Smith, N. and Gazeau, M.-C. and Ramı́rez, S.I. and Cernogora, G. and Isra{\"{e}}l, G. and Raulin, F.},
    number = {10-11},
    pages = {1331--1340},
    volume = {47},
    isbn = {0032-0633},
    doi = {10.1016/S0032-0633(99)00054-9},
    issn = {00320633},
    keywords = {aerosol analysis, c 4 n 2, laboratory simulation, planetary atmosphere, titan}
}

@article{Singh2017b,
    title = {{Experimental reflectance study of methane and ethane ice at Titan’s surface conditions}},
    year = {2017},
    journal = {Astrophysics and Space Science},
    author = {Singh, G. and Singh, S. and Wagner, A. and Chevrier, V. F. and Combe, J.-P. and Gainor, M.},
    number = {10},
    pages = {184},
    volume = {362},
    publisher = {Springer Science+Business Media B.V.},
    url = {http://link.springer.com/10.1007/s10509-017-3166-0},
    doi = {10.1007/s10509-017-3166-0},
    issn = {0004-640X},
    keywords = {atmospheres, planetary surfaces, titan}
}

@article{Ringbauer2014,
    title = {{Experimental simulation of closed timelike curves}},
    year = {2014},
    journal = {Nature Communications},
    author = {Ringbauer, Martin and Broome, Matthew A and Myers, Casey R and White, Andrew G and Ralph, Timothy C},
    number = {May},
    pages = {4145},
    volume = {5},
    url = {http://www.nature.com/ncomms/2014/140619/ncomms5145/full/ncomms5145.html%5Cnhttp://www.nature.com/doifinder/10.1038/ncomms5145},
    doi = {10.1038/ncomms5145},
    issn = {2041-1723},
    pmid = {24942489},
    arxivId = {arXiv:1501.0501}
}

@article{Gautier2013,
    title = {{Experimental simulation of Titan’s aerosols formation}},
    year = {2013},
    author = {Gautier, Thomas and Bousquet, Pr Philippe and Rannou, Pr Pascal and Lellouch, Pr Emmanuel and Fichtner, Pr Horst}
}

@article{Gudmundsson1999,
    title = {{Experimental studies of O 2 /Ar plasma in a planar inductive discharge}},
    year = {1999},
    journal = {Plasma Sources Science and Technology},
    author = {Gudmundsson, J T and Kimura, T. and Lieberman, M.},
    number = {1},
    pages = {22--30},
    volume = {8},
    url = {http://stacks.iop.org/0963-0252/8/i=1/a=003?key=crossref.47514f9adf2b7c80d343b6ddf2104a36},
    isbn = {0963-0252},
    doi = {10.1088/0963-0252/8/1/003},
    issn = {0963-0252}
}

@article{Hong2018,
    title = {{Experimental study of heterogeneous organic chemistry induced by far ultraviolet light: Implications for growth of organic aerosols by CH 3 addition in the atmospheres of Titan and early Earth}},
    year = {2018},
    journal = {Icarus},
    author = {Hong, Peng and Sekine, Yasuhito and Sasamori, Tsutoni and Sugita, Seiji},
    pages = {25--39},
    volume = {307},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103516304997},
    doi = {10.1016/j.icarus.2018.02.019},
    issn = {00191035},
    keywords = {"Titan, atmosphere", Atmospheric chemistry, Organic chemistry, Photochemistry, atmospheric chemistry}
}

@article{Vidali2004,
    title = {{Experimental study of the formation of molecular hydrogen and carbon dioxide on dust grain analogues}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Vidali, G. and Roser, J. E. and Manic{\`{o}}, G. and Pirronello, V.},
    number = {1},
    pages = {6--13},
    volume = {33},
    doi = {10.1016/j.asr.2003.08.003},
    issn = {02731177},
    keywords = {Dust grains, ISM, Molecular hydrogen}
}

@article{Barge2017,
    title = {{Experimentally Testing Hydrothermal Vent Origin of Life on Enceladus and Other Icy/Ocean Worlds}},
    year = {2017},
    journal = {Astrobiology},
    author = {Barge, Laura M. and White, Lauren M.},
    number = {9},
    pages = {ast.2016.1633},
    volume = {17},
    url = {http://online.liebertpub.com/doi/10.1089/ast.2016.1633},
    isbn = {1531-1074},
    doi = {10.1089/ast.2016.1633},
    issn = {1531-1074}
}

@article{Mitri2017,
    title = {{Explorer of Enceladus and Titan (E 2 T): Investigating ocean worlds' evolution and habitability in the solar system}},
    year = {2017},
    journal = {Planetary and Space Science},
    author = {Mitri, Giuseppe and Postberg, Frank and Soderblom, Jason M. and Wurz, Peter and Tortora, Paolo and Abel, Bernd and Barnes, Jason W. and Berga, Marco and Carrasco, Nathalie and Coustenis, Athena and Paul de Vera, Jean Pierre and D'Ottavio, Andrea and Ferri, Francesca and Hayes, Alexander G. and Hayne, Paul O. and Hillier, Jon K. and Kempf, Sascha and Lebreton, Jean-Pierre and Lorenz, Ralph D. and Martelli, Andrea and Orosei, Roberto and Petropoulos, Anastassios E. and Reh, Kim and Schmidt, Juergen and Sotin, Christophe and Srama, Ralf and Tobie, Gabriel and Vorburger, Audrey and Vuitton, Véronique and Wong, Andre and Zannoni, Marco},
    publisher = {Elsevier Ltd},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0032063317301447},
    doi = {10.1016/j.pss.2017.11.001},
    issn = {00320633}
}

@article{Tinetti2010,
    title = {{Exploring Extrasolar Worlds Today and Tomorrow}},
    year = {2010},
    author = {Tinetti, G. and Griffith, C. A.},
    pages = {115},
    volume = {430},
    url = {http://adsabs.harvard.edu/abs/2010ASPC..430..115T},
    isbn = {1050-3390}
}

@article{Edberg2013,
    title = {{Extreme densities in Titan's ionosphere during the T85 magnetosheath encounter}},
    year = {2013},
    journal = {Geophysical Research Letters},
    author = {Edberg, N. J.T. and Andrews, D. J. and Shebanits, O. and {\AA}gren, K. and Wahlund, J. E. and Opgenoorth, H. J. and Roussos, E. and Garnier, P. and Cravens, T. E. and Badman, S. V. and Modolo, R. and Bertucci, C. and Dougherty, M. K.},
    number = {12},
    pages = {2879--2883},
    volume = {40},
    doi = {10.1002/grl.50579},
    issn = {00948276},
    keywords = {Cassini, Titan, ionization, ionosphere, magnetosheath}
}

@article{Friedlaender2013,
    title = {{Extreme diel variation in the feeding behavior of humpback whales along the western Antarctic Peninsula during autumn}},
    year = {2013},
    journal = {Marine Ecology Progress Series},
    author = {Friedlaender, A. S. and Tyson, R. B. and Stimpert, A. K. and Read, A. J. and Nowacek, D. P.},
    pages = {281--289},
    volume = {494},
    isbn = {0171-8630; 1616-1599},
    doi = {10.3354/meps10541},
    issn = {01718630},
    keywords = {Antarctica, Foraging ecology, Humpback whale, Tagging}
}

@article{Broadfoot1981,
    title = {{Extreme Ultraviolet Observations from Voyager 1 Encounter with Saturn}},
    year = {1981},
    author = {Broadfoot, A. L. and Sandel, B. R. and Shemansky, D and Holberg, J. B. and Smith, G. R.},
    number = {April},
    volume = {212}
}

@article{Modolo2007,
    title = {{Far plasma wake of Titan from the RPWS observations: A case study}},
    year = {2007},
    journal = {Geophysical Research Letters},
    author = {Modolo, R. and Wahlund, J. E. and Bostr{\"{o}}m, R. and Canu, P. and Kurth, W. S. and Gurnett, D. and Lewis, G. R. and Coates, Andrew J.},
    number = {24},
    volume = {34},
    isbn = {0094-8276},
    doi = {10.1029/2007GL030482},
    issn = {00948276}
}

@article{Kattenhorn2006,
    title = {{Fault-induced perturbed stress fields and associated tensile and compressive deformation at fault tips in the ice shell of Europa: implications for fault mechanics}},
    year = {2006},
    journal = {Journal of Structural Geology},
    author = {Kattenhorn, Simon A. and Marshall, Scott T.},
    number = {12},
    pages = {2204--2221},
    volume = {28},
    isbn = {0191-8141},
    doi = {10.1016/j.jsg.2005.11.010},
    issn = {01918141},
    keywords = {Anti-cracks, Compression, Europa, Faults, Stress, Strike-slip, Tailcracks}
}

@article{Friedlaender2014,
    title = {{Feeding rates and under-ice foraging strategies of the smallest lunge filter feeder, the Antarctic minke whale (Balaenoptera bonaerensis)}},
    year = {2014},
    journal = {Journal of Experimental Biology},
    author = {Friedlaender, Ari S. and Goldbogen, Jeremy A. and Nowacek, D. P. and Read, A. J. and Johnston, D. and Gales, N.},
    number = {16},
    pages = {2851--2854},
    volume = {217},
    url = {http://jeb.biologists.org/content/217/16/2851.abstract},
    isbn = {0022-0949},
    doi = {10.1242/jeb.106682},
    issn = {0022-0949},
    pmid = {25122916},
    keywords = {feeding, minke whales, performance}
}

@article{Sotin2008,
    title = {{Figure 2: Phase diagram of water ice with temperature pro- files to illustrate the structure described in Fig. 1. Figure 1: Internal structure of Europa (left) and Ganymede (right). Figure from [1].}},
    year = {2008},
    author = {Sotin, C. and Tobie, G. and Duval, P.},
    pages = {4--5}
}

@article{Kliore2008,
    title = {{First results from the Cassini radio occultations of the Titan ionosphere}},
    year = {2008},
    author = {Kliore, Avydas J and Nagy, Andrew F and Marouf, Essam A and French, Richard G and Flasar, F Michael and Rappaport, Nicole J and Anabttawi, Aseel and Asmar, Sami W and Kahann, Daniel S and Barbinis, Elias and Goltz, Gene L and Fleischman, Don U and Rochblatt, David J},
    pages = {1--9},
    volume = {113},
    doi = {10.1029/2007JA012965},
    keywords = {http://dx.doi.org/10.1029/2007JA012965, doi:10.102}
}

@article{Courtin2011,
    title = {{First results of Herschel -SPIRE observations of Titan}},
    year = {2011},
    journal = {Astronomy {\&} Astrophysics},
    author = {Courtin, R. and Swinyard, B. M. and Moreno, R. and Fulton, T. and Lellouch, E. and Rengel, M. and Hartogh, P.},
    pages = {L2},
    volume = {536},
    url = {http://www.aanda.org/articles/aa/full_html/2011/12/aa18304-11/aa18304-11.html},
    doi = {10.1051/0004-6361/201118304},
    issn = {0004-6361},
    keywords = {individual, planetary systems, planets and satellites, spectroscopic, submillimeter, techniques, titan}
}

@article{Bills2011,
    title = {{Forced obliquities and moments of inertia of Ceres and Vesta}},
    year = {2011},
    journal = {Icarus},
    author = {Bills, B. G. and Nimmo, F.},
    number = {2},
    pages = {496--509},
    volume = {213},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.09.002},
    doi = {10.1016/j.icarus.2010.09.002},
    issn = {00191035},
    keywords = {Asteroid Ceres, Asteroid Vesta, Asteroids, Dynamics, Rotational dynamics}
}

@article{Bills2008,
    title = {{Forced obliquity and moments of inertia of Titan}},
    year = {2008},
    journal = {Icarus},
    author = {Bills, Bruce G. and Nimmo, Francis},
    number = {1},
    pages = {293--297},
    volume = {196},
    doi = {10.1016/j.icarus.2008.03.002},
    issn = {00191035},
    keywords = {Rotational dynamics, Tides, Titan}
}

@article{Vuitton2008,
    title = {{Formation and distribution of benzene on Titan}},
    year = {2008},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Vuitton, V. and Yelle, R. V. and Cui, J.},
    number = {5},
    pages = {1--18},
    volume = {113},
    doi = {10.1029/2007JE002997},
    issn = {01480227},
    keywords = {http://dx.doi.org/10.1029/2007JE002997, doi:10.102}
}

@article{Coustenis2005,
    title = {{Formation and evolution of Titan's atmosphere}},
    year = {2005},
    journal = {Space Science Reviews},
    author = {Coustenis, A.},
    number = {1-2},
    pages = {171--184},
    volume = {116},
    isbn = {0038-6308},
    doi = {10.1007/s11214-005-1954-2},
    issn = {00386308},
    keywords = {Atmospheres, Infrared, Satellites, Solar System, Space missions, Titan}
}

@article{Horst2012,
    title = {{Formation of Amino Acids and Nucleotide Bases in a Titan Atmosphere Simulation Experiment}},
    year = {2012},
    journal = {Astrobiology},
    author = {H{\"{o}}rst, S.M. and Yelle, R.V. and Buch, A. and Carrasco, N. and Cernogora, G. and Dutuit, O. and Quirico, E. and Sciamma-O'Brien, E. and Smith, M.a. and Somogyi, Á. and Szopa, C. and Thissen, R. and Vuitton, V.},
    number = {9},
    pages = {809--817},
    volume = {12},
    url = {http://online.liebertpub.com/doi/abs/10.1089/ast.2011.0623},
    isbn = {1531-1074},
    doi = {10.1089/ast.2011.0623},
    issn = {1531-1074},
    pmid = {22917035}
}

@article{Hoppa1999,
    title = {{Formation of cycloidal features on Europa}},
    year = {1999},
    journal = {Science},
    author = {Hoppa, G V and Tufts, B R and Greenberg, R and Geissler, P E},
    number = {5435},
    pages = {1899--902},
    volume = {285},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/10489365},
    doi = {10.1126/science.285.5435.1899},
    issn = {0036-8075},
    pmid = {10489365},
    keywords = {Extraterrestrial Environment, Ice, Jupiter}
}

@article{Yelle2010,
    title = {{Formation of NH3 and CH2NH in Titan's upper atmosphere}},
    year = {2010},
    journal = {Faraday Discussions},
    author = {Yelle, Roger V and Vuitton, V and Lavvas, P and Klippenstein, S J and Smith, M a and H{\"{o}}rst, S M and Cui, J},
    pages = {31},
    volume = {147},
    url = {http://xlink.rsc.org/?DOI=c004787m},
    isbn = {1359-6640},
    doi = {10.1039/c004787m},
    issn = {1359-6640}
}

@article{Drilling2010,
    title = {{Formation of NH3 and HCN in atmospheric glow discharge fed by gaseous CH4-N2 mixture discharge fed by gaseous CH 4 -N 2 mixture}},
    year = {2010},
    author = {Drilling, Horvath G A and Republic, Slovak},
    number = {June 2014},
    pages = {4--6}
}

@article{Sun2015,
    title = {{Formation of Polyynes C4H2, C6H2, C8H2, and C10H2 from Reactions of C2H, C4H, C6H, and C8H Radicals with C2H2}},
    year = {2015},
    journal = {The Journal of Physical Chemistry Letters},
    author = {Sun, Y-L. and Huang, W-J. and Lee, S-H.},
    number = {3},
    pages = {909--911},
    volume = {47},
    url = {http://dx.doi.org/10.1016/j.carbon.2008.11.049},
    doi = {10.1016/j.carbon.2008.11.049},
    issn = {0008-6223}
}

@article{Tooke1988,
    title = {{Fourier self-deconvolution in IR spectroscopy}},
    year = {1988},
    journal = {Trends in Analytical Chemistry},
    author = {Tooke, P. B.},
    number = {4},
    pages = {130--136},
    volume = {7},
    isbn = {0165-9936},
    doi = {10.1016/0165-9936(88)87010-9},
    issn = {01659936}
}

@article{Branscomb2018,
    title = {{Frankenstein or a Submarine Alkaline Vent: Who is Responsible for Abiogenesis?: Part 1: What is life-that it might create itself?}},
    year = {2018},
    journal = {BioEssays},
    author = {Branscomb, Elbert and Russell, Michael J.},
    number = {8},
    pages = {1--8},
    volume = {40},
    doi = {10.1002/bies.201700182},
    issn = {15211878}
}

@article{Branscomb2018a,
    title = {{Frankenstein or a Submarine Alkaline Vent: Who is Responsible for Abiogenesis?: Part 2: As life is now, so it must have been in the beginning}},
    year = {2018},
    journal = {BioEssays},
    author = {Branscomb, Elbert and Russell, Michael J.},
    number = {8},
    pages = {1--10},
    volume = {40},
    doi = {10.1002/bies.201700182},
    issn = {15211878}
}

@article{Bills2005,
    title = {{Free and forced obliquities of the Galilean satellites of Jupiter}},
    year = {2005},
    journal = {Icarus},
    author = {Bills, Bruce G.},
    number = {1},
    pages = {233--247},
    volume = {175},
    isbn = {-},
    doi = {10.1016/j.icarus.2004.10.028},
    issn = {00191035},
    keywords = {Callisto, Europa, Ganymede, Io, Obliquity, Rotational dynamics}
}

@article{Capone1983,
    title = {{Galactic Cosmic Rays and N2 Dissociation on Titan}},
    year = {1983},
    journal = {Icarus},
    author = {Capone, L A and Dubach, J and Prasad, S S and Whitten, R C},
    number = {1},
    pages = {73--82},
    volume = {55},
    keywords = {GALACTIC COSMIC RAYS, GAS DISSOCIATION, NITROGEN}
}

@article{Rathbun2014,
    title = {{Galileo PPR Observations of Europa: Correlations of Thermophysical Properties with Exogenic and Endogenic Processes}},
    year = {2014},
    journal = {Workshop on the Habitability of Icy Worlds},
    author = {Rathbun, Julie A. and Spencer, J. R. and Howett, C. J A},
    pages = {85719}
}

@article{Rathbun2010,
    title = {{Galileo PPR observations of Europa: Hotspot detection limits and surface thermal properties}},
    year = {2010},
    journal = {Icarus},
    author = {Rathbun, Julie A. and Rodriguez, Nathaniel J. and Spencer, John R.},
    number = {2},
    pages = {763--769},
    volume = {210},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.07.017},
    doi = {10.1016/j.icarus.2010.07.017},
    issn = {00191035},
    keywords = {Europa, Satellites, Surfaces, Thermal histories}
}

@article{Ling2005,
    title = {{Gamma-Ray Spectral Characteristics of Thermal and Non-Thermal Emission from Three Black Holes}},
    year = {2005},
    journal = {Chinese Journal of Astronomy and Astrophysics},
    author = {Ling, J. C. and Wheaton, W.},
    volume = {80}
}

@article{Vance2014,
    title = {{Ganymede's internal structure including thermodynamics of magnesium sulfate oceans in contact with ice}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Vance, Steve and Bouffard, Mathieu and Choukroun, Mathieu and Sotin, Christophe},
    pages = {62--70},
    volume = {96},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2014.03.011},
    isbn = {00320633},
    doi = {10.1016/j.pss.2014.03.011},
    issn = {00320633},
    keywords = {Equations of state, Ganymede, Geophysics, High pressure, JUICE, Oceanography}
}

@article{Scattergood1987a,
    title = {{Gas chromatographic instrumention for the analysis of aerosols and gases in Titan's atmosphere}},
    year = {1987},
    author = {Scattergood, T W and Valentin, J R and Hara, B J O and Kojiro, D R and Carle, G C},
    number = {6},
    keywords = {doi:10., http://dx.doi.org/10.1029/JB092iB04p0E723}
}

@article{Torokova2015a,
    title = {{Gas Chromatography Analysis of Discharge Products in N2-CH4 Gas Mixture at Atmospheric Pressure: Study of Mimic Titan's Atmosphere}},
    year = {2015},
    journal = {Contributions to Plasma Physics},
    author = {Torokova, L. and Watson, J. and Krcma, F. and Mazankova, V. and Mason, N. J. and Horvath, G. and Matejcik, S.},
    number = {X},
    pages = {n/a-n/a},
    volume = {11},
    url = {http://doi.wiley.com/10.1002/ctpp.201400052},
    doi = {10.1002/ctpp.201400052},
    issn = {08631042},
    keywords = {atmospheric pressure glow discharge, gas chromatography, nitrogen-methane gas mixture}
}

@article{Sharpe2004,
    title = {{Gas Phase Database for Quantitative Infrared Spectroscopy}},
    year = {2004},
    journal = {Applied Spectroscopy},
    author = {Sharpe, S.N. and Johnson, T.J. and James, R.L. and Chu, P.M. and Rhoderick, G.C. and Johnson, P.a.},
    number = {12},
    pages = {1452--1461},
    volume = {58},
    isbn = {0003-7028 (Print){\textbackslash}r0003-7028 (Linking)},
    doi = {10.1366/0003702042641281},
    issn = {0003-7028},
    pmid = {15606959},
    arxivId = {arXiv:1011.1669v3}
}

@article{Jolly2015,
    title = {{Gas phase dicyanoacetylene (C4N2) on Titan: New experimental and theoretical spectroscopy results applied to Cassini CIRS data}},
    year = {2015},
    journal = {Icarus},
    author = {Jolly, A. and Cottini, V. and Fayt, A. and Manceron, L. and Kwabia-Tchana, F. and Benilan, Y. and Guillemin, J. C. and Nixon, C. and Irwin, P.},
    pages = {340--346},
    volume = {248},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.10.049},
    doi = {10.1016/j.icarus.2014.10.049},
    issn = {10902643},
    keywords = {Abundance, atmosphere, IR observations, IR spectroscopy, Titan}
}

@inproceedings{Romanzin2018,
    title = {{Gas phase ion-molecule chemistry: controlled reactions of methyl cations with O-bearing compounds and hydrocarbons}},
    year = {2018},
    booktitle = {XXIst Symposium on Atomic, Cluster and Surface Physics 2018 (SASP 2018)},
    author = {Romanzin, C. and Thissen, R. and Lopes, A. and Miranda, Barbara Cunha De and Alcaraz, C.}
}

@article{Shi2000,
    title = {{Gas-phase acidity and C – H bond energy of diacetylene}},
    year = {2000},
    journal = {Chem. Phys. Lett.},
    author = {Shi, Yang and Ervin, Kent M.},
    number = {February},
    pages = {149--154},
    volume = {318}
}

@article{Blagojevic2003,
    title = {{Gas-phase syntheses for interstellar carboxylic and amino acids}},
    year = {2003},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Blagojevic, Voislav and Petrie, Simon and Bohme, Diethard K.},
    number = {1},
    volume = {339},
    isbn = {0035-8711},
    doi = {10.1046/j.1365-8711.2003.06351.x},
    issn = {00358711},
    keywords = {Astrobiology, Astrochemistry, Comets: general, ISM: molecules}
}

@article{Heideman1965,
    title = {{Gauss and the History of the Fast Fourier Transform}},
    year = {1965},
    author = {Heideman, Michael T and Johnson, D O N H and Burrus, C Sidney and Truesdell, Communicated C}
}

@article{Jacquinet2014,
    title = {{GEISA 2014 spectroscopic database : context , contents , quality requirements , evolution 1 . GEISA presentation ; involvement in atmospheric remote sensing applications 2 . General description and examples of GEISA-2014 contents 3 . Spectroscopic data qu}},
    year = {2014},
    author = {Jacquinet, N and Cr{\'{e}}peau, L and Bouhdaoui, A and Boutammine, C},
    pages = {9--10}
}

@article{Head1998,
    title = {{Geologic History of the E4 Region of Europa: Implications for Ridge Formation, Cryo- Volcanism, and Chaos Formation}},
    year = {1998},
    author = {Head, J W and Sherman, N D and Pappalardo, R T and Greeley, R and Sullivan, R and Senske, D and Mcewen, A},
    pages = {6--7}
}

@article{Pappalardo1998,
    title = {{Geological evidence for solid-state convection in Europa's ice shell.}},
    year = {1998},
    journal = {Nature},
    author = {Pappalardo, Robert T and Head, James W. and Greeley, Ronald and Sullivan, R J and Pilcher, C and Schubert, Gerald and Moore, William B. and Carr, Michael H. and Moore, J M and Belton, Michael J S and Goldsby, David L.},
    number = {6665},
    pages = {365--368},
    volume = {391},
    isbn = {0028-0836 (Print){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/34862},
    issn = {0028-0836},
    pmid = {9450750}
}

@article{Malaska2016,
    title = {{Geomorphological map of the Afekan Crater region, Titan: Terrain relationships in the equatorial and mid-latitude regions}},
    year = {2016},
    journal = {Icarus},
    author = {Malaska, Michael J. and Lopes, Rosaly M C and Williams, David A. and Neish, Catherine D. and Solomonidou, Anezina and Soderblom, Jason M. and Schoenfeld, Ashley M. and Birch, Sam P D and Hayes, Alex G. and Le Gall, Alice and Janssen, Michael A. and Farr, Thomas G. and Lorenz, Ralph D. and Radebaugh, Jani and Turtle, Elizabeth P.},
    pages = {130--161},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.02.021},
    doi = {10.1016/j.icarus.2016.02.021},
    issn = {10902643},
    keywords = {Geological processes, Titan, Titan, surface}
}

@article{Vance2016,
    title = {{Geophysical controls of chemical disequilibria in Europa}},
    year = {2016},
    journal = {Geophysical Research Letters},
    author = {Vance, S. D. and Hand, K. P. and Pappalardo, R. T.},
    number = {10},
    pages = {4871--4879},
    volume = {43},
    doi = {10.1002/2016GL068547},
    issn = {19448007},
    keywords = {Europa, habitability, hydrothermal, life, microfracture, serpentinization}
}

@book{Island,
    title = {{Geophysical Monograph Series}},
    author = {Island, South and Zealand, New and Okaya, David and Stem, Tim and Centers, Spreading and Lowell, Robert P and Freymueller, Jeffrey T and Haeussler, Peter J and Robert, L and Kintner, Paul M and Coster, Anthea J and Fuller-rowell, Tim and Mannucci, Anthony J and Mendillo, Michael and Carbon, Global and Brian, Cycle and Cycling, Carbon and Andrew, Peatlands},
    isbn = {9781119066774}
}

@article{Dai2014,
    title = {{Geophysical Research Letters}},
    year = {2014},
    journal = {Geophysical Research Letters},
    author = {Dai, S and Seol, Y},
    number = {May},
    pages = {4176--4184},
    volume = {41},
    doi = {10.1002/2014GL060535.Received}
}

@article{Vance2017,
    title = {{Geophysical tests for habitability in ice-covered ocean worlds}},
    year = {2017},
    author = {Vance, Steven D. and Panning, Mark P. and St{\"{a}}hler, Simon and Cammarano, Fabio and Bills, Bruce G. and Kedar, Sharon and Sotin, Christophe and Pike, William T. and Lorenz, Ralph and Tsai, Victor and Huang, Hsin-Hua and Jackson, Jennifer M. and Banerdt, Bruce},
    pages = {1--44},
    url = {http://arxiv.org/abs/1705.03999},
    arxivId = {1705.03999}
}

@article{Bland2013a,
    title = {{Giant Convecting Mudballs of the Early Solar System}},
    year = {2013},
    journal = {44th Lunar and Planetary Science Conference},
    author = {Bland, P A and Travis, B J and Dyl, K A and Schubert, G},
    number = {July},
    pages = {Abstract {\#}1447},
    volume = {4},
    url = {http://www.lpi.usra.edu/meetings/lpsc2013/pdf/1447.pdf%5Cnpapers3://publication/uuid/9F3FE2B4-6243-4602-82D4-955537BA078C}
}

@article{Teanby2008,
    title = {{Global and temporal variations in hydrocarbons and nitriles in Titan's stratosphere for northern winter observed by Cassini/CIRS}},
    year = {2008},
    journal = {Icarus},
    author = {Teanby, N. A. and Irwin, P. G J and de Kok, R. and Nixon, C. A. and Coustenis, A. and Royer, E. and Calcutt, S. B. and Bowles, N. E. and Fletcher, L. and Howett, C. and Taylor, F. W.},
    number = {2},
    pages = {595--611},
    volume = {193},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2007.08.017},
    issn = {00191035},
    keywords = {Atmospheres, Titan, composition}
}

@article{Rodriguez2009,
    title = {{Global circulation as the main source of cloud activity on Titan.}},
    year = {2009},
    journal = {Nature},
    author = {Rodriguez, Sébastien and Le Mou{\'{e}}lic, Stéphane and Rannou, Pascal and Tobie, Gabriel and Baines, Kevin H and Barnes, Jason W and Griffith, Caitlin a and Hirtzig, Mathieu and Pitman, Karly M and Sotin, Christophe and Brown, Robert H and Buratti, Bonnie J and Clark, Roger N and Nicholson, Phil D},
    number = {7247},
    pages = {678--682},
    volume = {459},
    isbn = {1476-4687 (Electronic){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/NATURE08014},
    issn = {0028-0836},
    pmid = {19494910},
    arxivId = {0907.0606}
}

@article{Cook-Hallett2015,
    title = {{Global contraction/expansion and polar lithospheric thinning on Titan from patterns of tectonism}},
    year = {2015},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Cook-Hallett, Casey and Barnes, Jason W. and Kattenhorn, Simon A. and Hurford, Terry and Radebaugh, Jani and Stiles, Bryan and Beuthe, Mikael},
    number = {6},
    pages = {1220--1236},
    volume = {120},
    doi = {10.1002/2014JE004645},
    issn = {21699100},
    keywords = {Titan, global stress fields, tectonics}
}

@article{Elliot1998,
    title = {{Global warming on Triton}},
    year = {1998},
    journal = {Nature},
    author = {Elliot, J. L. and Hammel, H. B. and Wasserman, L. H. and Franz, O. G. and McDonald, S. W. and Person, M. J. and Olkin, C. B. and Dunham, E. W. and Spencer, J. R. and Stansberry, J. A. and Buie, M. W. and Pasachoff, J. M. and Babcock, B. A. and McConnochie, T. H.},
    number = {6687},
    pages = {765--767},
    volume = {393},
    url = {http://dx.doi.org/10.1038/31651%5Cnhttp://www.nature.com/doifinder/10.1038/31651},
    doi = {10.1038/31651},
    issn = {00280836}
}

@article{Zent1989,
    title = {{Grain metamorphism in polar nitrogen ice on Triton}},
    year = {1989},
    journal = {Geophysical Research Letters},
    author = {Zent, Aaron P and Mckay, Christopher P and Pollack, James B and Cruikshank, Dale P},
    number = {8},
    pages = {965--968},
    volume = {16}
}

@article{Yin2015,
    title = {{Gravitational spreading, bookshelf faulting, and tectonic evolution of the South Polar Terrain of Saturn's moon Enceladus}},
    year = {2015},
    journal = {Icarus},
    author = {Yin, An and Pappalardo, Robert T.},
    pages = {409--439},
    volume = {260},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.07.017},
    doi = {10.1016/j.icarus.2015.07.017},
    issn = {10902643},
    keywords = {Enceladus, Geological processes, Ices, mechanical properties}
}

@article{Penteado2010,
    title = {{Ground-based measurements of the methane distribution on Titan}},
    year = {2010},
    journal = {Icarus},
    author = {Penteado, Paulo F and Griffith, Caitlin A},
    number = {1},
    pages = {345--351},
    volume = {206},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.08.022},
    doi = {10.1016/j.icarus.2009.08.022},
    issn = {0019-1035}
}

@article{Evans1991,
    title = {{H C N Dimers : Iminoacetonitrile and N-Cyanomethanimine}},
    year = {1991},
    author = {Evans, Richard A and Loreneak, Primoi and Ha, Tae-kyu and Wentrup, Curt},
    number = {34},
    pages = {7261--7276},
    volume = {99}
}

@article{Silva2008,
    title = {{H elimination and metastable lifetimes in the UV photoexcitation of diacetylene.}},
    year = {2008},
    journal = {Proceedings of the National Academy of Sciences of the United States of America},
    author = {Silva, R and Gichuhi, W K and Huang, C and Doyle, M B and Kislov, V V and Mebel, A M and Suits, A G},
    number = {35},
    pages = {12713--8},
    volume = {105},
    url = {http://www.pnas.org/content/105/35/12713},
    doi = {10.1073/pnas.0801180105},
    issn = {1091-6490},
    pmid = {18697925}
}

@article{Dimitrov2003,
    title = {{Hardening of Titan's aerosols by their charging}},
    year = {2003},
    journal = {Icarus},
    author = {Dimitrov, Vasili and Bar-Nun, Akiva},
    number = {2},
    pages = {440--443},
    volume = {166},
    doi = {10.1016/j.icarus.2003.07.007},
    issn = {00191035},
    keywords = {Charging, Forced aging, Titan's aerosols}
}

@article{DeKok2014,
    title = {{HCN ice in Titan's high-altitude southern polar cloud}},
    year = {2014},
    journal = {Nature},
    author = {de Kok, Remco J and Teanby, Nicholas A and Maltagliati, Luca and Irwin, Patrick G J and Vinatier, Sandrine},
    number = {7520},
    pages = {65--7},
    volume = {514},
    publisher = {Nature Publishing Group},
    url = {http://adsabs.harvard.edu/abs/2014Natur.514...65D},
    doi = {10.1038/nature13789},
    issn = {1476-4687},
    pmid = {25279918},
    arxivId = {1410.5563}
}

@article{Mamajanov2014,
    title = {{HCN polymers characterized by solid state NMR : Chains and sheets formed in the neat liquid HCN polymers characterized by solid state NMR : Chains and sheets}},
    year = {2014},
    author = {Mamajanov, Irena and Herzfeld, Judith},
    number = {2009},
    volume = {134503},
    doi = {10.1063/1.3092908}
}

@article{Ruiz2007,
    title = {{Heat flow and thickness of a convective ice shell on Europa for grain size-dependent rheologies}},
    year = {2007},
    journal = {Icarus},
    author = {Ruiz, Javier and Alvarez-Gimez, Jos A. and Tejero, Rosa and Sanchez, Nieves},
    number = {1},
    pages = {145--154},
    volume = {190},
    doi = {10.1016/j.icarus.2007.03.015},
    issn = {00191035},
    keywords = {Europa, Jupiter, Thermal histories, Tides, satellites, solid body}
}

@article{Ruiz2000,
    title = {{Heat flows through the ice lithosphere of Europa}},
    year = {2000},
    journal = {Journal of Geophysical Research},
    author = {Ruiz, Javier and Tejero, Rosa},
    number = {E12},
    pages = {29283},
    volume = {105},
    doi = {10.1029/1999JE001228},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/1999JE001228, doi:10.102}
}

@article{Berkowitz1962,
    title = {{Heat of formation of the CN radical}},
    year = {1962},
    journal = {The Journal of Chemical Physics},
    author = {Berkowitz, J},
    number = {1962},
    pages = {2533--2539},
    volume = {1555},
    url = {http://link.aip.org/link/?JCPSA6/36/2533/1},
    doi = {10.1063/1.1732330},
    issn = {00219606}
}

@article{Choblet2017,
    title = {{Heat transport in the high-pressure ice mantle of large icy moons}},
    year = {2017},
    journal = {Icarus},
    author = {Choblet, G. and Tobie, G. and Sotin, C. and Kalousov{\'{a}}, K. and Grasset, O.},
    pages = {252--262},
    volume = {285},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.12.002},
    doi = {10.1016/j.icarus.2016.12.002},
    issn = {10902643},
    keywords = {Callisto, Ganymede, Ices, Interiors, Titan}
}

@article{Sittler2009,
    title = {{Heavy ion formation in Titan's ionosphere: Magnetospheric introduction of free oxygen and a source of Titan's aerosols?}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Sittler, E.C. and Ali, A. and Cooper, J.F. and Hartle, R.E. and Johnson, R.E. and Coates, A.J. and Young, D.T.},
    number = {13},
    month = {11},
    pages = {1547--1557},
    volume = {57},
    url = {http://www.sciencedirect.com/science/article/pii/S0032063309002268},
    doi = {10.1016/j.pss.2009.07.017},
    issn = {00320633},
    keywords = {Aerosols, Astrobiology, Heavy negative ions, Oxygen, Saturn's magnetosphere, Titan}
}

@article{Crary2009,
    title = {{Heavy ions, temperatures and winds in Titan's ionosphere: Combined Cassini CAPS and INMS observations}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Crary, F. J. and Magee, B. A. and Mandt, K. and Waite, J. H. and Westlake, J. and Young, D. T.},
    number = {14-15},
    pages = {1847--1856},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.09.006},
    doi = {10.1016/j.pss.2009.09.006},
    issn = {00320633},
    keywords = {Heavy ions, Ion temperature, Ionosphere, Ionospheric winds, Titan}
}

@article{Coates2009,
    title = {{Heavy negative ions in Titan's ionosphere: Altitude and latitude dependence}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Coates, A. J. and Wellbrock, A. and Lewis, G. R. and Jones, G. H. and Young, D. T. and Crary, F. J. and Waite, J. H.},
    number = {14-15},
    pages = {1866--1871},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.05.009},
    doi = {10.1016/j.pss.2009.05.009},
    issn = {00320633},
    keywords = {Ionosphere, Loss, Negative ions, Production Tholins, Titan}
}

@article{Rengel2014,
    title = {{Herschel/PACS spectroscopy of trace gases of the stratosphere of Titan}},
    year = {2014},
    journal = {Astronomy {\&} Astrophysics},
    author = {Rengel, M. and Sagawa, H. and Hartogh, P. and Lellouch, E. and Feuchtgruber, H. and Moreno, R. and Jarchow, C. and Courtin, R. and Cernicharo, J. and Lara, L. M.},
    pages = {A4},
    volume = {561},
    url = {http://www.aanda.org/10.1051/0004-6361/201321945},
    isbn = {1342199146},
    doi = {10.1051/0004-6361/201321945},
    issn = {0004-6361},
    arxivId = {1404.2164},
    keywords = {atmospheres, individual, planets and satellites, spectroscopic, techniques, titan}
}

@misc{Kossacki1996,
    title = {{Hiding Titan's ocean: Densification and hydrocarbon storage in an icy regolith}},
    year = {1996},
    booktitle = {Planetary and Space Science},
    author = {Kossacki, Konrad J. and Lorenz, Ralph D.},
    number = {9},
    pages = {1029--1037},
    volume = {44},
    doi = {10.1016/0032-0633(96)00022-0},
    issn = {00320633}
}

@article{Ferus2017,
    title = {{High Energy Radical Chemistry Formation of HCN-rich Atmospheres on early Earth}},
    year = {2017},
    journal = {Scientific Reports},
    author = {Ferus, Martin and Kubel{\'{i}}k, Petr and Kn{\'{i}}{\v{z}}ek, Antonín and Pastorek, Adam and Sutherland, John and Civi{\v{s}}, Svatopluk},
    number = {1},
    pages = {1--9},
    volume = {7},
    isbn = {4159801706},
    doi = {10.1038/s41598-017-06489-1},
    issn = {20452322},
    pmid = {28740207}
}

@misc{McKay1988,
    title = {{High-temperature shock formation of N2 and organics on primordial Titan}},
    year = {1988},
    booktitle = {Nature},
    author = {McKay, C P and Scattergood, T W and Pollack, J B and Borucki, W J and Van Ghyseghem, H T},
    number = {6164},
    pages = {520--522},
    volume = {332},
    isbn = {0028-0836 (Print){\textbackslash}r0028-0836},
    doi = {10.1038/332520a0},
    issn = {0028-0836},
    pmid = {11536599},
    keywords = {*Atmosphere, *Evolution, Planetary, *Extraterrestrial Environment, *Hot Temperature, *Saturn, Ammonia/analysis/*chemistry, Hydrocarbons/analysis/chemistry, Hydrogen Cyanide/analysis/chemistry, Hydrogen/analysis/chemistry, Lasers, Methane/analysis/chemistry, Models, Chemical, Nitrogen/analysis/*chemistry}
}

@article{Gudipati1995a,
    title = {{Higher excited states of aromatic hydrocarbons. III. Assigning the in-plane polarized transitions of low-symmetry molecules: chrysene and E-stilbene}},
    year = {1995},
    journal = {Chemical Physics},
    author = {Gudipati, Murthy S. and Maus, Michael and Daverkausen, Johannes and Hohlneicher, Georg},
    number = {1},
    pages = {37--47},
    volume = {192},
    isbn = {0301-0104},
    doi = {10.1016/0301-0104(94)00367-J},
    issn = {03010104}
}

@article{Burr2015,
    title = {{Higher-than-predicted saltation threshold wind speeds on Titan}},
    year = {2015},
    journal = {Nature},
    author = {Burr, Devon M. and Bridges, Nathan T. and Marshall, John R. and Smith, James K. and White, Bruce R. and Emery, Joshua P.},
    number = {7532},
    pages = {60--63},
    volume = {517},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/nature14088},
    isbn = {1476-4687 (Electronic){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/nature14088},
    issn = {14764687},
    pmid = {25487154}
}

@article{Treut2007,
    title = {{Historical Overview of Climate Change Science}},
    year = {2007},
    journal = {Earth},
    author = {Treut, Le and Somerville, R and Cubasch, U and Ding, Y and Mauritzen, C and Mokssit, a and Peterson, T and Prather, M and Qin, D and Manning, M and Chen, Z and Marquis, M and Averyt, K B and Tignor, M},
    number = {October},
    pages = {93--127},
    volume = {Chapter 1},
    url = {http://www.meteosat.com/ipcc4/Ch01_SOD_Text_TSU_FINAL.pdf},
    isbn = {9780521880091},
    doi = {10.1016/j.soilbio.2010.04.001},
    issn = {00380717},
    pmid = {10490603}
}

@misc{Buratti1994,
    title = {{Historical Photometric Evidence for Volatile Migration on Triton}},
    year = {1994},
    booktitle = {Icarus},
    author = {Buratti, B and Goguen, J. D. and Gibson, J. and Mosher, J.},
    number = {2},
    pages = {303--314},
    volume = {110},
    url = {http://linkinghub.elsevier.com/retrieve/doi/10.1006/icar.1994.1124},
    doi = {10.1006/icar.1994.1124},
    issn = {00191035}
}

@article{Muller-Wodarg2008,
    title = {{Horizontal structures and dynamics of Titan's thermosphere}},
    year = {2008},
    journal = {Journal of Geophysical Research E: Planets},
    author = {M{\"{u}}ller-Wodarg, I. C F and Yelle, R. V. and Cui, J. and Waite, J. H.},
    number = {10},
    pages = {1--17},
    volume = {113},
    doi = {10.1029/2007JE003033},
    issn = {01480227}
}

@article{Moore2017,
    title = {{How habitable zones and super-Earths lead us astray}},
    year = {2017},
    journal = {Nature Astronomy},
    author = {Moore, William B. and Lenardic, A. and Jellinek, A. M. and Johnson, C. L. and Goldblatt, C. and Lorenz, R. D.},
    number = {2},
    pages = {0043},
    volume = {1},
    publisher = {Macmillan Publishers Limited},
    url = {http://www.nature.com/articles/s41550-017-0043},
    doi = {10.1038/s41550-017-0043},
    issn = {2397-3366}
}

@article{Hebrard2009,
    title = {{How measurements of rate coefficients at low temperature increase the predictivity of photochemical models of titan's atmosphere}},
    year = {2009},
    journal = {Journal of Physical Chemistry A},
    author = {H{\'{e}}brard, E. and Dobrijevic, M. and Pernot, P. and Carrasco, N. and Bergeat, A. and Hickson, K. M. and Canosa, A. and Le Picard, S. D. and Sims, I. R.},
    number = {42},
    pages = {11227--11237},
    volume = {113},
    isbn = {1089-5639},
    doi = {10.1021/jp905524e},
    issn = {10895639},
    pmid = {19775112}
}

@article{Alon2009,
    title = {{How To Choose a Good Scientific Problem}},
    year = {2009},
    journal = {Molecular Cell},
    author = {Alon, Uri},
    number = {6},
    pages = {726--728},
    volume = {35}
}

@article{Ben-Jaffel2013,
    title = {{Hubble Space Telescope detection of carbon and oxygen in the atmosphere of exoplanet HD 189733b}},
    year = {2013},
    journal = {Astronomy {\&} Astrophysics},
    author = {Ben-Jaffel, Lotfi and Ballester, Gilda},
    pages = {1--12},
    volume = {52},
    url = {http://arxiv.org/abs/1303.4232},
    doi = {10.1051/0004-6361/201221014},
    issn = {0004-6361},
    arxivId = {1303.4232},
    keywords = {activity, general, hd 189733, individual, magnetic fields, planet-star interactions, planets and satellites, stars, sun, ultraviolet}
}

@article{Helden,
    title = {{Huygens and his times}},
    author = {Helden, Albert Van}
}

@article{Bos,
    title = {{Huygens and Mathematics}},
    author = {Bos, Henk J M}
}

@article{Chareix2004,
    title = {{Huygens and Mechanics}},
    year = {2004},
    author = {Chareix, Fabien}
}

@article{Dijksterhuis2004,
    title = {{Huygens and optics}},
    year = {2004},
    journal = {European Space Agency, (Special Publication) ESA SP},
    author = {Dijksterhuis, Fokko Jan},
    number = {1278},
    pages = {81--89},
    issn = {03796566}
}

@article{Lebreton2010,
    title = {{Huygens Science and Instrumentation : Lessons Learned For The Future In Situ Exploration of Titan}},
    year = {2010},
    author = {Lebreton, J and Estec, E S A and Noordwijk, A G},
    pages = {9215},
    volume = {5},
    doi = {10.1007/978-1-4020-9217-6}
}

@article{McCord1999,
    title = {{Hydrated salt minerals on Europa's Surface from the Galileo near-infrared mapping spectrometer (NIMS) investigation}},
    year = {1999},
    journal = {Journal of Geophysical Research},
    author = {McCord, Thomas B and Hansen, Gary B and Matson, Dennis L and Johnson, Torrence V and Crowley, James K and Fanale, Fraser P and Carlson, Robert W and Smythe, William D and Martin, Patrick D and Hibbitts, Charles A and Granahan, James C and Ocampo, Adriana},
    number = {E5},
    pages = {11827--11851},
    volume = {104},
    url = {http://www.agu.org/pubs/crossref/1999/1999JE900005.shtml},
    isbn = {0148-0227},
    doi = {10.1029/1999JE900005},
    issn = {0148-0227},
    pmid = {102},
    keywords = {http://dx.doi.org/10.1029/1999JE900005, doi:10.102}
}

@article{Fox1997,
    title = {{Hydrocarbon ions in the ionosphere of Titan}},
    year = {1997},
    journal = {Geophysical Research Letters},
    author = {Fox, Jane L. and Yelle, Roger V.},
    number = {17},
    pages = {2179--2182},
    volume = {24},
    doi = {10.1029/97GL02051},
    issn = {1944-8007},
    keywords = {doi:10.1029/9, http://dx.doi.org/10.1029/97GL02051}
}

@article{Ghosh1977,
    title = {{Hydrogen bond distance and phase change in crystalline HCN}},
    year = {1977},
    journal = {Journal of Physics C: Solid State Physics},
    author = {Ghosh, P. N.},
    number = {22},
    pages = {4421--4424},
    volume = {10},
    doi = {10.1088/0022-3719/10/22/012},
    issn = {00223719}
}

@article{Theule2011a,
    title = {{Hydrogenation of solid hydrogen cyanide HCN and methanimine CH <sub>2</sub> NH at low temperature}},
    year = {2011},
    journal = {Astronomy {\&} Astrophysics},
    author = {Theule, P. and Borget, F. and Mispelaer, F. and Danger, G. and Duvernay, F. and Guillemin, J. C. and Chiavassa, T.},
    number = {2011},
    pages = {A64},
    volume = {534},
    url = {http://www.aanda.org/10.1051/0004-6361/201117494},
    doi = {10.1051/0004-6361/201117494},
    issn = {0004-6361}
}

@article{Theule2011,
    title = {{Hydrogenation of solid hydrogen cyanide HCN and methanimine CH2NH at low temperature}},
    year = {2011},
    journal = {Astronomy {\&} Astrophysics},
    author = {Theule, P and Borget, F and Mispelaer, F and Danger, G and Duvernay, F and Guillemin, J-C C and Chiavassa, T},
    pages = {A64},
    volume = {534},
    doi = {10.1051/0004-6361/201117494},
    issn = {0004-6361},
    keywords = {astrochemistry, ism, molecular processes, molecules}
}

@article{Danger2012,
    title = {{Hydroxyacetonitrile (HOCH2CN) formation in astrophysical conditions. competition with the aminomethanol, a glycine precursor}},
    year = {2012},
    journal = {Astrophysical Journal},
    author = {Danger, G. and Duvernay, F. and Theul{\'{e}}, P. and Borget, F. and Chiavassa, T.},
    number = {1},
    volume = {756},
    isbn = {0004-637X},
    doi = {10.1088/0004-637X/756/1/11},
    issn = {15384357},
    keywords = {ISM: molecules, astrochemistry, comets: general, meteorites, meteors, meteoroids, methods: laboratory, molecular processes}
}

@article{Ghail1998,
    title = {{Ice Crust Thickness and Internal Composition of Europa}},
    year = {1998},
    journal = {Lunar and Planetary Science Abstracts},
    author = {Ghail, R C},
    pages = {7--8}
}

@article{Vance,
    title = {{Icy Satellite Processes in the Solar System : A plurality of worlds}},
    author = {Vance, Steven Douglas and Collins, Geoffrey C},
    number = {November 2014}
}

@article{Cloutis2016,
    title = {{Identification and discrimination of polycyclic aromatic hydrocarbons using Raman spectroscopy}},
    year = {2016},
    journal = {Icarus},
    author = {Cloutis, Edward and Szymanski, Paul and Applin, Daniel and Goltz, Douglas},
    pages = {211--230},
    volume = {274},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.03.023},
    doi = {10.1016/j.icarus.2016.03.023},
    issn = {10902643},
    keywords = {Cosmochemistry, Organic chemistry, Prebiotic chemistry, Spectroscopy}
}

@article{He2014,
    title = {{Identification of nitrogenous organic species in Titan aerosols analogs: Implication for prebiotic chemistry on Titan and early Earth}},
    year = {2014},
    journal = {Icarus},
    author = {He, Chao and Smith, Mark A.},
    pages = {86--92},
    volume = {238},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.05.012},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.05.012},
    issn = {10902643},
    keywords = {Organic chemistry, Prebiotic chemistry, Titan, atmosphere, Titan, surface}
}

@article{Cable2014,
    title = {{Identification of primary amines in Titan tholins using microchip nonaqueous capillary electrophoresis}},
    year = {2014},
    journal = {Earth and Planetary Science Letters},
    author = {Cable, M. L. and H{\"{o}}rst, S. M. and He, C. and Stockton, A. M. and Mora, M. F. and Tolbert, M. A. and Smith, M. A. and Willis, P. A.},
    pages = {99--107},
    volume = {403},
    isbn = {0012-821X},
    doi = {10.1016/j.epsl.2014.06.028},
    issn = {0012821X},
    keywords = {Ethanol, Ethylamine, Lab-on-a-chip, Microfluidics, Titan}
}

@article{Planetary2018,
    title = {{Identifying the enigmatic Haystack and HASP ice clouds observed by CIRS in Titan's stratosphere}},
    year = {2018},
    author = {Planetary, European and Congress, Science},
    pages = {1--2},
    volume = {12}
}

@article{Moran2016,
    title = {{Identifying the Species Threat Hotspots from Global Supply Chains}},
    year = {2016},
    journal = {Nature Ecology and Evolution},
    author = {Moran, Daniel and Kanemoto, Keiichiro},
    number = {7491},
    pages = {1--13},
    volume = {6},
    url = {http://biorxiv.org/lookup/doi/10.1101/076869},
    doi = {10.1101/076869},
    issn = {2397-334X}
}

@article{Porco2005,
    title = {{Imaging of Titan from the Cassini spacecraft}},
    year = {2005},
    author = {Porco, Carolyn C and Baker, Emily and Barbara, John and Beurle, Kevin and Brahic, Andre and Burns, Joseph A and Charnoz, Sebastien and Cooper, Nick and Dawson, Douglas D and Genio, Anthony D Del and Denk, Tilmann and Dones, Luke and Dyudina, Ulyana and Evans, Michael W and Fussner, Stephanie and Giese, Bernd and Grazier, Kevin and Helfenstein, Paul and Ingersoll, Andrew P and Jacobson, Robert A and Johnson, Torrence V and Mcewen, Alfred and Tiscareno, Matthew and Turtle, Elizabeth P and Vasavada, Ashwin R and Veverka, Joseph and Wagner, Roland and West, Robert},
    pages = {159--168}
}

@misc{1976BAAS____8__473G.pdf,
    title = {{1976BAAS{\_}{\_}{\_}{\_}8{\_}{\_}473G.pdf}}
}

@misc{HCNSynthesis,
    title = {{HCN and CN- in synthesis}}
}
@article{Sekine2014,
    title = {{Impact chemistry of methanol: Implications for volatile evolution on icy satellites and dwarf planets, and cometary delivery to the Moon}},
    year = {2014},
    journal = {Icarus},
    author = {Sekine, Yasuhito and Genda, Hidenori and Muto, Yuta and Sugita, Seiji and Kadono, Toshihiko and Matsui, Takafumi},
    pages = {39--47},
    volume = {243},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.08.034},
    doi = {10.1016/j.icarus.2014.08.034},
    issn = {10902643},
    keywords = {Impact processes, Moon, surface, Satellites, atmospheres, Satellites, formation}
}

@article{Silber2017,
    title = {{Impact Crater Morphology and the Structure of Europa's Ice Shell}},
    year = {2017},
    journal = {Journal of Geophysical Research: Planets},
    author = {Silber, Elizabeth A. and Johnson, Brandon C.},
    url = {http://doi.wiley.com/10.1002/2017JE005456},
    doi = {10.1002/2017JE005456},
    issn = {21699097},
    arxivId = {arXiv:1711.08997v1},
    keywords = {Europa, ice shell thickness, impact crater morphology, warm convective ice}
}

@article{Gans2013,
    title = {{Impact of a new wavelength-dependent representation of methane photolysis branching ratios on the modeling of Titan's atmospheric photochemistry}},
    year = {2013},
    journal = {Icarus},
    author = {Gans, B. and Peng, Z. and Carrasco, N. and Gauyacq, D. and Lebonnois, S. and Pernot, P.},
    number = {1},
    pages = {330--343},
    volume = {223},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.11.024},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2012.11.024},
    issn = {00191035},
    keywords = {Atmospheres, Chemistry, Atmospheres, Composition, Photochemistry, Titan}
}

@article{Dubrovin2014,
    title = {{Impact of lightning on the lower ionosphere of Saturn and possible generation of halos and sprites}},
    year = {2014},
    journal = {Icarus},
    author = {Dubrovin, D. and Luque, A. and Gordillo-Vazquez, F. J. and Yair, Y. and Parra-Rojas, F. C. and Ebert, U. and Price, C.},
    pages = {313--328},
    volume = {241},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.06.025},
    doi = {10.1016/j.icarus.2014.06.025},
    issn = {10902643},
    keywords = {Ionospheres, Lightning, Saturn}
}

@article{Tokano2009,
    title = {{Impact of seas / lakes on polar meteorology of Titan : Simulation by a coupled GCM-Sea model}},
    year = {2009},
    journal = {Icarus},
    author = {Tokano, Tetsuya},
    number = {2},
    pages = {619--636},
    volume = {204},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.07.032},
    doi = {10.1016/j.icarus.2009.07.032},
    issn = {0019-1035}
}

@article{Asphaug2016,
    title = {{Implications of Europa's global cycloid population}},
    year = {2016},
    author = {Mohr, K. J. and Rhoden, A. R. and Hurford, T. A. and Dubois, D.},
    pages = {9--10},
    isbn = {1189985144},
    doi = {10.1016/j.icarus.2007.12.027.}
}

@article{Harris2006,
    title = {{Improved HCN/HNC linelist, model atmospheres and synthetic spectra for WZ Cas}},
    year = {2006},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Harris, G. J. and Tennyson, J. and Kaminsky, B. M. and Pavlenko, Ya V. and Jones, H. R A},
    number = {1},
    pages = {400--406},
    volume = {367},
    doi = {10.1111/j.1365-2966.2005.09960.x},
    issn = {00358711},
    keywords = {Infrared: stars, Molecular data, Stars: AGB, Stars: atmospheres, Stars: carbon}
}

@article{Dubois2018,
    title = {{In Situ Investigation of Neutrals Involved in the Formation of Titan Tholins}},
    year = {2019},
    journal = {Icarus},
    author = {Dubois, D. and Carrasco, N. and Petrucciani, M. and Vettier, L. and Tigrine, S. and Pernot, P.},
    number = {July 2018},
    pages = {182--196},
    volume = {317},
    publisher = {Elsevier},
    url = {https://doi.org/10.1016/j.icarus.2018.07.006},
    doi = {10.1016/j.icarus.2018.07.006},
    issn = {00191035},
    keywords = {Atmospheres, Chemistry, Experimental techniques, Plasma discharge, Saturn, Titan}
}

@article{Fulchignoni2005,
    title = {{In situ measurements of the physical characteristics of Titan's environment}},
    year = {2005},
    journal = {Nature},
    author = {Fulchignoni, M. and Ferri, F. and Angrilli, F. and Ball, A. J. and Bar-Nun, A. and Barucci, M. A. and Bettanini, C. and Bianchini, G. and Borucki, W. and Colombatti, G. and Coradini, M. and Coustenis, A. and Debei, S. and Falkner, P. and Fanti, G. and Flamini, E. and Gaborit, V. and Grard, R. and Hamelin, M. and Harri, A. M. and Hathi, B. and Jernej, I. and Leese, M. R. and Lehto, A. and Lion Stoppato, P. F. and L{\'{o}}pez-Moreno, J. J. and M{\"{a}}kinen, T. and McDonnell, J. A. M. and McKay, C. P. and Molina-Cuberos, G. and Neubauer, F. M. and Pirronello, V. and Rodrigo, R. and Saggin, B. and Schwingenschuh, K. and Seiff, A. and Simões, F. and Svedhem, H. and Tokano, T. and Towner, M. C. and Trautner, R. and Withers, P. and Zarnecki, J. C.},
    number = {7069},
    pages = {785--791},
    volume = {438},
    url = {http://www.nature.com/doifinder/10.1038/nature04314},
    isbn = {1476-4687 (Electronic){\textbackslash}n0028-0836 (Linking)},
    doi = {10.1038/nature04314},
    issn = {0028-0836},
    pmid = {16319827}
}

@article{Horst2013haze,
    title = {{In situ measurements of the size and density of titan aerosol analogs}},
    year = {2013},
    journal = {Astrophysical Journal Letters},
    author = {H{\"{o}}rst, S. M. and Tolbert, M. A.},
    number = {1},
    pages = {1--21},
    volume = {770},
    isbn = {2041-8205},
    doi = {10.1088/2041-8205/770/1/L10},
    issn = {20418205},
    arxivId = {1305.2211},
    keywords = {astrobiology, planets and satellites: atmospheres, planets and satellites: composition}
}

@article{Hebrard2006,
    title = {{Incertitudes photochimiques dans les mod{\`{e}}les de l’atmosph{\`{e}}re de Titan : Revue et cons{\'{e}}quences}},
    year = {2006},
    journal = {Th{\`{e}}se},
    author = {H{\'{e}}brard, Eric}
}

@article{Vigren2014,
    title = {{Increasing positive ion number densities below the peak of ion-electron pair production in titan's ionosphere}},
    year = {2014},
    journal = {Astrophysical Journal},
    author = {Vigren, E. and Galand, M. and Shebanits, O. and Wahlund, J. E. and Geppert, W. D. and Lavvas, P. and Vuitton, V. and Yelle, R. V.},
    number = {1},
    volume = {786},
    isbn = {doi:10.1088/0004-637X/786/1/69},
    doi = {10.1088/0004-637X/786/1/69},
    issn = {15384357},
    keywords = {molecular processes, planets and satellites: individual (Titan)}
}

@article{Khurana1998,
    title = {{Induced magnetic fields as evidence for subsurface oceans in Europa and Callisto}},
    year = {1998},
    journal = {Nature},
    author = {Khurana, K.K. and Kivelson, M.G. and Stevenson, David J. and Schubert, Gerald and Russell, Christopher T. and Walker, R.J. and Polanskey, C.},
    number = {6704},
    pages = {777--780},
    volume = {395},
    url = {http://www.nature.com.ezproxy4.lib.le.ac.uk/nature/journal/v395/n6704/full/395777a0.html},
    isbn = {0028-0836 (Print){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/27394},
    issn = {0028-0836},
    pmid = {9796812},
    arxivId = {physics/9810036},
    keywords = {Extraterrestrial Environment, Jupiter, Magnetics, Salts, Water}
}

@article{Fleury2014,
    title = {{Influence of CO on Titan atmospheric reactivity}},
    year = {2014},
    journal = {Icarus},
    author = {Fleury, B. and Carrasco, N. and Gautier, T. and Mahjoub, A. and He, J. and Szopa, C. and Hadamcik, E. and Buch, A. and Cernogora, G.},
    pages = {221--229},
    volume = {238},
    doi = {10.1016/j.icarus.2014.05.027},
    issn = {10902643},
    keywords = {Experimental techniques, Saturn, satellites, Titan, atmosphere}
}

@article{Molina-Cuberos2000,
    title = {{Influence of electrophilic species on the lower ionosphere of Titan}},
    year = {2000},
    journal = {Geophysical Research Letters},
    author = {Molina-Cuberos, G. J. and Lopez-Moreno, J. J. and Rodrigo, R.},
    number = {9},
    pages = {1351--1354},
    volume = {27},
    doi = {10.1029/1999GL010771},
    issn = {00948276}
}

@article{Borucki2008,
    title = {{Influence of high abundances of aerosols on the electrical conductivity of the Titan atmosphere}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Borucki, W. J. and Whitten, R. C.},
    number = {1},
    pages = {19--26},
    volume = {56},
    doi = {10.1016/j.pss.2007.03.013},
    issn = {00320633},
    keywords = {Planetary atmosphere, Titan}
}

@article{Salvador2015,
    title = {{Influence of initial CO 2 content on a planet surface conditions at the end of the magma ocean phase}},
    year = {2015},
    journal = {EPSC Abstracts},
    author = {Salvador, Arnaud},
    pages = {3--4},
    volume = {10}
}

@article{Mahjoub2012,
    title = {{Influence of methane concentration on the optical indices of titan's aerosols analogues}},
    year = {2012},
    journal = {Icarus},
    author = {Mahjoub, A. and Carrasco, N. and Dahoo, P. R. and Gautier, T. and Szopa, C. and Cernogora, G.},
    number = {2},
    pages = {670--677},
    volume = {221},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.08.015},
    doi = {10.1016/j.icarus.2012.08.015},
    issn = {00191035},
    keywords = {Photometry, Radiative transfer, Titan, Titan, atmosphere}
}

@article{Carrasco2007,
    title = {{Influence of neutral transport on ion chemistry uncertainties in Titan ionosphere}},
    year = {2007},
    journal = {Icarus},
    author = {Carrasco, N. and H{\'{e}}brard, E. and Banaszkiewicz, M. and Dobrijevic, M. and Pernot, P.},
    number = {2},
    month = {12},
    pages = {519--526},
    volume = {192},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103507003533},
    doi = {10.1016/j.icarus.2007.08.016},
    issn = {00191035},
    keywords = {Atmospheres, Ionospheres, Titan, chemistry, composition, dynamics}
}

@article{Modolo2005,
    title = {{Influence of the solar EUV flux on the Martian plasma environment}},
    year = {2005},
    journal = {Annales Geophysicae},
    author = {Modolo, R. and Chanteur, G.~M. M. and Dubinin, E. and Matthews, A.~P. P.},
    number = {2},
    pages = {433--444},
    volume = {23},
    url = {http://www.ann-geophys.net/23/433/2005/},
    doi = {10.5194/angeo-23-433-2005},
    issn = {1432-0576},
    keywords = {actions with unmagnetized bodies, ionization processes, magnetospheric physics, numerical simulation suites, solar wind and inter-, space plasma physics}
}

@article{Palumbo2004,
    title = {{Infrared and Raman spectroscopies of refractory residues left over after ion irradiation of nitrogen-bearing icy mixtures}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Palumbo, M. E. and Ferini, G. and Baratta, G. A.},
    number = {1},
    pages = {49--56},
    volume = {33},
    doi = {10.1016/j.asr.2003.03.002},
    issn = {02731177},
    keywords = {Cosmic ion processing, Frozen CH4 (methane), Ices in the solar system, Infrared spectroscopy, Laboratory measurements, Raman spectroscopy}
}

@article{Khanna1988,
    title = {{Infrared band extinctions and complex refractive indices of crystalline C2H2and C4H2}},
    year = {1988},
    journal = {Icarus},
    author = {Khanna, R. K. and Ospina, Mario J. and Zhao, Guizhi},
    number = {3},
    pages = {527--535},
    volume = {73},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(88)90062-0},
    issn = {10902643}
}

@article{Ennis2017,
    title = {{Infrared characterisation of acetonitrile and propionitrile aerosols under Titan's atmospheric conditions}},
    year = {2017},
    journal = {Phys. Chem. Chem. Phys.},
    author = {Ennis, C. and Auchettl, R. and Ruzi, M. and Robertson, E. G.},
    number = {4},
    pages = {2915--2925},
    volume = {19},
    publisher = {Royal Society of Chemistry},
    url = {http://xlink.rsc.org/?DOI=C6CP08110J},
    doi = {10.1039/C6CP08110J},
    issn = {1463-9076}
}

@article{P.1983,
    title = {{INFRARED IN THE 12-14pm ABSORPTION BY ACETYLENE REGION AT LOW TEMPERATURES?}},
    year = {1983},
    journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
    author = {P., Varanasi and P., L., Giver and F., P., J., Valero},
    volume = {139}
}

@article{Hanel1981,
    title = {{Infrared Observations of the Saturnian System from Voyager 1}},
    year = {1981},
    journal = {Science},
    author = {Hanel, R. and Conrath, B. and Flasar, F. M. and Kunde, V. G. and Maguire, W. C. and Pearl, J. and Pirraglia, J. and Samuelson, R. E. and Herath, L. and Allison, M. and Cruikshank, D. and Gautier, D. and Gierasch, P. and Horn, L. and Koppany, R. and Ponnamperuma, C.},
    number = {4491},
    month = {4},
    pages = {192--200},
    volume = {212},
    url = {http://www.sciencemag.org/cgi/doi/10.1126/science.212.4491.192},
    doi = {10.1126/science.212.4491.192},
    issn = {0036-8075}
}

@article{Cernicharo2001,
    title = {{Infrared Space Observatory's Discovery of C4H2, C6H2, and Benzene in CRL 618}},
    year = {2001},
    journal = {The Astrophysical Journal},
    author = {Cernicharo, José and Heras, Ana M. and Tielens, A. G. G. M. and Pardo, Juan R. and Herpin, Fabrice and Gu{\'{e}}lin, Michel and Waters, L. B. F. M.},
    number = {2},
    pages = {L123-L126},
    volume = {546},
    url = {http://stacks.iop.org/1538-4357/546/i=2/a=L123},
    isbn = {1538-4357},
    doi = {10.1086/318871},
    issn = {0004637X}
}

@article{Hudson2017,
    title = {{Infrared spectra and band strengths of amorphous and crystalline N2O}},
    year = {2017},
    journal = {Journal of Chemical Physics},
    author = {Hudson, R. L. and Loeffler, M. J. and Gerakines, P. A.},
    number = {2},
    volume = {146},
    doi = {10.1063/1.4973548},
    issn = {00219606}
}

@article{Moore2010,
    title = {{INFRARED SPECTRA AND OPTICAL CONSTANTS OF NITRILE ICES RELEVANT TO TITAN's ATMOSPHERE}},
    year = {2010},
    journal = {The Astrophysical Journal Supplement Series},
    author = {Moore, Marla H. and Ferrante, Robert F. and James Moore, W. and Hudson, Reggie},
    number = {1},
    pages = {96--112},
    volume = {191},
    url = {http://stacks.iop.org/0067-0049/191/i=1/a=96?key=crossref.f20ef1fba1838e3f1faf076976ddd850},
    doi = {10.1088/0067-0049/191/1/96},
    issn = {0067-0049},
    keywords = {catalogs, individual, infrared, laboratory, machine-readable tables, methods, online-only material, planetary systems, planets and satellites, spectroscopic, techniques, titan}
}

@article{Cerceau1985,
    title = {{Infrared spectra of gaseous mononitriles: Application to the atmosphere of Titan}},
    year = {1985},
    journal = {Icarus},
    author = {Cerceau, F. and Raulin, F. and Courtin, R. and Gautier, D.},
    number = {2},
    pages = {207--220},
    volume = {62},
    doi = {10.1016/0019-1035(85)90118-6},
    issn = {10902643}
}

@article{Armen2007,
    title = {{Infrared spectroscopy of acetylene}},
    year = {2007},
    author = {Armen, G Bradley},
    pages = {1--34}
}

@article{Zhou2009,
    title = {{Infrared spectroscopy of crystalline and amorphous diacetylene (C4H2) and implications for Titan’s atmospheric composition}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Zhou, Li and Kaiser, Ralf I and Tokunaga, Alan T},
    pages = {830--835},
    volume = {57},
    doi = {10.1016/j.pss.2009.02.003}
}

@article{Moore2003a,
    title = {{Infrared study of ion-irradiated N2-dominated ices relevant to Triton and Pluto: Formation of HCN and HNC}},
    year = {2003},
    journal = {Icarus},
    author = {Moore, M. H. and Hudson, R. L.},
    number = {2},
    pages = {486--500},
    volume = {161},
    isbn = {1301286044},
    doi = {10.1016/S0019-1035(02)00037-4},
    issn = {00191035},
    keywords = {Ices, Pluto, Radiation chemistry, Spectroscopy, Triton}
}

@article{Hartle2006,
    title = {{Initial interpretation of Titan plasma interaction as observed by the Cassini plasma spectrometer: Comparisons with Voyager 1}},
    year = {2006},
    journal = {Planetary and Space Science},
    author = {Hartle, R. E. and Sittler, E. C. and Neubauer, F. M. and Johnson, R. E. and Smith, H. T. and Crary, F. and McComas, D. J. and Young, D. T. and Coates, A. J. and Simpson, D. and Bolton, S. and Reisenfeld, D. and Szego, K. and Berthelier, J. J. and Rymer, A. and Vilppola, J. and Steinberg, J. T. and Andre, N.},
    number = {12},
    pages = {1211--1224},
    volume = {54},
    doi = {10.1016/j.pss.2006.05.029},
    issn = {00320633},
    keywords = {Cassini, Composition, Mass loading, Pickup ions, Plasma, Titan}
}

@article{Zanazzi2017,
    title = {{Initiation of Plate Tectonics on Exoplanets with Significant Tidal Stress}},
    year = {2017},
    author = {Zanazzi, J. J. and Triaud, Amaury},
    url = {http://arxiv.org/abs/1711.09898},
    arxivId = {1711.09898},
    keywords = {extra-solar planets, geophysics, tectonics, terrestrial planets}
}

@article{Magee2009,
    title = {{INMS-derived composition of Titan's upper atmosphere: Analysis methods and model comparison}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Magee, Brian A. and Waite, J. Hunter and Mandt, Kathleen E. and Westlake, Joseph and Bell, Jared and Gell, David A.},
    number = {14-15},
    pages = {1895--1916},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.06.016},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2009.06.016},
    issn = {00320633},
    keywords = {Mass spectrometry, Neutral composition, Titan}
}

@article{Coates2009a,
    title = {{Interaction of Titan's ionosphere with Saturn's magnetosphere}},
    year = {2009},
    journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
    author = {Coates, A. J},
    number = {1889},
    pages = {773--788},
    volume = {367},
    url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.2008.0248},
    doi = {10.1098/rsta.2008.0248},
    issn = {1364-503X},
    keywords = {1, 1982, 2005, an ionosphere, backes et al, however, introduction, ionosphere, it does have a, magnetosphere, moment, negative ions, ness et al, photoelectrons, s space environment, saturn, substantial neutral atmosphere and, titan, titan is a body, with no significant dipole}
}

@article{Tolansky1930,
    title = {{Interferometric evaluation of thicknesses of thin films}},
    year = {1930},
    journal = {Le Journal de Physique et le Radium},
    author = {Tolansky, S.},
    isbn = {0195000110}
}

@article{Cordiner2018,
    title = {{Interferometric imaging of Titan's HC3N, H13CCCN and HCCC15N}},
    year = {2018},
    journal = {Astrophysical Journal Letters},
    author = {Cordiner, M. A. and Nixon, C. A. and Charnley, S. B. and Teanby, N. A. and Molter, E. M. and Kisiel, Z. and Vuitton, V.},
    pages = {10--15},
    url = {http://arxiv.org/abs/1805.04416},
    arxivId = {1805.04416}
}

@article{Schubert2004,
    title = {{Interior Composition , Structure and Dynamics of the Galilean Satellites}},
    year = {2004},
    journal = {Jupiter. The planet, satellites and magnetosphere},
    author = {Schubert, G. and Anderson, J. D. and Spohn, T. and Mckinnon, William B.},
    number = {Danby},
    pages = {281 - 306},
    isbn = {0-521-81808-7}
}

@article{Sohl2003,
    title = {{Interior structure models and tidal Love numbers of Titan}},
    year = {2003},
    journal = {Journal of Geophysical Research},
    author = {Sohl, F.},
    number = {E12},
    pages = {1--13},
    volume = {108},
    isbn = {0148-0227},
    doi = {10.1029/2003JE002044},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/2003JE002044, doi:10.102}
}

@article{Hussmann2004,
    title = {{Internal Structure and Tidal Heating of Ganymede}},
    year = {2004},
    journal = {Geophysical Research Abstracts},
    author = {Hussmann, Hauke and Sohl, Frank and Spohn, Tilman},
    pages = {9--10},
    volume = {6}
}

@article{Bonnet2013,
    title = {{International Journal of Mass Spectrometry Compositional and structural investigation of HCN polymer through high resolution mass spectrometry}},
    year = {2013},
    author = {Bonnet, J-Y. and Thissen, Roland and Frisari, Maëliss and Vuitton, Véronique and Quirico, Éric and Dutuit, Odile and Le, Léna and Fray, Nicolas and Cottin, Hervé and H{\"{o}}rst, Sarah M and Yelle, Roger V},
    pages = {193--203},
    volume = {355},
    doi = {10.1016/j.ijms.2013.06.015}
}

@article{Vuitton2003,
    title = {{Intrinsic lifetime of metastable excited C4H2: Implications for the photochemistry of C4H2in Titan's atmosphere}},
    year = {2003},
    journal = {Planetary and Space Science},
    author = {Vuitton, V. and G{\'{e}}e, C. and Raulin, F. and B{\'{e}}nilan, Y. and Cr{\'{e}}pin, C. and Gazeau, M. C.},
    number = {13},
    pages = {847--852},
    volume = {51},
    doi = {10.1016/j.pss.2003.07.001},
    issn = {00320633},
    keywords = {Diacetylene, Lifetime, Rare gas matrices, Titan}
}

@article{Shebanits2016,
    title = {{Ion and aerosol precursor densities in Titan's ionosphere: A multi‐instrument case study}},
    year = {2016},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Shebanits, O and Wahlund, J.‐E. and Edberg, N J T and Crary, F J and Wellbrock, A and Andrews, D J and Vigren, E and Desai, R T and Coates, A J and Mandt, K E and Waite, J H},
    number = {10},
    pages = {10--75},
    volume = {121},
    url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1002/2016JA022980},
    doi = {10.1002/2016JA022980},
    keywords = {Titan's ionosphere, dusty ion‐ion plasma, ion and dust densities, mean ion mass, negative ion and dust charge}
}

@article{Vuitton2007,
    title = {{Ion chemistry and N-containing molecules in Titan's upper atmosphere}},
    year = {2007},
    journal = {Icarus},
    author = {Vuitton, V. and Yelle, R. V. and McEwan, M. J.},
    number = {2},
    pages = {722--742},
    volume = {191},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2007.06.023},
    issn = {00191035},
    keywords = {Atmospheres, Ionospheres, Organic chemistry, Titan, composition}
}

@article{Larsson2012,
    title = {{Ion chemistry in space}},
    year = {2012},
    journal = {Reports on Progress in Physics},
    author = {Larsson, M. and Geppert, W. D. and Nyman, G.},
    number = {6},
    volume = {75},
    isbn = {9783527408528},
    doi = {10.1088/0034-4885/75/6/066901},
    issn = {00344885},
    pmid = {22790651}
}

@article{Woodson2015,
    title = {{Ion composition in Titan's exosphere via the Cassini Plasma Spectrometer I: T40 encounter}},
    year = {2015},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Woodson, A. K. and Smith, H. T. and Crary, F. J. and Johnson, R. E.},
    number = {1},
    pages = {212--234},
    volume = {120},
    doi = {10.1002/2014JA020499},
    issn = {21699402},
    keywords = {Titan}
}

@article{Mandt2012,
    title = {{Ion densities and composition of Titan's upper atmosphere derived from the Cassini Ion Neutral Mass Spectrometer: Analysis methods and comparison of measured ion densities to photochemical model simulations}},
    year = {2012},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Mandt, Kathleen E. and Gell, David A. and Perry, Mark and Hunter Waite, J. and Crary, Frank A. and Young, David and Magee, Brian A. and Westlake, Joseph H. and Cravens, Thomas and Kasprzak, Wayne and Miller, Greg and Wahlund, Jan Erik and Gren, Karin and Edberg, Niklas J T and Heays, Alan N. and Lewis, Brenton R. and Gibson, Stephen T. and De La Haye, V. and Liang, Mao Chang},
    number = {10},
    pages = {1--22},
    volume = {117},
    doi = {10.1029/2012JE004139},
    issn = {01480227},
    keywords = {Cassini, INMS, Titan, ionosphere}
}

@article{Wang1999,
    title = {{Ion energy distributions in inductively coupled radio-frequency discharges in argon, nitrogen, oxygen, chlorine, and their mixtures}},
    year = {1999},
    journal = {Journal of Applied Physics},
    author = {Wang, Yicheng and Olthoff, J. K.},
    number = {9},
    pages = {6358},
    volume = {85},
    url = {http://link.aip.org/link/JAPIAU/v85/i9/p6358/s1&Agg=doi},
    isbn = {0021-8979},
    doi = {10.1063/1.370138},
    issn = {00218979}
}

@article{Field1991,
    title = {{Ion energy distributions in radio-frequency discharges}},
    year = {1991},
    journal = {Journal of Applied Physics},
    author = {Field, D. and Klemperer, D. F. and May, P. W. and Song, Y. P.},
    number = {1},
    pages = {82--92},
    volume = {70},
    doi = {10.1063/1.350247},
    issn = {00218979}
}

@article{kawamura1999,
    title = {{Ion energy distributions in rf sheaths; review, analysis and simulation}},
    year = {1999},
    journal = {Plasma Sources Science and Technology},
    author = {Kawamura, E},
    pages = {R45-R64},
    volume = {8}
}

@article{Kawamura1999b,
    title = {{Ion energy distributions in rf sheaths; review, analysis and simulation}},
    year = {1999},
    journal = {Plasma Sources Science and Technology},
    author = {Kawamura, E. and Vahedi, V. and Lieberman, M. A. and Birdsall, C. K.},
    pages = {R45-R64},
    volume = {8}
}

@article{Waite2005,
    title = {{Ion Neutral Mass Spectrometer Results from the First Flyby of Titan}},
    year = {2005},
    journal = {Science},
    author = {Waite, J. H. and Niemann, H. B. and Yelle, R. V. and Kasprzak, W. T. and Cravens, T. E. and Luhmann, J. G. and McNutt, R. L. and Ip, W. H. and Gell, D. and De La Haye, V. and Muller-Wordag, I. and Magee, B. A. and Borggren, N and Ledvina, S. A. and Fletcher, G. G. and Walter, E. M. and Miller, R. and Scherer, S. and Thorpe, R. L. and Xu, Xing and Block, B. P. and Arnett, K.},
    number = {2},
    pages = {195--209},
    volume = {85},
    isbn = {0022-4073},
    doi = {10.1016/S0022-4073(03)00225-5},
    issn = {00224073}
}

@article{Cui2010,
    title = {{Ion transport in Titan’s upper atmosphere}},
    year = {2010},
    journal = {Journal of Geophysical Research},
    author = {Cui, J and Galand, M and Yelle, R V and Wahlund, J E and {\AA}gren, K and Jr, J H Waite and Dougherty, M K},
    pages = {1--12},
    volume = {115},
    doi = {10.1029/2009JA014563}
}

@article{Coolbaugh1989,
    title = {{Ion-molecule chemistry within doubly charged ammonia clusters}},
    year = {1989},
    author = {Coolbaugh, M Todd and Peifer, William R and Garvey, James F}
}

@article{Peifer1989,
    title = {{Ion-Molecule Chemistry within Triply Charged Ammonia Clusters}},
    year = {1989},
    journal = {Journal of Physical Chemistry},
    author = {Peifer, William R and Coolbaugh, M Todd and Garvey, James F},
    number = {11},
    pages = {4700--4703}
}

@article{Molina-Cuberos1999a,
    title = {{Ionization by cosmic rays of the atmosphere of Titan}},
    year = {1999},
    journal = {Planetary and Space Science},
    author = {Molina-Cuberos, G.J. and L{\'{o}}pez-Moreno, J.J. and Rodrigo, R. and Lara, L.M. and O’Brien, K.},
    number = {10-11},
    pages = {1347--1354},
    volume = {47},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0032063399000562},
    doi = {10.1016/S0032-0633(99)00056-2},
    issn = {00320633}
}

@article{Galand2010,
    title = {{Ionization sources in Titan's deep ionosphere}},
    year = {2010},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Galand, Marina and Yelle, Roger and Cui, Jun and Wahlund, Jan Erik and Vuitton, Vronique and Wellbrock, Anne and Coates, Andrew},
    number = {7},
    pages = {1--14},
    volume = {115},
    doi = {10.1029/2009JA015100},
    issn = {21699402}
}

@article{Coates2007,
    title = {{Ionospheric electrons in Titan’s tail : Plasma structure during the Cassini T9 encounter}},
    year = {2007},
    journal = {Geophysical Research Letters},
    author = {Coates, A J and Crary, F J and Young, D T and Szego, K and Arridge, C S and Bebesi, Z and Jr, E C Sittler and Hartle, R E and Hill, T W},
    pages = {1--6},
    volume = {34},
    doi = {10.1029/2007GL030919},
    keywords = {Titan, doi:10.1029/2007GL030919, http://dx.doi.org/10.1029/2007GL030919, ionosphere, plasma}
}

@article{Molina-Cuberos2001,
    title = {{Ionospheric layer induced by meteoric ionization in Titan's atmosphere}},
    year = {2001},
    journal = {Planetary and Space Science},
    author = {Molina-Cuberos, G. J. and Lammer, H. and Stumptner, W. and Schwingenschuh, K. and Rucker, H. O. and L{\'{o}}pez-Moreno, J. J. and Rodrigo, R. and Tokano, T.},
    number = {2},
    pages = {143--153},
    volume = {49},
    isbn = {0032-0633},
    doi = {10.1016/S0032-0633(00)00133-1},
    issn = {00320633},
    keywords = {Cassini, Dust, Huygens, Ionosphere, Meteoroid, Titan}
}

@misc{David1996,
    title = {{IR Vibrational-Rotational Spectra of the Ammonia Molecule}},
    year = {1996},
    booktitle = {Journal of Chemical Education},
    author = {David, C. W.},
    number = {1},
    pages = {46--50},
    volume = {73},
    doi = {10.1021/ed073p46},
    issn = {00219584}
}

@article{Donnell2012,
    title = {{IR-UV Spectroscopic Studies of OH and CN Radical Complexes}},
    year = {2012},
    author = {Donnell, Bridget Anne O}
}

@article{Serigano2016,
    title = {{Isotopic Ratios of Carbon and Oxygen in Titan's CO using ALMA}},
    year = {2016},
    journal = {The Astrophysical Journal Letters},
    author = {Serigano, Joseph and Nixon, Conor A. and Cordiner, Martin A. and Irwin, Patrick G. J. and Teanby, Nicholas A. and Charnley, Steven B. and Lindberg, Johan E.},
    number = {1},
    pages = {1--6},
    volume = {821},
    publisher = {IOP Publishing},
    url = {http://arxiv.org/abs/1602.07707%0Ahttp://dx.doi.org/10.3847/2041-8205/821/1/L8},
    doi = {10.3847/2041-8205/821/1/L8},
    issn = {2041-8213},
    arxivId = {1602.07707},
    keywords = {atmospheres, imaging, individual, interferometric, planets and satellites, planets and satellites: atmospheres, planets and satellites: individual (Titan), spectroscopy, techniques, techniques: imaging spectroscopy, techniques: interferometric, titan}
}

@article{Bloxham2017,
    title = {{Jupiter ’ s interior and deep atmosphere: The initial pole-to-pole passes with the Juno spacecraft}},
    year = {2017},
    author = {Bloxham, J and Brown, S and Connerney, J E P and Dejong, E and Folkner, W and Gautier, D},
    number = {May},
    pages = {821--825},
    volume = {825}
}

@misc{Drossart1999,
    title = {{Jupiter's H3+ aurorae observed with the Galileo/NIMS experiment}},
    year = {1999},
    author = {Drossart, P. and Encrenaz, T. and Carlson, R. W. and Kamp, L. W.}
}

@article{Melin2016,
    title = {{Jupiter's hydrogen bulge: A Cassini perspective}},
    year = {2016},
    journal = {Icarus},
    author = {Melin, Henrik and Stallard, T. S.},
    pages = {238--247},
    volume = {278},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.06.023},
    doi = {10.1016/j.icarus.2016.06.023},
    issn = {10902643},
    keywords = {Aeronomy, Atmosphere, Aurorae, Jupiter, Magnetic fields, Ultraviolet observations}
}

@article{Dobrijevic2010,
    title = {{Key reactions in the photochemistry of hydrocarbons in Neptune's stratosphere}},
    year = {2010},
    journal = {Planetary and Space Science},
    author = {Dobrijevic, M. and Cavali, T. and Hbrard, E. and Billebaud, F. and Hersant, F. and Selsis, F.},
    number = {12},
    pages = {1555--1566},
    volume = {58},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2010.07.024},
    issn = {00320633},
    keywords = {Hydrocarbons, Key reactions, Neptune, Photochemistry, Sensitivity analysis, Uncertainty propagation}
}

@article{Kamath1993,
    title = {{Kinetics of Diacetylene Polymerization: An FT-Raman Study}},
    year = {1993},
    journal = {Macromolecules},
    author = {Kamath, M. and Kim, W. H. and Li, L. and Kumar, J. and Tripathy, S. and Babu, K. N. and Talwar, S. S.},
    number = {22},
    pages = {5954--5958},
    volume = {26},
    isbn = {0387312781},
    doi = {10.1021/ma00074a017},
    issn = {15205835},
    pmid = {7633532},
    arxivId = {arXiv:1011.1669v3}
}

@article{Moore1990,
    title = {{Koyaanismuuyaw: the hypothesis of a perennially dichotomous Triton}},
    year = {1990},
    journal = {Geophysical Research Letters},
    author = {Moore, Jeffrey M and Spencer, John R},
    number = {10},
    pages = {1757--1760},
    volume = {17}
}

@article{Carrasco2016,
    title = {{Laboratory analogues simulating titan's atmospheric aerosols: Compared chemical compositions of grains and thin films}},
    year = {2016},
    journal = {Planetary and Space Science},
    author = {Carrasco, N. and Jomard, François and Vigneron, Jackie and Etcheberry, Arnaud and Cernogora, Guy},
    publisher = {Elsevier},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0032063316300459},
    doi = {10.1016/j.pss.2016.05.006},
    issn = {00320633}
}

@article{Lutz1976,
    title = {{Laboratory band strengths of methane and their application to the atmospheres of Jupiter, Saturn, Uranus, Neptune, and Titan}},
    year = {1976},
    journal = {The Astrophysical Journal},
    author = {Lutz, B. L. and Owen, T. and Cess, R. D.},
    pages = {541},
    volume = {203},
    url = {http://adsabs.harvard.edu/abs/1976ApJ...203..541L},
    doi = {10.1086/154110},
    issn = {0004-637X},
    keywords = {Abundance, Atmospheric Radiation, Jupiter Atmosphere, Methane, Molecular Spectra, Neptune (Planet), Planetary Atmospheres, Saturn (Planet), Spectral Bands, Spectral Line Width, Spectrum Analysis, Titan, Uranus (Planet)}
}

@article{Thissen2006,
    title = {{Laboratory experiments for Titan's ionosphere: the chemistry of N2+ , N+ , and N2++ nitrogen ions Laboratory experiments for Titan’s ionosphere : the chemistry of N+2 , N , and N2 nitrogen ions}},
    year = {2006},
    author = {Thissen, R. and Alcaraz, C. and Dutuit, O. and Nicolas, C. and Soldi-Lose, H. and Zabka, Jan and Franceschi, Pietro},
    number = {January},
    pages = {2--4}
}

@article{Imanaka2004,
    title = {{Laboratory experiments of Titan tholin formed in cold plasma at various pressures: Implications for nitrogen-containing polycyclic aromatic compounds in Titan haze}},
    year = {2004},
    journal = {Icarus},
    author = {Imanaka, Hiroshi and Khare, Bishun N. and Elsila, Jamie E. and Bakes, Emma L O and McKay, Christopher P. and Cruikshank, Dale P. and Sugita, Seiji and Matsui, Takafumi and Zare, Richard N.},
    number = {2},
    pages = {344--366},
    volume = {168},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2003.12.014},
    issn = {00191035},
    keywords = {Haze, Nitrogen-containing polycyclic aromatic compounds, Organic chemistry, Spectroscopy, Tholin, Titan}
}

@article{Horst2018,
    title = {{Laboratory investigations of Titan haze formation: In situ measurement of gas and particle composition}},
    year = {2018},
    journal = {Icarus},
    author = {H{\"{o}}rst, Sarah M. and Yoon, Y. Heidi and Ugelow, Melissa S. and Parker, Alex H. and Li, Rui and de Gouw, Joost A. and Tolbert, Margaret A.},
    pages = {136--151},
    volume = {301},
    doi = {10.1016/j.icarus.2017.09.039},
    issn = {10902643},
    arxivId = {1709.10131},
    keywords = {Atmospheres, Organic chemistry, Photochemistry, Titan, atmosphere, chemistry}
}

@article{Hadamcik2009,
    title = {{Laboratory light-scattering measurements with Titan's aerosols analogues produced by a dusty plasma}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Hadamcik, E. and Renard, J. B. and Alcouffe, G. and Cernogora, G. and Levasseur-Regourd, A. C. and Szopa, C.},
    number = {13},
    pages = {1631--1641},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.06.013},
    doi = {10.1016/j.pss.2009.06.013},
    issn = {00320633},
    keywords = {Dusty plasma, Laboratory experiment, Light scattering, Linear polarization, Titan's haze analogue}
}

@article{Mitchell2015,
    title = {{Laboratory measurements of cryogenic liquid alkane microwave absorptivity and implications for the composition of Ligeia Mare, Titan}},
    year = {2015},
    journal = {Geophysical Research Letters},
    author = {Mitchell, Karl L. and Barmatz, Martin B. and Jamieson, Corey S. and Lorenz, Ralph D. and Lunine, Jonathan I.},
    number = {5},
    pages = {1340--1345},
    volume = {42},
    doi = {10.1002/2014GL059475},
    issn = {19448007},
    keywords = {Titan, composition, liquid alkanes, loss tangent, microwave, seas}
}

@article{Saykally1976,
    title = {{Laboratory Microwave Spectrum and Rest Frequencies of the N2H+ Ion}},
    year = {1976},
    journal = {The Astrophysical Journal},
    author = {Saykally, R. J. and Dixon, T. and Anderson, T. and Szanto, P. and Woods, R. C.}
}

@article{Nelson2018,
    title = {{Laboratory simulations of planetary surfaces: Understanding regolith physical properties from remote photopolarimetric observations}},
    year = {2018},
    journal = {Icarus},
    author = {Nelson, Robert M. and Boryta, Mark D. and Hapke, Bruce W. and Manatt, Kenneth S. and Shkuratov, Yuriy and Psarev, V. and Vandervoort, Kurt and Kroner, Desire and Nebedum, Adaze and Vides, Christina L. and Qui{\~{n}}ones, John},
    pages = {483--498},
    volume = {302},
    publisher = {Elsevier Inc.},
    url = {https://doi.org/10.1016/j.icarus.2017.11.021},
    doi = {10.1016/j.icarus.2017.11.021},
    issn = {10902643},
    keywords = {Europa, Jupiter, satellites, Photometry, Polarimetry, Radiative transfer, Satellites, surfaces}
}

@article{Castillo-Rogez2012,
    title = {{Laboratory studies in support of planetary geophysics}},
    year = {2012},
    journal = {Jet Propulsion},
    author = {Castillo-Rogez, JC and Durham, WB},
    number = {1},
    pages = {1--8},
    volume = {1},
    url = {http://www.psi.edu/sites/default/files/imported/about/staff/sykes/sbag/roadmap/JulieCCastillo_lab_white_paper.pdf}
}

@article{Curtis2008,
    title = {{Laboratory studies of methane and ethane adsorption and nucleation onto organic particles: Application to Titan's clouds}},
    year = {2008},
    journal = {Icarus},
    author = {Curtis, Daniel B. and Hatch, Courtney D. and Hasenkopf, Christa A. and Toon, Owen B. and Tolbert, Margaret A. and McKay, Christopher P. and Khare, Bishun N.},
    number = {2},
    pages = {792--801},
    volume = {195},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2008.02.003},
    issn = {00191035},
    keywords = {Atmospheres, IR spectroscopy, Ices, Organic chemistry, Titan, chemistry}
}

@article{Kobayashi2017,
    title = {{Laboratory Studies of Methane and Its Relationship to Prebiotic Chemistry}},
    year = {2017},
    journal = {Astrobiology},
    author = {Kobayashi, Kensei and Geppert, Wolf D. and Carrasco, Nathalie and Holm, Nils G. and Mousis, Olivier and Palumbo, Maria Elisabetta and Waite, J. Hunter and Watanabe, Naoki and Ziurys, Lucy M.},
    number = {8},
    pages = {786--812},
    volume = {17},
    url = {http://online.liebertpub.com/doi/10.1089/ast.2016.1492},
    doi = {10.1089/ast.2016.1492},
    issn = {1531-1074},
    pmid = {28727932}
}

@article{Thissen2009,
    title = {{Laboratory studies of molecular growth in the titan ionosphere}},
    year = {2009},
    journal = {Journal of Physical Chemistry A},
    author = {Thissen, Roland and Vuitton, Veronique and Lavvas, Panayotis and Lemaire, Joel and Dehon, Christophe and Dutuit, Odile and Smith, Mark A. and Turchini, Stefano and Catone, Daniele and Yelle, Roger V. and Pernot, Pascal and Somogyi, Arpad and Coreno, Marcello},
    number = {42},
    pages = {11211--11220},
    volume = {113},
    isbn = {1520-5215 (Electronic){\textbackslash}n1089-5639 (Linking)},
    doi = {10.1021/jp9050353},
    issn = {10895639},
    pmid = {19769328}
}

@article{Gudipati2015a,
    title = {{Laboratory Studies Towards Understanding Comets}},
    year = {2015},
    journal = {Space Science Reviews},
    author = {Gudipati, Murthy S. and Abou Mrad, Ninette and Blum, Jürgen and Charnley, Steven B. and Chiavassa, Thierry and Cordiner, Martin A. and Mousis, Olivier and Danger, Grégoire and Duvernay, Fabrice and Gundlach, Bastian and Hartogh, Paul and Marboeuf, Ulysse and Simonia, Irakli and Simonia, Tsitsino and Theul{\'{e}}, Patrice and Yang, Rui},
    number = {1-4},
    pages = {101--150},
    volume = {197},
    publisher = {Springer Science+Business Media Dordrecht},
    url = {http://dx.doi.org/10.1007/s11214-015-0192-5},
    doi = {10.1007/s11214-015-0192-5},
    issn = {15729672},
    keywords = {Clathrates, Coma, Comets, Experimental, Ice, Isotope ratios, Laboratory, Negative ions, Organics, Origin of life, Origin of solar systems, Outgassing, Review, Volatiles}
}

@article{Helfenstein1992,
    title = {{Large Quasi-Circular Features Beneath Frost on Triton}},
    year = {1992},
    journal = {Science},
    author = {Helfenstein, Paul and Veverka, Joseph and Mccarthy, Derek and Lee, Pascal and Hillier, John and Helfenstein, Paul and Veverka, Joseph and Mccarthy, Derek and Lee, Pascal and Hillier, John},
    number = {5046},
    pages = {824--826},
    volume = {255},
    issn = {00368075}
}

@article{Trafton1984,
    title = {{Large seasonal variations in Triton's atmosphere}},
    year = {1984},
    journal = {Icarus},
    author = {Trafton, L.},
    number = {2},
    pages = {312--324},
    volume = {58},
    doi = {10.1016/0019-1035(84)90048-4},
    issn = {10902643}
}

@article{Li1984,
    title = {{Laser measurements of the effects of vibrational energy on the reactions of CN}},
    year = {1984},
    journal = {The Journal of Chemical Physics},
    author = {Li, Xuechu and Sayah, Nahid and Jackson, William M.},
    number = {2},
    pages = {833--840},
    volume = {81},
    doi = {10.1063/1.447717},
    issn = {00219606}
}

@article{Bouley2016,
    title = {{Late Tharsis formation and implications for early Mars.}},
    year = {2016},
    journal = {Nature},
    author = {Bouley, Sylvain and Baratoux, David and Matsuyama, Isamu and Forget, Francois and S{\'{e}}journ{\'{e}}, Antoine and Turbet, Martin and Costard, Francois},
    number = {7594},
    pages = {344--347},
    volume = {531},
    url = {http://dx.doi.org/10.1038/nature17171},
    doi = {10.1038/nature17171},
    issn = {1476-4687},
    pmid = {26934230}
}

@article{Hofstadter1989,
    title = {{Latitudinal variations of ammonia in the atmosphere of Uranus: An analysis of microwave observations}},
    year = {1989},
    journal = {Icarus},
    author = {Hofstadter, Mark D. and Muhleman, Duane O.},
    number = {2},
    pages = {396--412},
    volume = {81},
    doi = {10.1016/0019-1035(89)90060-2},
    issn = {10902643}
}

@article{Teanby2006,
    title = {{Latitudinal variations of HCN, HC3N, and C2 N2 in Titan's stratosphere derived from Cassini CIRS data}},
    year = {2006},
    journal = {Icarus},
    author = {Teanby, N. A. and Irwin, P. G J and de Kok, R. and Nixon, C. A. and Coustenis, A. and B{\'{e}}zard, B. and Calcutt, S. B. and Bowles, N. E. and Flasar, F. M. and Fletcher, L. and Howett, C. and Taylor, F. W.},
    number = {1},
    pages = {243--255},
    volume = {181},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2005.11.008},
    issn = {00191035},
    keywords = {Atmospheres, composition, Titan}
}

@article{Lammer2001,
    title = {{Lightning activity on Titan: Can Cassini detect it?}},
    year = {2001},
    journal = {Planetary and Space Science},
    author = {Lammer, H. and Tokano, T. and Fischer, G. and Stumptner, W. and Molina-Cuberos, G. J. and Schwingenschuh, K. and Rucker, H. O.},
    number = {6},
    pages = {561--574},
    volume = {49},
    doi = {10.1016/S0032-0633(00)00171-9},
    issn = {00320633}
}

@article{Olgin2011,
    title = {{Limits of Enceladus's ice shell thickness from tidally driven tiger stripe shear failure}},
    year = {2011},
    journal = {Geophysical Research Letters},
    author = {Olgin, John G. and Smith-Konter, Bridget R. and Pappalardo, Robert T.},
    number = {2},
    pages = {1--5},
    volume = {38},
    doi = {10.1029/2010GL044950},
    issn = {00948276}
}

@article{Tomasko2009a,
    title = {{Limits on the size of aerosols from measurements of linear polarization in Titan's atmosphere}},
    year = {2009},
    journal = {Icarus},
    author = {Tomasko, M. G. and Doose, L. R. and Dafoe, L. E. and See, C.},
    number = {1},
    pages = {271--283},
    volume = {204},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.05.034},
    doi = {10.1016/j.icarus.2009.05.034},
    issn = {00191035},
    keywords = {Titan}
}

@article{Pieri1981,
    title = {{Lineament and polygon patterns on Europa}},
    year = {1981},
    journal = {Nature},
    author = {Pieri, D.}
}

@article{Rhoden2013,
    title = {{Lineament azimuths on Europa: Implications for obliquity and non-synchronous rotation}},
    year = {2013},
    journal = {Icarus},
    author = {Rhoden, Alyssa Rose and Hurford, Terry A.},
    number = {1},
    pages = {841--859},
    volume = {226},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.06.029},
    doi = {10.1016/j.icarus.2013.06.029},
    issn = {00191035},
    keywords = {Europa, Rotational dynamics, Tectonics}
}

@article{Rhoden2015,
    title = {{Linking Europa's plume activity to tides, tectonics, and liquid water}},
    year = {2015},
    journal = {Icarus},
    author = {Rhoden, Alyssa Rose and Hurford, Terry A. and Roth, Lorenz and Retherford, Kurt},
    pages = {169--178},
    volume = {253},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.02.023},
    doi = {10.1016/j.icarus.2015.02.023},
    issn = {10902643},
    arxivId = {1502.06854},
    keywords = {Europa, Jupiter, satellites, Satellites, surfaces, Tectonics}
}

@article{Fallis2013b,
    title = {{Linking Europa's plume activity to tides, tectonics, and liquid water}},
    year = {2013},
    journal = {Journal of Chemical Information and Modeling},
    author = {Fallis, A.G},
    number = {9},
    pages = {1689--1699},
    volume = {53},
    isbn = {9788578110796},
    doi = {10.1017/CBO9781107415324.004},
    issn = {1098-6596},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {icle}
}

@article{Squyres1983,
    title = {{Liquid water and active resurfacing on Europa}},
    year = {1983},
    journal = {Nature},
    author = {Squyres, S. W. and Reynolds, R. T. and Cassen, P.},
    number = {20},
    pages = {225--226},
    volume = {301}
}

@article{Poggiali2016,
    title = {{Liquid-filled canyons on Titan}},
    year = {2016},
    journal = {Geophysical Research Letters},
    author = {Poggiali, V and Mastrogiuseppe, M and Hayes, A G and Seu, R and Birch, S P D and Lorenz, R and Grima, C and Hofgartner, J D},
    number = {May},
    pages = {1--8},
    doi = {10.1002/2016GL069679.Received},
    issn = {19448007},
    keywords = {10.1002/2016GL069679 and spaceborne radar, Titan, altimetry, geophysical measurement techniques, hydrology, planetary science}
}

@article{Hammel2007,
    title = {{Long-term atmospheric variability on Uranus and Neptune}},
    year = {2007},
    journal = {Icarus},
    author = {Hammel, H. B. and Lockwood, G. W.},
    number = {1},
    pages = {291--301},
    volume = {186},
    doi = {10.1016/j.icarus.2006.08.027},
    issn = {00191035},
    keywords = {Neptune, Photometry, Uranus, atmosphere}
}

@article{Sagan1971b,
    title = {{Long-wavelength ultraviolet photoproduction of amino acids on the primitive earth}},
    year = {1971},
    journal = {Science},
    author = {Sagan, C. and Khare, B. N.},
    number = {3995},
    pages = {417--420},
    volume = {173},
    doi = {10.1126/science.173.3995.417},
    issn = {00368075},
    pmid = {17770442}
}

@article{Berteloite2008,
    title = {{Low temperature (39-298 K) kinetics study of the reactions of the C4H radical with various hydrocarbons observed in Titan's atmosphere}},
    year = {2008},
    journal = {Icarus},
    author = {Berteloite, C. and Le Picard, Sébastien D. and Birza, Petre and Gazeau, Marie Claire and Canosa, André and B{\'{e}}nilan, Yves and Sims, Ian R.},
    number = {2},
    pages = {746--757},
    volume = {194},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2007.10.012},
    issn = {00191035},
    keywords = {Atmospheres, Organic chemistry, Titan, chemistry, composition}
}

@article{Neish2009,
    title = {{Low temperature hydrolysis of laboratory tholins in ammonia-water solutions: Implications for prebiotic chemistry on Titan}},
    year = {2009},
    journal = {Icarus},
    author = {Neish, C. D. and Somogyi, Á. and Lunine, J. I. and Smith, M. A.},
    number = {1},
    pages = {412--421},
    volume = {201},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.01.003},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.01.003},
    issn = {00191035},
    keywords = {Prebiotic chemistry, Prebiotic environments, Titan}
}

@article{Biennier2014,
    title = {{Low temperature reaction kinetics of CN-+HC3N and implications for the growth of anions in Titan's atmosphere}},
    year = {2014},
    journal = {Icarus},
    author = {Biennier, Ludovic and Carles, Sophie and Cordier, Daniel and Guillemin, Jean Claude and Le Picard, Sébastien D. and Faure, Alexandre},
    pages = {123--131},
    volume = {227},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.09.004},
    isbn = {00191035},
    doi = {10.1016/j.icarus.2013.09.004},
    issn = {00191035},
    keywords = {Atmospheres, Ionospheres, Titan, atmosphere, chemistry}
}

@article{Joalland2016,
    title = {{Low-Temperature Reactivity of C2n+1N- Anions with Polar Molecules}},
    year = {2016},
    journal = {Journal of Physical Chemistry Letters},
    author = {Joalland, Baptiste and Jamal-Eddine, Nour and K??os, Jacek and Lique, Fran??ois and Trolez, Yann and Guillemin, Jean Claude and Carles, Sophie and Biennier, Ludovic},
    number = {15},
    pages = {2957--2961},
    volume = {7},
    doi = {10.1021/acs.jpclett.6b01191},
    issn = {19487185}
}

@article{Santamaria2014,
    title = {{Low-temperature spectroscopy of the {\$}{\^{}}{\{}12{\}}{\$}C{\$}{\_}2{\$}H{\$}{\_}2{\$} ({\$}{\textbackslash}upsilon{\_}1 +{\textbackslash}upsilon{\_}3{\$}) band in a helium buffer gas}},
    year = {2014},
    author = {Santamaria, L. and Di Sarno, V. and Ricciardi, I. and De Rosa, M. and Mosca, S. and Santambrogio, G. and Maddaloni, P. and De Natale, P.},
    pages = {1--15},
    url = {http://arxiv.org/abs/1410.5310%5Cnhttp://dx.doi.org/10.1088/0004-637X/801/1/50},
    doi = {10.1088/0004-637X/801/1/50},
    arxivId = {1410.5310},
    keywords = {buffer gas cooling, cold, submitted to, the astrophysical journal, vibrational spectroscopy}
}

@article{Stress2005,
    title = {{Lunar and Planetary Science XXXVI ( 2005 ) Lunar and Planetary Science XXXVI ( 2005 )}},
    year = {2005},
    author = {Stress, Diurnal and Pappalardo, Robert T. and Barr, Amy C. and Gleeson, Damhnait and Mullen, Mccall and Stempel, Michelle M and Wahr, John and Physics, Space and Sciences, Planetary and Louis, Saint},
    pages = {3--4}
}

@article{Singh2014,
    title = {{Lyot-based Low Order Wavefront Sensor : Implementation on the Subaru Coronagraphic Extreme Adaptive Optics System and its Laboratory Performance}},
    year = {2014},
    author = {Singh, Garima and Guyon, Olivier and Baudoz, Pierre and Jovanovic, Nemanja and Martinache, Frantz and Janssen, Place Jules and Meudon, F- and Lagrange, Laboratoire},
    pages = {1--9},
    volume = {9148},
    doi = {10.1117/12.2057211},
    keywords = {coronagraph, extreme adaptive optics, high contrast imaging}
}

@article{Singh2014a,
    title = {{Lyot-based low order wavefront sensor for phase-mask coronagraphs: principle, simulations and laboratory experiments}},
    year = {2014},
    journal = {Astronomical Society of the Pacific},
    author = {Singh, Garima and Martinache, Frantz and Baudoz, Pierre and Guyon, Olivier and Matsuo, Taro and Jovanovic, Nemanja},
    number = {940},
    pages = {586--594},
    volume = {126},
    doi = {10.1086/677048},
    issn = {00046280},
    arxivId = {arXiv:1404.7201v1}
}

@article{LeMouelic2018,
    title = {{Mapping polar atmospheric features on Titan with VIMS: from the dissipation of the northern cloud to the onset of a southern polar vortex}},
    year = {2018},
    journal = {Icarus},
    author = {Le Mou{\'{e}}lic, S. and Rodriguez, S. and Robidel, R. and Rousseau, B. and Seignovert, Benoît and Sotin, C. and Barnes, J. W. and Brown, R. H. and Baines, K. H. and Buratti, B. J. and Clark, R. N. and Nicholson, P. D. and Rannou, P. and Cornet, T.},
    number = {December 2006},
    volume = {2004},
    url = {http://www.nature.com/articles/s41550-018-0434-z},
    isbn = {1844251411},
    doi = {10.1038/s41550-018-0434-z},
    issn = {2397-3366},
    arxivId = {arXiv:1805.01017v1},
    keywords = {10, 1038, doi, image processing, infrared observations, s41550-018-0434-z, titan, titan atmosphere, titan clouds}
}

@article{Marchi2004,
    title = {{Mass transfer in the satellite system of Neptune: Implications for Triton's crater asymmetry}},
    year = {2004},
    journal = {Planetary and Space Science},
    author = {Marchi, S. and Barbieri, C. and Lazzarin, M.},
    number = {8},
    pages = {671--677},
    volume = {52},
    doi = {10.1016/j.pss.2004.02.002},
    issn = {00320633}
}

@article{Cassidy2009,
    title = {{Massive Satellites of Close-in Gas Giant Exoplanets}},
    year = {2009},
    journal = {The Astrophysical Journal},
    author = {Cassidy, Timothy A. and Mendez, Rolando and Arras, Phil and Johnson, Robert E. and Skrutskie, Michael F.},
    number = {2},
    pages = {1341--1348},
    volume = {704},
    url = {http://stacks.iop.org/0004-637X/704/i=2/a=1341?key=crossref.2ff52bf82fc4e17e20efbeed472c386b},
    doi = {10.1088/0004-637X/704/2/1341},
    issn = {0004-637X},
    keywords = {celestial mechanics, general, planetary systems, planets and satellites}
}

@article{Malaska2016a,
    title = {{Material transport map of Titan: The fate of dunes}},
    year = {2016},
    journal = {Icarus},
    author = {Malaska, Michael J. and Lopes, Rosaly M. and Hayes, Alex G. and Radebaugh, Jani and Lorenz, Ralph D. and Turtle, Elizabeth P.},
    pages = {183--196},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.09.029},
    doi = {10.1016/j.icarus.2015.09.029},
    issn = {10902643},
    keywords = {Geological processes, Titan, Titan, surface}
}

@article{Chiang2010,
    title = {{Measurement of Cosmic Microwave Background Polarization Power Spectra From Two Years of Bicep Data}},
    year = {2010},
    journal = {The Astrophysical Journal},
    author = {Chiang, H. C. and Ade, P. A. R. and Barkats, D. and Battle, J. O. and Bierman, E. M. and Bock, J. J. and Dowell, C. D. and Duband, L. and Hivon, E. F. and Holzapfel, W. L. and Hristov, V. V. and Jones, W. C. and Keating, B. G. and Kovac, J. M. and Kuo, C. L. and Lange, A. E. and Leitch, E. M. and Mason, P. V. and Matsumura, T. and Nguyen, H. T. and Ponthieu, N. and Pryke, C. and Richter, S. and Rocha, G. and Sheehy, C. and Takahashi, Y. D. and Tolan, J. E. and Yoon, K. W.},
    number = {2},
    pages = {1123--1140},
    volume = {711},
    url = {http://stacks.iop.org/0004-637X/711/i=2/a=1123?key=crossref.cf19587425351fdee979981c6961439d},
    doi = {10.1088/0004-637X/711/2/1123},
    issn = {0004-637X},
    keywords = {cosmic background radiation, cosmology, gravitational waves, inflation, observations}
}

@article{Tomasko2008a,
    title = {{Measurements of methane absorption by the descent imager/spectral radiometer (DISR) during its descent through Titan's atmosphere}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Tomasko, M. G. and B{\'{e}}zard, B. and Doose, L. and Engel, S. and Karkoschka, E.},
    number = {5},
    pages = {624--647},
    volume = {56},
    doi = {10.1016/j.pss.2007.10.009},
    issn = {00320633},
    keywords = {Huygens, Methane absorption, Titan}
}

@article{Yin2016,
    title = {{Mechanics of evenly spaced strike-slip faults and its implications for the formation of tiger-stripe fractures on Saturn's moon Enceladus}},
    year = {2016},
    journal = {Icarus},
    author = {Yin, An and Zuza, Andrew V. and Pappalardo, Robert T.},
    pages = {466},
    volume = {277},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.10.027},
    doi = {10.1016/j.icarus.2016.06.025},
    issn = {10902643}
}

@article{Peale1979,
    title = {{Melting of Io by Tidal Dissipation}},
    year = {1979},
    journal = {Science},
    author = {Peale, S. J. and Cassen, P. and Reynolds, R. T.},
    number = {2},
    pages = {81--87},
    volume = {XXXIII},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/15003161%5Cnhttp://cid.oxfordjournals.org/lookup/doi/10.1093/cid/cir991%5Cnhttp://www.scielo.cl/pdf/udecada/v15n26/art06.pdf%5Cnhttp://www.scopus.com/inward/record.url?eid=2-s2.0-84861150233&partnerID=tZOtx3y1},
    isbn = {9780874216561},
    doi = {10.1007/s13398-014-0173-7.2},
    issn = {0717-6163},
    pmid = {15003161},
    arxivId = {arXiv:gr-qc/9809069v1},
    archivePrefix = {arXiv},
    eprint = {9809069v1},
    primaryClass = {gr-qc},
    keywords = {Adolescence, Adolescencia, Adolescent, Adolescent Behavior, Adolescent Behavior: psychology, Adult, Agresiones al cuerpo, Attachment to the body, Attaque au corps, Autolesiones deliberadas, Automutilation d{\'{e}}lib{\'{e}}r{\'{e}}e, Body Piercing, Body Piercing: psychology, Body Piercing: statistics {\&} numerical data, Body image, CUERPO, Chile, Chile: epidemiology, Cosmetic Techniques, Deliberate self-harm, Epidemiologic Methods, Female, Humans, Image corporelle, Imagen corporal, JUVENTUD, MODIFICACIONES CORPORALES, Male, Motivation, Movement, Risk-Taking, Self Mutilation, Self Mutilation: physiopathology, Self Mutilation: ultrasonography, Sex Distribution, Speech Articulation Tests, Speech Intelligibility, Tattooing, Tattooing: psychology, Tattooing: statistics {\&} numerical data, Tongue, Tongue: injuries, Tongue: physiopathology, Tongue: ultrasonography, aesthetics, and on cor-, as none were found, autoinjury and health, body, complications did not, complications from inserting a, constituci{\'{o}}n del yo, control postural- estabilizaci{\'{o}}n- v{\'{i}}as, corporal modifications, corps, cuerpo, culturas juveniles, cultures juv{\'{e}}niles, epidural, esth{\'{e}}tique, est{\'{e}}tica, find any reports of, high resolution images, if neuraxial anes-, ing with neuraxial anesthesia, jeunesse, juvenile cultures, juventud, mecanismos de anteroalimentaci{\'{o}}n y, modificacio -, needle through a, nes corporales, perforaci{\'{o}}n corporal, piel, pr{\'{a}}ctica autolesiva, psicoan{\'{a}}lisis, research, retroalimentaci{\'{o}}n, risks management, segunda piel, sensitivas y motoras, spinal, sustainable reconstruction, tattoo, tattooing, tattoos, tatuaje, the literature on tattoos, was reviewed to see, youth}
}

@article{Soter1966,
    title = {{Mercury : Infrared Evidence for Nonsynchronous Rotation}},
    year = {1966},
    journal = {Science},
    author = {Soter, S. L.},
    pages = {14--15},
    volume = {153}
}

@article{Stevenson2012,
    title = {{Mercury's mysteries start to unfold}},
    year = {2012},
    journal = {Nature},
    author = {Stevenson, David J.},
    pages = {52--53},
    volume = {485},
    isbn = {1476-4687 (Electronic){\textbackslash}r0028-0836 (Linking)},
    doi = {10.1038/485052a},
    issn = {00280836},
    pmid = {22552095}
}

@article{Guerlet2010,
    title = {{Meridional distribution of CH3C2H and C4H2 in Saturn’s stratosphere from CIRS / Cassini limb and nadir observations}},
    year = {2010},
    journal = {Icarus},
    author = {Guerlet, Sandrine and Fouchet, Thierry and B{\'{e}}zard, Bruno and Moses, Julianne I and Fletcher, Leigh N and Simon-miller, Amy A and Flasar, F Michael},
    number = {2},
    pages = {682--695},
    volume = {209},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.03.033},
    doi = {10.1016/j.icarus.2010.03.033},
    issn = {0019-1035}
}

@article{Adamkovics2016,
    title = {{Meridional variation in tropospheric methane on Titan observed with AO spectroscopy at Keck and VLT}},
    year = {2016},
    journal = {Icarus},
    author = {{\'{A}}d{\'{a}}mkovics, Máté and Mitchell, Jonathan L. and Hayes, Alexander G. and Rojo, Patricio M. and Corlies, Paul and Barnes, Jason W. and Ivanov, Valentin D. and Brown, Robert H. and Baines, Kevin H. and Buratti, Bonnie J. and Clark, Roger N. and Nicholson, Philip D. and Sotin, Christophe},
    pages = {376--388},
    volume = {270},
    doi = {10.1016/j.icarus.2015.05.023},
    issn = {10902643},
    arxivId = {1509.08835},
    keywords = {Adaptive optics, Atmospheres, Titan, atmosphere, evolution, structure}
}

@article{Sundberg2012,
    title = {{Messenger observations of dipolarization events in Mercury's magnetotail}},
    year = {2012},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Sundberg, Torbjörn and Slavin, James A. and Boardsen, Scott A. and Anderson, Brian J. and Korth, Haje and Ho, George C. and Schriver, David and Uritsky, Vadim M. and Zurbuchen, Thomas H. and Raines, Jim M. and Baker, Daniel N. and Krimigis, Stamatios M. and McNutt, Ralph L. and Solomon, Sean C.},
    number = {9},
    pages = {1--11},
    volume = {117},
    isbn = {2156-2202},
    doi = {10.1029/2012JA017756},
    issn = {21699402}
}

@article{Zwier1996,
    title = {{Metastable Diacetylene Reactions as Routes to Large Hydrocarbons in Titan’s Atmosphere}},
    year = {1996},
    journal = {Icarus},
    author = {Zwier, Timothy S and Allen, Mark},
    pages = {578--583},
    volume = {583}
}

@article{Tokano2005a,
    title = {{Meteorological assessment of the surface temperatures on Titan : constraints on the surface type}},
    year = {2005},
    author = {Tokano, Tetsuya},
    pages = {222--242},
    volume = {173},
    doi = {10.1016/j.icarus.2004.08.019},
    keywords = {atmospheres, meteorology, satellite, structure, surfaces, titan}
}

@article{Scattergood1977,
    title = {{Methane absorption in the visible spectra of the outer planets and Titan}},
    year = {1975},
    journal = {The Astrophysical Journal},
    author = {Owen, T and Cess, RD},
    pages = {L37-L40},
    volume = {197},
    url = {http://adsabs.harvard.edu/full/1975ApJ...197L..37O},
    doi = {10.1086/181771}
}

@article{Fletcher2009a,
    title = {{Methane and its isotopologues on Saturn from Cassini/CIRS observations}},
    year = {2009},
    journal = {Icarus},
    author = {Fletcher, L. N. and Orton, G. S. and Teanby, N. A. and Irwin, P. G.J. and Bjoraker, G. L.},
    number = {2},
    pages = {351--367},
    volume = {199},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2008.09.019},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2008.09.019},
    issn = {00191035},
    keywords = {Atmospheres, Saturn, composition, structure}
}

@article{Giver1976,
    title = {{Methane Contamination of H2 Features in the Spectrum of Titan}},
    year = {1976},
    author = {Giver, P.}
}

@article{Pintassilgo1999,
    title = {{Methane decomposition and active nitrogen in a N2-CH4 glow discharge at low pressures}},
    year = {1999},
    journal = {Plasma Sources Science Technology},
    author = {Pintassilgo, C D and Loureiro, J and Cernogora, G and Touzeau, M},
    number = {1},
    pages = {463--478},
    isbn = {0963-0252},
    doi = {http://dx.doi.org/10.1016/0019-1035(91)90068-5},
    issn = {0019-1035}
}

@article{Lovesday2001,
    title = {{Methane drizzle on Titan}},
    year = {2006},
    journal = {Nature},
    author = {Tokano, Tetsuya and McKay, Christopher P. and Neubauer, Fritz M. and Atreya, Sushil K. and Ferri, Francesca and Fulchignoni, Marcello and Niemann, Hasso B.},
    number = {7101},
    pages = {432--435},
    volume = {442},
    isbn = {0028-0836},
    doi = {10.1038/nature04948},
    issn = {14764687},
    pmid = {16871213}
}

@article{Romanzin2005,
    title = {{Methane photochemistry: A brief review in the frame of a new experimental program of Titan's atmosphere simulations}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {Romanzin, C. and Gazeau, M. C. and B{\'{e}}nilan, Y. and H{\'{e}}brard, E. and Jolly, A. and Raulin, F. and Boy{\'{e}}-P{\'{e}}ronne, S. and Douin, S. and Gauyacq, D.},
    number = {2},
    pages = {258--267},
    volume = {36},
    doi = {10.1016/j.asr.2005.03.079},
    issn = {02731177},
    keywords = {Atmosphere, Atmospheric simulations, Methane photolysis, Photochemical models, Titan}
}

@article{Charnay2015,
    title = {{Methane storms as a driver of Titan’s dune orientation}},
    year = {2015},
    journal = {Nature Geoscience},
    author = {Charnay, Benjamin and Barth, Erika and Rafkin, Scot and Narteau, Clément and Lebonnois, Sébastien and Rodriguez, Sébastien and Courrech du Pont, Sylvain and Lucas, Antoine},
    number = {April},
    pages = {1--5},
    volume = {8},
    url = {http://www.nature.com/doifinder/10.1038/ngeo2406},
    doi = {10.1038/ngeo2406},
    issn = {1752-0894},
    arxivId = {arXiv:1504.03404v1}
}

@article{Barth2006,
    title = {{Methane, ethane, and mixed clouds in Titan's atmosphere: Properties derived from microphysical modeling}},
    year = {2006},
    journal = {Icarus},
    author = {Barth, Erika L. and Toon, Owen B.},
    number = {1},
    pages = {230--250},
    volume = {182},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2005.12.017},
    issn = {00191035},
    keywords = {Atmospheres, Titan, structure}
}

@article{Stoker1990,
    title = {{Microbial metabolism of tholin}},
    year = {1990},
    journal = {Icarus},
    author = {Stoker, C. R. and Boston, P. J. and Mancinelli, R. L. and Segal, W. and Khare, B. N. and Sagan, C.},
    number = {1},
    pages = {241--256},
    volume = {85},
    isbn = {0019-1035 (Print){\textbackslash}n0019-1035 (Linking)},
    doi = {10.1016/0019-1035(90)90114-O},
    issn = {10902643},
    pmid = {11538367}
}

@article{Barth2003,
    title = {{Microphysical modeling of ethane ice clouds in Titan's atmosphere}},
    year = {2003},
    journal = {Icarus},
    author = {Barth, Erika L. and Toon, Owen B.},
    number = {1},
    pages = {94--113},
    volume = {162},
    doi = {10.1016/S0019-1035(02)00067-2},
    issn = {00191035},
    keywords = {Atmospheres, Clouds, Structure, Titan}
}

@article{Gautier2012,
    title = {{Mid- and far-infrared absorption spectroscopy of Titan's aerosols analogues}},
    year = {2012},
    journal = {Icarus},
    author = {Gautier, Thomas and Carrasco, Nathalie and Mahjoub, Ahmed and Vinatier, Sandrine and Giuliani, Alexandre and Szopa, Cyril and Anderson, Carrie M. and Correia, Jean Jacques and Dumas, Paul and Cernogora, Guy},
    number = {1},
    pages = {320--327},
    volume = {221},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.07.025},
    doi = {10.1016/j.icarus.2012.07.025},
    issn = {00191035},
    keywords = {Infrared observations, Prebiotic chemistry, Titan, atmosphere}
}

@article{Hidayat1997,
    title = {{Millimeter and Submillimeter Heterodyne Observations of Titan : Retrieval of the Vertical Profile of HCN and the 12 C / 13 C Ratio}},
    year = {1997},
    author = {Hidayat, T and Marten, A and B{\'{e}}zard, B. and Gautier, D. and Owen, T. C. and Matthews, H. E. and Paubert, G.},
    pages = {170--182},
    volume = {182}
}

@article{Encrenaz1996,
    title = {{Millimeter Spectroscopy of Uranus and Neptune : Constraints on CO and PH 3 Tropospheric Abundances}},
    year = {1996},
    journal = {Icarus},
    author = {Encrenaz, T. and Serabyn, E. and Weisstein, E. W.},
    pages = {616--624},
    volume = {624},
    doi = {10.1006/icar.1996.0235},
    issn = {00191035}
}

@misc{Winglee2000,
    title = {{Mini-magnetospheric plasma propulsion: Tapping energy of the solar wind for spacecraft propulsion}},
    year = {2000},
    author = {Winglee, R. M. and Slough, J. and Ziemba, T. and Goodson, A.}
}

@article{Stempel2005,
    title = {{Model constraints on the opening rates of bands on Europa}},
    year = {2005},
    journal = {Icarus},
    author = {Stempel, Michelle M. and Barr, Amy C. and Pappalardo, Robert T.},
    number = {2},
    pages = {297--304},
    volume = {177},
    doi = {10.1016/j.icarus.2005.03.025},
    issn = {00191035},
    keywords = {Europa, Geological processes, Geophysics, Satellites of Jupiter, Tectonics}
}

@article{Keller1998,
    title = {{Model of Titan's ionosphere with detailed hydrocarbon ion chemistry}},
    year = {1998},
    journal = {Planet. Space Sci.},
    author = {Keller, C. N. and Anicich, V. G. and Cravens, T. E.},
    pages = {1157--1174},
    volume = {46},
    isbn = {0032-0633},
    doi = {Doi: 10.1016/s0032-0633(98)00053-1},
    issn = {00320633}
}

@article{Cravens2009,
    title = {{Model-data comparisons for Titan’s nightside ionosphere}},
    year = {2009},
    journal = {Icarus},
    author = {Cravens, T. E. and Robertson, I. P. and Jr, J H Waite and Yelle, R V and Vuitton, V and Coates, A J and Wahlund, J and Agren, K and Richard, M S and Haye, V De La and Wellbrock, A and Neubauer, F M},
    number = {1},
    pages = {174--188},
    volume = {199},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2008.09.005},
    doi = {10.1016/j.icarus.2008.09.005},
    issn = {0019-1035}
}

@article{Carrasco2007b,
    title = {{Modeling of branching ratio uncertainty in chemical networks by dirichlet distributions}},
    year = {2007},
    journal = {Journal of Physical Chemistry A},
    author = {Carrasco, N. and Pernot, P.},
    number = {18},
    pages = {3507--3512},
    volume = {111},
    isbn = {1089-5639 (Print){\textbackslash}n1089-5639 (Linking)},
    doi = {10.1021/jp067306y},
    issn = {10895639},
    pmid = {17439103}
}

@article{Wahr2009,
    title = {{Modeling stresses on satellites due to nonsynchronous rotation and orbital eccentricity using gravitational potential theory}},
    year = {2009},
    journal = {Icarus},
    author = {Wahr, John and Selvans, Zane A. and Mullen, McCall E. and Barr, Amy C. and Collins, Geoffrey C. and Selvans, Michelle M. and Pappalardo, Robert T.},
    number = {1},
    pages = {188--206},
    volume = {200},
    isbn = {00191035},
    doi = {10.1016/j.icarus.2008.11.002},
    issn = {00191035},
    keywords = {Europa, Geophysics, Satellites, Tectonics, Tides, general, solid body}
}

@article{Wahr2009a,
    title = {{Modeling stresses on satellites due to nonsynchronous rotation and orbital eccentricity using gravitational potential theory}},
    year = {2009},
    journal = {Icarus},
    author = {Wahr, John and Selvans, Zane A. and Mullen, McCall E. and Barr, Amy C. and Collins, Geoffrey C. and Selvans, Michelle M. and Pappalardo, Robert T.},
    number = {1},
    pages = {188--206},
    volume = {200},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2008.11.002},
    isbn = {00191035},
    doi = {10.1016/j.icarus.2008.11.002},
    issn = {00191035},
    keywords = {Europa, Geophysics, Satellites, Tectonics, Tides, general, solid body}
}

@article{Barth2017,
    title = {{Modeling survey of ices in Titan's stratosphere}},
    year = {2017},
    journal = {Planetary and Space Science},
    author = {Barth, Erika L.},
    number = {January},
    pages = {20--31},
    volume = {137},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2017.01.003},
    isbn = {3035469687},
    doi = {10.1016/j.pss.2017.01.003},
    issn = {00320633},
    keywords = {Atmosphere, Condensation, Hydrocarbons, Ices, Titan}
}

@article{Turc2014,
    title = {{Modelling Ganymede ’ s neutral environment : A 3D test-particle simulation}},
    year = {2014},
    journal = {ICARUS},
    author = {Turc, L and Leclercq, L and Leblanc, F and Modolo, R and Chaufray, J},
    pages = {157--169},
    volume = {229},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.11.005},
    doi = {10.1016/j.icarus.2013.11.005},
    issn = {0019-1035}
}

@article{Tokano2001,
    title = {{Modelling of thunderclouds and lightning generation on Titan}},
    year = {2001},
    journal = {Planetary and Space Science},
    author = {Tokano, T. and Molina-Cuberos, G. J. and Lammer, H. and Stumptner, W.},
    number = {6},
    pages = {539--560},
    volume = {49},
    doi = {10.1016/S0032-0633(00)00170-7},
    issn = {00320633}
}

@article{Lee2015,
    title = {{Modelling the local and global cloud formation on HD 189733b}},
    year = {2015},
    journal = {Astronomy {\&} Astrophysics},
    author = {Lee, G and Juncher, D},
    pages = {1--23},
    volume = {A12},
    doi = {10.1051/0004-6361/201525982},
    issn = {0004-6361},
    arxivId = {arXiv:1505.06576v1},
    keywords = {atmospheres, hd 189733b, individual, methods, planets and satellites}
}

@article{CunhaMiranda2016,
    title = {{Molecular Isomer Identification of Titan ' s Tholins Organic Aerosols by Photoelectron / photoion Coincidence Spectroscopy Coupled to VUV Synchrotron Radiation Molecular Isomer Identification of Titan ’ s Tholins Organic Aerosols by Photoelectron / Photoi}},
    year = {2016},
    journal = {The journal of physical chemistry. A},
    author = {Cunha De Miranda, Barbara and Garcia, Gustavo A and Gaie-levrel, Francois and Mahjoub, Ahmed and Gautier, Thomas and Fleury, Benjamin and Nahon, Laurent and Pernot, Pascal and Carrasco, Nathalie},
    doi = {10.1021/acs.jpca.6b03346}
}

@article{Stevens2015,
    title = {{Molecular nitrogen and methane density retrievals from Cassini UVIS dayglow observations of Titan's upper atmosphere}},
    year = {2015},
    journal = {Icarus},
    author = {Stevens, Michael H. and Evans, J. Scott and Lumpe, Jerry and Westlake, Joseph H. and Ajello, Joseph M. and Bradley, E. Todd and Esposito, Larry W.},
    pages = {301--312},
    volume = {247},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.10.008},
    doi = {10.1016/j.icarus.2014.10.008},
    issn = {10902643},
    keywords = {Aeronomy, Atmospheres, composition, Spectroscopy, Titan, atmosphere}
}

@article{Fukuzawa1997,
    title = {{Molecular Orbital Study of Neutral‐Neutral Reactions concerning HC3N Formation in Interstellar Space}},
    year = {1997},
    journal = {The Astrophysical Journal},
    author = {Fukuzawa, Kaori and Osamura, Yoshihiro},
    number = {1},
    pages = {113--121},
    volume = {489},
    url = {http://stacks.iop.org/0004-637X/489/i=1/a=113},
    doi = {10.1086/304782},
    issn = {0004-637X},
    arxivId = {https://www.mendeley.com/research/molecular-orbital-study-neutralneutral-reactions-concerning-hc-3-n-formation-interstellar-space/?utm{\_}source=desktop{\&}utm{\_}medium=1.15.3{\&}utm{\_}campaign=open{\_}catalog{\&}userDocumentId={\{}3495e5e3-b7df-4875-9368-b9a3712e722c{\}}}
}

@article{Swain2009a,
    title = {{MOLECULAR SIGNATURES IN THE NEAR-INFRARED DAYSIDE SPECTRUM OF HD 189733b}},
    year = {2009},
    journal = {The Astrophysical Journal},
    author = {Swain, M. R. and Vasisht, G. and Tinetti, G. and Bouwman, J. and Chen, Pin and Yung, Y. and Deming, D. and Deroo, P.},
    number = {2},
    pages = {L114-L117},
    volume = {690},
    url = {http://arxiv.org/abs/0812.1844%5Cnhttp://stacks.iop.org/1538-4357/690/i=2/a=L114?key=crossref.abe9d068ddc0057ad0d6b3a3d82b63cd},
    doi = {10.1088/0004-637X/690/2/L114},
    issn = {0004-637X},
    arxivId = {0812.1844},
    keywords = {0004-637x, 10, 1088, 2, 2009 january 10, 690, a, all rights reserved, astrophysical journal, c 2009, doi, hd 189733b, l114, l117, molecular signatures in the, near-infrared dayside spectrum of, printed in the u, s, the american astronomical society}
}

@article{Sagan1960,
    title = {{Molecular Synthesis in Simulated Reducing Planetary Atmospheres}},
    year = {1960},
    journal = {AAS},
    author = {Sagan, C. and Miller, S.},
    pages = {6800}
}

@article{Dorn2011,
    title = {{Monomer abundance distribution patterns as a universal biosignature: Examples from terrestrial and digital life}},
    year = {2011},
    journal = {Journal of Molecular Evolution},
    author = {Dorn, Evan D. and Nealson, Kenneth H. and Adami, Christoph},
    number = {3},
    pages = {283--295},
    volume = {72},
    isbn = {1432-1432 (Electronic){\textbackslash}r0022-2844 (Linking)},
    doi = {10.1007/s00239-011-9429-4},
    issn = {00222844},
    pmid = {21253717},
    arxivId = {1101.1013},
    keywords = {Amino acids, Artificial life, Astrobiology, Carboxylic acids, Evolution, Exobiology, Meteorites}
}

@article{Cassidy2005,
    title = {{Monte Carlo model of sputtering and other ejection processes within a regolith}},
    year = {2005},
    journal = {Icarus},
    author = {Cassidy, T. A. and Johnson, R. E.},
    number = {2},
    pages = {499--507},
    volume = {176},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2005.02.013},
    issn = {00191035},
    keywords = {Atmospheres, composition, Moon, surface, Regoliths, Surfaces, satellites}
}

@article{Friedlaender2016,
    title = {{Multiple-stage decisions in a marine central-place forager Subject Category : Subject Areas : Author for correspondence :}},
    year = {2016},
    author = {Friedlaender, Ari S and Johnston, David W and Reny, B and Kaltenberg, Amanda and Goldbogen, Jeremy A and Stimpert, Alison K and Curtice, Corrie and Hazen, Elliott L and Halpin, Patrick N and Read, Andrew J and Douglas, P},
    doi = {10.1098/rsos.160043},
    issn = {20545703},
    pmid = {27293784},
    keywords = {behaviour, ecology, oceanography}
}

@article{Lavvas2015,
    title = {{N2 state population in Titan’s atmosphere}},
    year = {2015},
    journal = {Icarus},
    author = {Lavvas, P. and Yelle, R.V. and Heays, A.N. and Campbell, L. and Brunger, M.J. and Galand, M. and Vuitton, V.},
    month = {11},
    pages = {29--59},
    volume = {260},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103515002778},
    doi = {10.1016/j.icarus.2015.06.033},
    issn = {00191035},
    keywords = {Aeronomy, Atmospheres, chemistry, Titan, atmosphere, Ultraviolet observations}
}

@article{Johnson2017,
    title = {{Nanograin Density Outside Saturn’s A Ring}},
    year = {2017},
    journal = {The Astrophysical Journal},
    author = {Johnson, Robert E. and Tseng, Wei-Lin and Elrod, M. K. and Persoon, A. M.},
    number = {1},
    pages = {L6},
    volume = {834},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/2041-8205/834/i=1/a=L6?key=crossref.700a8566324e7a06897533dade9d4031},
    doi = {10.3847/2041-8213/834/1/L6},
    issn = {2041-8213},
    keywords = {individual, planets and satellites, planets and satellites: individual (Saturn), planets and satellites: rings, rings, saturn}
}

@article{Lopes2016,
    title = {{Nature, distribution, and origin of Titan's Undifferentiated Plains}},
    year = {2016},
    journal = {Icarus},
    author = {Lopes, Rosaly M C and Malaska, M. J. and Solomonidou, A. and Le Gall, A. and Janssen, M. A. and Neish, C. D. and Turtle, E. P. and Birch, S. P D and Hayes, A. G. and Radebaugh, J. and Coustenis, A. and Schoenfeld, A. and Stiles, B. W. and Kirk, R. L. and Mitchell, K. L. and Stofan, E. R. and Lawrence, K. J.},
    number = {July 2013},
    pages = {162--182},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.11.034},
    doi = {10.1016/j.icarus.2015.11.034},
    issn = {10902643},
    keywords = {Infrared observations, Radar observations, Satellites, surface, Titan, Titan, surface}
}

@article{Grundy2004,
    title = {{Near-infrared spectral monitoring of Triton with IRTF/SpeX I: Establishing a baseline for rotational variability}},
    year = {2004},
    journal = {Icarus},
    author = {Grundy, W. M. and Young, L. A.},
    number = {2},
    pages = {455--465},
    volume = {172},
    doi = {10.1016/j.icarus.2004.07.013},
    issn = {00191035},
    keywords = {Ices, Infrared observations, Satellite surfaces, Satellites of Neptune, Volatile transport}
}

@article{Grundy2010,
    title = {{Near-infrared spectral monitoring of Triton with IRTF/SpeX II: Spatial distribution and evolution of ices}},
    year = {2010},
    journal = {Icarus},
    author = {Grundy, W. M. and Young, L. A. and Stansberry, J. A. and Buie, M. W. and Olkin, C. B. and Young, E. F.},
    number = {2},
    pages = {594--604},
    volume = {205},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.08.005},
    doi = {10.1016/j.icarus.2009.08.005},
    issn = {00191035},
    arxivId = {0908.2623},
    keywords = {Ices, Infrared observations, Neptune, Spectroscopy, Triton, satellites}
}

@article{Vuitton2009a,
    title = {{Negative ion chemistry in Titan's upper atmosphere}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Vuitton, V. and Lavvas, P. and Yelle, R. V. and Galand, M. and Wellbrock, A. and Lewis, G. R. and Coates, A. J. and Wahlund, J. E.},
    number = {13},
    pages = {1558--1572},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.04.004},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2009.04.004},
    issn = {00320633},
    keywords = {Atmospheres, Composition, Ionospheres, Organic chemistry, Titan}
}

@article{Shebanits2013,
    title = {{Negative ion densities in the ionosphere of Titan-Cassini RPWS/LP results}},
    year = {2013},
    journal = {Planetary and Space Science},
    author = {Shebanits, O. and Wahlund, J. E. and Mandt, K. and {\AA}gren, K. and Edberg, N. J.T. and Waite, J. H.},
    pages = {153--162},
    volume = {84},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2013.05.021},
    doi = {10.1016/j.pss.2013.05.021},
    issn = {00320633},
    keywords = {Cassini, Dust-plasma interaction, Ionospheric physics, Negative ions, Titan}
}

@article{Coates2010a,
    title = {{Negative ions at Titan and Enceladus: recent results}},
    year = {2010},
    journal = {Faraday Discussions},
    author = {Coates, Andrew J. and Wellbrock, Anne and Lewis, Gethyn R. and Jones, Geraint H. and Young, David T. and Crary, Frank J. and Waite, J. Hunter and Johnson, Robert E. and Hill, Thomas W. and Sittler Jr., Edward C.},
    pages = {293},
    volume = {147},
    url = {http://xlink.rsc.org/?DOI=c004700g},
    doi = {10.1039/c004700g},
    issn = {1359-6640},
    pmid = {21302552}
}

@article{Horvath2009,
    title = {{Negative ions formed in N 2 /CH 4 /Ar discharge – A simulation of Titan's atmosphere chemistry}},
    year = {2009},
    journal = {The European Physical Journal Applied Physics},
    author = {Horvath, G. and Aranda-Gonzalvo, Y. and Mason, N. J. and Zahoran, M. and Matejcik, S.},
    number = {1},
    pages = {13105},
    volume = {49},
    url = {http://www.epjap.org/10.1051/epjap/2009192},
    doi = {10.1051/epjap/2009192},
    issn = {1286-0042}
}

@article{Millar2017,
    title = {{Negative ions in space}},
    year = {2017},
    journal = {Chemical Reviews},
    author = {Millar, Thomas J. and Walsh, Catherine and Field, Thomas A.},
    number = {3},
    pages = {1765--1795},
    volume = {117},
    doi = {10.1021/acs.chemrev.6b00480},
    issn = {15206890},
    pmid = {28112897}
}

@article{Coates2010,
    title = {{Negative ions in the Enceladus plume}},
    year = {2010},
    journal = {Icarus},
    author = {Coates, A. J. and Jones, G. H. and Lewis, G. R. and Wellbrock, A. and Young, D. T. and Crary, F. J. and Johnson, R. E. and Cassidy, T. A. and Hill, T. W.},
    number = {2},
    pages = {618--622},
    volume = {206},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.07.013},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.07.013},
    issn = {00191035},
    keywords = {Aeronomy, Atmospheres, composition, Enceladus, Ionospheres, Saturn, magnetosphere}
}

@article{Masters2014,
    title = {{Neptune and triton: Essential pieces of the solar system puzzle}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Masters, A. and Achilleos, N. and Agnor, C. B. and Campagnola, S. and Charnoz, S. and Christophe, B. and Coates, A. J. and Fletcher, L. N. and Jones, G. H. and Lamy, L. and Marzari, F. and Nettelmann, N. and Ruiz, J. and Ambrosi, R. and Andre, N. and Bhardwaj, A. and Fortney, J. J. and Hansen, C. J. and Helled, R. and Moragas-Klostermeyer, G. and Orton, G. and Ray, L. and Reynaud, S. and Sergis, N. and Srama, R. and Volwerk, M.},
    number = {PA},
    pages = {108--121},
    volume = {104},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2014.05.008},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2014.05.008},
    issn = {00320633},
    keywords = {Neptune, Solar, System exploration, Triton}
}

@article{Agnor2006,
    title = {{Neptune's capture of its moon Triton in a binary-planet gravitational encounter.}},
    year = {2006},
    journal = {Nature},
    author = {Agnor, Craig B. and Hamilton, Douglas P.},
    number = {7090},
    pages = {192--194},
    volume = {441},
    url = {http://www.nature.com/doifinder/10.1038/nature04792%5Cnhttp://www.ncbi.nlm.nih.gov/pubmed/16688170},
    isbn = {0028-0836},
    doi = {10.1038/nature04792},
    issn = {1476-4687},
    pmid = {16688170}
}

@article{Goldreich1989,
    title = {{Neptune's Story}},
    year = {1989},
    journal = {Science},
    author = {Goldreich, P and Murray, N and Longaretti, P. Y. and Banfield, D},
    number = {4917},
    pages = {500--504},
    volume = {245}
}

@article{Hebrard2012,
    title = {{Neutral production of hydrogen isocyanide (HNC) and hydrogen cyanide (HCN) in Titan’s upper atmosphere}},
    year = {2012},
    journal = {Astronomy {\&} Astrophysics},
    author = {H{\'{e}}brard, E. and Dobrijevic, M. and Loison, J. C. and Bergeat, A. and Hickson, K. M.},
    pages = {A21},
    volume = {541},
    url = {http://www.aanda.org/10.1051/0004-6361/201218837},
    doi = {10.1051/0004-6361/201218837},
    issn = {0004-6361},
    keywords = {atmospheres, composition, individual, planets and satellites, titan}
}

@article{Kammer2017,
    title = {{New Horizons Upper Limits on O{\$}{\_}2{\$} in Pluto's Present Day Atmosphere}},
    year = {2017},
    author = {Kammer, J. A. and Stern, S. A. and Gladstone, G. R. and Young, L. A. and Olkin, C. B. and Steffl, A. and Weaver, H. A. and Ennico, K.},
    pages = {0--4},
    url = {http://arxiv.org/abs/1706.04232},
    arxivId = {1706.04232},
    keywords = {atmospheres, individual, planets and satellites, pluto}
}

@article{Pereira2010,
    title = {{New Insight into the Formation of Nitrogen Sulfide : A Quantum Chemical Study}},
    year = {2010},
    author = {Pereira, Priscila S S and Macedo, Luiz G M and Pimentel, S},
    pages = {509--515}
}

@article{Noyelles2014,
    title = {{New insights on Titan's interior from its obliquity}},
    year = {2014},
    journal = {Arxiv},
    author = {{Noyelles} and {Nimmo}},
    arxivId = {1403.2276},
    keywords = {Titanobliquity}
}

@article{Marten2002,
    title = {{New Millimeter Heterodyne Observations of Titan: Vertical Distributions of Nitriles HCN, HC3N, CH3CN, and the Isotopic Ratio 15N/14N in Its Atmosphere}},
    year = {2002},
    journal = {Icarus},
    author = {Marten, A and Hidayat, T and Biraud, Y and Moreno, R},
    number = {2},
    pages = {532--544},
    volume = {158},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103502968971},
    isbn = {0019-1035},
    doi = {10.1006/icar.2002.6897},
    issn = {00191035},
    keywords = {Titan, atmospheres, atmospheres, composition, radio observations, radio observations}
}

@article{Vervack2004,
    title = {{New perspectives on Titan's upper atmosphere from a reanalysis of the Voyager 1 UVS solar occultations}},
    year = {2004},
    journal = {Icarus},
    author = {Vervack, Ronald J. and Sandel, Bill R. and Strobel, Darrell F.},
    number = {1},
    pages = {91--112},
    volume = {170},
    doi = {10.1016/j.icarus.2004.03.005},
    issn = {00191035},
    keywords = {Aeronomy, Atmospheres, Occultations, Structure, Titan}
}

@article{Yair2012,
    title = {{New results on planetary lightning}},
    year = {2012},
    journal = {Advances in Space Research},
    author = {Yair, Yoav},
    number = {3},
    pages = {293--310},
    volume = {50},
    publisher = {COSPAR},
    url = {http://dx.doi.org/10.1016/j.asr.2012.04.013},
    doi = {10.1016/j.asr.2012.04.013},
    issn = {02731177},
    keywords = {Discharge processes, Electromagnetic radiation, Lightning, Planetary atmospheres, Sprites}
}

@article{Gall,
    title = {{New thermal anomalies in the subsurface of Enceladus ’ South Polar Terrain}},
    journal = {Nature Astronomy},
    author = {Gall, A Le and Leyrat, C and Janssen, M A and Choblet, G and Tobie, G and Bourgeois, O and Lucas, A},
    pages = {1--20}
}

@article{Thiemann2012,
    title = {{Nitric Acid , Nitrous Acid , and Nitrogen Oxides}},
    year = {2012},
    journal = {Ullmann's Encyclopedia of Industrial Chemistry, Vol. 24},
    author = {Thiemann, Michael and Scheibler, Erich and Wiegand, Karl Wilhelm},
    number = {Ieo 2003},
    pages = {177--223},
    volume = {2003},
    isbn = {9783527306732},
    doi = {10.1002/14356007.a17}
}

@article{Gautier2011,
    title = {{Nitrile gas chemistry in Titan's atmosphere}},
    year = {2011},
    journal = {Icarus},
    author = {Gautier, Thomas and Carrasco, Nathalie and Buch, Arnaud and Szopa, Cyril and Sciamma-O'Brien, Ella and Cernogora, Guy},
    number = {2},
    pages = {625--635},
    volume = {213},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2011.04.005},
    issn = {00191035},
    keywords = {Atmospheres, Chemistry, Experimental techniques, Prebiotic chemistry, Saturn, Satellites}
}

@article{Strobel1991,
    title = {{Nitrogen Airglow Sources: Comparison of Triton, Titan, and Earth}},
    year = {1991},
    journal = {Geophysical Research Letters},
    author = {Strobel, D. F. and Meier, R. R. and Strickland, D. J.},
    number = {24},
    pages = {999--1000},
    volume = {20}
}

@article{Trainer2012,
    title = {{Nitrogen Incorporation in CH <sub>4</sub> -N <sub>2</sub> Photochemical Aerosol Produced by Far Ultraviolet Irradiation}},
    year = {2012},
    journal = {Astrobiology},
    author = {Trainer, Melissa G. and Jimenez, Jose L. and Yung, Yuk L. and Toon, Owen B. and Tolbert, Margaret A.},
    number = {4},
    pages = {315--326},
    volume = {12},
    url = {http://online.liebertpub.com/doi/abs/10.1089/ast.2011.0754},
    isbn = {1531-1074; 1557-8070},
    doi = {10.1089/ast.2011.0754},
    issn = {1531-1074},
    pmid = {22519972}
}

@article{Gautier2014,
    title = {{Nitrogen incorporation in titan's tholins inferred by high resolution orbitrap mass spectrometry and gas chromatography-mass spectrometry}},
    year = {2014},
    journal = {Earth and Planetary Science Letters},
    author = {Gautier, Thomas and Carrasco, Nathalie and Schmitz-Afonso, Isabelle and Touboul, David and Szopa, Cyril and Buch, Arnaud and Pernot, Pascal},
    pages = {33--42},
    volume = {404},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.epsl.2014.07.011},
    isbn = {0012-821X},
    doi = {10.1016/j.epsl.2014.07.011},
    issn = {0012821X},
    keywords = {Aerosols, High resolution mass spectrometry, Nitrogen, Tholins, Titan's atmosphere}
}

@article{Raulin1982,
    title = {{No Title}},
    year = {1982},
    author = {Raulin, Francois and Mourey, Didier and Toupance, Gerard},
    number = {October 1981},
    pages = {267--279},
    volume = {12}
}

@article{Yelle1991,
    title = {{Non-LTE Models of Titan's Upper Atmosphere}},
    year = {1991},
    journal = {The Astrophysical Journal},
    author = {Yelle, R.V.}
}

@article{Shoji2014,
    title = {{Non-steady state tidal heating of Enceladus}},
    year = {2014},
    journal = {Icarus},
    author = {Shoji, D. and Hussmann, H. and Sohl, F. and Kurita, K.},
    pages = {75--85},
    volume = {235},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.03.006},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.03.006},
    issn = {10902643},
    keywords = {Enceladus, Satellites, dynamics, Saturn, Tides, solid body}
}

@article{Greenberg,
    title = {{Non-synchronous Rotation of Europa}},
    author = {Greenberg, R and Hoppa, G V and Tufts, B R and Geissler, P},
    pages = {11--12},
    volume = {0092}
}

@article{Gao2013,
    title = {{Nonhydrostatic effects and the determination of icy satellites' moment of inertia}},
    year = {2013},
    journal = {Icarus},
    author = {Gao, Peter and Stevenson, David J.},
    number = {2},
    pages = {1185--1191},
    volume = {226},
    doi = {10.1016/j.icarus.2013.07.034},
    issn = {00191035},
    arxivId = {1309.1205},
    keywords = {Callisto, Enceladus, Ganymede, Interiors}
}

@article{Kattenhorn2002,
    title = {{Nonsynchronous Rotation Evidence and Fracture History in the Bright Plains Region, Europa}},
    year = {2002},
    journal = {Icarus},
    author = {Kattenhorn, Simon a},
    number = {2},
    pages = {490--506},
    volume = {157},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103502968259},
    isbn = {00191035},
    doi = {10.1006/icar.2002.6825},
    issn = {00191035},
    keywords = {europa, geological processes, satellite, surfaces}
}

@article{Brien2005,
    title = {{Numerical calculations of the longevity of impact oases on Titan}},
    year = {2005},
    author = {Brien, David P O and Lorenz, Ralph D and Lunine, Jonathan I},
    pages = {243--253},
    volume = {173},
    doi = {10.1016/j.icarus.2004.08.001},
    keywords = {cratering, impact processes, prebiotic chemistry, prebiotic environments, titan}
}

@article{Broks2005,
    title = {{Numerical investigation of the discharge characteristics of the pulsed discharge nozzle}},
    year = {2005},
    journal = {Physical Reviews},
    author = {Broks, B H P and Brok, W J M and Remy, J and Mullen, J J A M Van Der},
    pages = {1--8},
    doi = {10.1103/PhysRevE.71.036409}
}

@article{Abramov2008,
    title = {{Numerical modeling of endogenic thermal anomalies on Europa}},
    year = {2008},
    journal = {Icarus},
    author = {Abramov, Oleg and Spencer, John R.},
    number = {1},
    pages = {378--385},
    volume = {195},
    doi = {10.1016/j.icarus.2007.11.027},
    issn = {00191035},
    keywords = {Europa, Geological processes, Ices, Thermal histories, Volcanism}
}

@article{Stamnes1988,
    title = {{Numerically Stable Algorithm for Discrete-Ordinate-Method Radiative-Transfer in Multiple-Scattering and Emitting Layered Media}},
    year = {1988},
    journal = {Applied Optics},
    author = {Stamnes, K and Tsay, S C and Wiscombe, W and Jayaweera, K},
    number = {12},
    pages = {2502--2509},
    volume = {27}
}

@article{Chen2011,
    title = {{Obliquity tides do not significantly heat Enceladus}},
    year = {2011},
    journal = {Icarus},
    author = {Chen, E. M A and Nimmo, F.},
    number = {2},
    pages = {779--781},
    volume = {214},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.06.007},
    doi = {10.1016/j.icarus.2011.06.007},
    issn = {00191035},
    keywords = {Enceladus, Rotational dynamics, Saturn, Satellites}
}

@article{Rodriguez2010,
    title = {{Observational evidence for active dust storms on Titan at equinox}},
    year = {2010},
    author = {Rodriguez, S and Mou{\'{e}}lic, S Le and Barnes, J W and Kok, J F and Rafkin, S C R and Lorenz, R D and Charnay, B and Radebaugh, J and Narteau, C and Cornet, T and Bourgeois, O and Lucas, A and Rannou, P and Griffith, C A},
    doi = {10.1038/s41561-018-0233-2}
}

@article{Sola1908,
    title = {{Observations des satellites principaux de Jupiter et de Titan.}},
    year = {1908},
    journal = {Astronomische Nachrichten},
    author = {Sol{\'{a}} Comas, José},
    number = {18},
    pages = {4290},
    volume = {179}
}

@article{Mcgrath1978,
    title = {{Observations of Europa’s Tenuous Atmosphere}},
    year = {1978},
    author = {Mcgrath, M a and Hansen, C J and Hendrix, a R},
    pages = {485--505}
}

@article{Crossfield2015,
    title = {{Observations of Exoplanet Atmospheres}},
    year = {2015},
    journal = {Publications of the Astronomical Society of the Pacific},
    author = {Crossfield, Ian J. M.},
    number = {956},
    pages = {941--960},
    volume = {127},
    url = {http://arxiv.org/pdf/1507.03966v3.pdf%5Cnhttp://arxiv.org/abs/1507.03966%5Cnhttp://iopscience.iop.org/article/10.1086/683115%5Cnhttp://arxiv.org/pdf/1507.03966.pdf},
    doi = {10.1086/683115},
    issn = {00046280},
    arxivId = {1507.03966},
    keywords = {127, 2, 2015, 2015 october, 941, 960, a, all rights reserved, blications of the a, c rossfield 1, ft version july 22, i an j, m, observations of exoplanet atmospheres, printed in u, s, stronomical s ociety of, the astronomical society of, the p acific, the pacific}
}

@article{Snell1981,
    title = {{OBSERVATIONS OF HC3N, HC5N, AND HC7N IN MOLECULAR CLOUDS}},
    year = {1980},
    author = {Snell, Ronald L and Schloerb, F Peter and Young, Judith S and Hjalmarson, A and Friberg, P.}
}

@article{Brown2003,
    title = {{Observations with the Visual and Infrared Mapping Spectrometer (VIMS) during Cassini's flyby of Jupiter}},
    year = {2003},
    journal = {Icarus},
    author = {Brown, R. H. and Baines, K. H. and Bellucci, G. and Bibring, J. P. and Buratti, B. J. and Capaccioni, F. and Cerroni, P. and Clark, R. N. and Coradini, A. and Cruikshank, D. P. and Drossart, P. and Formisano, V. and Jaumann, R. and Langevin, Y. and Matson, D. L. and McCord, T. B. and Mennella, V. and Nelson, R. M. and Nicholson, P. D. and Sicardy, B. and Sotin, C. and Amici, S. and Chamberlain, M. A. and Filacchione, G. and Hansen, G. and Hibbitts, K. and Showalter, M.},
    number = {2},
    pages = {461--470},
    volume = {164},
    isbn = {00191035},
    doi = {10.1016/S0019-1035(03)00134-9},
    issn = {00191035},
    keywords = {Cassini mission, Jovian satellites, Jupiter, Jupiter's ring, Planetary atmospheres, Planetary surfaces, Spectroscopy}
}

@article{Bertrand2016,
    title = {{Observed glacier and volatile distribution on Pluto from atmosphere–topography processes}},
    year = {2016},
    journal = {Nature},
    author = {Bertrand, Tanguy and Forget, François},
    pages = {1--8},
    publisher = {Nature Publishing Group},
    url = {http://www.nature.com/doifinder/10.1038/nature19337},
    doi = {10.1038/nature19337},
    issn = {0028-0836}
}

@article{Morley2017,
    title = {{Observing the Atmospheres of Known Temperate Earth-sized Planets with JWST}},
    year = {2017},
    author = {Morley, Caroline V. and Kreidberg, Laura and Rustamkulov, Zafar and Robinson, Tyler and Fortney, Jonathan J.},
    pages = {1--19},
    url = {http://arxiv.org/abs/1708.04239},
    arxivId = {1708.04239},
    keywords = {atmospheres, gj 1132b, individual, lhs 1140b, planets and satellites, terrestrial planets, trappist-1b, trappist-1c, trappist-1d, trappist-1e, trappist-1f, trappist-1g, trappist-1h}
}

@article{Matsuyama2018,
    title = {{Ocean tidal heating in icy satellites with solid shells}},
    year = {2018},
    author = {Matsuyama, Isamu and Beuthe, Mikael and Hay, Hamish C. F. C. and Nimmo, Francis and Kamata, Shunichi},
    url = {http://arxiv.org/abs/1804.07727},
    arxivId = {1804.07727},
    keywords = {dynamics, enceladus, europa, rotational dynamics, satellites, solid body, tides}
}

@article{Lunine2017a,
    title = {{Ocean worlds exploration}},
    year = {2017},
    journal = {Acta Astronautica},
    author = {Lunine, Jonathan I.},
    pages = {123--130},
    volume = {131},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.actaastro.2016.11.017},
    doi = {10.1016/j.actaastro.2016.11.017},
    issn = {00945765},
    keywords = {Exobiology, Jupiter, Moons, Planetary exploration, Saturn}
}

@article{Lunine2017,
    title = {{Ocean worlds exploration}},
    year = {2017},
    journal = {Acta Astronautica},
    author = {Lunine, Jonathan I.},
    number = {November 2016},
    pages = {123--130},
    volume = {131},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.actaastro.2016.11.017},
    isbn = {00945765},
    doi = {10.1016/j.actaastro.2016.11.017},
    issn = {00945765},
    keywords = {Exobiology, Jupiter, Moons, Planetary exploration, Saturn}
}

@article{Nimmo2016,
    title = {{Ocean worlds in the outer solar system}},
    year = {2016},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Nimmo, F. and Pappalardo, R. T.},
    number = {8},
    pages = {1378--1399},
    volume = {121},
    isbn = {2169-9100},
    doi = {10.1002/2016JE005081},
    issn = {21699100},
    keywords = {Callisto, Enceladus, Europa, Ganymede, Pluto, Titan}
}

@article{Auclair-Desrotour2018,
    title = {{Oceanic tides from Earth-like to ocean planets}},
    year = {2018},
    journal = {Astronomy {\&} Astrophysics},
    author = {Auclair-Desrotour, P and Mathis, S and Laskar, J and Leconte, J},
    number = {Laplace 1798},
    url = {https://arxiv.org/pdf/1801.08742.pdf},
    arxivId = {1801.08742},
    keywords = {oceans – planets and satellites, terrestrial planets}
}

@article{Agren2007,
    title = {{On magnetospheric electron impact ionisation and dynamics in Titan's ram-side and polar ionosphere–a Cassini case study}},
    year = {2007},
    journal = {Annales Geophysicae},
    author = {{\AA}gren, K. and Wahlund, J.-E. and Modolo, R. and Lummerzheim, D. and Galand, M. and M{\"{u}}ller-Wodarg, I. and Canu, P. and Kurth, W.S. and Cravens, T.E. and Yelle, R.V. and Waite, J.H. and Coates, A.J. and Lewis, G.R. and Young, D.T. and Bertucci, C. and Dougherty, M.K.},
    number = {11},
    pages = {2359--2369},
    volume = {25},
    url = {http://hal.archives-ouvertes.fr/hal-00330154/},
    doi = {10.5194/angeo-25-2359-2007},
    issn = {1432-0576},
    keywords = {ionosphere, magnetosphere-ionosphere interactions, magnetospheric physics, planetary ionospheres, plasma, temperature and density}
}

@article{Wahlund2009,
    title = {{On the amount of heavy molecular ions in Titan’s ionosphere}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Wahlund, J.‐E. and Galand, M. and Yelle, R V and Crary, F J and Mandt, K and Magee, B and Andr, M and Jr, J H Waite and Young, D T and Coates, A J and Garnier, P and Agren, K and Vuitton, V and Gurnett, D A and Kurth, W S},
    pages = {1857--1865},
    volume = {57},
    doi = {10.1016/j.pss.2009.07.014}
}

@article{Ivory1842,
    title = {{On the constitution of the atmosphere}},
    year = {1842},
    journal = {Philosophical Magazine Series 3},
    author = {Ivory, James},
    number = {130},
    pages = {197--201},
    volume = {20},
    url = {http://www.tandfonline.com/doi/abs/10.1080/14786444208650553},
    doi = {10.1080/14786444208650553},
    issn = {1941-5966}
}

@article{Fortenberry2017,
    title = {{On the Detectability of the {\$}{\{}{\textbackslash}tilde{\{}{\{}{\textbackslash}boldsymbol{\{}X{\}}{\}}{\}}{\}}{\^{}}{\{}2{\}}{\{}{\textbackslash}boldsymbol{\{}A{\}}{\}}{\^{}}{\{}{\textbackslash}prime{\textbackslash}prime{\}} {\$} HSS, HSO, and HOS Radicals in the Interstellar Medium}},
    year = {2017},
    journal = {The Astrophysical Journal},
    author = {Fortenberry, Ryan C. and Francisco, Joseph S.},
    number = {2},
    pages = {243},
    volume = {835},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/835/i=2/a=243?key=crossref.8de25b9a058eb5d1d65fa7254053708f},
    doi = {10.3847/1538-4357/aa582d},
    issn = {1538-4357},
    keywords = {ISM: lines and bands, ISM: molecules, infrared, infrared: ISM, ism, lines and bands, molecular data, molecular processes, molecules, radio lines: ISM}
}

@article{Milhaud1975,
    title = {{On the formation of CH<sub>4</sub><sup>+</sup>, CH<sub>3</sub><sup>+</sup>, CH<sub>2</sub><sup>+</sup>, CH<sup>+</sup> and C<sup>+</sup> secondary ions in methane}},
    year = {1975},
    journal = {International Journal of Mass Spectrometry and Ion Physics},
    author = {Milhaud, J.},
    number = {3},
    pages = {327--337},
    volume = {16},
    url = {http://www.sciencedirect.com/science/article/pii/0020738175870306%5Cnhttp://www.sciencedirect.com/science/article/pii/0020738175870306/pdf?md5=912592811c2ff301df15acb0dd2fcbd9&pid=1-s2.0-0020738175870306-main.pdf},
    doi = {10.1016/0020-7381(75)87030-6},
    issn = {0020-7381}
}

@article{Huybrighs2017,
    title = {{On the in-situ detectability of Europa's water vapour plumes from a flyby mission}},
    year = {2017},
    journal = {Icarus},
    author = {Huybrighs, Hans L.F. and Futaana, Yoshifumi and Barabash, Stanislav and Wieser, Martin and Wurz, Peter and Krupp, Norbert and Glassmeier, Karl Heinz and Vermeersen, Bert},
    number = {November 2014},
    pages = {270--280},
    volume = {289},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.10.026},
    isbn = {4955138497},
    doi = {10.1016/j.icarus.2016.10.026},
    issn = {10902643},
    arxivId = {1704.00912}
}

@article{Reynolds1979,
    title = {{On the Internal Structure of the Major Satellites of the Outer Planets}},
    year = {1979},
    journal = {Geophysical Research Letters},
    author = {Reynolds, Ray T and Cassen, Patrick M},
    number = {2},
    pages = {121--124},
    volume = {6}
}

@article{Agren2009,
    title = {{On the ionospheric structure of Titan}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {{\AA}gren, K. and Wahlund, J and Garnier, P and Modolo, R and Cui, J and Galand, M and Mu, I},
    pages = {1821--1827},
    volume = {57},
    doi = {10.1016/j.pss.2009.04.012}
}

@article{VanHoolst2013,
    title = {{On the librations and tides of large icy satellites}},
    year = {2013},
    journal = {Icarus},
    author = {Van Hoolst, Tim and Baland, Rose Marie and Trinh, Antony},
    number = {1},
    pages = {299--315},
    volume = {226},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.05.036},
    doi = {10.1016/j.icarus.2013.05.036},
    issn = {00191035},
    keywords = {Callisto, Europa, Ganymede, Rotational dynamics, Tides, solid body, Titan}
}

@article{Schenk2007,
    title = {{On the negligible surface age of Triton}},
    year = {2007},
    journal = {Icarus},
    author = {Schenk, Paul M. and Zahnle, Kevin},
    number = {1},
    pages = {135--149},
    volume = {192},
    doi = {10.1016/j.icarus.2007.07.004},
    issn = {00191035},
    keywords = {Comets, Cratering, Neptune, Triton, satellites}
}

@article{Jankowski1989,
    title = {{On the obliquity and tidal heating of Triton}},
    year = {1989},
    journal = {Icarus},
    author = {Jankowski, David G. and Chyba, Christopher F. and Nicholson, Philip D.},
    number = {1},
    pages = {211--219},
    volume = {80},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(89)90169-3},
    issn = {10902643}
}

@article{Leblanc2017,
    title = {{On the orbital variability of Ganymede’s atmosphere}},
    year = {2017},
    journal = {Icarus},
    author = {Leblanc, F and Oza, A V and Leclercq, L and Schmidt, C and Cassidy, T and Modolo, R and Chaufray, J Y and Johnson, R E},
    pages = {185--198},
    volume = {293},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2017.04.025},
    doi = {10.1016/j.icarus.2017.04.025},
    issn = {0019-1035}
}

@article{McKinnon1984,
    title = {{On the origin of Triton and Pluto}},
    year = {1984},
    journal = {Nature Letters},
    author = {McKinnon, William B.}
}

@article{Rosenberg2009,
    title = {{On the possibility of ion-acoustic instability in Titan’s ionosphere}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Rosenberg, M Ã and Shukla, P K},
    number = {14-15},
    pages = {2030--2031},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.09.004},
    doi = {10.1016/j.pss.2009.09.004},
    issn = {0032-0633},
    keywords = {Aerosol, Ion-acoustic instability, Titan ionosphere}
}

@article{Trafton1972b,
    title = {{On the possible detection of H2 in titan's atmosphere}},
    year = {1972},
    journal = {The Astrophysical Journal},
    author = {Trafton, L.},
    number = {175},
    pages = {285--293},
    volume = {5},
    url = {http://articles.adsabs.harvard.edu/cgi-bin/nph-iarticle_query?bibcode=1972ApJ...175..285T&db_key=AST&page_ind=0&data_type=GIF&type=SCREEN_VIEW&classic=YES},
    doi = {10.1086/151556},
    issn = {0004-637X}
}

@article{Dubois2017a,
    title = {{On the Presence of Aminomethyl (CH2NH2+) in Titan's Upper Atmosphere}},
    year = {2017},
    journal = {ALMA proposal},
    author = {Dubois, D. and Carrasco, N. and Sciamma-O’Brien, E. and Fortenberry, Ryan and Oza, A. and Thelen, A. and Desai, R.},
    pages = {14--17}
}

@article{Kislyakova2016,
    title = {{On the ultraviolet anomalies of the WASP-12 and HD 189733 systems: Trojan satellites as a plasma source}},
    year = {2016},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Kislyakova, K. G. and Pilat-Lohinger, E. and Funk, B. and Lammer, H. and Fossati, L. and Eggl, S. and Schwarz, R. and Boudjada, M. Y. and Erkaev, N. V.},
    number = {1},
    pages = {988--999},
    volume = {461},
    doi = {10.1093/mnras/stw1110},
    issn = {13652966},
    arxivId = {1605.02507},
    keywords = {Planet-star interactions, Planets and satellites: atmospheres, Planets and satellites: dynamical evolution and st, Planets and satellites: individual: HD 189733b, Planets and satellites: individual:WASP-12b, Stars: activity}
}

@article{Singh2015,
    title = {{On-sky demonstration of low-order wavefront sensing and control with focal plane phase mask coronagraphs}},
    year = {2015},
    journal = {Astronomical Society of the Pacific},
    author = {Singh, Garima and Lozi, Julien and Guyon, Olivier and Baudoz, Pierre and Jovanovic, Nemanja and Martinache, Frantz},
    number = {955},
    volume = {127},
    doi = {10.1086/682726},
    issn = {00046280},
    arxivId = {arXiv:1506.06298v1}
}

@article{Puhl-Quinn1995,
    title = {{One-Dimensional Hybrid Simulations of the Diamagnetic Cavity Boundary Region of Comet Halley}},
    year = {1995},
    journal = {Journal of Geophysical Research},
    author = {Puhl-Quinn, P and Cravens, T E},
    number = {A11},
    pages = {21631--21644},
    volume = {100},
    url = {http://www.agu.org/pubs/crossref/1995/95JA01820.shtml},
    doi = {10.1029/2002JA009622},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/95JA01820, doi:10.1029/9}
}

@article{Sciamma-OBrien2012,
    title = {{Optical constants from 370nm to 900nm of Titan tholins produced in a low pressure RF plasma discharge}},
    year = {2012},
    journal = {Icarus},
    author = {Sciamma-O'Brien, E. and Dahoo, P. R. and Hadamcik, E. and Carrasco, N. and Quirico, E. and Szopa, C. and Cernogora, G.},
    number = {1},
    pages = {353--363},
    volume = {218},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.12.014},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2011.12.014},
    issn = {00191035},
    keywords = {Photometry, Titan}
}

@article{Khare1984a,
    title = {{Optical constants of organic tholins produced in a simulated Titanian atmosphere: From soft x-ray to microwave frequencies}},
    year = {1984},
    journal = {Icarus},
    author = {Khare, B. N. and Sagan, Carl and Arakawa, E. T. and Suits, F. and Callcott, T. A. and Williams, M. W.},
    number = {1},
    pages = {127--137},
    volume = {60},
    doi = {10.1016/0019-1035(84)90142-8},
    issn = {10902643}
}

@article{Vinatier2012,
    title = {{Optical constants of Titan's stratospheric aerosols in the 70-1500cm -1 spectral range constrained by Cassini/CIRS observations}},
    year = {2012},
    journal = {Icarus},
    author = {Vinatier, Sandrine and Rannou, Pascal and Anderson, Carrie M. and B??zard, Bruno and De Kok, Remco and Samuelson, Robert E.},
    number = {1},
    pages = {5--12},
    volume = {219},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.02.009},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2012.02.009},
    issn = {00191035},
    keywords = {Atmospheres, composition, Spectroscopy, Titan, atmosphere}
}

@article{Cauley2015,
    title = {{Optical hydrogen absorption consistent with a thin bow shock leading the hot Jupiter HD 189733b}},
    year = {2015},
    author = {Cauley, P. Wilson and Redfield, Seth and Jensen, Adam G. and Barman, Travis and Endl, Michael and Cochran, William D.},
    pages = {10},
    url = {http://arxiv.org/abs/1507.05916},
    doi = {10.1088/0004-637X/810/1/13},
    issn = {15384357},
    arxivId = {1507.05916}
}

@article{Riedel1990,
    title = {{Optical Navigation During the Voyager Neptune Encounter}},
    year = {1990},
    journal = {AIAA paper},
    author = {Riedel, J E and Owen Jr, W M and Stuve, J A and Synnott, S P},
    url = {http://pdf.aiaa.org/GetFileGoogle.cfm?gID=65945&gTable=mtgpaper%5Cnpapers://23322e7b-a0cc-4788-a6e0-544263a1c348/Paper/p674},
    doi = {10.2514/6.1990-2877}
}

@article{Hadamcik2013,
    title = {{Optical properties of analogs of Titan's aerosols produced by dusty plasma}},
    year = {2013},
    journal = {Earth, Planets and Space},
    author = {Hadamcik, E. and Renard, J. -B. and Mahjoub, A. and Gautier, Thomas and Carrasco, N. and Cernogora, Guy and Szopa, C.},
    number = {10},
    pages = {1175--1184},
    volume = {65},
    url = {http://labs.adsabs.harvard.edu/adsabs/abs/2013EP%26S...65.1175H/},
    doi = {10.5047/eps.2013.05.019},
    issn = {13438832},
    keywords = {aerosol, light scattering, polarization, refractive indices, tholins, titan}
}

@article{Khare1994,
    title = {{Optical properties of poly-HCN and their astronomical applications.}},
    year = {1994},
    journal = {Canadian journal of chemistry},
    author = {Khare, B N and Sagan, C and Thompson, W R and Arakawa, E T and Meisse, C and Tuminello, P S},
    number = {9},
    pages = {678--694},
    volume = {72},
    doi = {10.1139/v94-093},
    issn = {0008-4042},
    pmid = {11540502}
}

@article{Lee2012,
    title = {{Optimal estimation retrievals of the atmospheric structure and composition of HD189733b from secondary eclipse spectroscopy}},
    year = {2012},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Lee, J. M. and Fletcher, L. N. and Irwin, P. G J},
    number = {1},
    pages = {170--182},
    volume = {420},
    isbn = {0035-8711},
    doi = {10.1111/j.1365-2966.2011.20013.x},
    issn = {00358711},
    arxivId = {1110.2934v2},
    keywords = {Methods: analytical, Planetary systems: individual: HD189733b, Planets and satellites: atmospheres, Radiative transfer}
}

@article{Hubbard1989,
    title = {{Optimized Jupiter, Saturn, and Uranus interior models}},
    year = {1989},
    journal = {Icarus},
    author = {Hubbard, W. B. and Marley, Mark S.},
    number = {1},
    pages = {102--118},
    volume = {78},
    isbn = {00191035},
    doi = {10.1016/0019-1035(89)90072-9},
    issn = {10902643}
}

@article{Sugla2013,
    title = {{Orbital and Structural Evolution of Triton Advisors : Saswata Hier-Majumder}},
    year = {2013},
    author = {Sugla, Rishi and Hamilton, Douglas and Leki, Vedran},
    number = {April}
}

@article{Roth2014,
    title = {{Orbital apocenter is not a sufficient condition for HST/STIS detection of Europa's water vapor aurora.}},
    year = {2014},
    journal = {Proceedings of the National Academy of Sciences of the United States of America},
    author = {Roth, Lorenz and Retherford, Kurt D and Saur, Joachim and Strobel, Darrell F and Feldman, Paul D and McGrath, Melissa A and Nimmo, Francis},
    number = {48},
    pages = {5123--32},
    volume = {111},
    url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=4260579&tool=pmcentrez&rendertype=abstract},
    doi = {10.1073/pnas.1416671111},
    issn = {1091-6490},
    pmid = {25404343},
    keywords = {Exobiology, Exobiology: methods, Extraterrestrial Environment, Hydrogen, Hydrogen: analysis, Hydrogen: chemistry, Ice, Jupiter, Oxygen, Oxygen: analysis, Oxygen: chemistry, Steam, Telescopes, Water, Water: analysis, Water: chemistry}
}

@article{Zhang2007,
    title = {{Orbital resonances in the inner neptunian system. I. The 2:1 Proteus-Larissa mean-motion resonance}},
    year = {2007},
    journal = {Icarus},
    author = {Zhang, Ke and Hamilton, Douglas P.},
    number = {2},
    pages = {386--399},
    volume = {188},
    doi = {10.1016/j.icarus.2006.12.002},
    issn = {00191035},
    keywords = {Neptune, Resonances, Satellites, Triton, dynamics, orbital, satellites}
}

@article{Zhang2008,
    title = {{Orbital resonances in the inner neptunian system. II. Resonant history of Proteus, Larissa, Galatea, and Despina}},
    year = {2008},
    journal = {Icarus},
    author = {Zhang, Ke and Hamilton, Douglas P.},
    number = {1},
    pages = {267--282},
    volume = {193},
    doi = {10.1016/j.icarus.2007.08.024},
    issn = {00191035},
    keywords = {Neptune, Resonances, Satellites, Triton, dynamics, orbital, satellites}
}

@article{Gavilan2018,
    title = {{Organic Aerosols in Anoxic and Oxic Atmospheres of Earth-like Exoplanets: VUV-MIR Spectroscopy of CHON Tholins}},
    year = {2018},
    journal = {The Astrophysical Journal},
    author = {Gavilan, Lisseth and Carrasco, Nathalie and Hoffmann, Søren Vrønning and Jones, Nykola C. and Mason, Nigel J.},
    number = {2},
    pages = {110},
    volume = {861},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/861/i=2/a=110?key=crossref.4966ef8b113b56542ecb25658138b39c},
    doi = {10.3847/1538-4357/aac8df},
    issn = {1538-4357},
    keywords = {atmospheres, fundamental parameters, laboratory, methods, planets and, planets and satellites, planets and satellites:,fundamental parameters,met, satellites, solid state, spectroscopic, techniques}
}

@article{Gavilan2017,
    title = {{Organic Aerosols in the Presence of CO<inf>2</inf> in the Early Earth and Exoplanets: UV-Vis Refractive Indices of Oxidized Tholins}},
    year = {2017},
    journal = {Astrophysical Journal Letters},
    author = {Gavilan, L. and Broch, L. and Carrasco, N. and Fleury, B. and Vettier, L.},
    number = {1},
    pages = {L5},
    volume = {848},
    publisher = {IOP Publishing},
    url = {http://dx.doi.org/10.3847/2041-8213/aa8cc4},
    doi = {10.3847/2041-8213/aa8cc4},
    issn = {20418213},
    keywords = {laboratory: solid state, planets and satellites: atmospheres, planets and satellites: fundamental parameters, techniques: spectroscopic}
}

@article{Raulin2002,
    title = {{Organic chemistry and exobiology on Titan}},
    year = {2002},
    journal = {Space Science Reviews},
    author = {Raulin, François and Owen, Tobias},
    number = {1-4},
    pages = {377--394},
    volume = {104},
    isbn = {0038-6308},
    doi = {10.1023/A:1023636623006},
    issn = {00386308}
}

@article{Raulin1987,
    title = {{Organic chemistry in the oceans of Titan}},
    year = {1987},
    journal = {Advances in Space Research},
    author = {Raulin, F.},
    number = {5},
    pages = {71--81},
    volume = {7},
    doi = {10.1016/0273-1177(87)90358-9},
    issn = {02731177}
}

@article{Coll1995,
    title = {{Organic chemistry in Titan's atmosphere: New data from laboratory simulations at low temperature}},
    year = {1995},
    journal = {Advances in Space Research},
    author = {Coll, P. and Coscia, D. and Gazeau, M. C. and de Vanssay, E. and Guillemin, J. C. and Raulin, F.},
    number = {2},
    pages = {93--103},
    volume = {16},
    isbn = {0273-1177{\textbackslash}r0-08-042622-0},
    doi = {10.1016/0273-1177(95)00197-M},
    issn = {02731177},
    pmid = {11543541}
}

@article{Ali2015,
    title = {{Organic chemistry in Titan's upper atmosphere and its astrobiological consequences: I. Views towards Cassini plasma spectrometer (CAPS) and ion neutral mass spectrometer (INMS) experiments in space}},
    year = {2015},
    journal = {Planetary and Space Science},
    author = {Ali, A. and Sittler, E. C. and Chornay, D. and Rowe, B. R. and Puzzarini, C.},
    number = {1},
    pages = {46--63},
    volume = {109-110},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2015.01.015},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2015.01.015},
    issn = {00320633},
    keywords = {Astronomical observations, Carbanions, Carbonium ions, Prebiotic chemistry, Titan, Upper atmosphere}
}

@article{Ramirez2005,
    title = {{Organic chemistry induced by corona discharges in Titan's troposphere: Laboratory simulations}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {Ram{\'{i}}rez, Sandra I. and Navarro-Gonz{\'{a}}lez, Rafael and Coll, Patrice and Raulin, François},
    number = {2},
    pages = {274--280},
    volume = {36},
    doi = {10.1016/j.asr.2005.09.010},
    issn = {02731177},
    keywords = {Cassini-Huygens, Corona discharges, Hydrocarbons, Nitriles, Titan, Troposphere}
}

@article{Chang1979,
    title = {{Organic Chemistry on Titan}},
    year = {1979},
    journal = {Reviews of Geophysics and Space Physics},
    author = {Chang, S. and Scattergood, Thomas and Aronowitz, S. and Flores, J.},
    number = {8},
    pages = {1923--1933},
    volume = {17}
}

@article{Chang1979a,
    title = {{Organic Chemistry titan}},
    year = {1979},
    author = {Chang, Shemood and Scattergood, T. and Aronowitz, Sheldon and Flotes, Jose},
    isbn = {1979000859}
}

@article{Miller1959,
    title = {{Organic Compound Synthesis on the Primitive Earth}},
    year = {1959},
    author = {Miller, Stanley L and Urey, Harold C},
    number = {3370},
    pages = {245--251},
    volume = {130}
}

@article{Goesmann2015,
    title = {{Organic compounds on comet 67P/Churyumov-Gerasimenko revealed by COSAC mass spectrometry}},
    year = {2015},
    journal = {Science},
    author = {Goesmann, Fred and Rosenbauer, Helmut and Bredeh{\"{o}}ft, Jan Hendrik and Cabane, Michel and Ehrenfreund, Pascale and Gautier, Thomas and Giri, Chaitanya and Kr{\"{u}}ger, Harald and Roy, Léna Le and Macdermott, Alexandra J and Mckenna-lawlor, Susan and Meierhenrich, Uwe J and Caro, Guillermo M Muñoz and Raulin, Francois and Roll, Reinhard and Steele, Andrew and Steininger, Harald and Sternberg, Robert and Szopa, Cyril},
    pages = {2--5},
    url = {http://www.sciencemag.org/content/349/6247/aab0689.full.pdf}
}

@article{Khare1981,
    title = {{Organic solids produced by electrical discharge in reducing atmospheres: Tholin molecular analysis}},
    year = {1981},
    journal = {Icarus},
    author = {Khare, B. N. and Sagan, Carl and Zumberge, John E. and Sklarew, Deborah S. and Nagy, Bartholomew},
    number = {2},
    pages = {290--297},
    volume = {48},
    isbn = {1102900850},
    doi = {10.1016/0019-1035(81)90110-X},
    issn = {10902643}
}

@article{Chadha1971,
    title = {{Organic Synthesis in a Simulated Jovian Atmosphere}},
    year = {1971},
    journal = {Icarus},
    author = {Chadha, M. S. and Flores, J. J. and Lawless, J. G. and Ponnamperuma, C.},
    pages = {39--44},
    volume = {15}
}

@article{Woeller1969,
    title = {{Organic synthesis in a simulated Jovian atmosphere-II}},
    year = {1969},
    journal = {Icarus},
    author = {Woeller, F. and Ponnamperuma, Cyril},
    number = {1},
    pages = {39--44},
    volume = {15},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(71)90031-5},
    issn = {10902643}
}

@article{Molton1974,
    title = {{Organic synthesis in a simulated Jovian atmosphere. III. Synthesis of Aminonitriles}},
    year = {1974},
    journal = {Icarus},
    author = {Molton, P. M. and Ponnamperuma, Cyril},
    number = {2},
    pages = {166--174},
    volume = {21},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(74)90133-X},
    issn = {10902643}
}

@article{Gupta1981,
    title = {{Organic synthesis in the atmosphere of Titan}},
    year = {1981},
    journal = {Nature},
    author = {Gupta, S. and Ochiai, E. and Ponnamperuma, C.},
    volume = {293}
}

@misc{Yung,
    title = {{Organic synthesis in the Atmosphere of Titan: Modeling and recent Observations}},
    author = {Yung, Yuk L. and Liang, Mao Chang and Zhang, Xi and Kammer, J. A. and Shemansky, D}
}

@article{Lammer2018,
    title = {{Origin and evolution of the atmospheres of early Venus, Earth and Mars}},
    year = {2018},
    journal = {Astron Astrophys Rev},
    author = {Lammer, Helmut and Zerkle, Aubrey L and Gebauer, Stefanie and Tosi, Nicola and Noack, Lena and Scherf, Manuel and Pilat-Lohinger, Elke and G{\"{u}}del, Manuel and Grenfell, John Lee and Godolt, Mareike and Nikolaou, Athanasia},
    number = {2},
    volume = {26},
    publisher = {Springer Berlin Heidelberg},
    url = {https://doi.org/10.1007/s00159-018-0108-y},
    doi = {10.1007/s00159-018-0108-y},
    issn = {1432-0754},
    keywords = {Mars {\textperiodcentered} Habitability, Venus}
}

@article{Horst2008,
    title = {{Origin of oxygen species in Titan's atmosphere}},
    year = {2008},
    journal = {Journal of Geophysical Research E: Planets},
    author = {H{\"{o}}rst, S. M. and Vuitton, Veronique and Yelle, R. V.},
    number = {10},
    pages = {1--14},
    volume = {113},
    doi = {10.1029/2008JE003135},
    issn = {01480227}
}

@article{Pearce2017,
    title = {{Origin of the RNA world : The fate of nucleobases in warm little ponds}},
    year = {2017},
    author = {Pearce, Ben K D and Pudritz, Ralph E and Semenov, Dmitry A and Henning, Thomas K},
    pages = {1--6},
    doi = {10.1073/pnas.1710339114},
    issn = {0027-8424},
    arxivId = {1710.00434}
}

@article{Raymond2017,
    title = {{Origin of water in the inner Solar System: planetesimals scattered inward during Jupiter and Saturn's rapid gas accretion ACCEPTED MANUSCRIPT Origin of water in the inner Solar System: planetesimals scattered inward during Jupiter and Saturn's rapid gas a}},
    year = {2017},
    journal = {Icarus},
    author = {Raymond, Sean N and Izidoro, Andre},
    url = {http://ac.els-cdn.com/S0019103517302592/1-s2.0-S0019103517302592-main.pdf?_tid=a9a4240c-60ab-11e7-a2c0-00000aacb35d&acdnat=1499167786_c1321166d49c761d34edb92a85f96df8},
    doi = {10.1016/j.icarus.2017.06.030},
    arxivId = {1707.01234},
    keywords = {Origins of Solar System, Planetary formation}
}

@article{Sasaki2012,
    title = {{Outcomes and Duration of Tidal Evolution in a Star-Planet-Moon System}},
    year = {2012},
    journal = {The Astrophysical Journal},
    author = {Sasaki, Takashi and Barnes, Jason W. and O'Brien, David P.},
    pages = {51},
    volume = {754},
    doi = {10.1088/0004-637X/754/1/51},
    issn = {0004-637X},
    arxivId = {1206.0334},
    keywords = {celestial mechanics, color figures, general, online-only material, planetary systems, planets and satellites}
}

@article{Counselman1973,
    title = {{Outcomes of tidal evolution}},
    year = {1973},
    journal = {The Astrophysical Journal},
    author = {Counselman, Charles C. III},
    pages = {307--314},
    volume = {180},
    url = {http://adsabs.harvard.edu/full/1973ApJ...180..307C},
    doi = {10.1086/151964},
    issn = {0004-637X},
    keywords = {celestial mechanics, planets}
}

@article{Greenberg1974,
    title = {{Outcomes of tidal evolution for orbits with arbitrary inclination}},
    year = {1974},
    journal = {Icarus},
    author = {Greenberg, Richard},
    number = {1},
    pages = {51--58},
    volume = {23},
    doi = {10.1016/0019-1035(74)90103-1},
    issn = {10902643}
}

@article{Carrasco2008b,
    title = {{PAMPRE}},
    year = {2008},
    author = {Carrasco, Nathalie}
}

@article{Szopa2006,
    title = {{PAMPRE: A dusty plasma experiment for Titan's tholins production and study}},
    year = {2006},
    journal = {Planetary and Space Science},
    author = {Szopa, Cyril and Cernogora, Guy and Boufendi, Laifa and Correia, Jean J. and Coll, Patrice},
    number = {4},
    month = {4},
    pages = {394--404},
    volume = {54},
    url = {http://www.sciencedirect.com/science/article/pii/S003206330600002X},
    doi = {10.1016/j.pss.2005.12.012},
    issn = {00320633},
    keywords = {Aerosols, Cold plasma, Laboratory simulation, Physico-chemical properties, Tholins, Titan}
}

@article{Anderson2010,
    title = {{Particle size and abundance of HC3N ice in Titan's lower stratosphere at high northern latitudes}},
    year = {2010},
    journal = {Icarus},
    author = {Anderson, C. M. and Samuelson, R. E. and Bjoraker, G. L. and Achterberg, R. K.},
    number = {2},
    pages = {914--922},
    volume = {207},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.12.024},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.12.024},
    issn = {00191035},
    keywords = {Radiative transfer, Titan}
}

@article{Helfenstein1985,
    title = {{Patterns of fracture and tidal stresses due to nonsynchronous rotation: Implications for fracturing on Europa}},
    year = {1985},
    journal = {Icarus},
    author = {Helfenstein, Paul and Parmentier, E. M.},
    number = {2},
    pages = {175--184},
    volume = {61},
    doi = {10.1016/0019-1035(85)90099-5},
    issn = {10902643}
}

@article{Helfenstein1985a,
    title = {{Patterns of fracture and tidal stresses due to nonsynchronous rotation: Implications for fracturing on Europa}},
    year = {1985},
    journal = {Icarus},
    author = {Helfenstein, Paul and Parmentier, E. M.},
    number = {2},
    pages = {175--184},
    volume = {61},
    doi = {10.1016/0019-1035(85)90099-5},
    issn = {10902643}
}

@article{Young1975,
    title = {{Phase diagrams of the elements}},
    year = {1975},
    journal = {Lawrence Livermore Laboratory},
    author = {Young, David a},
    pages = {64},
    isbn = {0520074831},
    doi = {10.2172/4010212}
}

@article{Yasuda2008,
    title = {{Phase equilibrium for clathrate hydrates formed with methane, ethane, propane, or carbon dioxide at temperatures below the freezing point of water}},
    year = {2008},
    journal = {Journal of Chemical and Engineering Data},
    author = {Yasuda, Keita and Ohmura, Ryo},
    number = {9},
    pages = {2182--2188},
    volume = {53},
    isbn = {0021-9568},
    doi = {10.1021/je800396v},
    issn = {00219568}
}

@article{Fletcher2009,
    title = {{Phosphine on Jupiter and Saturn from Cassini/CIRS}},
    year = {2009},
    journal = {Icarus},
    author = {Fletcher, L. N. and Orton, G. S. and Teanby, N. A. and Irwin, P. G.J.},
    number = {2},
    pages = {543--564},
    volume = {202},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.03.023},
    doi = {10.1016/j.icarus.2009.03.023},
    issn = {00191035},
    keywords = {Atmospheres, Jupiter, Saturn, composition, structure}
}

@article{Gudipati2013,
    title = {{Photochemical activity of Titan's low-altitude condensed haze.}},
    year = {2013},
    journal = {Nature communications},
    author = {Gudipati, Murthy S and Jacovi, Ronen and Couturier-Tamburelli, Isabelle and Lignell, Antti and Allen, Mark},
    number = {April},
    pages = {1648},
    volume = {4},
    publisher = {Nature Publishing Grouphttps://www.regonline.com/builder/site/default.aspx?EventID=1929367},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/23552063},
    isbn = {2041-1723},
    doi = {10.1038/ncomms2649},
    issn = {2041-1723},
    pmid = {23552063}
}

@article{Gudipati2015,
    title = {{Photochemical Evolution of Condensed Organics in Titan's Atmosphere and on the Surface How Earth-Like is Titan ? Outline Titan – A Habitable Body ? Titan – Rich Organic Inventory Titan – Photochemistry Conclusions}},
    year = {2015},
    author = {Gudipati, Murthy S and Couturier-tamburelli, Isabelle and Fleury, Benjamin and Lignell, Antti and Jacovi, Ronen}
}

@misc{Toublanc1995,
    title = {{Photochemical modelling of Titan’s atmosphere}},
    year = {1995},
    booktitle = {Icarus},
    author = {Toublanc, D. and Parisot P., Brillet, J., Gautier, D., Raulin, F. and McKay, C. P.},
    pages = {2--16},
    volume = {113}
}

@article{Tran2005,
    title = {{Photochemical processes on Titan: Irradiation of mixtures of gases that simulate Titan's atmosphere}},
    year = {2005},
    journal = {Icarus},
    author = {Tran, Buu N. and Joseph, Jeffrey C. and Force, Michael and Briggs, Robert G. and Vuitton, Veronique and Ferris, James P.},
    number = {1},
    pages = {106--115},
    volume = {177},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2005.03.015},
    issn = {00191035},
    keywords = {Abundances atmosphere, Atmosphere composition, Organic chemistry, Photochemistry, Titan}
}

@article{Cottin2014,
    title = {{Photochemical studies in low Earth orbit for organic compounds related to small bodies, Titan and Mars. Current and future facilities}},
    year = {2014},
    journal = {Bulletin de la Societe Royale des Sciences de Liege},
    author = {Cottin, H. and Saiagh, K. and Nguyen, D. and Grand, N. and B{\'{e}}nilan, Y. and Cloix, M. and Coll, P. and Gazeau, M. C. and Fray, N. and Khalaf, D. and Raulin, F. and Stalport, F. and Carrasco, N. and Szopa, C. and Chaput, D. and Bertrand, M. and Westall, F. and Mattioda, A. and Quinn, R. and Ricco, A. and Santos, O. and Baratta, G. A. and Strazzulla, G. and Palumbo, M. E. and Postollec, A. Le and Dobrijevic, M. and Coussot, G. and Vigier, F. and Vandenabeele-Trambouze, O. and Incerti, S. and Berger, T.},
    number = {July 2014},
    pages = {60--73},
    volume = {84},
    issn = {17835720}
}

@article{Coupeaud2006,
    title = {{Photochemical Synthesis of the Cyanodiacetylene HC 5 N : A Cryogenic Matrix Experiment}},
    year = {2006},
    author = {Coupeaud, A and Ko{\l}os, R and Aycard, J P and Pie, N},
    pages = {2371--2377}
}

@article{Fleury2015,
    title = {{Photochemistry of condensed species on Titan's aerosols analogues}},
    year = {2015},
    author = {Fleury, Benjamin and Carrasco, Nathalie and Gudipati, Murthy S}
}

@article{Glicker1987,
    title = {{Photochemistry of Diacetylene}},
    year = {1987},
    journal = {Journal of Physical Chemistry},
    author = {Glicker, S. and Okabe, H.},
    number = {9},
    pages = {437--440}
}

@article{Dubois2017b,
    title = {{Photochemistry of HCN Ice on Tholins Simulated in Titan’s Lower Atmosphere Conditions}},
    year = {2017},
    journal = {EPSC 2017},
    author = {Dubois, D. and Gudipati, Murthy S. and Henderson, B. and Carrasco, N. and Fleury, B. and Couturier-Tamburelli, Isabelle},
    pages = {9--10},
    volume = {11}
}

@article{Yung1984,
    title = {{Photochemistry of the atmosphere of Titan: Comparison between model and observations}},
    year = {1984},
    journal = {The Astrophysical Journal},
    author = {Yung, Yuk L. and Allen, Mark and Pinto, Joseph},
    number = {1981},
    pages = {465--506},
    volume = {212}
}

@article{Singh2010,
    title = {{Photodissociation Dynamics of Methylamine Cation and Its Relevance To Titan'S Ionosphere}},
    year = {2010},
    journal = {The Astrophysical Journal},
    author = {Singh, Prashant Chandra and Shen, Lei and Zhou, Jia and Schlegel, H. Bernhard and Suits, Arthur G.},
    number = {1},
    pages = {112--116},
    volume = {710},
    url = {http://iopscience.iop.org/article/10.1088/0004-637X/710/1/112},
    doi = {10.1088/0004-637X/710/1/112},
    issn = {0004-637X},
    keywords = {astrochemistry, clouds, general, individual, ism, planets and satellites}
}

@article{Richards1981a,
    title = {{Photodissociation of N2 - A significant source of thermospheric atomic nitrogen}},
    year = {1981},
    author = {Richards, P. G. and Torr, D. G. and Torr, M. R.},
    number = {80},
    pages = {1495--1498},
    volume = {86},
    doi = {10.1029/JA086iA03p01495},
    issn = {0148-0227}
}

@article{Huang2010,
    title = {{PHOTODISSOCIATION OF THE DIACETYLENE DIMER AND IMPLICATIONS FOR HYDROCARBON GROWTH IN TITAN’S ATMOSPHERE}},
    year = {2010},
    journal = {The Astrophysical Journal},
    author = {Huang, Cunshun and Zhang, Fangtong and Kaiser, Ralf I and Kislov, Vadim V and Mebel, Alexander M and Silva, Ruchira and Gichuhi, Wilson K and Suits, Arthur G},
    pages = {1249--1255},
    doi = {10.1088/0004-637X/714/2/1249},
    keywords = {astrochemistry, clouds, general, individual, ism, planets and satellites}
}

@article{Woon2004,
    title = {{Photoionization in ultraviolet processing of astrophysical ice analogs at cryogenic temperatures}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Woon, David E.},
    number = {1},
    pages = {44--48},
    volume = {33},
    isbn = {*************},
    doi = {10.1016/j.asr.2003.07.003},
    issn = {02731177},
    keywords = {Astrochemistry, ISM: molecules, Molecular processes}
}

@article{Tomasko1982,
    title = {{Photometry and polarimetry of Titan: Pioneer 11 observations and their implications for aerosol properties}},
    year = {1982},
    journal = {Icarus},
    author = {Tomasko, Martin G. and Smith, Peter H.},
    number = {1},
    pages = {65--95},
    volume = {51},
    doi = {10.1016/0019-1035(82)90030-6},
    issn = {10902643}
}

@article{Bassler1984,
    title = {{Photopolymerization of diacetylenes under hydrostatic pressure}},
    year = {1984},
    journal = {Chemical Physics},
    author = {B{\"{a}}ssler, H.},
    number = {2},
    pages = {307--318},
    volume = {93},
    isbn = {0065-3195},
    doi = {10.1016/0301-0104(85)80027-6},
    issn = {03010104}
}

@article{Cernogora2009,
    title = {{Physical properties of dust produced in a N 2 - CH 4 RF plasma discharge}},
    year = {2009},
    journal = {Ispc{\_}19},
    author = {Cernogora, G and Alcouffe, G and Hadamcik, E and Renard, J B and Carrasco, N and Szopa, C},
    pages = {4--7},
    volume = {6},
    keywords = {aerosols, atmosphere, dusty plasmas, light scattering, linear polarization, titan}
}

@article{McKay2001,
    title = {{Physical properties of the organic aerosols and clouds on Titan}},
    year = {2001},
    journal = {Planetary and Space Science},
    author = {McKay, C.P and Coustenis, A and Samuelson, R.E and Lemmon, M.T and Lorenz, R.D and Cabane, M and Rannou, P and Drossart, P},
    number = {1},
    pages = {79--99},
    volume = {49},
    doi = {10.1016/S0032-0633(00)00051-9},
    issn = {00320633}
}

@article{BallA.J.GarryR.C.2007,
    title = {{Planetary Landers And Entry Probes}},
    year = {2007},
    author = {Ball A.J., Garry R.C., Lorenz R.D.},
    pages = {364},
    isbn = {9780521820028},
    doi = {10.1017/CBO9780511536052},
    pmid = {14973856}
}

@article{Crida2015,
    title = {{Planetary science: Shepherds of Saturn's ring}},
    year = {2015},
    journal = {Nature Geoscience},
    author = {Crida, Aurélien},
    number = {9},
    pages = {666--667},
    volume = {8},
    publisher = {Nature Publishing Group},
    url = {http://www.nature.com/doifinder/10.1038/ngeo2512},
    doi = {10.1038/ngeo2512},
    issn = {1752-0894}
}

@article{Touvelle1987,
    title = {{Plasma Chemical Synthesis. II. Effect of Wall Surface on the Synthesis of Ammonia}},
    year = {1987},
    journal = {Plasma Chemistry and Plasma Processing},
    author = {Touvelle, M and Licea, J L Mufioz and Venugopalan, M and Mufioz Licea, J L and Venugopalan, M},
    number = {1},
    pages = {101},
    volume = {7},
    keywords = {ammonia, catalysis, nitrogen-, plasma synthesis, wall effect}
}

@article{Bagenal2015,
    title = {{Plasma conditions at Europa's orbit}},
    year = {2015},
    journal = {Icarus},
    author = {Bagenal, Fran and Sidrow, Evan and Wilson, Robert J. and Cassidy, Timothy A. and Dols, Vincent and Crary, Frank J. and Steffl, Andrew J. and Delamere, Peter A. and Kurth, William S. and Paterson, William R.},
    pages = {1--13},
    volume = {261},
    doi = {10.1016/j.icarus.2015.07.036},
    issn = {10902643},
    keywords = {Atmospheres, structure, Europa, Jupiter, magnetosphere, Satellites, atmospheres}
}

@article{Thompson1991,
    title = {{Plasma discharge in N{\$}{\_}2{\$} + CH{\$}{\_}4{\$} at low pressures: Experimental results and applications to Titan}},
    year = {1991},
    journal = {Icarus},
    author = {Thompson, W Reid and Henry, Todd J and Schwartz, Joel M and Khare, B N and Sagan, Carl},
    number = {1},
    pages = {57--73},
    volume = {90},
    doi = {http://dx.doi.org/10.1016/0019-1035(91)90068-5},
    issn = {0019-1035}
}

@article{Behounkova2017,
    title = {{Plume Activity and Tidal Deformation on Enceladus Influenced by Faults and Variable Ice Shell Thickness}},
    year = {2017},
    journal = {Astrobiology},
    author = {B{\v{e}}hounkov{\'{a}}, M. and Sou{\v{c}}ek, Ondřej and Hron, Jaroslav and {\v{C}}adek, Ondřej},
    number = {9},
    pages = {ast.2016.1629},
    volume = {17},
    url = {http://online.liebertpub.com/doi/10.1089/ast.2016.1629},
    doi = {10.1089/ast.2016.1629},
    issn = {1531-1074}
}

@article{Teolis2017,
    title = {{Plume and surface feature structure and compositional effects on Europa's global exosphere: Preliminary Europa mission predictions}},
    year = {2017},
    journal = {Icarus},
    author = {Teolis, B. D. and Wyrick, D. Y. and Bouquet, A. and Magee, B. A. and Waite, J. H.},
    pages = {18--29},
    volume = {284},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.10.027},
    doi = {10.1016/j.icarus.2016.10.027},
    issn = {10902643},
    keywords = {Abundances, atmospheres, Atmospheres, dynamics, Europa, Ices, Jupiter, Jupiter, satellites, Satellites, atmospheres, Satellites, composition, Volcanism}
}

@article{Wong2015,
    title = {{Pluto's implications for a Snowball Titan}},
    year = {2015},
    journal = {Icarus},
    author = {Wong, Michael L. and Yung, Yuk L. and Randall Gladstone, G.},
    number = {C},
    pages = {192--196},
    volume = {246},
    publisher = {Elsevier Inc.},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.05.019},
    issn = {10902643},
    keywords = {Photochemistry, Pluto, Pluto, atmosphere, Titan, Titan, atmosphere}
}

@article{Delamere2004,
    title = {{Pluto's kinetic interaction with the solar wind}},
    year = {2004},
    journal = {Geophysical Research Letters},
    author = {Delamere, P. A. and Bagenal, F.},
    number = {4},
    pages = {L04807},
    volume = {31},
    url = {http://doi.wiley.com/10.1029/2003GL018122},
    doi = {10.1029/2003GL018122},
    issn = {0094-8276}
}

@article{Ojakangas1989,
    title = {{Polar Wander of an Ice Shell on Europa}},
    year = {1989},
    journal = {Icarus},
    author = {Ojakangas, G. W. and Stevenson, D. J.},
    pages = {242--270},
    volume = {270}
}

@article{Sagan1993,
    title = {{Polycyclic aromatic hydrocarbons in the atmospheres of Titan and Jupiter.}},
    year = {1993},
    journal = {The Astrophysical journal},
    author = {Sagan, C and Khare, B N and Thompson, W R and McDonald, G D and Wing, M R and Bada, J L and Vo-Dinh, T and Arakawa, E T},
    number = {1},
    pages = {399--405},
    volume = {414},
    url = {http://articles.adsabs.harvard.edu/full/1993ApJ...414..399S},
    isbn = {0004-637X (Print){\textbackslash}r0004-637X (Linking)},
    doi = {10.1086/173086},
    issn = {0004-637X},
    pmid = {11539501},
    arxivId = {ISSN 0004-637X},
    keywords = {NASA Discipline Exobiology, Non-NASA Center}
}

@article{Rahm2016,
    title = {{Polymorphism and electronic structure of polyimine and its potential significance for prebiotic chemistry on Titan}},
    year = {2016},
    author = {Rahm, Martin and Lunine, Jonathan I and Usher, David A and Shalloway, David},
    pages = {1--6},
    doi = {10.1073/pnas.1606634113}
}

@article{Johnson2017a,
    title = {{Porosity and salt content determine if subduction can occur in Europa's ice shell}},
    year = {2017},
    journal = {Journal of Geophysical Research: Planets},
    author = {Johnson, Brandon C. and Sheppard, Rachel Y. and Pascuzzo, Alyssa C. and Fisher, Elizabeth A. and Wiggins, Sean E.},
    number = {8147},
    url = {http://doi.wiley.com/10.1002/2017JE005370},
    doi = {10.1002/2017JE005370},
    issn = {21699097},
    keywords = {europa, ice shell, plate tectonics, subduction}
}

@article{McKay2005,
    title = {{Possibilities for methanogenic life in liquid methane on the surface of Titan}},
    year = {2005},
    journal = {Icarus},
    author = {McKay, C. P. and Smith, H. D.},
    number = {1},
    pages = {274--276},
    volume = {178},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2005.05.018},
    issn = {00191035},
    keywords = {Life, Methanogens, Titan}
}

@article{Pena-Cabrera2004,
    title = {{Possible biotic distribution in our galaxy}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Pena-Cabrera, G. V Y and Durand-Manterola, H. J.},
    number = {1},
    pages = {114--117},
    volume = {33},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2003.07.016},
    issn = {02731177},
    keywords = {Astrobiology, Biotic distribution, Galaxy}
}

@article{Lorenz2005,
    title = {{Post-Cassini exploration of Titan: Science goals, instrumentation and mission concepts}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {Lorenz, R. D. and Lunine, J. I. and Zimmerman, W.},
    number = {2},
    pages = {281--285},
    volume = {36},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2005.03.080},
    issn = {02731177},
    keywords = {Astrobiology, Exploration, Prebiotic chemistry, Titan}
}

@article{Nimmo2014,
    title = {{Powering Triton's recent geological activity by obliquity tides: Implications for Pluto geology}},
    year = {2014},
    journal = {Icarus},
    author = {Nimmo, F. and Spencer, J. R.},
    pages = {1--9},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.01.044},
    doi = {10.1016/j.icarus.2014.01.044},
    issn = {00191035},
    keywords = {Pluto, Satellites, dynamics, Tides, solid body, Triton}
}

@article{Raulin2012,
    title = {{Prebiotic-like chemistry on Titan}},
    year = {2012},
    journal = {Chemical Society Reviews},
    author = {Raulin, François and Brass{\'{e}}, Coralie and Poch, Olivier and Coll, Patrice},
    number = {16},
    pages = {5380},
    volume = {41},
    url = {http://xlink.rsc.org/?DOI=c2cs35014a},
    isbn = {0306-0012},
    doi = {10.1039/c2cs35014a},
    issn = {0306-0012},
    pmid = {22481630}
}

@article{Lilensten2005,
    title = {{Prediction of a N2++ layer in the upper atmosphere of Titan}},
    year = {2005},
    journal = {Geophysical Research Letters},
    author = {Lilensten, Jean and Witasse, O. and Simon, C. and Soldi-Lose, H. and Dutuit, O. and Thissen, R. and Alcaraz, C.},
    number = {3},
    pages = {1--4},
    volume = {32},
    doi = {10.1029/2004GL021432},
    issn = {00948276}
}

@article{Neveu2014,
    title = {{Prerequisites for explosive cryovolcanism on dwarf planet-class Kuiper belt objects}},
    year = {2014},
    journal = {Icarus},
    author = {Neveu, M. and Desch, S. J. and Shock, E. L. and Glein, C. R.},
    pages = {48--64},
    volume = {246},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.03.043},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.03.043},
    issn = {10902643},
    keywords = {Charon, Interiors, Pluto, Satellites, Volcanism, formation}
}

@article{Nordheim2018,
    title = {{Preservation of potential biosignatures in the shallow subsurface of Europa}},
    year = {2018},
    journal = {Nature Astronomy},
    author = {Nordheim, T A and Hand, K P and Paranicas, C},
    publisher = {Springer US},
    url = {http://dx.doi.org/10.1038/s41550-018-0499-8},
    doi = {10.1038/s41550-018-0499-8},
    issn = {2397-3366}
}

@article{Mordaunt1993,
    title = {{Primary Product Channels in the Photodissociation of Methane at 121.6 nm}},
    year = {1993},
    journal = {Journal of Chemical Physics},
    author = {Mordaunt, D. H. and Lambert, I. R. and Morley, G. P. and Ashfold, Michael N. R. and Dixon, R. N. and Western, C. M.},
    number = {3},
    pages = {2054--2065},
    volume = {98},
    doi = {10.1063/1.464237},
    issn = {0021-9606},
    keywords = {FREE RADICALS, HYDROGEN ATOMS, METHANE, PHOTOCHEMI, HYDROGEN ATOMS, METHANE, PHOTOCHEMI}
}

@article{Ponnamperuna1971,
    title = {{Primiordial organic chemistry and the origin of life}},
    year = {1971},
    journal = {Quarterly Reviews of Biophysics},
    author = {Ponnamperuna, C},
    number = {2 and 3},
    pages = {77--106},
    volume = {4},
    publisher = {ECOLE CENTRALE PARIS},
    keywords = {LIFE, ORIGIN, ORIGIN OF LIFE}
}

@article{Bellucci2004,
    title = {{Principal components analysis of Jupiter VIMS spectra}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Bellucci, G. and Formisano, V. and D'Aversa, E. and Brown, R. H. and Baines, K. H. and Bibring, J. P. and Buratti, B. J. and Capaccioni, F. and Cerroni, P. and Clark, R. N. and Coradini, A. and Cruikshank, D. P. and Drossart, P. and Jaumann, R. and Langevin, Y. and Matson, D. L. and McCord, T. B. and Mennella, V. and Nelson, R. M. and Nicholson, P. D. and Sicardy, B. and Sotin, C. and Chamberlain, M. C. and Hansen, G. and Hibbits, K. and Showalter, M. and Filacchione, G.},
    number = {8},
    pages = {1640--1646},
    volume = {34},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2003.05.062},
    issn = {02731177},
    keywords = {Cassini, Great red spot, Jupiter, Visual-Infrared mapping spectrometer}
}

@article{Joy2002,
    title = {{Probabilistic models of the Jovian magnetopause and bow shock locations}},
    year = {2002},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Joy, S. P. and Kivelson, M. G. and Walker, R. J. and Khurana, K. K. and Russell, C. T. and Ogino, T.},
    number = {A10},
    pages = {1--17},
    volume = {107},
    isbn = {0148-0227},
    doi = {10.1029/2001JA009146},
    issn = {21699402},
    keywords = {Bow shock, Jupiter, MHD, Magnetopause, Solar wind}
}

@article{Kaplan2015,
    title = {{Probing a cell-embedded megadalton protein complex by DNP-supported solid-state NMR}},
    year = {2015},
    author = {Kaplan, Mohammed and Cukkemane, Abhishek and Zundert, Gydo C P Van and Narasimhan, Siddarth and Dani{\"{e}}ls, Mark and Mance, Deni and Waksman, Gabriel and Bonvin, Alexandre M J J and Fronzes, Rémi and Folkers, Gert E and Baldus, Marc},
    number = {May},
    doi = {10.1038/nmeth.3406}
}

@article{Sparks2016,
    title = {{PROBING FOR EVIDENCE OF PLUMES ON EUROPA WITH HST / STIS}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Sparks, W B and Hand, K P and Mcgrath, M A and Bergeron, E and Cracraft, M and Deustua, S E},
    number = {2},
    pages = {1--21},
    volume = {829},
    publisher = {IOP Publishing},
    url = {http://dx.doi.org/10.3847/0004-637X/829/2/121},
    doi = {10.3847/0004-637X/829/2/121},
    issn = {1538-4357},
    keywords = {general, planets and satellites, planets and satellites: general}
}

@article{Sparks2016a,
    title = {{PROBING FOR EVIDENCE OF PLUMES ON EUROPA WITH HST/STIS}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Sparks, W.},
    keywords = {general, planets and satellites}
}

@article{Swain2013,
    title = {{Probing the extreme planetary atmosphere of WASP-12b}},
    year = {2013},
    journal = {Icarus},
    author = {Swain, Mark and Deroo, Pieter and Tinetti, Giovanna and Hollis, Morgan and Tessenyi, Marcell and Line, Michael and Kawahara, Hajime and Fujii, Yuka and Showman, Adam P. and Yurchenko, Sergey N.},
    number = {1},
    pages = {432--445},
    volume = {225},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.04.003},
    doi = {10.1016/j.icarus.2013.04.003},
    issn = {00191035},
    arxivId = {1205.4736},
    keywords = {Atmospheres, Composition, Eclipses, Extrasolar planets, Jovian planets, Spectroscopy}
}

@article{Sagan1984a,
    title = {{Production and condensation of organic gases in the atmosphere of Titan}},
    year = {1984},
    journal = {Icarus},
    author = {Sagan, Carl and Reid Thompson, W.},
    number = {2},
    month = {8},
    pages = {133--161},
    volume = {59},
    url = {http://www.sciencedirect.com/science/article/pii/0019103584900186},
    doi = {10.1016/0019-1035(84)90018-6},
    issn = {00191035}
}

@article{Sagan1984,
    title = {{Production and Condensation of organic gases in the Atmosphere of Titan}},
    year = {1984},
    journal = {Statewide Agricultural Land Use Baseline 2015},
    author = {Sagan, C. and Thompson, W. R.},
    volume = {1},
    isbn = {9788578110796},
    doi = {10.1017/CBO9781107415324.004},
    issn = {1098-6596},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {icle}
}

@article{Scattergood1989,
    title = {{Production of organic compounds in plasmas: A comparison among electric sparks, laser-induced plasmas, and UV light}},
    year = {1989},
    journal = {Icarus},
    author = {Scattergood, Thomas W. and McKay, Christopher P. and Borucki, William J. and Giver, Lawrence P. and van Ghyseghem, Hilde and Parris, James E. and Miller, Stanley L.},
    number = {2},
    pages = {413--428},
    volume = {81},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(89)90061-4},
    issn = {10902643},
    pmid = {11542165}
}

@article{Scattergood1975,
    title = {{Production of organic molecules in the outer solar system by proton irradiation - Laboratory simulations}},
    year = {1975},
    author = {Scattergood, T. and Lesser, P. and Owen, T.},
    pages = {465--471},
    volume = {471}
}

@article{Johnson2006a,
    title = {{Production, ionization and redistribution of O 2 in Saturn’s ring atmosphere}},
    year = {2006},
    author = {Johnson, R E and Luhmann, J G and Tokar, R L and Bouhram, M and Berthelier, J J and Sittler, E C},
    pages = {393--402},
    volume = {180},
    doi = {10.1016/j.icarus.2005.08.021},
    keywords = {atmosphere, magnetosphere, rings, saturn}
}

@article{Vinatier,
    title = {{Profils verticaux de temperature}},
    author = {Vinatier, Sandrine},
    pages = {151},
    volume = {2}
}

@article{Schwingenschuh2001,
    title = {{Propagation of electromagnetic waves in the lower ionosphere of Titan}},
    year = {2001},
    journal = {Advances in Space Research},
    author = {Schwingenschuh, K. and Molina-Cuberos, G.J. J. and Eichelberger, H.U. U. and Torkar, K. and Friedrich, M. and Grard, R. and Falkner, P. and L{\'{o}}pez-Moreno, J.J. J. and Rodrigo, R.},
    number = {10},
    pages = {1505--1510},
    volume = {28},
    url = {http://www.sciencedirect.com/science/article/pii/S0273117701005841},
    doi = {10.1016/S0273-1177(01)00584-1},
    issn = {02731177}
}

@article{Clifford1998,
    title = {{Properties of diazocarbene [CNN] and the diazomethyl radical [HCNN] via ion chemistry and spectroscopy}},
    year = {1998},
    journal = {Journal of Physical Chemistry A},
    author = {Clifford, Eileen P. and Wenthold, Paul G. and Lineberger, W. Carl and Petersson, George A. and Broadus, Katherine M. and Kass, Steven R. and Kato, Shuji and DePuy, Charles H. and Bierbaum, Veronica M. and Ellison, G. Barney},
    number = {36},
    pages = {7100--7112},
    volume = {102},
    isbn = {1089-5639},
    doi = {10.1021/jp9802735},
    issn = {10895639}
}

@article{Mandt2014,
    title = {{PROTOSOLAR AMMONIA AS THE UNIQUE SOURCE OF TITAN ’ s NITROGEN}},
    year = {2014},
    author = {Mandt, Kathleen E and Mousis, Olivier and Lunine, Jonathan and Gautier, Daniel},
    volume = {24},
    doi = {10.1088/2041-8205/788/2/L24},
    keywords = {and satellites, atmospheres, comets, composition, formation, general, planets, planets and satellites}
}

@article{Stevenson2016,
    title = {{Quantifying and Predicting the Presence of Clouds in Exoplanet Atmospheres}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Stevenson, Kevin B.},
    number = {2},
    pages = {L16},
    volume = {817},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/2041-8205/817/i=2/a=L16?key=crossref.f3c58469d361765ff5431af100f45eab},
    doi = {10.3847/2041-8205/817/2/L16},
    issn = {2041-8213},
    keywords = {analytical, atmospheres, methods, methods: analytical, planets and satellites, planets and satellites: atmospheres, spectroscopic, techniques, techniques: spectroscopic}
}

@article{Fortenberry2017review,
    title = {{Quantum astrochemical spectroscopy}},
    year = {2017},
    journal = {International Journal of Quantum Chemistry},
    author = {Fortenberry, Ryan C.},
    number = {2},
    pages = {81--91},
    volume = {117},
    doi = {10.1002/qua.25180},
    issn = {1097461X},
    keywords = {anions, astrochemistry, cations, cloud computing, noble gases, quartic force fields, radicals}
}

@article{Fortenberry2017b,
    title = {{Quantum Chemical Spectral Characterization of CH 2 NH 2 + for Remote Sensing of Titan’s Atmosphe}},
    year = {2017},
    journal = {Icarus},
    author = {Fortenberry, Ryan and Thackston, Russell and Fortenberry, Ryan and Nicholson, Prof Philip and Fortenberry, Ryan C and Ph, D}
}

@article{Thackston2018,
    title = {{Quantum chemical spectral characterization of CH2NH2+ for remote sensing of Titan’s atmosphere}},
    year = {2018},
    journal = {Icarus},
    author = {Thackston, Russell and Fortenberry, Ryan C.},
    pages = {187--193},
    volume = {299},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103517302932},
    doi = {10.1016/j.icarus.2017.07.029},
    issn = {00191035},
    keywords = {"Atmospheres, "Titan, Infrared observations, Radio observations, Spectroscopy, atmosphere", chemistry", composition"}
}

@article{Singh2017,
    title = {{Quantum Decimation in Hilbert Space: Coarse-Graining without Structure}},
    year = {2017},
    author = {Singh, Ashmeet and Carroll, Sean M},
    arxivId = {arXiv:1709.01066v1}
}

@article{Harmon2008,
    title = {{Radar imagery of the southern Caloris region, Mercury}},
    year = {2008},
    journal = {Icarus},
    author = {Harmon, John K.},
    number = {1},
    pages = {298--301},
    volume = {196},
    doi = {10.1016/j.icarus.2008.03.003},
    issn = {00191035},
    keywords = {Mercury, Radar observations, surface}
}

@article{Sandwell2004,
    title = {{Radar interferometry for measuring tidal strains across cracks on Europa}},
    year = {2004},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Sandwell, David and Rosen, Paul and Moore, William and Gurrola, Eric},
    number = {11},
    pages = {1--9},
    volume = {109},
    doi = {10.1029/2004JE002276},
    issn = {01480227},
    keywords = {Crack, Europa, Interferometry}
}

@article{Heggy2016,
    title = {{Radar Probing of Jovian Icy Moons: Understanding Subsurface water and structure Detectability in the JUICE and Europa Missions}},
    year = {2016},
    journal = {Icarus},
    author = {Heggy, Essam and Scabbia, Giovanni and Bruzzone, Lorenzo and Pappalardo, Robert T.},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103516307953},
    doi = {10.1016/j.icarus.2016.11.039},
    issn = {00191035},
    keywords = {Callisto, Dielectric, Europa, Ganymede, Juice, Radar}
}

@article{Elachi2004,
    title = {{Radar: the Cassini Titan radar mapper}},
    year = {2004},
    journal = {Space Sci. Rev.},
    author = {Elachi, C and Allison, M D and Borgarelli, L and Encrenaz, P and Im, E and Janssen, M A and Johnson, W T K and Kirk, R L and Lorenz, R D and Lunine, J I and {others}},
    number = {1},
    pages = {71--110},
    volume = {115}
}

@article{Horst2013,
    title = {{Radiative Equilibrium: the Insolation of an Atmosphere}},
    year = {1913},
    author = {A., Milne E.},
    number = {5},
    volume = {lxxviii}
}

@article{Tyler1981,
    title = {{Radio Science Investigations of the Saturn System with Voyager 1: Preliminary Results.}},
    year = {1981},
    journal = {Science (New York, N.Y.)},
    author = {Tyler, G L and Eshleman, V R and Anderson, J D and Levy, G S and Lindal, G F and Wood, G E and Croft, T a},
    number = {4491},
    pages = {201--206},
    volume = {212},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/17783830},
    doi = {10.1126/science.212.4491.201},
    issn = {0036-8075},
    pmid = {17783830}
}

@article{Tomasko2005,
    title = {{Rain, winds and haze during the Huygens probe's descent to Titan's surface}},
    year = {2005},
    journal = {Nature},
    author = {Tomasko, M G and Archinal, B and Becker, T and B{\'{e}}zard, B and Bushroe, M and Combes, M and Cook, D and Coustenis, A and de Bergh, C and Dafoe, L E and Doose, L and Dout{\'{e}}, S and Eibl, A and Engel, S and Gliem, F and Grieger, B and Holso, K and Howington-Kraus, E and Karkoschka, E and Keller, H U},
    number = {7069},
    pages = {765--778},
    volume = {438},
    url = {http://libraries.ou.edu/access.aspx?url=http://search.ebscohost.com/login.aspx?direct=true&db=aph&AN=19071750&site=ehost-live},
    isbn = {00280836},
    doi = {10.1038/nature04126},
    issn = {0028-0836},
    pmid = {19071750}
}

@article{Pezolet1969,
    title = {{Raman spectra of liquid and crystalline HCN and DCN}},
    year = {1969},
    journal = {Notes},
    author = {Pezolet, M. and Savoie, R.},
    number = {1},
    pages = {4226--4229}
}

@article{Turtle2011,
    title = {{Rapid and extensive surface changes near Titan's equator: evidence of April showers.}},
    year = {2011},
    journal = {Science (New York, N.Y.)},
    author = {Turtle, E P and Perry, J E and Hayes, a G and Lorenz, R D and Barnes, J W and McEwen, a S and West, R a and Del Genio, a D and Barbara, J M and Lunine, J I and Schaller, E L and Ray, T L and Lopes, R M C and Stofan, E R},
    number = {6023},
    pages = {1414--1417},
    volume = {331},
    isbn = {0036-8075},
    doi = {10.1126/science.1201063},
    issn = {0036-8075},
    pmid = {21415347}
}

@article{Vuitton2012,
    title = {{Rapid Association Reactions At Low Pressure: Impact on the Formation of Hydrocarbons on Titan}},
    year = {2012},
    journal = {The Astrophysical Journal},
    author = {Vuitton, V. and Yelle, R. V. and Lavvas, P. and Klippenstein, S. J.},
    number = {1},
    pages = {11},
    volume = {744},
    url = {http://stacks.iop.org/0004-637X/744/i=1/a=11?key=crossref.1737dcd2fbdc1d6e7392d7016a086f4f},
    doi = {10.1088/0004-637X/744/1/11},
    issn = {0004-637X},
    keywords = {astrochemistry, color figures, individual, methods, numerical, online-only material, planets and satellites, titan}
}

@misc{Prange1996,
    title = {{Rapid energy dissipation and variability of the Io-Jupiter electrodynamic circuit}},
    year = {1996},
    author = {Prange, R and Rego, D. and Southwood, David J. and Zarka, P. and Miller, S. and Ip, W.}
}

@article{Hoobler1997,
    title = {{Rate coefficients for reactions of ethynyl radical (C2H) with HCN and CH3CN: Implications for the formation of complex nitriles on Titan}},
    year = {1997},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Hoobler, Ray J. and Leone, Stephen R.},
    number = {E12},
    pages = {28717--28723},
    volume = {102},
    doi = {10.1029/97JE02526},
    issn = {01480227},
    keywords = {Analytical protocol, Multi-frequency resonant excitation, Polychlorodibenzo-p-dioxins, Polychlorodibenzofurans, Quadrupole ion trap}
}

@article{Glavin2004,
    title = {{Re-examination of amino acids in Antarctic micrometeorites}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Glavin, D. P. and Matrajt, G. and Bada, J. L.},
    number = {1},
    pages = {106--113},
    volume = {33},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2003.02.011},
    issn = {02731177},
    keywords = {Amino acids, Micrometeorites, Prebiotic organic inventory}
}

@article{Bhasi2015,
    title = {{Reaction between HN and SN : a possible channel for the interstellar formation of N2 and SH in the}},
    year = {2015},
    journal = {Physical Chemistry Chemical Physics},
    author = {Bhasi, Priya and Nhlabatsi, Zanele P and Sitha, Sanyasi},
    pages = {32455--32463},
    volume = {17},
    publisher = {Royal Society of Chemistry},
    url = {http://dx.doi.org/10.1039/C5CP05190H},
    doi = {10.1039/C5CP05190H},
    issn = {1463-9076}
}

@article{Koyama2015,
    title = {{Reaction Dynamics of CN Radicals in Acetonitrile Solutions}},
    year = {2015},
    journal = {Journal of Physical Chemistry A},
    author = {Koyama, Daisuke and Coulter, Philip and Grubb, Michael P. and Greetham, Gregory M. and Clark, Ian P. and Orr-Ewing, Andrew J.},
    number = {52},
    pages = {12924--12934},
    volume = {119},
    doi = {10.1021/acs.jpca.5b10720},
    issn = {15205215}
}

@article{Seki1996,
    title = {{Reaction rates of the CN radical with diacetylene and dicyanoacetylene}},
    year = {1996},
    journal = {Chemical Physics Letters},
    author = {Seki, K. and Yagi, M. and He, M. and Halpem, J. and Okabe, H.},
    number = {August},
    pages = {0--5},
    volume = {4}
}

@article{Wang2015,
    title = {{Reactions of Azine Anions with Nitrogen and Oxygen Atoms: Implications for Titan's Upper Atmosphere and Interstellar Chemistry}},
    year = {2015},
    journal = {Journal of the American Chemical Society},
    author = {Wang, Zhe Chen and Cole, Callie A. and Demarais, Nicholas J. and Snow, Theodore P. and Bierbaum, Veronica M.},
    number = {33},
    pages = {10700--10709},
    volume = {137},
    doi = {10.1021/jacs.5b06089},
    issn = {15205126},
    pmid = {26281019}
}

@article{Hudson2004,
    title = {{Reactions of nitriles in ices relevant to Titan, comets, and the interstellar medium: Formation of cyanate ion, ketenimines, and isonitriles}},
    year = {2004},
    journal = {Icarus},
    author = {Hudson, R. L. and Moore, M. H.},
    number = {2},
    pages = {466--478},
    volume = {172},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2004.06.011},
    issn = {00191035},
    keywords = {Comets, Ices, Photochemistry, Radiation chemistry, Titan}
}

@article{CunhadeMiranda2015,
    title = {{Reactions of State-Selected Atomic Oxygen Ions O(+)((4)S, (2)D, (2)P) with Methane.}},
    year = {2015},
    journal = {The journal of physical chemistry. A},
    author = {Cunha de Miranda, Barbara and Romanzin, Claire and Chefdeville, Simon and Vuitton, Véronique and {\v{Z}}abka, Jan and Pol{\'{a}}{\v{s}}ek, Miroslav and Alcaraz, Christian},
    number = {23},
    pages = {6082--98},
    volume = {119},
    url = {http://dx.doi.org/10.1021/jp512846v},
    isbn = {1520-5215 (Electronic)
1089-5639 (Linking)},
    doi = {10.1021/jp512846v},
    issn = {1520-5215},
    pmid = {25721439}
}

@article{Wang2016,
    title = {{Reactions of substituted benzene anions with N and O atoms: Chemistry in Titan's upper atmosphere and the interstellar medium}},
    year = {2016},
    journal = {Journal of Chemical Physics},
    author = {Wang, Zhe Chen and Bierbaum, Veronica M.},
    number = {21},
    volume = {144},
    url = {http://dx.doi.org/10.1063/1.4952454},
    doi = {10.1063/1.4952454},
    issn = {00219606},
    pmid = {27276954}
}

@article{Espinosa2003,
    title = {{Reanalysis of Saturn's magnetospheric field data view of spin-periodic perturbations}},
    year = {2003},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Espinosa, Stéphane A. and Southwood, David J. and Dougherty, Michèle K.},
    number = {A2},
    pages = {1--8},
    volume = {108},
    doi = {10.1029/2001JA005083},
    issn = {21699402},
    keywords = {Magnetic, Magnetosphere, Periodicity, Pioneer, Saturn, Voyager}
}

@article{Nogueira2011,
    title = {{Reassessing the origin of Triton}},
    year = {2011},
    journal = {Icarus},
    author = {Nogueira, E. and Brasser, R. and Gomes, R.},
    number = {1},
    pages = {113--130},
    volume = {214},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.05.003},
    doi = {10.1016/j.icarus.2011.05.003},
    issn = {00191035},
    arxivId = {1105.1179},
    keywords = {Irregular satellites, Neptune, Satellites, Satellites, Dynamics, Tides, Solid body, Triton}
}

@article{Salama2016,
    title = {{Recent Progresses in Laboratory Astrophysics with Ames’ COSmIC Facility}},
    year = {2016},
    author = {Salama, Farid and Contreras, Cesar and Sciamma-O'Brien, Ella and Bejaoui, Salma},
    number = {332},
    pages = {364--369},
    url = {https://ui.adsabs.harvard.edu/#abs/2016AAS...22811605S},
    doi = {10.1017/S1743921317011619},
    issn = {1743-9213}
}

@article{Coates2011,
    title = {{Recent results from titan's ionosphere}},
    year = {2011},
    journal = {Space Science Reviews},
    author = {Coates, A. J. and Wahlund, J. E. and Agren, K. and Edberg, N. and Cui, J. and Wellbrock, A. and Szego, K.},
    number = {1-4},
    pages = {85--111},
    volume = {162},
    isbn = {1121401198},
    doi = {10.1007/s11214-011-9826-4},
    issn = {00386308},
    keywords = {Ionosphere, Mars, Titan, Venus}
}

@article{Khare1973,
    title = {{Red clouds in reducing atmospheres}},
    year = {1973},
    journal = {Icarus},
    author = {Khare, B. and Sagan, C.},
    number = {3},
    month = {11},
    pages = {311--321},
    volume = {20},
    url = {http://www.sciencedirect.com/science/article/pii/0019103573900080},
    doi = {10.1016/0019-1035(73)90008-0},
    issn = {00191035}
}

@article{Faulk2017,
    title = {{Regional patterns of extreme precipitation on Titan consistent with observed alluvial fan distribution}},
    year = {2017},
    journal = {Nature Geoscience},
    author = {Faulk, S P and Mitchell, J L and Moon, S and Lora, J M},
    number = {October},
    pages = {1--6},
    doi = {10.1038/NGEO3043}
}

@article{Sotin2005,
    title = {{Release of volatiles from a possible cryovolcano from near-infrared imaging of Titan.}},
    year = {2005},
    journal = {Nature},
    author = {Sotin, C. and Jaumann, Ralf and Buratti, Bonnie J and Brown, Robert H and Clark, Roger N. and Soderblom, Laurence a and Baines, K H and Bellucci, Giancarlo and Bibring, Jean-Pierre and Capaccioni, Fabrizio and Cerroni, Pricilla and Combes, Michel and Coradini, Angioletta and Cruikshank, Dale P and Drossart, Pierre and Formisano, Vittorio and Langevin, Yves and Matson, Dennis L and McCord, Thomas B and Nelson, Robert M and Nicholson, Philip D and Sicardy, B and LeMou{\'{e}}lic, Stéphane and Rodriguez, S and Stephan, Klaas E and Scholz, C K},
    number = {7043},
    pages = {786--789},
    volume = {435},
    isbn = {1476-4687 (Electronic)},
    doi = {10.1038/nature03596},
    issn = {0028-0836},
    pmid = {15944697}
}

@article{Everett1848,
    title = {{Report on the Discovery and Name of an Eighth Satellite of Saturn}},
    year = {1848},
    journal = {Memoirs of the American Academy of Arts and Sciences},
    author = {Everett, E.},
    number = {4},
    pages = {275--290},
    volume = {47}
}

@article{Coustenis2009,
    title = {{Results from the Huygens probe on Titan}},
    year = {2009},
    author = {Coustenis, Jean-pierre Lebreton Athena and Lunine, Jonathan and Raulin, François and Owen, Tobias and Strobel, Darrell},
    pages = {149--179},
    doi = {10.1007/s00159-009-0021-5}
}

@article{Mitri2008,
    title = {{Resurfacing of Titan by ammonia-water cryomagma}},
    year = {2008},
    journal = {Icarus},
    author = {Mitri, Giuseppe and Showman, Adam P. and Lunine, Jonathan I. and Lopes, Rosaly M C},
    number = {1},
    pages = {216--224},
    volume = {196},
    doi = {10.1016/j.icarus.2008.02.024},
    issn = {00191035},
    keywords = {Geophysics, Ices, Interiors, Satellites, Saturn, Titan, Volcanism, surfaces}
}

@article{Bauduin2018,
    title = {{Retrieval of H2O abundance in Titan's stratosphere: A (re)analysis of CIRS/Cassini and PACS/Herschel observations}},
    year = {2018},
    journal = {Icarus},
    author = {Bauduin, S. and Irwin, P. G.J. and Lellouch, E. and Cottini, V. and Moreno, R. and Nixon, C. A. and Teanby, N. A. and Ansty, T. and Flasar, F. M.},
    pages = {288--305},
    volume = {311},
    publisher = {Elsevier Inc.},
    url = {https://doi.org/10.1016/j.icarus.2018.04.003},
    doi = {10.1016/j.icarus.2018.04.003},
    issn = {10902643},
    keywords = {Atmosphere, Infrared observations, Satellite, Spectroscopy, Titan, atmosphere, composition}
}

@article{Pappalardo2012,
    title = {{Revealing Europa’s Ocean The Galilean Satellites : January 1610}},
    year = {2012},
    author = {Pappalardo, Robert T}
}

@article{Coll1999,
    title = {{Review and latest results of laboratory investigations of Titan's aerosols.}},
    year = {1998},
    journal = {Origins of life and evolution of the biosphere : the journal of the International Society for the Study of the Origin of Life},
    author = {Coll, P and Coscia, D and Gazeau, M C and Guez, L and Raulin, F},
    pages = {195--213},
    volume = {28},
    url = {http://dx.doi.org/10.1023/A:1006521601133},
    isbn = {0169-6149 (Print)},
    doi = {10.1023/A:1006521601133},
    issn = {1573-0875},
    pmid = {11536864}
}

@article{Jolly2014,
    title = {{Revised infrared bending mode intensities for diacetylene (C4H2): Application to Titan}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Jolly, A and Manceron, L and Kwabia-tchana, F and Benilan, Y and Gazeau, M},
    pages = {60--64},
    volume = {97},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2014.03.020},
    doi = {10.1016/j.pss.2014.03.020},
    issn = {0032-0633},
    keywords = {Band intensities, Diacetylene, Far infrared, Titan}
}

@article{Charnoz2012a,
    title = {{Rings in the Solar System : a short review}},
    year = {2012},
    journal = {Handbooks of Exoplanets},
    author = {Charnoz, Sébastien and Crida, Aurélien and Hyodo, Ryuki},
    number = {1},
    volume = {4}
}

@article{Liu2016a,
    title = {{Role of fluids in the tectonic evolution of Titan}},
    year = {2016},
    journal = {Icarus},
    author = {Liu, Zac Yung Chun and Radebaugh, Jani and Harris, Ron A. and Christiansen, Eric H. and Rupper, Summer},
    pages = {2--13},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.02.016},
    doi = {10.1016/j.icarus.2016.02.016},
    issn = {10902643},
    keywords = {Geological processes, Tectonics, Titan, hydrology, Titan, surface}
}

@article{Imanaka2007,
    title = {{Role of photoionization in the formation of complex organic molecules in Titan's upper atmosphere}},
    year = {2007},
    journal = {Geophysical Research Letters},
    author = {Imanaka, Hiroshi and Smith, Mark A.},
    number = {2},
    pages = {1--5},
    volume = {34},
    isbn = {0094-8276},
    doi = {10.1029/2006GL028317},
    issn = {00948276}
}

@article{Brogi2016,
    title = {{ROTATION AND WINDS OF EXOPLANET HD 189733b MEASURED WITH HIGH-DISPERSION TRANSMISSION SPECTROSCOPY}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Brogi, M and De Kok, R J and Albrecht, S and Snellen, I A G and Birkby, J L and Schwarz, H},
    number = {2},
    pages = {106},
    volume = {817},
    publisher = {IOP Publishing},
    url = {http://dx.doi.org/10.3847/0004-637X/817/2/106},
    doi = {10.3847/0004-637X/817/2/106},
    issn = {1538-4357},
    keywords = {planets and satellites: atmospheres, planets and satellites: fundamental parameters, planets and satellites: individual (HD 189733 b), techniques: spectroscopic}
}

@article{Douglas1952,
    title = {{Rotation--vibration spectra of diatomic and simple polyatomic molecules with long absorbing paths. IX.{\~{}}The spectra of the HCN and DCN molecules from 2.5{\~{}}{$\mu$} to 0.5{\~{}}{$\mu$}}},
    year = {1952},
    author = {Douglas, A E and Sharma, D},
    pages = {448--458},
    volume = {21},
    doi = {10.1063/1.1698927},
    issn = {00219606}
}

@article{Bills2011a,
    title = {{Rotational dynamics and internal structure of Titan}},
    year = {2011},
    journal = {Icarus},
    author = {Bills, Bruce G. and Nimmo, Francis},
    number = {1},
    pages = {351--355},
    volume = {214},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.04.028},
    doi = {10.1016/j.icarus.2011.04.028},
    issn = {00191035},
    keywords = {Rotational dynamics}
}

@article{Lewis1971b,
    title = {{Satellites of the Outer Planets : Thermal Models Runoff of Deicing Salt : Effect on Irondequoit Bay , Rochester , New York}},
    year = {1971},
    journal = {Science},
    author = {Lewis, J.},
    pages = {1127--1128},
    volume = {172}
}

@article{Lewis1971a,
    title = {{Satellites of the outer planets: Their physical and chemical nature}},
    year = {1971},
    journal = {Icarus},
    author = {Lewis, J.},
    number = {2},
    pages = {174--185},
    volume = {15},
    doi = {10.1016/0019-1035(71)90072-8},
    issn = {10902643}
}

@article{Dojcansky1974,
    title = {{Saturated vapour pressure of acetonitrile}},
    year = {1974},
    journal = {Chem. Zvesti},
    author = {Dojcansky, J and Heinrich, J},
    number = {September 1973},
    pages = {157--159},
    volume = {28}
}

@article{Lunine2009,
    title = {{Saturn ' s Titan : A Strict Test for Life ' s Cosmic Ubiquity Linked references are available on JSTOR for this article : Saturn ' s Titan : A Strict Test for Life ' s Cosmic Ubiquity1}},
    year = {2009},
    journal = {American Philosphical Society},
    author = {Lunine, Jonathan I},
    number = {4},
    pages = {403--418},
    volume = {153}
}

@article{Hyodo2015,
    title = {{Saturn's F ring and shepherd satellites a natural outcome of satellite system formation}},
    year = {2015},
    journal = {Nature Geoscience},
    author = {Hyodo, Ryuki and Ohtsuki, Keiji},
    number = {9},
    pages = {686--689},
    volume = {8},
    doi = {10.1038/ngeo2508},
    issn = {17520908}
}

@article{Ronnet2018,
    title = {{Saturn's formation and early evolution at the origin of Jupiter's massive moons}},
    year = {2018},
    journal = {The Astronomical Journal},
    author = {Ronnet, Thomas and Mousis, Olivier and Vernazza, Pierre and Lunine, Jonathan I. and Crida, Aurélien},
    number = {5},
    pages = {224},
    volume = {155},
    publisher = {IOP Publishing},
    url = {http://arxiv.org/abs/1804.02892},
    doi = {10.3847/1538-3881/aabcc7},
    issn = {1538-3881},
    arxivId = {1804.02892},
    keywords = {formation, galilean satellites, individual, jupiter, methods, methods: numerical,planets and satellites: formati, numerical, planets and satellites, protoplanetary disks, saturn}
}

@article{Lunine2009b,
    title = {{Saturn's Titan: A Strict Test for Life's Cosmic Ubiquity}},
    year = {2009},
    author = {Lunine, Jonathan},
    pages = {1--30}
}

@article{Nelson2009,
    title = {{Saturn's Titan: Surface change, ammonia, and implications for atmospheric and tectonic activity}},
    year = {2009},
    journal = {Icarus},
    author = {Nelson, R. M. and Kamp, L. W. and Matson, D. L. and Irwin, P. G J and Baines, K. H. and Boryta, M. D. and Leader, F. E. and Jaumann, R. and Smythe, W. D. and Sotin, C. and Clark, R. N. and Cruikshank, D. P. and Drossart, P. and Pearl, J. C. and Hapke, B. W. and Lunine, J. and Combes, M. and Bellucci, G. and Bibring, J. P. and Capaccioni, F. and Cerroni, P. and Coradini, A. and Formisano, V. and Filacchione, G. and Langevin, R. Y. and McCord, T. B. and Mennella, V. and Nicholson, P. D. and Sicardy, B.},
    number = {2},
    pages = {429--441},
    volume = {199},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2008.08.013},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2008.08.013},
    issn = {00191035},
    keywords = {Ices, Infrared observations, Spectrophotometry, Spectroscopy, Titan}
}

@article{Belenkaya2006,
    title = {{Saturn’s aurora in the January 2004 events}},
    year = {2006},
    journal = {Annales Geophysicae},
    author = {Belenkaya, E S and Cowley, S W H and Alexeev, I I and Belenkaya, E S and Cowley, S W H and Saturn, I I Alexeev},
    number = {January 2004},
    pages = {1649--1663},
    volume = {24}
}

@article{Bagenal2005,
    title = {{Saturn’s mixed magnetosphere}},
    year = {2005},
    journal = {Nature},
    author = {Bagenal, Fran},
    number = {February 1955},
    pages = {695--696},
    volume = {433}
}

@article{Lee2015a,
    title = {{Scale height — A parameter for characterizing atmosphere}},
    year = {2015},
    journal = {The Physics Teacher},
    author = {Lee, Kevin M and Ryan, Dominic M},
    number = {2},
    pages = {122--123},
    volume = {53},
    url = {http://scitation.aip.org/content/aapt/journal/tpt/53/2/10.1119/1.4905820},
    doi = {doi:http://dx.doi.org/10.1119/1.4905820},
    issn = {19434928},
    keywords = {atmosphere, exponential, physics education, scaleheight, teaching}
}

@article{Gudipati1995,
    title = {{Schumann-Runge bands of O2 in Ar, Kr and Xe matrices revisited: potential curves of the B 3??u- state}},
    year = {1995},
    journal = {Chemical Physics},
    author = {Gudipati, Murthy S.},
    number = {2-3},
    pages = {451--462},
    volume = {201},
    doi = {10.1016/0301-0104(95)00273-1},
    issn = {03010104}
}

@article{Pappalardo2015,
    title = {{Science and Reconnaissance from the Europa Clipper Mission Concept: Exploring Europa's Habitability}},
    year = {2015},
    author = {Pappalardo, Robert T. and Senske, D and Prockter, L M and Paczkowski, B. and Vance, S and Goldstein, B. and Magner, T and Cooke, B C},
    pages = {2347}
}

@article{Tobie2014,
    title = {{Science goals and mission concept for the future exploration of Titan and Enceladus}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Tobie, G. and Teanby, N. A. and Coustenis, A. and Jaumann, R. and Raulin, F. and Schmidt, J. and Carrasco, N. and Coates, A. J. and Cordier, D. and De Kok, R. and Geppert, W. D. and Lebreton, J. P. and Lefevre, A. and Livengood, T. A. and Mandt, K. E. and Mitri, G. and Nimmo, F. and Nixon, C. A. and Norman, L. and Pappalardo, R. T. and Postberg, F. and Rodriguez, S. and Schulze-Makuch, D. and Soderblom, J. M. and Solomonidou, A. and Stephan, K. and Stofan, E. R. and Turtle, E. P. and Wagner, R. J. and West, R. A. and Westlake, J. H.},
    number = {PA},
    pages = {59--77},
    volume = {104},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2014.10.002},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2014.10.002},
    issn = {00320633},
    keywords = {Atmosphere, Enceladus, Interior, Missions, Ocean, Surface, Titan}
}

@article{Pappalardo2013,
    title = {{Science potential from a Europa lander.}},
    year = {2013},
    journal = {Astrobiology},
    author = {Pappalardo, R T and Vance, S and Bagenal, F and Bills, B G and Blaney, D L and Blankenship, D D and Brinckerhoff, W B and Connerney, J E P and Hand, K P and Hoehler, T M and Leisner, J S and Kurth, W S and McGrath, M a and Mellon, M T and Moore, J M and Patterson, G W and Prockter, L M and Senske, D a and Schmidt, B E and Shock, E L and Smith, D E and Soderlund, K M},
    number = {8},
    pages = {740--73},
    volume = {13},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/23924246},
    isbn = {1557-8070 (Electronic){\textbackslash}r1557-8070 (Linking)},
    doi = {10.1089/ast.2013.1003},
    issn = {1557-8070},
    pmid = {23924246},
    keywords = {Exobiology, Geology, Jupiter, Oceans and Seas, Space Flight}
}

@article{Mousis2014,
    title = {{Scientific rationale for Saturn's in situ exploration}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Mousis, O. and Fletcher, L. N. and Lebreton, J. P. and Wurz, P. and Cavali??, T. and Coustenis, A. and Courtin, R. and Gautier, D. and Helled, R. and Irwin, P. G J and Morse, A. D. and Nettelmann, N. and Marty, B. and Rousselot, P. and Venot, O. and Atkinson, D. H. and Waite, J. H. and Reh, K. R. and Simon, A. A. and Atreya, S. and Andr??, N. and Blanc, M. and Daglis, I. A. and Fischer, G. and Geppert, W. D. and Guillot, T. and Hedman, M. M. and Hueso, R. and Lellouch, E. and Lunine, J. I. and Murray, C. D. and O'Donoghue, J. and Rengel, M. and S??nchez-Lavega, A. and Schmider, F. X. and Spiga, A. and Spilker, T. and Petit, J. M. and Tiscareno, M. S. and Ali-Dib, M. and Altwegg, K. and Bolton, S. J. and Bouquet, A. and Briois, C. and Fouchet, T. and Guerlet, S. and Kostiuk, T. and Lebleu, D. and Moreno, R. and Orton, G. S. and Poncy, J.},
    number = {PA},
    pages = {29--47},
    volume = {104},
    doi = {10.1016/j.pss.2014.09.014},
    issn = {00320633},
    arxivId = {arXiv:1404.4811v1},
    keywords = {Elemental and isotopic composition, Entry probe, Giant planet formation, In situ measurements, Saturn atmosphere, Solar system formation}
}

@article{Kuan2004,
    title = {{Searches for interstellar molecules of potential prebiotic importance}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Kuan, Yi Jehng and Charnley, Steven B. and Huang, Hui Chun and Kisiel, Zbigniew and Ehrenfreund, Pascale and Tseng, Wei Ling and Yan, Chi Hung},
    number = {1},
    pages = {31--39},
    volume = {33},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2003.04.004},
    issn = {02731177},
    keywords = {Astrobiology, ISM: Abundances, ISM: Individual (Orion Kleinmann-Low, Sagittarius, ISM: Molecules, Line: Identification, Radio Lines: ISM}
}

@article{Hofstadter2003,
    title = {{Seasonal change in the deep atmosphere of Uranus}},
    year = {2003},
    journal = {Icarus},
    author = {Hofstadter, Mark D. and Butler, Bryan J.},
    number = {1},
    pages = {168--180},
    volume = {165},
    doi = {10.1016/S0019-1035(03)00174-X},
    issn = {00191035},
    keywords = {Giant planet, Microwave, Uranus}
}

@article{Teanby2010,
    title = {{SEASONAL CHANGES IN TITAN'S POLAR TRACE GAS ABUNDANCE OBSERVED BY <i>CASSINI</i>}},
    year = {2010},
    journal = {The Astrophysical Journal},
    author = {Teanby, N. A. and Irwin, P. G. J. and de Kok, R. and Nixon, C. A.},
    number = {1},
    pages = {L84-L89},
    volume = {724},
    url = {http://stacks.iop.org/2041-8205/724/i=1/a=L84?key=crossref.3b97b6c7e947e493f44cf0804b9d0772},
    doi = {10.1088/2041-8205/724/1/L84},
    issn = {2041-8205},
    keywords = {atmospheres, color figures, machine-readable table, online-only material, planets and satellites}
}

@article{Jennings2012a,
    title = {{Seasonal disappearance of far-infrared haze in Titan's stratosphere}},
    year = {2012},
    journal = {Astrophysical Journal Letters},
    author = {Jennings, Donald E. and Anderson, C. M. and Samuelson, R. E. and Flasar, F. M. and Nixon, C. A. and Kunde, V. G. and Achterberg, R. K. and Cottini, V. and De Kok, R. and Coustenis, A. and Vinatier, S. and Calcutt, S. B.},
    number = {1},
    pages = {1--4},
    volume = {754},
    isbn = {doi:10.1088/2041-8205/754/1/L3},
    doi = {10.1088/2041-8205/754/1/L3},
    issn = {20418205},
    keywords = {molecular processes, planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: individual (Titan), radiation mechanisms: thermal}
}

@article{Moses2018,
    title = {{Seasonal Stratospheric Photochemistry on Uranus and Neptune}},
    year = {2018},
    journal = {Icarus},
    author = {Moses, Julianne I. and Fletcher, Leigh N. and Greathouse, Thomas K. and Orton, Glenn S. and Hue, Vincent},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103517307935},
    doi = {10.1016/j.icarus.2018.02.004},
    issn = {00191035},
    arxivId = {1803.10338}
}

@article{Karkoschka2016,
    title = {{Seasonal variation of Titan's haze at low and high altitudes from HST-STIS spectroscopy}},
    year = {2016},
    journal = {Icarus},
    author = {Karkoschka, Erich},
    pages = {339--354},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.07.007},
    doi = {10.1016/j.icarus.2015.07.007},
    issn = {10902643},
    keywords = {Atmospheres, Satellites, atmospheres, Titan, atmosphere, dynamics, structure}
}

@article{Vinatier2015,
    title = {{Seasonal variations in Titan's middle atmosphere during the northern spring derived from Cassini/CIRS observations}},
    year = {2015},
    journal = {Icarus},
    author = {Vinatier, Sandrine and B{\'{e}}zard, Bruno and Lebonnois, Sébastien and Teanby, Nick A. and Achterberg, Richard K. and Gorius, Nicolas and Mamoutkine, Andrei and Guandique, Ever and Jolly, Antoine and Jennings, Donalds E. and Flasar, F. Michael},
    pages = {95--115},
    volume = {250},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.11.019},
    doi = {10.1016/j.icarus.2014.11.019},
    issn = {10902643},
    keywords = {Atmospheres, composition, Atmospheres, structure, Infrared observations, Titan, atmosphere}
}

@article{Teanby,
    title = {{Seasonal variations in Titan’s atmospheric composition : observations and implications}},
    author = {Teanby, Nicholas}
}

@article{Lebonnois2001,
    title = {{Seasonal Variations of Titan's Atmospheric Composition}},
    year = {2001},
    journal = {Icarus},
    author = {Lebonnois, S. and Toublanc, D. and Hourdin, F. and Rannou, P.},
    number = {2},
    pages = {384--406},
    volume = {152},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103501966321},
    isbn = {0019-1035},
    doi = {10.1006/icar.2001.6632},
    issn = {00191035},
    keywords = {atmospheres, been developed, composition, dynamics, of titan, photochemistry, photochemistry in the atmosphere, several photochemical models have, titan, to understand the complex}
}

@article{Crespin2005,
    title = {{Seasonal variations of Titan’s stratospheric composition in the LMD/SA Global ClimateModel}},
    year = {2005},
    journal = {Bull. Am. Astron. Soc.},
    author = {Crespin, A. and Lebonnois, S. and Hourdin, F. and Rannou, P.},
    volume = {37, 718}
}

@article{Correia2009,
    title = {{Secular evolution of a satellite by tidal effect. application to triton.}},
    year = {2009},
    journal = {The Astrophysical Journal Letters},
    author = {Correia, Alexandre C M},
    number = {3},
    arxivId = {arXiv:0909.4210v1}
}

@article{Correia2009b,
    title = {{Secular Evolution of a Satellite By Tidal Effect: Application To Triton}},
    year = {2009},
    journal = {The Astrophysical Journal},
    author = {Correia, Alexandre C. M.},
    number = {1},
    pages = {L1-L4},
    volume = {704},
    url = {http://stacks.iop.org/1538-4357/704/i=1/a=L1},
    doi = {10.1088/0004-637X/704/1/L1},
    issn = {0004-637X},
    arxivId = {0909.4210},
    keywords = {analytical, celestial mechanics, general, individual, methods, neptune, planets and satellites, triton}
}

@article{Pappalardo2010,
    title = {{Seeking Europa's Ocean}},
    year = {2010},
    journal = {Proceedings of the International Astronomical Union},
    author = {Pappalardo, Robert T.},
    number = {S269},
    pages = {101--114},
    volume = {6},
    url = {http://www.journals.cambridge.org/abstract_S1743921310007325},
    doi = {10.1017/S1743921310007325},
    issn = {1743-9213},
    keywords = {and the copernican revolution, center, changed our sense of, claim, convection, europa, figure 1, four galilean moons of, four hundred years ago, habitability, ice, jupiter forever, no longer could humans, ocean, place in the universe, the discovery of the, to be at its, today one of those, was underway}
}

@article{Beghin2015,
    title = {{Self-consistent modeling of induced magnetic field in Titan's atmosphere accounting for the generation of Schumann resonance}},
    year = {2015},
    journal = {Icarus},
    author = {B{\'{e}}ghin, Christian},
    pages = {126--136},
    volume = {247},
    doi = {10.1016/j.icarus.2014.10.005},
    issn = {10902643},
    keywords = {Magnetic fields, Saturn, magnetosphere, Titan, atmosphere, Titan, surface}
}

@article{Hebrard2005,
    title = {{Sensitivity effects of photochemical parameters uncertainties on hydrocarbon production in the atmosphere of Titan}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {H{\'{e}}brard, E. and B{\'{e}}nilan, Y. and Raulin, F.},
    number = {2},
    pages = {268--273},
    volume = {36},
    doi = {10.1016/j.asr.2005.03.093},
    issn = {02731177},
    keywords = {Atmospheric composition, Monte-Carlo calculations, Photochemistry, Titan}
}

@article{Carrasco2008,
    title = {{Sensitivity of a Titan ionospheric model to the ion-molecule reaction parameters}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Carrasco, N. and Alcaraz, C. and Dutuit, O. and Plessis, S. and Thissen, R. and Vuitton, V. and Yelle, R. and Pernot, P.},
    number = {12},
    month = {11},
    pages = {1644--1657},
    volume = {56},
    url = {http://www.sciencedirect.com/science/article/pii/S0032063308001025},
    doi = {10.1016/j.pss.2008.04.007},
    issn = {00320633},
    keywords = {Branching ratio, Ion-molecule reaction, Ionospheric chemistry model, Sensitivity analysis, Titan, Uncertainty propagation}
}

@article{Muntener2010,
    title = {{Serpentine and serpentinization: A link between planet formation and life}},
    year = {2010},
    journal = {Geology},
    author = {M{\"{u}}ntener, Othmar},
    number = {10},
    pages = {959--960},
    volume = {38},
    doi = {10.1130/focus102010.1},
    issn = {00917613}
}

@article{Nimmo2007,
    title = {{Shear heating as the origin of the plumes and heat flux on Enceladus.}},
    year = {2007},
    journal = {Nature},
    author = {Nimmo, F and Spencer, J R and Pappalardo, R T and Mullen, M E},
    number = {7142},
    pages = {289--291},
    volume = {447},
    isbn = {0028-0836},
    doi = {10.1038/nature05783},
    issn = {0028-0836},
    pmid = {17507976}
}

@misc{Scattergood1987,
    title = {{Shock formation of N2 and organic compounds in a primodrial NH3-CH4 atmosphere on Titan}},
    year = {1987},
    author = {Scattergood, T W and Mckay, C P and Pollack, J. B. and Borucki, W. J. and van Ghyseghem, H. T.}
}

@article{Vuitton2018,
    title = {{Simulating the density of organic species in the atmosphere of Titan with a coupled ion-neutral photochemical model}},
    year = {2018},
    journal = {Icarus},
    author = {Vuitton, V and Yelle, R V and Klippenstein, S J},
    number = {iii},
    keywords = {atmosphere, atmospheres, chemistry, ionospheres, organic chemistry, photochemistry, titan}
}

@article{Salz2016,
    title = {{Simulating the escaping atmospheres of hot gas planets in the solar neighborhood}},
    year = {2016},
    journal = {Astronomy {\&} Astrophysics},
    author = {Salz, M. and Czesla, S. and Schneider, P. C. and Schmitt, J. H. M. M.},
    pages = {A75},
    volume = {586},
    url = {http://arxiv.org/abs/1511.09341%5Cnhttp://www.aanda.org/10.1051/0004-6361/201526109},
    doi = {10.1051/0004-6361/201526109},
    issn = {0004-6361},
    arxivId = {1511.09341},
    keywords = {and satellites, atmospheres, dynamical evolution and stability, general, hydrodynamics, methods, numerical, planets, planets and satellites, radiation mechanisms}
}

@article{Bell2010,
    title = {{Simulating the one-dimensional structure of Titan's upper atmosphere: 1. Formulation of the Titan Global Ionosphere-Thermosphere Model and benchmark simulations}},
    year = {2010},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Bell, Jared M. and Bougher, Stephen W. and Waite, J. Hunter and Ridley, Aaron J. and Magee, Brian A. and Mandt, Kathleen E. and Westlake, Joseph and DeJong, Anna D. and Bar-Nun, Akiva and Jacovi, Ronen and Toth, Gabor and De La Haye, Virginie},
    number = {12},
    pages = {1--20},
    volume = {115},
    doi = {10.1029/2010JE003636},
    issn = {01480227},
    keywords = {http://dx.doi.org/10.1029/2010JE003636, doi:10.102}
}

@article{Larson2014,
    title = {{Simulating Titan's aerosols in a three dimensional general circulation model}},
    year = {2014},
    journal = {Icarus},
    author = {Larson, Erik J L and Toon, Owen B. and Friedson, Andrew J.},
    pages = {400--419},
    volume = {243},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.09.003},
    doi = {10.1016/j.icarus.2014.09.003},
    issn = {10902643},
    keywords = {Atmospheres, dynamics, Atmospheres, structure, Titan, atmosphere}
}

@article{Newman2016,
    title = {{Simulating Titan's methane cycle with the TitanWRF General Circulation Model}},
    year = {2016},
    journal = {Icarus},
    author = {Newman, Claire E. and Richardson, Mark I. and Lian, Yuan and Lee, Christopher},
    pages = {106--134},
    volume = {267},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.11.028},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2015.11.028},
    issn = {10902643},
    keywords = {Atmospheres dynamics, Atmospheres structure, Meteorology, Titan, Titan atmosphere}
}

@article{Godinho2014,
    title = {{Simulation of surface dynamics during dissolution as a function of the surface orientation: Implications for non-constant dissolution rates}},
    year = {2014},
    journal = {Earth and Planetary Science Letters},
    author = {Godinho, J. R A and Piazolo, S. and Evans, L.},
    pages = {163--170},
    volume = {408},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.epsl.2014.10.018},
    doi = {10.1016/j.epsl.2014.10.018},
    issn = {0012821X},
    keywords = {Dissolution, Kinetics, Modeling, Rate constant, Surface, Topography}
}

@article{Couturier-Tamburelli2015,
    title = {{Simulation of Titan’s atmospheric photochemistry Formation of non-volatile residue from polar nitrile ices}},
    year = {2015},
    journal = {Astronomy and Astrophysics},
    author = {Couturier-Tamburelli, I. and Pi{\'{e}}tri, N. and Gudipati, M.},
    volume = {111},
    doi = {10.1051/0004-6361/201425518},
    issn = {14320746},
    keywords = {astrochemistry, atmospheres, planetary systems, planets and satellites, planets and satellites: atmospheres, planets and satellites: surfaces, surfaces, ultraviolet, ultraviolet: planetary systems}
}

@article{Poppe2010,
    title = {{Simulations of the photoelectron sheath and dust levitation on the lunar surface}},
    year = {2010},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Poppe, Andrew and Hor{\'{a}}nyi, Miáhly},
    number = {8},
    pages = {1--9},
    volume = {115},
    isbn = {0148-0227},
    doi = {10.1029/2010JA015286},
    issn = {21699402}
}

@article{Minaev2004,
    title = {{Singlet-triplet transitions in three-atomic molecules studied by time-dependent MCSCF and density functional theory}},
    year = {2004},
    journal = {Molecular Physics},
    author = {Minaev, Boris and Tunell, Ingvar and Salek, Pawel and Loboda, Oleksandr and Vahtras, Olav and {\AA}gren, Hans},
    number = {13},
    pages = {1391--1406},
    volume = {102},
    isbn = {0026-8976},
    doi = {10.1080/00268970410001668435},
    issn = {00268976}
}

@article{Redfield2007,
    title = {{Sodium Absorption From the Exoplanetary Atmosphere of HD189733b Detected in the Optical Transmission Spectrum}},
    year = {2008},
    journal = {The Astrophysical Journal},
    author = {Redfield, Seth and Endl, Michael and Cochran, William D. and Koesterke, Lars},
    number = {1},
    pages = {12},
    volume = {673},
    url = {http://arxiv.org/abs/0712.0761%5Cnhttp://stacks.iop.org/1538-4357/673/i=1/a=L87},
    doi = {10.1086/527475},
    issn = {0004-637X},
    arxivId = {0712.0761}
}

@article{Edberg2013a,
    title = {{Solar cycle modulation of Titan's ionosphere}},
    year = {2013},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Edberg, N. J T and Andrews, D. J. and Shebanits, O. and {\AA}gren, K. and Wahlund, J. E. and Opgenoorth, H. J. and Cravens, T. E. and Girazian, Z.},
    number = {8},
    pages = {5255--5264},
    volume = {118},
    doi = {10.1002/jgra.50463},
    issn = {21699402},
    keywords = {Cassini, Titan, ionosphere, solar cycle}
}

@article{Madanian2016,
    title = {{Solar cycle variations in ion composition in the dayside ionosphere of Titan}},
    year = {2016},
    author = {Madanian, H and Cravens, T E and Richard, M S and Waite, J H and Edberg, N J T and Westlake, J H and Wahlund, J},
    pages = {8013--8037},
    doi = {10.1002/2015JA022274.Received},
    keywords = {10.1002/2015JA022274 and solar cycle, Cassini INMS, Titan, ion density, planetary ionospheres}
}

@article{Capalbo2015,
    title = {{Solar Occultation by Titan Measured by CASSINI/UVIS}},
    year = {2015},
    author = {Capalbo, Fernando J and Yves, B and Yelle, Roger V and Koskinen, Tommi T and Sandel, R and Holsclaw, Gregory M and Mcclintock, William E and Capalbo, Fernando J and Yves, B and Yelle, Roger V and Koskinen, Tommi T and Bill, R}
}

@article{Bunce,
    title = {{Solar System Ice Giants : Exoplanets in our Backyard .}},
    author = {Bunce, Emma and Arridge, Christopher and Masters, Adam and Hofstadter, Mark and Hospodarsky, George and Kurth, William and Romani, Paul and Lamy, Laurent and Zarka, Philippe},
    pages = {1--6},
    volume = {1}
}

@article{Anderson2016,
    title = {{Solid-state chemistry as a formation mechanism for Titan's stratospheric C4N2 ice clouds}},
    year = {2016},
    journal = {Geophysical Research Letters},
    author = {Anderson, C. M. and Samuelson, R. E. and Yung, Y. L. and McLain, J. L.},
    pages = {n/a-n/a},
    url = {http://doi.wiley.com/10.1002/2016GL067795},
    doi = {10.1002/2016GL067795},
    issn = {00948276},
    keywords = {10.1002/2016GL067795 and solid-state chemistry, far infrared, ice formation, radiative transfer, remote sensing}
}

@article{Baughman1987,
    title = {{Solid-State Polymerization of Diacetylenes.}},
    year = {1987},
    journal = {American Chemical Society, Polymer Preprints, Division of Polymer Chemistry},
    author = {Baughman, R. H.},
    number = {2},
    pages = {445--446},
    volume = {28},
    isbn = {0021-8979},
    doi = {10.1063/1.1660929},
    issn = {00323934}
}

@article{Barnett2016,
    title = {{Solubility and Reactivity of Tholins in Liquid Hydrocarbons on Titan}},
    year = {2016},
    journal = {LPSC2016},
    author = {Barnett, K. N. and Chevrier, V. F.},
    pages = {1--2},
    volume = {1814}
}

@article{Garvey1988,
    title = {{Solvated NH5+ formed within ionized clusters of ammonia and ammonia-benzene}},
    year = {1988},
    journal = {Chemical Physics Letters},
    author = {Garvey, James F and Bernstein, Richard B},
    number = {1},
    pages = {13--18},
    volume = {143}
}

@article{Edwards2009,
    title = {{Some ion chemistry of HC5N}},
    year = {2009},
    journal = {International Journal of Mass Spectrometry},
    author = {Edwards, Samuel J. and Freeman, Colin G. and McEwan, Murray J.},
    number = {2-3},
    pages = {82--86},
    volume = {279},
    isbn = {13873806},
    doi = {10.1016/j.ijms.2008.10.003},
    issn = {13873806},
    keywords = {Cyanopolyynes, HC5N, Proton affinity, SIFT, Titan}
}

@article{StetefeldtC.A.1896,
    title = {{Some large perturbations in the motions of celestrial bodies}},
    year = {1896},
    journal = {Astronomical Society of the Pacific},
    author = {{Stetefeldt C. A.}},
    number = {34},
    pages = {67--68},
    volume = {6}
}

@article{Ainslie2016,
    title = {{Sonar equations for planetary exploration}},
    year = {2016},
    author = {Ainslie, Michael A and Leighton, Timothy G},
    number = {2},
    volume = {140},
    url = {http://dx.doi.org/10.1121/1.4960786},
    doi = {10.1121/1.4960786},
    issn = {00014966}
}

@article{Lombardo2019,
    title = {{Spatial and seasonal variations in C3Hxhydrocarbon abundance in Titan's stratosphere from Cassini CIRS observations}},
    year = {2019},
    journal = {Icarus},
    author = {Lombardo, Nicholas A. and Nixon, Conor A. and Achterberg, Richard K. and Jolly, Antoine and Sung, Keeyoon and Irwin, Patrick G.J. and Flasar, F. Michael},
    pages = {454--469},
    volume = {317},
    doi = {10.1016/j.icarus.2018.08.027},
    issn = {10902643},
    arxivId = {1809.04102},
    keywords = {Atmospheres, Atmospheres–Infrared Observations–Satellites, Atmosphere–Abundances, Titan}
}

@article{Beuthe2013,
    title = {{Spatial patterns of tidal heating}},
    year = {2013},
    journal = {Icarus},
    author = {Beuthe, Mikael},
    number = {1},
    pages = {308--329},
    volume = {223},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.11.020},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2012.11.020},
    issn = {00191035},
    arxivId = {1212.4630},
    keywords = {Europa, Io, Planetary dynamics, Tides, Solid body, Titan}
}

@article{Thelen2017,
    title = {{Spatial variations in Titan's atmospheric temperature: ALMA and Cassini comparisons from 2012 to 2015}},
    year = {2017},
    journal = {Icarus},
    author = {Thelen, Alexander E. and Nixon, C. A. and Chanover, N. J. and Molter, E. M. and Cordiner, M. A. and Achterberg, R. K. and Serigano, J. and Irwin, P. G.J. and Teanby, N. and Charnley, S. B.},
    pages = {1--11},
    volume = {0},
    publisher = {Elsevier Inc.},
    doi = {10.1016/j.icarus.2017.10.042},
    issn = {10902643},
    keywords = {Atmosphere, Atmospheres, Dynamics, Radiative transfer, Radio observations, Spectroscopy, Titan}
}

@article{Louden2015,
    title = {{SPATIALLY RESOLVED EASTWARD WINDS AND ROTATION OF HD 189733b}},
    year = {2015},
    journal = {The Astrophysical Journal},
    author = {Louden, Tom and Wheatley, Peter J.},
    number = {2},
    pages = {L24},
    volume = {814},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/2041-8205/814/i=2/a=L24?key=crossref.8da74ff16df90e615d23c791d2596b16},
    doi = {10.1088/2041-8205/814/2/L24},
    issn = {2041-8213},
    arxivId = {1511.03689},
    keywords = {atmospheres, atmospheric effects, celestial mechanics, hd 189733, hd 189733b, individual, planets and satellites, planets and satellites: atmospheres, planets and satellites: individual (HD 189733b), spectroscopic, stars, stars: individual (HD 189733), techniques, techniques: spectroscopic}
}

@article{Combes1997,
    title = {{Spatially Resolved Images of Titan by Means of Adaptive Optics}},
    year = {1997},
    journal = {Icarus},
    author = {Combes, M},
    number = {2},
    pages = {482--497},
    volume = {129},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103597957729},
    doi = {10.1006/icar.1997.5772},
    issn = {00191035}
}

@article{Adamkovics2004,
    title = {{Spatially-resolved spectroscopy at 1.6 {$\mu$}m of titan's atmosphere and surface}},
    year = {2004},
    journal = {Geophysical Research Letters},
    author = {{\'{A}}d{\'{a}}mkovics, M. and de Pater, I. and Roe, H. G. and Gibbard, S. G. and Griffith, C. A.},
    number = {17},
    pages = {1--4},
    volume = {31},
    doi = {10.1029/2004GL019929},
    issn = {00948276},
    keywords = {0305 Atmospheric composition and structure: Aeroso, 0317 Atmospheric composition and structure: Chemic, 0320 Atmospheric composition and structure: Cloud, 0343 Atmospheric composition and structure: Planet, 5494 Planetology: Solid surface planets: Instrumen}
}

@article{Neufeld2012,
    title = {{Special feature Discovery of interstellar mercapto radicals ( SH ) with the GREAT instrument on SOFIA}},
    year = {2012},
    author = {Neufeld, D A and Falgarone, E and Gerin, M and Godard, B and Herbst, E and For{\^{e}}ts, G Pineau and Vasyunin, A I and G{\"{u}}sten, R and Wiesemeyer, H and Ricken, O},
    pages = {1--4},
    volume = {6},
    keywords = {astrochemistry, clouds, ism, molecular processes, molecules, submillimeter}
}

@article{Wu2012,
    title = {{Spectra and Photolysis of Pure Nitrogen and Methane Dispersed in Solid Nitrogen With Vacuum-Ultraviolet Light}},
    year = {2012},
    journal = {The Astrophysical Journal},
    author = {Wu, Yu-Jong and Wu, C. Y. Robert and Chou, Sheng-Lung and Lin, Meng-Yeh and Lu, Hsiao-Chi and Lo, Jen-Iu and Cheng, Bing-Ming},
    number = {2},
    pages = {175},
    volume = {746},
    url = {http://stacks.iop.org/0004-637X/746/i=2/a=175?key=crossref.8db0972b34adefa1ac2d8dc201523312},
    doi = {10.1088/0004-637X/746/2/175},
    issn = {0004-637X},
    keywords = {astrochemistry, color figures, infrared, ism, laboratory, methods, molecular processes, molecules, online-only material}
}

@article{Bobrovnikoff1944,
    title = {{Spectra of the planets}},
    year = {1944},
    journal = {Reviews of Modern Physics},
    author = {Bobrovnikoff, N. T.},
    number = {3-4},
    pages = {271--285},
    volume = {16},
    doi = {10.1103/RevModPhys.16.271},
    issn = {00346861}
}

@article{Wyttenbach2015,
    title = {{Spectrally resolved detection of sodium in the atmosphere of HD 189733b with the HARPS spectrograph}},
    year = {2015},
    journal = {Astronomy {\&} Astrophysics},
    author = {Wyttenbach, A. and Ehrenreich, D. and Lovis, C. and Udry, S. and Pepe, F.},
    pages = {A62},
    volume = {577},
    url = {http://www.aanda.org/articles/aa/full_html/2015/05/aa25729-15/aa25729-15.html},
    doi = {10.1051/0004-6361/201525729},
    issn = {0004-6361},
    arxivId = {1503.05581},
    keywords = {atmospheres, hd 189733b, individual, instrumentation, methods, observational, planets and satellites, spectrographs, spectroscopic, techniques}
}

@article{Joo1999,
    title = {{Spectrophotometric analysis of aluminum nitride thin films}},
    year = {1999},
    journal = {Journal of Vacuum Science {\&} Technology A: Vacuum, Surfaces, and Films},
    author = {Joo, Han-Yong and Kim, Hyeong Joon and Kim, Sang June and Kim, Sang Youl},
    number = {3},
    pages = {862},
    volume = {17},
    doi = {10.1116/1.582035},
    issn = {07342101}
}

@article{Huang2011,
    title = {{Spectroscopic Constants for 13 C and Deuterium Isotopologues of Cyclic and Linear C 3 H 3 +}},
    year = {2011},
    journal = {The Astrophysical Journal},
    author = {Huang, Xinchuan and Lee, Timothy J.},
    number = {1},
    pages = {33},
    volume = {736},
    url = {http://iopscience.iop.org/0004-637X/736/1/33/fulltext/},
    doi = {10.1088/0004-637X/736/1/33},
    issn = {0004-637X},
    pmid = {21510653},
    keywords = {ISM: molecules, astrochemistry, circumstellar matter, molecular data, molecular processes}
}

@article{Couturier-Tamburelli2014,
    title = {{Spectroscopic studies of non-volatile residue formed by photochemistry of solid C4N2: A model of condensed aerosol formation on Titan}},
    year = {2014},
    journal = {Icarus},
    author = {Couturier-Tamburelli, I. and Gudipati, Murthy S. and Lignell, Antti and Jacovi, Ronen and Pi{\'{e}}tri, Nathalie},
    pages = {81--90},
    volume = {234},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.02.016},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.02.016},
    issn = {10902643},
    keywords = {Astrobiology, IR Spectroscopy, Ices, Photochemistry, Prebiotic environments, Titan}
}

@article{Couturier-Tamburelli2014a,
    title = {{Spectroscopic studies of non-volatile residue formed by photochemistry of solid C4N2: A model of condensed aerosol formation on Titan}},
    year = {2014},
    journal = {Icarus},
    author = {Couturier-Tamburelli, I. and Gudipati, Murthy S. and Lignell, Antti and Jacovi, Ronen and Pi{\'{e}}tri, Nathalie},
    number = {October},
    pages = {81--90},
    volume = {234},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.02.016},
    issn = {10902643},
    keywords = {Astrobiology, IR Spectroscopy, Ices, Photochemistry, Prebiotic environments, Titan}
}

@book{Tinetti2013,
    title = {{Spectroscopy of planetary atmospheres in our Galaxy}},
    year = {2013},
    booktitle = {Astronomy and Astrophysics Review},
    author = {Tinetti, Giovanna and Encrenaz, Thérèse and Coustenis, Athena},
    number = {1},
    volume = {21},
    isbn = {0015901300},
    doi = {10.1007/s00159-013-0063-6},
    issn = {09354956},
    keywords = {Extrasolar planets, Radiative transfer, Spectroscopy}
}

@article{Wisdom2004,
    title = {{SPIN-ORBIT SECONDARY RESONANCE DYNAMICS OF ENCELADUS}},
    year = {2004},
    author = {Wisdom, J},
    pages = {484--491},
    keywords = {analytical, celestial mechanics, enceladus, formation, gravitation, individual, methods, mimas, numerical, planets and satellites, saturn}
}

@misc{Johnson1998,
    title = {{Sputter contribution to the atmospheric corona on Mars}},
    year = {1998},
    author = {Johnson, R. E. and Luhmann, J. G.}
}

@article{Lovesday2001b,
    title = {{Stable methane hydrate above 2[thinsp]GPa and the source of Titan's atmospheric methane}},
    year = {2001},
    author = {Loveday, J. S. and Nelmes, R. J. and Guthrie, M. and Belmonte, S. A. and Allan, D. R. and Klug, D. D. and Tse, J. S. and Handa, Y. P.},
    number = {6829},
    pages = {661--663},
    volume = {410},
    url = {http://dx.doi.org/10.1038/35070513},
    doi = {10.1038/35070513},
    issn = {0028-0836}
}

@article{Navarro-Gonzalez2004,
    title = {{Steps toward the origin(s) of life: endogenous sources and chemistry}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Navarro-Gonzalez, Rafael and Raulin, F.},
    number = {1},
    pages = {79--80},
    volume = {33},
    url = {http://www.sciencedirect.com/science/article/B6V3S-4BHJV26-3/2/f7f879d39f79b6e6b126e094bec4b0f7},
    doi = {doi: DOI: 10.1016/j.asr.2003.11.002},
    issn = {0273-1177}
}

@article{Baines2009,
    title = {{Storm clouds on Saturn: Lightning-induced chemistry and associated materials consistent with Cassini/VIMS spectra}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Baines, Kevin H. and Delitsky, Mona L. and Momary, Thomas W. and Brown, Robert H. and Buratti, Bonnie J. and Clark, Roger N. and Nicholson, Philip D.},
    number = {14-15},
    pages = {1650--1658},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.06.025},
    doi = {10.1016/j.pss.2009.06.025},
    issn = {00320633},
    keywords = {Cassini-huygens, Lightning chemistry, Saturn:clouds, Saturn:lightning, Thunderstorm, Visual-infrared mapping spectrometer (VIMS)}
}

@article{Neish2018,
    title = {{Strategies for Detecting Biological Molecules on Titan}},
    year = {2018},
    journal = {Astrobiology},
    author = {Neish, Catherine D. and Lorenz, Ralph D. and Turtle, Elizabeth P. and Barnes, Jason W. and Trainer, Melissa G. and Stiles, Bryan and Kirk, Randolph and Hibbitts, Charles A. and Malaska, Michael J.},
    number = {5},
    pages = {ast.2017.1758},
    volume = {18},
    url = {http://www.liebertpub.com/doi/10.1089/ast.2017.1758},
    doi = {10.1089/ast.2017.1758},
    issn = {1531-1074}
}

@article{Barth2015,
    title = {{Stratospheric Ices in Titan's Atmosphere}},
    year = {2015},
    author = {Barth, E.},
    pages = {2015},
    volume = {10}
}

@article{Tanguy1990,
    title = {{Stratospheric Profile of HCN on Titan from Millimeter Observations}},
    year = {1990},
    author = {Tanguy, Loic and Zard, Bruno B I and Marten, Andri and Gautier, Daniel and Rard, Eric G I and Paubert, Gabriel and Lecacheux, Alain},
    volume = {57}
}

@article{Deming2008,
    title = {{Strong Infrared Emission from the Extrasolar Planet HD189733b}},
    year = {2008},
    journal = {arXiv.org},
    author = {Deming, Drake and Harrington, Joseph and Seager, Sara and Richardson, L Jeremy},
    pages = {2008},
    volume = {astro-ph},
    url = {http://arxiv.org/abs/astro-ph/0602443v1%5Cnpapers3://publication/doi/10.1086/503358},
    doi = {10.1086/503358},
    issn = {0004-637X},
    arxivId = {astro-ph/0602443}
}

@article{Grillmair2008,
    title = {{Strong water absorption in the dayside emission spectrum of the planet HD 189733b.}},
    year = {2008},
    journal = {Nature},
    author = {Grillmair, Carl J and Burrows, Adam and Charbonneau, David and Armus, Lee and Stauffer, John and Meadows, Victoria and van Cleve, Jeffrey and von Braun, Kaspar and Levine, Deborah},
    number = {7223},
    pages = {767--769},
    volume = {456},
    doi = {10.1038/nature07574},
    issn = {0028-0836},
    pmid = {19079054},
    arxivId = {0901.4774}
}

@article{Sohl2014,
    title = {{Structural and tidal models of Titan and inferences on cryovolcanism}},
    year = {2014},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Sohl, F. and Solomonidou, A. and Wagner, F. W. and Coustenis, A. and Hussmann, H. and Schulze-Makuch, D.},
    number = {5},
    pages = {1013--1036},
    volume = {119},
    doi = {10.1002/2013JE004512},
    issn = {21699100},
    keywords = {Astrobiology, Interiors, Tectonics, Titan, Volcanism}
}

@article{Cameron1989,
    title = {{Structure and properties of C3H3+ cations}},
    year = {1989},
    journal = {Journal of Physical Chemistry},
    author = {Cameron, A. and Leszczynski, J. and Zerner, M. C. and Weiner, B.},
    number = {8},
    pages = {143--152}
}

@article{Cordier2016,
    title = {{Structure of Titan's evaporites}},
    year = {2016},
    journal = {Icarus},
    author = {Cordier, D. and Cornet, T. and Barnes, J. W. and MacKenzie, S. M. and Le Bahers, T. and Nna-Mvondo, D. and Rannou, P. and Ferreira, A. G.},
    pages = {41--56},
    volume = {270},
    doi = {10.1016/j.icarus.2015.12.034},
    issn = {10902643},
    keywords = {Satellites, surfaces, Saturn, satellites, Titan, surface}
}

@article{Lopez-Moreno2008,
    title = {{Structure of Titan's low altitude ionized layer from the Relaxation Probe onboard Huygens}},
    year = {2008},
    journal = {Geophysical Research Letters},
    author = {L{\'{o}}pez-Moreno, J. J. and Molina-Cuberos, G. J. and Hamelin, M. and Grard, R. and Simões, F. and Godard, R. and Schwingenschuh, K. and B{\'{e}}ghin, C. and Berthelier, J. J. and Brown, V. J.G. and Falkner, P. and Ferri, F. and Fulchignoni, M. and Jernej, I. and Jer{\'{o}}nimo, J. M. and Rodrigo, R. and Trautner, R.},
    number = {22},
    volume = {35},
    doi = {10.1029/2008GL035338},
    issn = {00948276}
}

@article{Robertson2009,
    title = {{Structure of Titan’s ionosphere : Model comparisons with Cassini data}},
    year = {2009},
    author = {Robertson, I P and Cravens, T E and Jr, J H Waite and Yelle, R V and Vuitton, V and Coates, A J and Wahlund, J E and Agren, K},
    number = {April 2005},
    pages = {1834--1846},
    volume = {57},
    doi = {10.1016/j.pss.2009.07.011}
}

@article{V1984,
    title = {{Structures and reactions of C3H6+ ions generated in cyclopropane}},
    year = {1984},
    journal = {International Journal of Mass Spectrometry and Ion Physics},
    author = {V, Elsevier Science Publishers B and Lias, G and Buckley, J},
    pages = {123--137},
    volume = {56}
}

@article{Mizutani1975,
    title = {{Study of the photochemical reaction of HCN nd its polymer prodcts relating to primary chemical evolution}},
    year = {1975},
    journal = {Origins of Life},
    author = {Mizutani, Hiroshi and Mikuni, Hitoshi and Takahasi, Makoto and Noda, Haruhiko},
    number = {1975},
    pages = {513--525},
    volume = {6}
}

@article{Vinatier2018,
    title = {{Study of Titan's fall southern stratospheric polar cloud composition with Cassini/CIRS: Detection of benzene ice}},
    year = {2018},
    journal = {Icarus},
    author = {Vinatier, S. and Schmitt, B. and B{\'{e}}zard, B. and Rannou, P. and Dauphin, C. and de Kok, R. and Jennings, D. E. and Flasar, F. M.},
    number = {June 2010},
    pages = {1--16},
    volume = {0},
    publisher = {Elsevier Inc.},
    url = {https://doi.org/10.1016/j.icarus.2017.12.040},
    doi = {10.1016/j.icarus.2017.12.040},
    issn = {10902643},
    keywords = {Atmospheres, Infrared observations, Titan, atmosphere, composition, structures}
}

@article{Currie2017,
    title = {{Subaru/SCExAO First-Light Direct Imaging of a Young Debris Disk around HD 36546}},
    year = {2017},
    author = {Currie, Thayne and Guyon, Olivier and Tamura, Motohide and Kudo, Tomoyuki and Jovanovic, Nemanja and Lozi, Julien and Schlieder, Joshua and Brandt, Timothy and Kuhn, Jonas and Serabyn, Eugene and Janson, Markus and Carson, Joseph and Kasdin, Jeremy and Groff, Tyler and McElwain, Michael and Singh, Garima and Uyama, Taichi and Kuzuhara, Masayuki and Akiyama, Eiji and Grady, Carol and Hayashi, Saeko and Knapp, Gillian and Kwon, Jungmi and Oh, Daehyeon and Wisniewski, John and Sitko, Michael and Yang, Yi},
    pages = {1--6},
    url = {http://arxiv.org/abs/1701.02314},
    arxivId = {1701.02314}
}

@article{Fray2009,
    title = {{Sublimation of ices of astrophysical interest: A bibliographic review}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Fray, N. and Schmitt, B.},
    number = {14-15},
    pages = {2053--2080},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.09.011},
    doi = {10.1016/j.pss.2009.09.011},
    issn = {00320633},
    keywords = {Condensation, Ices, Solids, Sublimation, Vapour pressure, Volatiles}
}

@article{Komacek2016,
    title = {{Submitted to The Astrophysical Journal ATMOSPHERIC CIRCULATION OF HOT JUPITERS: DAYSIDE-NIGHTSIDE TEMPERATURE DIFFERENCES}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Komacek, Thaddeus D and Showman, Adam P},
    number = {1},
    pages = {0},
    volume = {821},
    publisher = {IOP Publishing},
    url = {http://dx.doi.org/10.3847/0004-637X/821/1/16},
    doi = {10.3847/0004-637X/821/1/16},
    issn = {1538-4357},
    keywords = {analytical, atmospheres, gaseous planets, hydrodynamics, methods, methods: analytical, methods: numerical, numerical, planets and satellites, planets and satellites: atmospheres, planets and satellites: gaseous planets}
}

@article{Anderson2014,
    title = {{Subsidence-induced methane clouds in Titan's winter polar stratosphere and upper troposphere}},
    year = {2014},
    journal = {Icarus},
    author = {Anderson, C. M. and Samuelson, R. E. and Achterberg, R. K. and Barnes, J. W. and Flasar, F. M.},
    pages = {129--138},
    volume = {243},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.09.007},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.09.007},
    issn = {10902643},
    keywords = {Atmosphere, IR spectroscopy, Ices, Radiative transfer, Titan, clouds}
}

@article{Sohl2010,
    title = {{Subsurface water oceans on icy satellites: Chemical composition and exchange processes}},
    year = {2010},
    journal = {Space Science Reviews},
    author = {Sohl, Frank and Choukroun, Mathieu and Kargel, Jeffrey and Kimura, Jun and Pappalardo, Robert and Vance, Steve and Zolotov, Mikhail},
    number = {1-4},
    pages = {485--510},
    volume = {153},
    isbn = {0038-6308},
    doi = {10.1007/s11214-010-9646-y},
    issn = {00386308},
    keywords = {Callisto, Chemical evolution, Clathrate hydrates, Enceladus, Europa, Ganymede, High-pressure ices, Hydrothermal activity, Oceanic composition, Organic compounds, Outer solar system, Porous rock, Serpentinization, Titan, Water oceans}
}

@article{Ranjan2018,
    title = {{Sulfidic Anion Concentrations on Early Earth for Surficial Origins-of-Life Chemistry}},
    year = {2018},
    author = {Ranjan, Sukrit and Todd, Zoe R. and Sutherland, John D. and Sasselov, Dimitar D.},
    number = {9},
    pages = {1--18},
    volume = {18},
    url = {http://arxiv.org/abs/1801.07725},
    doi = {10.1089/ast.2017.1770},
    issn = {1531-1074},
    arxivId = {1801.07725}
}

@article{Pasek2005,
    title = {{Sulfur chemistry with time-varying oxygen abundance during Solar System formation}},
    year = {2005},
    journal = {Icarus},
    author = {Pasek, Matthew A. and Milsom, John A. and Ciesla, Fred J. and Lauretta, Dante S. and Sharp, Christopher M. and Lunine, Jonathan I.},
    number = {1},
    pages = {1--14},
    volume = {175},
    isbn = {1520621493},
    doi = {10.1016/j.icarus.2004.10.012},
    issn = {00191035},
    keywords = {Cosmochemistry, Jupiter, Meteorites, Solar nebula}
}

@article{Gao2017,
    title = {{Sulfur Hazes in Giant Exoplanet Atmospheres: Impacts on Reflected Light Spectra}},
    year = {2017},
    author = {Gao, Peter and Marley, Mark S and Zahnle, Kevin and Robinson, Tyler D and Lewis, Nikole K},
    pages = {1--15},
    url = {http://arxiv.org/abs/1701.00318},
    arxivId = {1701.00318},
    keywords = {atmospheres, planets and satellites}
}

@article{Gibson1985,
    title = {{Sulfur in achondritic meteorites}},
    year = {1985},
    journal = {Meteoritics},
    author = {Gibson, Everett K. and Moore, Carleton B. and Primus, Thomas M. and Lewis, Charles F.},
    number = {3},
    pages = {503--511},
    volume = {20},
    url = {http://doi.wiley.com/10.1111/j.1945-5100.1985.tb00046.x},
    doi = {10.1111/j.1945-5100.1985.tb00046.x},
    issn = {00261114}
}

@article{Tokano2016,
    title = {{Sun-stirred Kraken Mare: Circulation in Titan's seas induced by solar heating and methane precipitation}},
    year = {2016},
    journal = {Icarus},
    author = {Tokano, Tetsuya and Lorenz, Ralph D.},
    pages = {67--84},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.08.033},
    doi = {10.1016/j.icarus.2015.08.033},
    issn = {10902643},
    keywords = {Titan, atmosphere, Titan, hydrology, Titan, surface}
}

@article{Vuitton2007a,
    title = {{Supplementary material - Vuitton et al. 2007}},
    year = {2007},
    journal = {Synthesis},
    author = {Vuitton, V. and Yelle, R. V. and McEwan, M. J.},
    pages = {1--10},
    volume = {1}
}

@article{Rahm,
    title = {{Supporting Information - Polymorphism and electronic structure of polyimine}},
    author = {Rahm, Martin and Lunine, Jonathan I and Usher, David A and Shalloway, David},
    pages = {1--22},
    volume = {3}
}

@article{Prockter2017,
    title = {{Surface composition of pull-apart bands in Argadnel Regio, Europa: Evidence of localized cryovolcanic resurfacing during basin formation}},
    year = {2017},
    journal = {Icarus},
    author = {Prockter, Louise M. and Shirley, James H. and Dalton, James B. and Kamp, L.},
    pages = {27--42},
    volume = {285},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.11.024},
    doi = {10.1016/j.icarus.2016.11.024},
    issn = {10902643},
    keywords = {Bands, Europa, Galileo, NIMS, SSI}
}

@article{Owen1993,
    title = {{Surface ices and the atmospheric composition of pluto.}},
    year = {1993},
    journal = {Science (New York, N.Y.)},
    author = {Owen, T. C. and Roush, T. L. and Cruikshank, D. P. and Elliot, J. L. and Young, L. A. and de Bergh, C. and Schmitt, B. and Geballe, T. R. and Brown, R. H. and Bartholomew, M. J.},
    number = {5122},
    pages = {745--748},
    volume = {261},
    doi = {10.1126/science.261.5122.745},
    issn = {0036-8075},
    pmid = {17757212}
}

@article{Roush1995,
    title = {{Surface ices in the outer solar system}},
    year = {1995},
    journal = {AIP Conference Proceedings},
    author = {Roush, Ted L. and Cruikshank, Dale P. and Owen, Tobias C.},
    pages = {143--153},
    volume = {341},
    url = {http://scitation.aip.org/content/aip/proceeding/aipcp/10.1063/1.48737},
    doi = {10.1063/1.48737},
    issn = {0094243X}
}

@article{Coustenis2003,
    title = {{Surfaces and atmospheres of the outer planets, their satellites and ring systems}},
    year = {2003},
    journal = {Planetary and Space Science},
    author = {Coustenis, A.},
    number = {14-15},
    pages = {v},
    volume = {51},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0032063303002095},
    doi = {10.1016/S0032-0633(03)00209-5},
    issn = {00320633}
}

@article{Fraser2004,
    title = {{SURFRESIDE: A novel experiment to study surface chemistry under interstellar and protostellar conditions}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Fraser, H. J. and van Dishoeck, E. F.},
    number = {1},
    pages = {14--22},
    volume = {33},
    doi = {10.1016/j.asr.2003.04.003},
    issn = {02731177},
    keywords = {Astrochemistry, ISM: molecules, Methods: laboratory, Molecular processes}
}

@article{Sittler1983,
    title = {{Survey of low-energy plasma electrons in Saturn's magnetosphere: Voyagers 1 and 2}},
    year = {1983},
    journal = {Journal of Geophysical Research},
    author = {Sittler, E. C. and Ogilvie, K. W. and Scudder, J. D.},
    number = {A11},
    pages = {8847},
    volume = {88},
    url = {http://doi.wiley.com/10.1029/JA088iA11p08847},
    doi = {10.1029/JA088iA11p08847},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/JA088iA11p08847, doi:10.}
}

@article{Gaeman2012,
    title = {{Sustainability of a subsurface ocean within Triton's interior}},
    year = {2012},
    journal = {Icarus},
    author = {Gaeman, Jodi and Hier-Majumder, Saswata and Roberts, James H.},
    number = {2},
    pages = {339--347},
    volume = {220},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.05.006},
    doi = {10.1016/j.icarus.2012.05.006},
    issn = {00191035},
    keywords = {Neptune, Satellites, Tides, Solid body, Triton}
}

@article{Brandsma2004,
    title = {{Synthesis of Acetylenes, Allenes and Cumulenes. Methods and Techniques}},
    year = {2004},
    journal = {Academic Press},
    author = {Brandsma, L.}
}

@article{Khare1971,
    title = {{Synthesis of Cystine in Simulated Primitive Conditions}},
    year = {1971},
    journal = {Nature},
    author = {Khare, B. N. and Sagan, C.},
    volume = {232}
}

@article{Padmanabhan1983,
    title = {{SYNTHESIS OF SKIPPED (1,4) DIYNES VIA COUPLING OF (PROPARGYL ACETATE)DICOBALT HEXACARBONYL COMPLEXES WITH ALKYNYL ALANES}},
    year = {1983},
    journal = {Tetrahedron Letters},
    author = {Padmanabhan, S. and Nicholas, K. M.},
    number = {22},
    pages = {2239--2242},
    volume = {24}
}

@article{Huygens1659a,
    title = {{Systema Saturnium}},
    year = {1659},
    author = {Huygens, Christiaan}
}

@book{Huygens1659,
    title = {{Systema Saturnium, sive de causis mirandorum Saturni phaenomenon, et comite ejus planeta novo}},
    year = {1659},
    author = {Huygens, Christiaan},
    editor = {Vlacq, The Hague: Adrian}
}

@article{Kimura2007,
    title = {{Tectonic history of Europa: Coupling between internal evolution and surface stresses}},
    year = {2007},
    journal = {Earth, Planets and Space},
    author = {Kimura, Jun and Yamagishi, Yasuko and Kurita, Kei},
    number = {2},
    pages = {113--125},
    volume = {59},
    issn = {13438832},
    keywords = {Crustal stress, Structural evolution, Tectonics, Thermal history}
}

@article{Greenberg1998,
    title = {{Tectonic Processes on Europa : Tidal Stresses, Mechanical Response , and Visible Features}},
    year = {1998},
    journal = {Icarus},
    author = {Greenberg, Richard and Geissler, Paul and Hoppa, Gregory and Tufts, B Randall and Durda, Daniel D and Pappalardo, Robert and Head, James W and Greeley, Ronald and Sullivan, Robert and Carr, Michael H},
    number = {1},
    pages = {64--78},
    volume = {135},
    url = {http://dx.doi.org/10.1006/icar.1998.5986},
    doi = {10.1006/icar.1998.5986},
    issn = {00191035},
    keywords = {europa, geological processes, ices, tectonics}
}

@article{Kattenhorn2009,
    title = {{Tectonics of Europa}},
    year = {2009},
    author = {Kattenhorn, Simon a and Hurford, Terry a.},
    pages = {199--236},
    keywords = {2008, convergent, date submitted, dec 5, divergent, ice shell, margins, polar wander, tectonics, water ice}
}

@article{McKay1997,
    title = {{Temperature lapse rate and methane in Titan's troposphere}},
    year = {1997},
    journal = {Icarus},
    author = {McKay, C P and Chau Martin, S and Griffith, C A and Keller, R M},
    number = {2},
    pages = {498--505},
    volume = {129},
    url = {http://www.ncbi.nlm.nih.gov/entrez/query.fcgi?cmd=Retrieve&db=PubMed&dopt=Citation&list_uids=11541736},
    isbn = {0019-1035 (Print){\textbackslash}n0019-1035 (Linking)},
    doi = {10.1006/icar.1997.5751},
    issn = {00191035},
    pmid = {11541736},
    keywords = {*Saturn, *Temperature, Atmosphere/*chemistry, Extraterrestrial Environment, Humidity, Methane/*analysis, Models, Chemical, Nitrogen/analysis}
}

@article{Hill2013,
    title = {{Temperature-dependent molecular absorption cross sections for exoplanets and other atmospheres}},
    year = {2013},
    journal = {Icarus},
    author = {Hill, Christian and Yurchenko, Sergei N. and Tennyson, Jonathan},
    number = {2},
    pages = {1673--1677},
    volume = {226},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.07.028},
    isbn = {00191035},
    doi = {10.1016/j.icarus.2012.07.028},
    issn = {00191035},
    arxivId = {astro-ph.EP/1205.6514},
    keywords = {Atmospheres, Composition, Extrasolar planets, Infrared observations, Radiative transfer}
}

@article{Ferradaz2009,
    title = {{Temperature-dependent photoabsorption cross-sections of cyanoacetylene and diacetylene in the mid- and vacuum-UV : Application to Titan’s atmosphere}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Ferradaz, T and B, Y},
    pages = {10--22},
    volume = {57},
    doi = {10.1016/j.pss.2008.10.005},
    keywords = {absorption cross-sections, cyanoacetylene, diacetylene, low temperatures, titan, vacuum ultraviolet}
}

@article{Achterberg2011,
    title = {{Temporal variations of Titan's middle-atmospheric temperatures from 2004 to 2009 observed by Cassini/CIRS}},
    year = {2011},
    journal = {Icarus},
    author = {Achterberg, R. K. and Gierasch, Peter J. and Conrath, Barney J. and Michael Flasar, F. and Nixon, Conor A.},
    number = {1},
    pages = {686--698},
    volume = {211},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.08.009},
    doi = {10.1016/j.icarus.2010.08.009},
    issn = {00191035},
    keywords = {Atmosphere, Atmospheres, Dynamics, Infrared observations, Structure, Titan}
}

@article{Molesini,
    title = {{TESTING THE LENSES OF CAMPANI , LENS-MAKER FOR CASSINI}},
    author = {Molesini, Giuseppe and Campani, Giuseppe}
}

@article{Armante2016,
    title = {{The 2015 edition of the GEISA spectroscopic database}},
    year = {2016},
    journal = {Journal of Molecular Spectroscopy},
    author = {Armante, R and Scott, N A and Ch, A and Cr, L and Bouhdaoui, A and Crevoisier, C and Capelle, V and Boonne, C}
}

@article{Chapman1931,
    title = {{The absorption and dissociative or ionizing effect of monochromatic radiation in an atmosphere on a rotating earth}},
    year = {1931},
    journal = {Proceedings of the Physical Society},
    author = {Chapman, S},
    number = {1},
    pages = {26--45},
    volume = {43},
    isbn = {0959-5309},
    doi = {10.1088/0959-5309/43/5/302},
    issn = {0959-5309}
}

@article{Chapman1931a,
    title = {{The absorption and dissociative or ionizing effect of monochromatic radiation in an atmosphere on a rotating earth}},
    year = {1931},
    journal = {Proceedings of the Physical Society},
    author = {Chapman, S.},
    number = {1},
    pages = {26--45},
    volume = {43},
    isbn = {0959-5309},
    doi = {10.1088/0959-5309/43/1/305},
    issn = {09595309}
}

@article{Price1934,
    title = {{The absorption spectra of formaldehyde and hydrogen cyanide in the far ultraviolet}},
    year = {1934},
    journal = {Physical Reviews},
    author = {Price, W. C.},
    number = {529},
    pages = {4},
    volume = {46}
}

@article{Price1945,
    title = {{THE Absorption Spectra of Triple Bond Molecules in the Vacuum Ultraviolet}},
    year = {1945},
    journal = {Trans. Faraday Society},
    author = {Price, W. C. and Walsh, A. D.},
    number = {381},
    volume = {41}
}

@article{Bettens1996,
    title = {{The abundance of very large hydrocarbons and carbon clusters in the diffuse interstellar medium}},
    year = {1996},
    journal = {The Astrophysical Journal},
    author = {Bettens, R. P. A. and Herbst, E.}
}

@article{Niemann2005,
    title = {{The abundances of constituents of Titan's atmosphere from the GCMS instrument on the Huygens probe}},
    year = {2005},
    journal = {Nature},
    author = {Niemann, H. B. and Atreya, S. K. and Bauer, S. J. and Carignan, G. R. and Demick, J. E. and Frost, R. L. and Gautier, D. and Haberman, J. A. and Harpold, D. N. and Hunten, D. M. and Israel, G. and Lunine, J. I. and Kasprzak, W. T. and Owen, T. C. and Paulkovich, M. and Raulin, F. and Raaen, E. and Way, S. H.},
    number = {7069},
    pages = {779--784},
    volume = {438},
    url = {http://www.nature.com/doifinder/10.1038/nature04122},
    isbn = {0028-0836},
    doi = {10.1038/nature04122},
    issn = {0028-0836},
    pmid = {16319830},
    keywords = {Argon, Argon: analysis, Atmosphere, Atmosphere: chemistry, Carbon, Carbon: analysis, Carbon: chemistry, Extraterrestrial Environment, Extraterrestrial Environment: chemistry, Gas Chromatography-Mass Spectrometry, Gas Chromatography-Mass Spectrometry: instrumentat, Isotopes, Isotopes: analysis, Methane, Methane: analysis, Methane: chemistry, Nitrogen, Nitrogen: analysis, Nitrogen: chemistry, Space Flight, Space Flight: instrumentation}
}

@misc{2008ModernChemistry,
    title = {{Modern Acetylene Chemistry}},
    year = {2008},
    publisher = {Wiley}
}
@article{Russell2007,
    title = {{The alkaline solution to the emergence of life: Energy, entropy and early evolution}},
    year = {2007},
    journal = {Acta Biotheoretica},
    author = {Russell, Michael J.},
    number = {2},
    pages = {133--179},
    volume = {55},
    isbn = {0001-5342},
    doi = {10.1007/s10441-007-9018-5},
    issn = {00015342},
    pmid = {17704896},
    keywords = {Acetyl phosphate, CODH/ACS, Hydrothermal, Iron sulfide, OEC, Pyrophosphate}
}

@article{Gladstone2016,
    title = {{The Atmosphere of Pluto as Observed by New Horizons}},
    year = {2016},
    author = {Gladstone, G Randall and Stern, S Alan and Ennico, Kimberly and Olkin, Catherine B and Harold, A and Young, Leslie A and Summers, Michael E and Strobel, Darrell F and Hinson, David P and Kammer, A and Parker, Alex H and Steffl, Andrew J and Linscott, Ivan R and Parker, Joel Wm and Andrew, F and Slater, David C and Versteeg, Maarten H and Greathouse, Thomas K and Retherford, Kurt D and Throop, Henry and Cunningham, Nathaniel J and Woods, William W and Singer, Kelsi N and Tsang, C C and Schindhelm, Eric and Lisse, Carey M and Wong, Michael L and Yung, Yuk L and Zhu, Xun and Curdt, Werner and Lavvas, Panayotis and Young, Eliot F and Tyler, G Leonard and Horizons, New},
    pages = {1--39}
}

@article{Lindal1983,
    title = {{The atmosphere of Titan: An analysis of the Voyager 1 radio occultation measurements}},
    year = {1983},
    journal = {Icarus},
    author = {Lindal, G. F. and Wood, G. E. and Hotz, H. B. and Sweetnam, D. N. and Eshleman, V. R. and Tyler, G. L.},
    number = {2},
    pages = {348--363},
    volume = {53},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(83)90155-0},
    issn = {10902643}
}

@article{Trafton1981,
    title = {{The atmospheres of the outer planets and satellites}},
    year = {1981},
    journal = {Reviews of Geophysics},
    author = {Trafton, L.},
    number = {1},
    pages = {43--89},
    volume = {19},
    isbn = {8755-1209},
    doi = {10.1029/RG019i001p00043},
    issn = {19449208}
}

@article{Cicerone1983,
    title = {{The atmospheric chemistry of hydrogen cyanide (HCN)}},
    year = {1983},
    journal = {Journal of Geophysical Research},
    author = {Cicerone, R J and Zellner, R.},
    number = {C15},
    pages = {10689},
    volume = {88},
    url = {http://doi.wiley.com/10.1029/JC088iC15p10689},
    doi = {10.1029/JC088iC15p10689},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/JC088iC15p10689, doi:10.}
}

@article{Pryor2011,
    title = {{The auroral footprint of Enceladus on Saturn}},
    year = {2011},
    journal = {Nature},
    author = {Pryor, Wayne R. and Rymer, Abigail M. and Mitchell, Donald G. and Hill, Thomas W. and Young, David T. and Saur, Joachim and Jones, Geraint H. and Jacobsen, Sven and Cowley, Stan W.H. and Mauk, Barry H. and Coates, Andrew J. and Gustin, Jacques and Grodent, Denis and G{\'{e}}rard, Jean Claude and Lamy, Laurent and Nichols, Jonathan D. and Krimigis, Stamatios M. and Esposito, Larry W. and Dougherty, Michele K. and Jouchoux, Alain J. and Stewart, A. Ian F. and McClintock, William E. and Holsclaw, Gregory M. and Ajello, Joseph M. and Colwell, Joshua E. and Hendrix, Amanda R. and Crary, Frank J. and Clarke, John T. and Zhou, Xiaoyan},
    number = {7343},
    pages = {331--333},
    volume = {472},
    isbn = {0028-0836},
    doi = {10.1038/nature09928},
    issn = {00280836},
    pmid = {21512570}
}

@article{Earth,
    title = {{The basic properties of the natural atmosphere}},
    author = {Earth, The},
    pages = {1--22}
}

@article{Charbonneau2008,
    title = {{The Broadband Infrared Emission Spectrum of the Exoplanet HD 189733b}},
    year = {2008},
    author = {Charbonneau, David and Knutson, Heather a. and Barman, Travis and Allen, Lori E. and Mayor, Michel and Megeath, S. Thomas and Queloz, Didier and Udry, Stephane},
    pages = {20},
    url = {http://arxiv.org/abs/0802.0845},
    doi = {10.1086/591635},
    issn = {0004-637X},
    arxivId = {0802.0845}
}

@article{Trafton1972a,
    title = {{The bulk composition of Titan's atmosphere}},
    year = {1972},
    journal = {The Astrophysical Journal},
    author = {Trafton, L},
    number = {Allen 1963},
    pages = {295--306}
}

@article{Srama2002,
    title = {{The Cassini cosmic dust analyzer}},
    year = {2004},
    journal = {Space Science Reviews},
    author = {Srama, R. and Ahrens, T. J. and Altobelli, N. and Auer, S. and Bradley, J. G. and Burton, M. and Dikarev, V. V. and Economou, T. and Fechtig, H. and G{\"{o}}rlich, M. and Grande, M. and Graps, A. and Gr{\"{u}}n, E. and Havnes, O. and Helfert, S. and Horanyi, M. and Igenbergs, E. and Jessberger, E. K. and Johnson, T. V. and Kempf, S. and Krivov, A. V. and Kr{\"{u}}ger, H. and Mocker-Ahlreep, A. and Moragas-Klostermeyer, G. and Lamy, P. and Landgraf, M. and Linkert, D. and Linkert, G. and Lura, F. and Mcdonnell, J. A.M. and M{\"{o}}hlmann, D. and Morfill, G. E. and M{\"{u}}ller, M. and Roy, M. and Sch{\"{a}}fer, G. and Schlotzhauer, G. and Schwehm, G. H. and Spahn, F. and St{\"{u}}big, M. and Svestka, J. and Tschernjawski, V. and Tuzzolino, A. J. and W{\"{a}}sch, R. and Zook, H. A.},
    number = {1-4},
    pages = {465--518},
    volume = {114},
    isbn = {0038-6308},
    doi = {10.1007/s11214-004-1435-z},
    issn = {00386308},
    keywords = {CDA, Cassini, Dust sensor, E-ring, Interplanetary dust}
}

@article{Waite2004a,
    title = {{The Cassini Ion and Neutral Mass Spectrometer (INMS) investigation}},
    year = {2004},
    author = {Waite, J. H. and Lewis, W. S. and Kasprzak, W. T. and Anicich, V. G. and Block, B. P. and Cravens, T. E. and Fletcher, G. G. and Ip, W. H. and Luhmann, J. G. and Mcnutt, R. L. and Niemann, H. B. and Parejko, J. K. and Richards, J. E. and Thorpe, R. L. and Walter, E. M. and Yelle, R. V.},
    number = {1-4},
    pages = {113--231},
    volume = {114},
    isbn = {00386308},
    doi = {10.1007/s11214-004-1408-2},
    issn = {00386308},
    keywords = {Cassini, Huygens, Mass Spectrometry, Saturn, Titan}
}

@article{Waite2004,
    title = {{The Cassini Ion and Neutral Mass Spectrometer (INMS) Investigation}},
    year = {2004},
    journal = {Space Science Reviews},
    author = {Waite, J H and Lewis, W S and Kasprzak, W T and Anicich, V G and Block, B P and Cravens, T E and Fletcher, G G and Luhmann, J G and Mcnutt, R L and Niemann, H B and Parejko, J K and Richards, J E and Thorpe, R L and Walter, E M and Yelle, R V},
    pages = {113--231}
}

@article{Esposito2004,
    title = {{The Cassini Ultraviolet Imaging Spectrograph Investigation}},
    year = {2004},
    author = {Esposito, Larry W and Barth, Charles A and Colwell, Joshua E and Lawrence, M and Mcclintock, William E and Stewart, A I A N F and Uwe, H and Korth, Axel and Lauche, Hans and Festou, Michel C and Arthur, L and Hansen, Candice J and Maki, Justin N and West, Robert A and Reulke, Ralf and Warlich, Kerstin and Shemansky, Donald E and Yung, Y U K L},
    pages = {299--361},
    keywords = {cassini, on saturn, rings, saturn, spectroscopy on titan and}
}

@article{LeMouelic2018a,
    title = {{The Cassini VIMS archive of Titan: from browse products to global infrared color maps}},
    year = {2018},
    journal = {Icarus},
    author = {Le Mou{\'{e}}lic, S. and Cornet, T. and Rodriguez, S. and Sotin, C. and Seignovert, B. and Barnes, J.W. and Brown, R.H. and Baines, K.H. and Buratti, B.J. and Clark, R.N. and Nicholson, P.D. and Lasue, J. and Pasek, V. and Soderblom, J.M.},
    url = {https://linkinghub.elsevier.com/retrieve/pii/S0019103518303993},
    doi = {10.1016/j.icarus.2018.09.017},
    issn = {00191035}
}

@article{Brown2005,
    title = {{The Cassini visual and infrared mapping spectrometer (VIMS) investigation}},
    year = {2005},
    journal = {Space Science Reviews},
    author = {Brown, R. H. and Baines, K. H. and Bellucci, G. and Bibring, J. P. and Buratti, B. J. and Capaccioni, F. and Cerroni, P. and Clark, R. N. and Coradini, A. and Cruikshank, D. P. and Drossart, P. and Formisano, V. and Jaumann, R. and Langevin, Y. and Matson, D. L. and Mccord, T. B. and Mennella, V. and Miller, E. and Nelson, R. M. and Nicholson, P. D. and Sicardy, B. and Sotin, C.},
    number = {1-4},
    pages = {111--168},
    volume = {115},
    isbn = {0038-6308},
    doi = {10.1007/s11214-004-1453-x},
    issn = {00386308},
    keywords = {Cassini, Saturn, infrared mapping spectrometer}
}

@article{Brown2004,
    title = {{The Cassini visual and infrared mapping spectrometer (VIMS) investigation}},
    year = {2004},
    journal = {Space Science Reviews},
    author = {Brown, R. H. and Baines, K. H. and Bellucci, G. and Bibring, J. P. and Buratti, B. J. and Capaccioni, F. and Cerroni, P. and Clark, R. N. and Coradini, A. and Cruikshank, D. P. and Drossart, P. and Formisano, V. and Jaumann, R. and Langevin, Y. and Matson, D. L. and Mccord, T. B. and Mennella, V. and Miller, E. and Nelson, R. M. and Nicholson, P. D. and Sicardy, B. and Sotin, C.},
    number = {1-4},
    pages = {111--168},
    volume = {115},
    isbn = {0038-6308},
    doi = {10.1007/s11214-004-1453-x},
    issn = {00386308},
    pmid = {13005473},
    keywords = {Cassini, Saturn, infrared mapping spectrometer}
}

@article{Czesla2015,
    title = {{The center-to-limb variation across the Fraunhofer lines of HD 189733}},
    year = {2015},
    journal = {Astronomy {\&} Astrophysics},
    author = {Czesla, S. and Klocov{\'{a}}, T. and Khalafinejad, S. and Wolter, U. and Schmitt, J. H. M. M.},
    pages = {A51},
    volume = {582},
    url = {http://arxiv.org/abs/1509.05657%5Cnhttp://www.aanda.org/10.1051/0004-6361/201526386},
    doi = {10.1051/0004-6361/201526386},
    issn = {0004-6361},
    arxivId = {1509.05657},
    keywords = {activity, atmospheres, hd 189733 b, individual, planets and satellites, stars}
}

@article{Turrini2014,
    title = {{The comparative exploration of the ice giant planets with twin spacecraft: Unveiling the history of our Solar System}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Turrini, Diego and Politi, Romolo and Peron, Roberto and Grassi, Davide and Plainaki, Christina and Barbieri, Mauro and Lucchesi, David M. and Magni, Gianfranco and Altieri, Francesca and Cottini, Valeria and Gorius, Nicolas and Gaulme, Patrick and Schmider, Fran??ois Xavier and Adriani, Alberto and Piccioni, Giuseppe},
    number = {PA},
    pages = {93--107},
    volume = {104},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2014.09.005},
    doi = {10.1016/j.pss.2014.09.005},
    issn = {00320633},
    arxivId = {1402.2650},
    keywords = {Neptune, Neptune, satellites, Planetary formation, Space missions, Uranus, Uranus, satellites}
}

@article{Owen1982,
    title = {{The composition and origin of Titan's atmosphere}},
    year = {1982},
    journal = {Planetary and Space Science},
    author = {Owen, T. C.},
    number = {8},
    pages = {833--838},
    volume = {30},
    url = {http://www.sciencedirect.com/science/article/pii/0032063382901155}
}

@article{Coustenis2007,
    title = {{The composition of Titan's stratosphere from Cassini/CIRS mid-infrared spectra}},
    year = {2007},
    journal = {Icarus},
    author = {Coustenis, A. and Achterberg, R. K. and Conrath, Barney J. and Jennings, Donald E. and Marten, André and Gautier, Daniel and Nixon, Conor A. and Flasar, F. Michael and Teanby, Nick A. and B{\'{e}}zard, Bruno and Samuelson, Robert E. and Carlson, Ronald C. and Lellouch, Emmanuel and Bjoraker, Gordon L. and Romani, Paul N. and Taylor, Fred W. and Irwin, Patrick G J and Fouchet, Thierry and Hubert, Augustin and Orton, Glenn S. and Kunde, Virgil G. and Vinatier, Sandrine and Mondellini, Jacqueline and Abbas, Mian M. and Courtin, Regis},
    number = {1},
    pages = {35--62},
    volume = {189},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2006.12.022},
    issn = {00191035},
    keywords = {Infrared observations, Satellites, Titan, atmospheres}
}

@article{Rhoden2011,
    title = {{The contribution of Io-raised tides to Europa's diurnally-varying surface stresses}},
    year = {2011},
    author = {Rhoden, A. R. and Hurford, T. A. and Manga, Michael},
    pages = {3--4}
}

@article{Zahnle2017,
    title = {{The cosmic shoreline: the evidence that escape determines which planets have atmospheres, and what this may mean for proxima centauri b}},
    year = {2017},
    author = {Zahnle, Kevin J and Catling, David C},
    arxivId = {1702.03386},
    keywords = {individual, planetary systems, proxima centauri, stars}
}

@article{Ross1990,
    title = {{The Coupled Orbital and Thermal Evolution of Triton}},
    year = {1990},
    journal = {Geophysical Research Letters},
    author = {Ross, M. N. and Schubert, G.},
    number = {5},
    pages = {1--4}
}

@article{Evans2013,
    title = {{THE DEEP BLUE COLOR OF HD 189733b: ALBEDO MEASUREMENTS WITH HUBBLE SPACE TELESCOPE/SPACE TELESCOPE IMAGING SPECTROGRAPH AT VISIBLE WAVELENGTHS}},
    year = {2013},
    journal = {The Astrophysical Journal Letters},
    author = {Evans, Thomas M and Pont, Frédéric and Sing, David K and Aigrain, Suzanne and Barstow, Joanna K and D{\'{e}}sert, Jean-Michel and Gibson, Neale and Heng, Kevin and Knutson, Heather A and Lecavelier, Alain and Etangs, Des},
    pages = {16--5},
    volume = {772},
    doi = {10.1088/2041-8205/772/2/L16},
    issn = {2041-8205},
    arxivId = {1307.3239},
    keywords = {atmospheres – stars, individual (HD 189733) – techniques, photometric, planets and satellites}
}

@article{Lavvas2009,
    title = {{The detached haze layer in Titan's mesosphere}},
    year = {2009},
    journal = {Icarus},
    author = {Lavvas, Panayotis and Yelle, Roger V. and Vuitton, Véronique},
    number = {2},
    pages = {626--633},
    volume = {201},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.01.004},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.01.004},
    issn = {00191035},
    keywords = {Atmospheres, Titan, structure}
}

@article{Loomis2013,
    title = {{THE DETECTION OF INTERSTELLAR ETHANIMINE (CH <sub>3</sub> CHNH) FROM OBSERVATIONS TAKEN DURING THE GBT PRIMOS SURVEY}},
    year = {2013},
    journal = {The Astrophysical Journal},
    author = {Loomis, Ryan A. and Zaleski, Daniel P. and Steber, Amanda L. and Neill, Justin L. and Muckle, Matthew T. and Harris, Brent J. and Hollis, Jan M. and Jewell, Philip R. and Lattanzi, Valerio and Lovas, Frank J. and Martinez, Oscar and McCarthy, Michael C. and Remijan, Anthony J. and Pate, Brooks H. and Corby, Joanna F.},
    number = {1},
    pages = {L9},
    volume = {765},
    url = {http://stacks.iop.org/2041-8205/765/i=1/a=L9?key=crossref.f87e155bdad4d41fe62a2578ce6caa98},
    doi = {10.1088/2041-8205/765/1/L9},
    issn = {2041-8205},
    arxivId = {1302.1121},
    keywords = {abundances, catalogs, color figures, individual objects, ism, laboratory, methods, molecules, online-only material, sgrb2n, surveys}
}

@article{Loren1984,
    title = {{The detection of Interstellar methyl-diacetylene}},
    year = {1984},
    journal = {The Astrophysical Journal},
    author = {Loren, R. and Wootten, A. and Mundy, L.}
}

@article{Hussey1903,
    title = {{The diameter of Titan}},
    year = {1903},
    journal = {Publications of the Astronomical Society of the Pacific},
    author = {Hussey, W. J. and Aitken, R. G.},
    number = {953},
    pages = {131--158},
    volume = {277}
}

@article{T.,
    title = {{The discovery of Titan}},
    author = {T., Lynn W.}
}

@article{Schmidt2011,
    title = {{The Double ElectroStatic Ion-Ring ExpEriment , DESIREE}},
    year = {2011},
    author = {Schmidt, Henning T and L{\"{o}}fgren, Patrik and Liljeby, Leif and Br{\"{a}}nnholm, Lars and Ros{\'{e}}n, Stefan and Thomas, Richard D and Haag, Nicole and Johansson, Henrik A B and Bj{\"{o}}rkhage, Mikael and Blom, Mikael and Leontein, Sven and P{\'{a}}al, Andras and Andler, Guillermo and Reinhed, Peter and Seitz, Fabian and Rensfelt, Karl G and K{\"{a}}llberg, Anders and Das, Susanta and Halld{\'{e}}n, Per and Weimer, Jan and Simonsson, Ansgar and Hellberg, Fredrik and Larsson, Mats and Geppert, Wolf D and Zettergren, Henning and Cederquist, Henrik},
    pages = {2011},
    doi = {10.1088/1742-6596/388/14/142022},
    issn = {17426588}
}

@article{Russell2014,
    title = {{The drive to life on wet and icy worlds.}},
    year = {2014},
    journal = {Astrobiology},
    author = {Russell, Michael J and Barge, Laura M and Bhartia, Rohit and Bocanegra, Dylan and Bracher, Paul J and Branscomb, Elbert and Kidd, Richard and McGlynn, Shawn and Meier, David H and Nitschke, Wolfgang and Shibuya, Takazo and Vance, Steve and White, Lauren and Kanik, Isik},
    number = {4},
    pages = {308--43},
    volume = {14},
    url = {http://online.liebertpub.com/doi/full/10.1089/ast.2013.1110?src=recsys%5Cnhttp://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3995032&tool=pmcentrez&rendertype=abstract},
    isbn = {1531-1074},
    doi = {10.1089/ast.2013.1110},
    issn = {1557-8070},
    pmid = {24697642},
    keywords = {Biogenesis, Carbon Cycle, Earth (Planet), Exobiology, Hydrogen-Ion Concentration, Hydrothermal Vents, Hydrothermal Vents: chemistry, Inorganic Pyrophosphatase, Inorganic Pyrophosphatase: metabolism, Oxidation-Reduction}
}

@article{Jeans1925,
    title = {{The Dynamical Theory of Gases}},
    year = {1925},
    author = {Jeans, J.},
    volume = {4th Editio}
}

@article{Sagan1997,
    title = {{The Early Faint Sun Paradox: Organic Shielding of Ultraviolet-Labile Greenhouse Gases}},
    year = {1997},
    journal = {Science},
    author = {Sagan, C. and Chyba, C. F.},
    number = {5316},
    pages = {1217--1221},
    volume = {276},
    url = {http://www.sciencemag.org/cgi/doi/10.1126/science.276.5316.1217},
    doi = {10.1126/science.276.5316.1217},
    issn = {00368075}
}

@article{Harada2004,
    title = {{The Effect of the Non-synchronous Rotation on the Surface Stress of Europa : Constraints for the Rotation Period and the Surface Viscosity}},
    year = {2004},
    author = {Harada, Yuji and Kurita, Kei}
}

@article{Hamelin2016,
    title = {{The electrical properties of Titan's surface at the Huygens landing site measured with the PWA-HASI Mutual Impedance Probe. New approach and new findings}},
    year = {2016},
    journal = {Icarus},
    author = {Hamelin, Michel and Lethuillier, Anthony and Le Gall, Alice and Grard, Réjean and B{\'{e}}ghin, Christian and Schwingenschuh, Konrad and Jernej, Irmgard and L{\'{o}}pez-Moreno, José Juan and Brown, Vic and Lorenz, Ralph D. and Ferri, Francesca and Ciarletti, Valérie},
    pages = {272--290},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.11.035},
    doi = {10.1016/j.icarus.2015.11.035},
    issn = {10902643},
    keywords = {Data reduction techniques, Satellites, Titan, surface, surfaces}
}

@article{Sutherland2017,
    title = {{the end of the beginning}},
    year = {2017},
    journal = {Nature Publishing Group},
    author = {Sutherland, John D},
    pages = {1--8},
    volume = {1},
    publisher = {Macmillan Publishers Limited},
    url = {http://dx.doi.org/10.1038/s41570-016-0012},
    doi = {10.1038/s41570-016-0012}
}

@article{Levi2018,
    title = {{The equation of state of mh-iii: a possible deep ch 4 reservoir in Titan, super-Titan exoplanets and moons}},
    year = {2018},
    author = {Levi, A and Cohen, R. E.},
    pages = {1--14},
    arxivId = {arXiv:1808.07925v1}
}

@article{Charnoz2012,
    title = {{The Equatorial Ridges of Pan and Atlas :}},
    year = {2012},
    journal = {Science},
    author = {Charnoz, Sébastien},
    number = {2007},
    volume = {1622},
    doi = {10.1126/science.1148631}
}

@article{Hunten1973,
    title = {{The escape of light gases from planetary atmospheres}},
    year = {1973},
    journal = {Journal of Atmospheric Sciences},
    author = {Hunten, Donald M.},
    number = {8},
    pages = {1481–1494},
    volume = {30},
    url = {http://adsabs.harvard.edu/abs/1973JAtS...30.1481H},
    doi = {10.1175/1520-0469(1973)030<1481:TEOLGF>2.0.CO;2},
    issn = {0022-4928}
}

@article{Pappalardo2017a,
    title = {{The Europa Clipper}},
    year = {2017},
    author = {Pappalardo, R. T. and Senske, D. A. and Korth, H and Klima, R. and Vance, S. D. and Craft, K.},
    volume = {11}
}

@article{Pappalardo2017,
    title = {{The Europa Multiple-Flyby Mission: Synergistic Science to Investigate Habitability}},
    year = {2017},
    journal = {LPSC},
    author = {Pappalardo, R. T. and Senske, D A and Korth, H and Blaney, D and Blankenship, D and Christensen, P and Raymond, C and Retherford, K and Turtle, E P and Waite, J H and Westlake, J and Collins, G C and Hand, K and Lunine, J and Mcgrath, M and Nimmo, F and Paty, C and Soderblom, J and Spencer, J R and Paranicas, C and Solomon, S and Antonio, San and View, Mountain and Cruz, Santa and Observatory, Lamont-doherty Earth and Goal, Mission and Shell, I Ice and Europa, Exploring and Synergistic, Through}
}

@article{Conselice2016,
    title = {{THE EVOLUTION OF GALAXY NUMBER DENSITY AT <i>z</i> {\&}lt; 8 AND ITS IMPLICATIONS}},
    year = {2016},
    journal = {The Astrophysical Journal},
    author = {Conselice, Christopher J. and Wilkinson, Aaron and Duncan, Kenneth and Mortlock, Alice},
    number = {2},
    pages = {83},
    volume = {830},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/830/i=2/a=83?key=crossref.fedbb5c2800ebd163f5760535b282aad},
    doi = {10.3847/0004-637X/830/2/83},
    issn = {1538-4357},
    arxivId = {arXiv:1607.03909v2},
    keywords = {evolution, fundamental parameters, galaxies, galaxies: evolution, galaxies: fundamental parameters, galaxies: general, galaxies: high-redshift, galaxies: luminosity function, mass function, galaxies: structure, general, high-redshift, luminosity function, mass function, structure}
}

@article{Consolmagno1978,
    title = {{The evolution of icy satellite interiors and surfaces}},
    year = {1978},
    journal = {Icarus},
    author = {Consolmagno, Guy J. and Lewis, John S.},
    number = {2},
    pages = {280--293},
    volume = {34},
    doi = {10.1016/0019-1035(78)90168-9},
    issn = {10902643}
}

@article{Hickson2014,
    title = {{The evolution of infalling sulfur species in Titan’s atmosphere}},
    year = {2014},
    journal = {Astronomy {\&} Astrophysics},
    author = {Hickson, K M and Loison, J C and Cavali{\'{e}}, T and H{\'{e}}brard, E and Dobrijevic, M},
    pages = {A58},
    volume = {572},
    url = {http://www.aanda.org/10.1051/0004-6361/201424703},
    isbn = {doi:10.1051/0004-6361/201424703},
    doi = {10.1051/0004-6361/201424703},
    issn = {0004-6361},
    keywords = {atmospheres, composition, individual, planets and satellites, titan}
}

@article{Nisbet2011,
    title = {{The evolution of the atmosphere in the Archaean and early Proterozoic}},
    year = {2011},
    journal = {Chinese Science Bulletin},
    author = {Nisbet, Euan and Fowler, C. Mary R},
    number = {1},
    pages = {4--13},
    volume = {56},
    isbn = {10016538 (ISSN)},
    doi = {10.1007/s11434-010-4199-8},
    issn = {10016538},
    keywords = {Archean, Atmosphere evolution, Hadean, Methane, Photosynthesis, Stromatolite}
}

@article{Carrasco2018,
    title = {{The evolution of Titan’s high-altitude aerosols under ultraviolet irradiation}},
    year = {2018},
    journal = {Nature Astronomy},
    author = {Carrasco, N. and Tigrine, Sarah and Gavilan, Lisseth and Nahon, Laurent and Gudipati, Murthy S},
    pages = {1},
    publisher = {Springer US},
    url = {http:https://doi.org/10.1038/s41550-018-0439-7},
    doi = {10.1038/s41550-018-0439-7},
    issn = {2397-3366}
}

@article{Tennyson2018,
    title = {{The ExoMol Atlas of Molecular Opacities}},
    year = {2018},
    author = {Tennyson, Jonathan and Yurchenko, Sergei N.},
    pages = {11--16},
    url = {http://arxiv.org/abs/1805.03711},
    arxivId = {1805.03711},
    keywords = {brown stars, cool stars, exomol, exoplanets, molecular spectra, opacity}
}

@article{Tennyson2016,
    title = {{The ExoMol database: molecular line lists for exoplanet and other hot atmospheres}},
    year = {2016},
    journal = {Journal of Molecular Spectroscopy},
    author = {Tennyson, J. and Yurchenko, Sergei N and Al-refaie, Ahmed F and Emma, J and Chubb, Katy L and Coles, Phillip A and Diamantopoulou, S and Maire, N and Hill, Christian and Lam, Aden Z and Lodi, Lorenzo and Mckemmish, Laura K and Na, Yueqi and Owens, Alec and Polyansky, Oleg L and Sousa-silva, Clara and Daniel, S and Yachmenev, Andrey and Zak, Emil},
    pages = {1--68},
    arxivId = {arXiv:1603.05890v2},
    keywords = {cooling functions, cross sections, einstein a coefficients, infrared, k coefficients, lifetimes, partition functions, transition frequencies, visible}
}

@article{Garnier2007,
    title = {{The exosphere of Titan and its interaction with the kronian magnetosphere: MIMI observations and modeling}},
    year = {2007},
    journal = {Planetary and Space Science},
    author = {Garnier, P. and Dandouras, I. and Toublanc, D. and Brandt, P. C. and Roelof, E. C. and Mitchell, D. G. and Krimigis, S. M. and Krupp, N. and Hamilton, D. C. and Waite, H.},
    number = {1-2},
    pages = {165--173},
    volume = {55},
    doi = {10.1016/j.pss.2006.07.006},
    issn = {00320633},
    keywords = {Cassini, Energetic neutral atoms, Exosphere, Magnetosphere, Titan}
}

@article{Baines2018,
    title = {{The Eye of Saturn's North Polar Vortex: Unexpected Cloud Structures Observed at High Spatial Resolution by Cassini/VIMS}},
    year = {2018},
    journal = {Geophysical Research Letters},
    author = {Baines, K. H. and Sromovsky, L. A. and Fry, P. M. and Momary, T. W. and Brown, R. H. and Buratti, B. J. and Clark, R. N. and Nicholson, P. D. and Sotin, C.},
    number = {12},
    pages = {5867--5875},
    volume = {45},
    doi = {10.1029/2018GL078168},
    issn = {19448007},
    keywords = {Cassini, Saturn atmosphere, Saturn clouds, Saturn dynamics, Saturn north pole, VIMS}
}

@article{Mousis2016,
    title = {{The fate of ethane in Titan's hydrocarbon lakes and seas}},
    year = {2016},
    journal = {Icarus},
    author = {Mousis, Olivier and Lunine, Jonathan I. and Hayes, Alexander G. and Hofgartner, Jason D.},
    pages = {37--40},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.06.024},
    doi = {10.1016/j.icarus.2015.06.024},
    issn = {10902643},
    arxivId = {1510.07677},
    keywords = {Titan, Titan, atmosphere, Titan, hydrology, Titan, surface}
}

@article{Orton2017,
    title = {{The first close-up images of Jupiter's polar regions: Results from the Juno mission JunoCam instrument}},
    year = {2017},
    journal = {Geophysical Research Letters},
    author = {Orton, Glenn S. and Hansen, Candice and Caplinger, Michael and Ravine, Michael and Atreya, Sushil and Ingersoll, Andrew P. and Jensen, Elsa and Momary, Thomas and Lipkaman, Leslie and Krysak, Daniel and Zimdar, Robert and Bolton, Scott},
    pages = {1--8},
    url = {http://doi.wiley.com/10.1002/2016GL072443},
    doi = {10.1002/2016GL072443},
    issn = {00948276}
}

@article{Olah1972,
    title = {{The General Concept and Structure of Carbocations Based on Differentiation of Trivalent (“Classical”) Carbenium Ions from Three-Center Bound Penta- or Tetracoordinated (“Nonclassical”) Carbonium Ions. the Role of Carbocations in Electrophilic Reactions1a–}},
    year = {1972},
    journal = {Journal of the American Chemical Society},
    author = {Olah, George A.},
    number = {3},
    pages = {808--820},
    volume = {94},
    isbn = {0002-7863},
    doi = {10.1021/ja00758a020},
    issn = {15205126}
}

@article{Smith1910,
    title = {{The Geologic Record of California Author}},
    year = {1910},
    journal = {The Journal of Geology},
    author = {Smith, J. P.},
    number = {3},
    pages = {216--227},
    volume = {18}
}

@article{Li2011,
    title = {{The global energy balance of Titan}},
    year = {2011},
    journal = {Geophysical Research Letters},
    author = {Li, Liming and Nixon, Conor A. and Achterberg, Richard K. and Smith, Mark A. and Gorius, Nicolas J.P. and Jiang, Xun and Conrath, Barney J. and Gierasch, Peter J. and Simon-Miller, Amy A. and Michael Flasar, F. and Baines, Kevin H. and Ingersoll, Andrew P. and West, Robert A. and Vasavada, Ashwin R. and Ewald, Shawn P.},
    number = {23},
    pages = {4--7},
    volume = {38},
    doi = {10.1029/2011GL050053},
    issn = {00948276},
    keywords = {http://dx.doi.org/10.1029/2011GL050053, doi:10.102}
}

@article{Nimmo2007a,
    title = {{The global shape of Europa: Constraints on lateral shell thickness variations}},
    year = {2007},
    journal = {Icarus},
    author = {Nimmo, F. and Thomas, P. C. and Pappalardo, R. T. and Moore, W. B.},
    number = {1},
    pages = {183--192},
    volume = {191},
    doi = {10.1016/j.icarus.2007.04.021},
    issn = {00191035},
    keywords = {Interiors, Jupiter, Satellites, Tides, satellites, shapes, solid body}
}

@article{Brin2015,
    title = {{The Great Silence - the Controversy Concerning Extraterrestrial Intelligent Life}},
    year = {2015},
    journal = {CEUR Workshop Proceedings},
    author = {Brin, G. D.},
    number = {August 1983},
    pages = {33--36},
    volume = {1542},
    isbn = {9788578110796},
    doi = {10.1017/CBO9781107415324.004},
    issn = {16130073},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {Mobile, Named entity disambiguation, Natural language processing, News, Recommender system}
}

@article{Billings2005,
    title = {{The great thickness debate: Ice shell thickness models for Europa and comparisons with estimates based on flexure at ridges}},
    year = {2005},
    journal = {Icarus},
    author = {Billings, Sandra E. and Kattenhorn, Simon A.},
    number = {2},
    pages = {397--412},
    volume = {177},
    doi = {10.1016/j.icarus.2005.03.013},
    issn = {00191035},
    keywords = {Europa, Geological processes, Satellite, Surfaces}
}

@article{Sagan1973,
    title = {{The greenhouse of Titan}},
    year = {1973},
    journal = {Icarus},
    author = {Sagan, C.},
    number = {4},
    pages = {649--656},
    volume = {18},
    doi = {10.1016/0019-1035(73)90068-7},
    issn = {10902643}
}

@article{Mousis2015,
    title = {{The Hera Saturn entry probe mission}},
    year = {2015},
    journal = {Planetary and Space Science},
    author = {Mousis, O. and Atkinson, D. H. and Spilker, T. and Venkatapathy, E. and Poncy, J. and Frampton, R. and Coustenis, A. and Reh, K. and Lebreton, J. P. and Fletcher, L. N. and Hueso, R. and Amato, M. J. and Colaprete, A. and Ferri, F. and Stam, D. and Wurz, P. and Atreya, S. and Aslam, S. and Banfield, D. J. and Calcutt, S. and Fischer, G. and Holland, A. and Keller, C. and Kessler, E. and Leese, M. and Levacher, P. and Morse, A. and Mu??oz, O. and Renard, J. B. and Sheridan, S. and Schmider, F. X. and Snik, F. and Waite, J. H. and Bird, M. and Cavali??, T. and Deleuil, M. and Fortney, J. and Gautier, D. and Guillot, T. and Lunine, J. I. and Marty, B. and Nixon, C. and Orton, G. S. and S??nchez-Lavega, A.},
    pages = {80--103},
    volume = {130},
    doi = {10.1016/j.pss.2015.06.020},
    issn = {00320633},
    keywords = {Atmosphere, ESA's Cosmic Vision Medium class size call, In situ measurements, Probe, Saturn}
}

@article{Claudepierre2016,
    title = {{The hidden dynamics of relativistic electrons (0.7-1.5 MeV) in the inner zone and slot region}},
    year = {2016},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Claudepierre, S. G. and O'Brien, T. P. and Fennell, J. F. and Blake, J. B. and Clemmons, J. H. and Looper, M. D. and Mazur, J. E. and Roeder, J. L. and Turner, D. L. and Reeves, G. D. and Spence, H. E.},
    pages = {1--18},
    doi = {10.1002/2016JA023719}
}

@article{Pappalardo1999a,
    title = {{The Hidden Ocean of Europa}},
    year = {1999},
    journal = {Scientific American},
    author = {Pappalardo, Robert T. and Head, James W. and Greeley, Ronald},
    number = {4},
    pages = {54--63},
    volume = {281},
    doi = {10.1038/scientificamerican1099-54},
    issn = {0036-8733}
}

@article{Lebreton2002,
    title = {{The Huygens probe: Science, payload and mission overview}},
    year = {2002},
    journal = {Space Science Reviews},
    author = {Lebreton, J. P. and Matson, D. L.},
    number = {1-4},
    pages = {59--100},
    volume = {104},
    doi = {10.1023/A:1023657127549},
    issn = {00386308}
}

@article{Zarnecki,
    title = {{The Huygens Surface Science Package}},
    author = {Zarnecki, J C and Banaszkiewicz, M and Boynton, M Bannister W V and Clark, P Challenor B and Daniell, P M and Delderfield, J and English, M A and Fulchignoni, M and Garry, J R C and Geake, J E and Green, S F and Hathi, B and Jaroslawski, S and Leese, M R and Lorenz, R D and Mcdonnell, J A M and Miller, C S Mil R J and Newton, G and Parker, D J and Rabbetts, P and Svedhem, H and Turner, R F and Wright, M J and So, Hampshire and Kingdom, United},
    pages = {177--195}
}

@article{Rhoden2017,
    title = {{The Implications of Tides on the Mimas Ocean Hypothesis}},
    year = {2017},
    journal = {Journal of Geophysical Research: Planets},
    author = {Rhoden, Alyssa Rose and Henning, Wade and Hurford, Terry A. and Patthoff, D. Alex and Tajeddine, Radwan},
    url = {http://doi.wiley.com/10.1002/2016JE005097},
    doi = {10.1002/2016JE005097},
    issn = {21699097}
}

@article{Russell2013,
    title = {{The inevitable journey to being.}},
    year = {2013},
    journal = {Philosophical transactions of the Royal Society of London. Series B, Biological sciences},
    author = {Russell, Michael J and Nitschke, Wolfgang and Branscomb, Elbert},
    number = {1622},
    pages = {20120254},
    volume = {368},
    url = {http://rstb.royalsocietypublishing.org/content/368/1622/20120254.abstract},
    isbn = {0962-8436},
    doi = {10.1098/rstb.2012.0254},
    issn = {1471-2970},
    pmid = {23754808},
    keywords = {Animals, Astronomical Phenomena, Autotrophic Processes, Biological Evolution, Carbon Dioxide, Carbon Sequestration, Energy Metabolism, Energy Transfer, Geological Phenomena, Hot Temperature, Hydrothermal Vents, Oceans and Seas, Proton-Motive Force, Seawater, Thermodynamics}
}

@article{Lewis2018,
    title = {{The influence of a sub-stellar continent on the climate of a tidally-locked exoplanet}},
    year = {2018},
    author = {Lewis, Neil T. and Lambert, F. Hugo and Boutle, Ian A. and Mayne, Nathan J. and Manners, James and Acreman, David M.},
    url = {http://arxiv.org/abs/1802.00378},
    arxivId = {1802.00378},
    keywords = {atmospheres - planets and, corresponding author, lewis, neil t, planets and satellites, satellites, terrestrial planets - astrobiology}
}

@article{Trainer2013,
    title = {{The influence of benzene as a trace reactant in titan aerosol analogs}},
    year = {2013},
    journal = {Astrophysical Journal Letters},
    author = {Trainer, Melissa G. and Sebree, Joshua A. and Heidi Yoon, Y. and Tolbert, Margaret A.},
    number = {1},
    volume = {766},
    doi = {10.1088/2041-8205/766/1/L4},
    issn = {20418205},
    keywords = {planets and satellites: atmospheres, planets and satellites: individual (Titan)}
}

@article{Mazankova2016,
    title = {{The Influence of CO2 Admixtures on the Product Composition in a Nitrogen-Methane Atmospheric Glow Discharge Used as a Prebiotic Atmosphere Mimic}},
    year = {2016},
    journal = {Origins of Life and Evolution of Biospheres},
    author = {Mazankova, V. and Torokova, L. and Krcma, F. and Mason, N. J. and Matejcik, S.},
    number = {4},
    pages = {499--506},
    volume = {46},
    publisher = {Origins of Life and Evolution of Biospheres},
    url = {http://dx.doi.org/10.1007/s11084-016-9504-3},
    isbn = {1573-0875},
    doi = {10.1007/s11084-016-9504-3},
    issn = {15730875},
    keywords = {Atmospheric glow discharge, FTIR spectroscopy, Prebiotic atmosphere}
}

@article{Hurford2009,
    title = {{The influence of obliquity on europan cycloid formation}},
    year = {2009},
    journal = {Icarus},
    author = {Hurford, T. A. and Sarid, A. R. and Greenberg, R. and Bills, B. G.},
    number = {1},
    pages = {197--215},
    volume = {202},
    doi = {10.1016/j.icarus.2009.02.036},
    issn = {00191035},
    keywords = {Europa, Rotational dynamics, Tectonics, Tides, solid body}
}

@article{Penz2005,
    title = {{The influence of the solar particle and radiation environment on Titan's atmosphere evolution}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {Penz, T. and Lammer, H. and Kulikov, Yu N. and Biernat, H. K.},
    number = {2},
    pages = {241--250},
    volume = {36},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2005.03.043},
    issn = {02731177},
    keywords = {Atmosphere evolution, Hydrodynamic conditions, Solar wind, Titan}
}

@article{Gerakines1995,
    title = {{The infrared band strengths of H2O, CO and CO2 in laboratory simulations of astrophysical ice mixtures}},
    year = {1995},
    journal = {Astronomy {\&} Astrophysics},
    author = {Gerakines, P. A. and Schutte, W. A. and Greenberg, J. M. and Dishoeck, E. F. van},
    pages = {A108},
    volume = {565},
    url = {http://www.aanda.org/10.1051/0004-6361/201423560},
    isbn = {0004-6361},
    doi = {10.1051/0004-6361/201423560},
    issn = {0004-6361},
    arxivId = {1406.7646},
    keywords = {ISM: molecules, absorption, amorphous solid water, astrochemistry, carbon-dioxide, features, ices, infrared: ISM, irradiation, methods: laboratory: molecular, optical-constants, planetary, spectra, spectroscopy, techniques: spectroscopic, ultraviolet}
}

@article{Bernstein2004,
    title = {{The infrared spectrum of matrix isolated aminoacetonitrile, a precursor to the amino acid glycine}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Bernstein, M. P. and Bauschlicher, C. W. and Sandford, S. A.},
    number = {1},
    pages = {40--43},
    volume = {33},
    doi = {10.1016/j.asr.2003.07.002},
    issn = {02731177},
    keywords = {Amino acid, Glycine, IR spectroscopy, Meteorite, Nitrile}
}

@article{McDoniel2017,
    title = {{The Interaction of Io’s Plumes and Sublimation Atmosphere}},
    year = {2017},
    journal = {Icarus},
    author = {McDoniel, William J. and Goldstein, David B. and Varghese, Philip L. and Trafton, Laurence M.},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103517303068},
    doi = {10.1016/j.icarus.2017.04.021},
    issn = {00191035},
    keywords = {Io, Satellites, Volcanism, surfaces}
}

@article{Tokar2006,
    title = {{The interaction of the atmosphere of Enceladus with Saturn's plasma}},
    year = {2006},
    journal = {Science},
    author = {Tokar, R. L. and Johnson, R. E. and Hill, T. W. and Pontius, D. H. and Kurth, W. S. and Crary, F. J. and Young, D. T. and Thomsen, M. F. and Reisenfeld, D. B. and Coates, A. J. and Lewis, G. R. and Sittler, E. C. and Gurnett, D. A.},
    number = {5766},
    pages = {1409--1412},
    volume = {311},
    isbn = {1095-9203 (Electronic){\textbackslash}r0036-8075 (Linking)},
    doi = {10.1126/science.1121061},
    issn = {00368075},
    pmid = {16527967}
}

@article{Cordier2017,
    title = {{The Interaction of Titan’s Aerosols with Hydrocarbons Seas}},
    year = {2017},
    author = {Cordier, D. and Carrasco, N.},
    number = {1},
    pages = {2--3},
    volume = {11}
}

@article{Freeman1978,
    title = {{The interstellar synthesis of HC3N and HC5N}},
    year = {1978},
    journal = {Astrophysical Letters},
    author = {Freeman, CG and Harland, PW and McEwan, MJ},
    number = {July},
    pages = {133},
    volume = {19},
    url = {http://adsabs.harvard.edu/abs/1978ApL....19..133F}
}

@article{Cravens2004,
    title = {{The ionosphere of Titan: An updated theoretical model}},
    year = {2004},
    journal = {Advances in Space Research},
    author = {Cravens, T. E. and Vann, J. and Clark, J. and Yu, J. and Keller, C. N. and Brull, C.},
    number = {2},
    pages = {212--215},
    volume = {33},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2003.02.012},
    issn = {02731177},
    keywords = {Auger electrons, Photoelectron spectrum, Titan ionosphere}
}

@misc{Hill2001,
    title = {{The Jovian auroral oval}},
    year = {2001},
    author = {Hill, T. W.}
}

@article{Modolo2018,
    title = {{The LatHyS database for planetary plasma environment investigations: Overview and a case study of data/model comparisons}},
    year = {2018},
    journal = {Planetary and Space Science},
    author = {Modolo, R. and Hess, S. and G{\'{e}}not, V. and Leclercq, L. and Leblanc, F. and Chaufray, J. Y. and Weill, P. and Gangloff, M. and Fedorov, A. and Budnik, E. and Bouchemit, M. and Steckiewicz, M. and Andr{\'{e}}, N. and Beigbeder, L. and Popescu, D. and Toniutti, J. P. and Al-Ubaidi, T. and Khodachenko, M. and Brain, D. and Curry, S. and Jakosky, B. and Holmstr{\"{o}}m, M.},
    number = {November 2016},
    pages = {13--21},
    volume = {150},
    doi = {10.1016/j.pss.2017.02.015},
    issn = {00320633},
    keywords = {Data management, Mars, Numerical modeling, Solar wind interactions with unmagnetized bodies}
}

@article{Sudbery2014,
    title = {{The logic of the future in the Everett-Wheeler understanding of quantum theory}},
    year = {2014},
    journal = {Synthese},
    author = {Sudbery, Anthony},
    number = {September 2014},
    pages = {19},
    publisher = {Springer Netherlands},
    url = {http://arxiv.org/abs/1409.0755},
    doi = {10.1007/s11229-016-1142-9},
    issn = {0039-7857},
    arxivId = {1409.0755},
    keywords = {Quantum theory, Temporal logic, probability, quantum theory, temporal logic}
}

@article{Capone1976,
    title = {{The lower ionosphere of Titan}},
    year = {1976},
    journal = {Icarus},
    author = {Capone, L. A. and Whitten, R. C. and Dubach, J. and Prasad, S. S. and Huntress, W. T.},
    number = {3},
    pages = {367--378},
    volume = {28},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(76)90150-0},
    issn = {10902643}
}

@book{Budavari1996,
    title = {{The Merck Index}},
    year = {1996},
    author = {Budavari, S. and O'Neil, M. J. and Smith, A.},
    edition = {12th ed.},
    publisher = {Co., Merck {\&}}
}

@article{Koskinen2011,
    title = {{The mesosphere and lower thermosphere of Titan revealed by Cassini/UVIS stellar occultations}},
    year = {2011},
    journal = {Icarus},
    author = {Koskinen, T. T. and Yelle, R. V. and Snowden, D. S. and Lavvas, P. and Sandel, B. R. and Capalbo, F. J. and Benilan, Y. and West, R. A.},
    number = {2},
    pages = {507--534},
    volume = {216},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.09.022},
    doi = {10.1016/j.icarus.2011.09.022},
    issn = {00191035},
    keywords = {Atmospheres, Occultations, Structure, Titan}
}

@article{Plane2015,
    title = {{The Mesosphere and Metals: Chemistry and Changes}},
    year = {2015},
    journal = {Chemical Reviews},
    author = {Plane, John M.C. and Feng, Wuhu and Dawkins, Erin C.M.},
    number = {10},
    pages = {4497--4541},
    volume = {115},
    isbn = {0009-2665},
    doi = {10.1021/cr500501m},
    issn = {15206890},
    pmid = {25751779}
}

@article{Lunine2008,
    title = {{The methane cycle on Titan}},
    year = {2008},
    journal = {Nature Geoscience},
    author = {Lunine, Jonathan and Atreya, Sushil},
    number = {5},
    pages = {335--335},
    volume = {1},
    url = {http://www.nature.com/doifinder/10.1038/ngeo187},
    isbn = {1752-0894},
    doi = {10.1038/ngeo187},
    issn = {1752-0894}
}

@article{Paubert1984,
    title = {{The millimeter spectrum of Titan: Detectability of HCN, HC3N, and CH3CN and the CO abundance}},
    year = {1984},
    journal = {Icarus},
    author = {Paubert, G. and Gautier, D. and Courtin, R.},
    number = {3},
    pages = {599--612},
    volume = {60},
    doi = {10.1016/0019-1035(84)90167-2},
    issn = {10902643}
}

@article{Helling2016,
    title = {{The mineral clouds on HD 209458b and HD 189733b}},
    year = {2016},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Helling, Ch and Lee, G. and Dobbs-Dixon, I. and Mayne, N. and Amundsen, D. S. and Khaimova, J. and Unger, A. A. and Manners, J. and Acreman, D. and Smith, C.},
    number = {1},
    pages = {855--883},
    volume = {460},
    doi = {10.1093/mnras/stw662},
    issn = {13652966},
    arxivId = {1603.04022},
    keywords = {Astrochemistry, HD 189733b, HD 209458b, Individual, Numerical, Opacity -methods, Planets and satellites}
}

@article{Nordheim2017,
    title = {{The near-surface electron radiation environment of Saturn's moon Mimas}},
    year = {2017},
    journal = {Icarus},
    author = {Nordheim, T A and Hand, K P and Paranicas, C and Howett, C J A and Hendrix, A R and Jones, G H and Coates, A J},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2017.01.002},
    doi = {10.1016/j.icarus.2017.01.002},
    issn = {0019-1035}
}

@article{Irwin2008,
    title = {{The NEMESIS planetary atmosphere radiative transfer and retrieval tool}},
    year = {2008},
    journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
    author = {Irwin, P. G J and Teanby, N. A. and de Kok, R. and Fletcher, L. N. and Howett, C. J A and Tsang, C. C C and Wilson, C. F. and Calcutt, S. B. and Nixon, C. A. and Parrish, P. D.},
    number = {6},
    pages = {1136--1150},
    volume = {109},
    isbn = {0022-4073},
    doi = {10.1016/j.jqsrt.2007.11.006},
    issn = {00224073},
    keywords = {Correlated-k, Radiative transfer, Retrievals}
}

@article{Loison2015,
    title = {{The neutral photochemistry of nitriles, amines and imines in the atmosphere of Titan}},
    year = {2015},
    journal = {Icarus},
    author = {Loison, J. C. and H{\'{e}}brard, E. and Dobrijevic, M. and Hickson, K. M. and Caralp, F. and Hue, V. and Gronoff, G. and Venot, O. and B{\'{e}}nilan, Y.},
    pages = {218--247},
    volume = {247},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.09.039},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.09.039},
    issn = {10902643},
    keywords = {Atmospheres, chemistry, Atmospheres, composition, Organic chemistry, Photochemistry, Titan}
}

@article{Falchi2016,
    title = {{The new world atlas of artificial night sky brightness}},
    year = {2016},
    author = {Falchi, Fabio and Cinzano, Pierantonio and Duriscoe, Dan and Kyba, Christopher C M and Elvidge, Christopher D and Baugh, Kimberly and Portnov, Boris A and Rybnikova, Nataliya A and Furgoni, Riccardo},
    number = {June},
    pages = {1--26},
    doi = {10.1126/sciadv.1600377}
}

@article{Corby2001,
    title = {{THE NITRILES PROJECT : MOLECULE FORMATION IN THE GALACTIC CENTER}},
    year = {2001},
    author = {Corby, Joanna}
}

@article{Vuitton2006a,
    title = {{The Nitrogen Chemistry of Titan's Upper Atmosphere Revealed}},
    year = {2006},
    journal = {The Astrophysical Journal},
    author = {Vuitton, V. and Yelle, R. V. and Anicich, V. G.},
    number = {2},
    pages = {L175-L178},
    volume = {647},
    url = {http://iopscience.iop.org/article/10.1086/507467},
    doi = {10.1086/507467},
    issn = {0004-637X}
}

@article{Tebbutt1894,
    title = {{The occultation of Saturn, May 25, 1893}},
    year = {1894},
    journal = {Publications of the Astronomical Society of the Pacific},
    author = {Tebbutt, J.},
    number = {34},
    pages = {180},
    volume = {261},
    issn = {1050-3390}
}

@article{Elkins-tanton2005,
    title = {{The onset and early evolution of life}},
    year = {2005},
    journal = {GSA},
    author = {Elkins-tanton, Linda T and Hall, A.},
    number = {303},
    volume = {80301},
    doi = {10.1130/2005.2388(27).},
    keywords = {delamination, lithospheric thinning, magmatism, rayleigh-taylor instability}
}

@article{Jacobson2009,
    title = {{the Orbits of the Neptunian Satellites and the Orientation of the Pole of Neptune}},
    year = {2009},
    journal = {The Astronomical Journal},
    author = {Jacobson, R. A.},
    number = {5},
    pages = {4322--4329},
    volume = {137},
    url = {http://iopscience.iop.org/article/10.1088/0004-6256/137/5/4322%5Cnhttp://dx.doi.org/10.1088/0004-6256/137/5/4322},
    isbn = {doi:10.1088/0004-6256/137/5/4322},
    doi = {10.1088/0004-6256/137/5/4322},
    issn = {0004-6256},
    keywords = {ephemerides, individual, neptune, nereid, planets and satellites, proteus, triton}
}

@article{Jacobson1991,
    title = {{The orbits of Triton and Nereid from spacecraft and Earthbased observations}},
    year = {1991},
    journal = {Astronomy {\&} Astrophysics},
    author = {Jacobson, R. A. and Riedel, J. E. and Taylor, A. H.}
}

@article{Khare1984,
    title = {{The organic aerosols of Titan}},
    year = {1984},
    journal = {Advances in Space Research},
    author = {Khare, B. N. and Sagan, C. and Thompson, W. R. and Arakawa, E. T. and Suits, F. and Callcott, T. A. and Williams, M. W. and Shrader, S. and Ogino, H. and Willingham, T. O. and Nagy, B.},
    number = {12},
    pages = {59--68},
    volume = {4},
    isbn = {0273-1177 (Print)},
    doi = {10.1016/0273-1177(84)90545-3},
    issn = {02731177},
    pmid = {11537796}
}

@article{Khurana2007,
    title = {{The origin of Ganymede's polar caps}},
    year = {2007},
    journal = {Icarus},
    author = {Khurana, Krishan K. and Pappalardo, Robert T. and Murphy, Nate and Denk, Tilmann},
    number = {1},
    pages = {193--202},
    volume = {191},
    isbn = {00191035},
    doi = {10.1016/j.icarus.2007.04.022},
    issn = {00191035},
    keywords = {Europa, Ganymede, Jupiter, Satellites, magnetosphere, surfaces}
}

@article{Sagan1974,
    title = {{The origin of life in a cosmic context}},
    year = {1974},
    journal = {Origins of Life},
    author = {Sagan, C.},
    number = {3-4},
    pages = {497--505},
    volume = {5},
    doi = {10.1007/BF01207649},
    issn = {03021688},
    pmid = {4416394}
}

@article{Sutherland2016,
    title = {{The Origin of Life — Out of the Blue Angewandte}},
    year = {2016},
    author = {Sutherland, John D},
    pages = {104--121},
    doi = {10.1002/anie.201506585},
    keywords = {amino acids, hydrogen cyanide, prebiotic chemistry}
}

@article{Owen2009,
    title = {{The origin of Titan's atmosphere: some recent advances}},
    year = {2009},
    journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
    author = {Owen, T. and Niemann, H.B},
    number = {1889},
    pages = {607--615},
    volume = {367},
    url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.2008.0247},
    isbn = {1364-503X (Print){\textbackslash}r1364-503X (Linking)},
    doi = {10.1098/rsta.2008.0247},
    issn = {1364-503X},
    pmid = {19019783},
    keywords = {atmosphere, composition, deuterium, noble gases, origin}
}

@article{Owen2007,
    title = {{The origin of Titan’s atmosphere : some recent advances}},
    year = {2007},
    author = {Owen, By Tobias and Niemann, H B},
    number = {Linsky 2003},
    pages = {1--9},
    volume = {4},
    keywords = {atmosphere, composition, deuterium, noble gases, origin}
}

@article{Teanby2018,
    title = {{THE Origin of Titan’s External Oxygen: Further Constraints From ALMA Upper Limits on CS and CH2NH}},
    year = {2018},
    author = {Teanby, N. A. and Cordiner, M A and Nixon, C A and Irwin, P G J and H{\"{o}}rst, S.M. and Sylvestre, M and Serigano, J and Thelen, A E and Richards, A. M. S. and Charnley, S B},
    keywords = {atmospheres, individual, planets and satellites, radiative, titan}
}

@article{Loison2017,
    title = {{The photochemical fractionation of oxygen isotopologues in Titan's atmosphere}},
    year = {2017},
    journal = {Icarus},
    author = {Loison, J. C. and Dobrijevic, M. and Hickson, K. M. and Heays, A. N.},
    pages = {17--30},
    volume = {291},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2017.02.032},
    doi = {10.1016/j.icarus.2017.02.032},
    issn = {10902643},
    keywords = {Atmospheres, Ionospheres, Photochemistry, Titan}
}

@article{Krasnopolsky2010,
    title = {{The photochemical model of Titan’s atmosphere and ionosphere: A version without hydrodynamic escape}},
    year = {2010},
    journal = {Planetary and Space Science},
    author = {Krasnopolsky, Vladimir A.},
    number = {12},
    month = {10},
    pages = {1507--1515},
    volume = {58},
    url = {http://www.sciencedirect.com/science/article/pii/S0032063310002126},
    doi = {10.1016/j.pss.2010.07.010},
    issn = {00320633},
    keywords = {Atmosphere, Composition, Evolution, Ionosphere, Photochemistry, Titan}
}

@article{Ramos,
    title = {{The photochemistry and photophysics of diacetylene and cyanoacetylene: applications to the atmosphere of Titan}},
    author = {Ramos, C.}
}

@article{Horne1970,
    title = {{The Photolysis of Acyclic Azines and the Electronic Spectra of RFormulaRFormulaCNFormula Radicals}},
    year = {1970},
    journal = {Proceedings of the Royal Society A: Mathematical, Physical and Engineering Sciences},
    author = {Horne, D. G. and Norrish, R. G. W.},
    number = {1522},
    pages = {301--322},
    volume = {315},
    url = {http://rspa.royalsocietypublishing.org/cgi/doi/10.1098/rspa.1970.0045},
    doi = {10.1098/rspa.1970.0045},
    issn = {1364-5021}
}

@article{Bott2016,
    title = {{The polarization of HD 189733}},
    year = {2016},
    journal = {Monthly Notices of the Royal Astronomical Society: Letters},
    author = {Bott, Kimberly and Bailey, Jeremy and Kedziora-Chudczer, Lucyna and Cotton, Daniel V. and Lucas, P. W. and Marshall, Jonathan P. and Hough, J. H.},
    number = {1},
    pages = {L109-L113},
    volume = {459},
    doi = {10.1093/mnrasl/slw046},
    issn = {17453933},
    arxivId = {1603.05745},
    keywords = {Planets and satellites: Atmospheres, Planets and satellites: Individual: HD 189733b, Polarization, Techniques: Polarimetric}
}

@article{Waite2007,
    title = {{The Process of Tholin Formation in Titan's Upper Atmosphere}},
    year = {2007},
    journal = {Science},
    author = {Waite, J. H. and Young, D.T. and Cravens, T. E. and Coates, A. J. and Crary, F. J. and Magee, B. and Westlake, J.},
    number = {2007},
    volume = {870},
    doi = {10.1126/science.1139727}
}

@article{Ordu2012,
    title = {{The quest for complex molecules in space: laboratory spectroscopy of <i>n</i> -butyl cyanide, <i>n</i> -C <sub>4</sub> H <sub>9</sub> CN, in the millimeter wave region and its astronomical search in Sagittarius B2(N)}},
    year = {2012},
    journal = {Astronomy {\&} Astrophysics},
    author = {Ordu, M. H. and M{\"{u}}ller, H. S. P. and Walters, A. and Nu{\~{n}}ez, M. and Lewen, F. and Belloche, A. and Menten, K. M. and Schlemmer, S.},
    pages = {A121},
    volume = {541},
    url = {http://www.aanda.org/10.1051/0004-6361/201118738},
    doi = {10.1051/0004-6361/201118738},
    issn = {0004-6361},
    arxivId = {1204.2686},
    keywords = {individual objects, ism, laboratory, methods, molecular data, molecules, radio lines, sagittarius b2, spectroscopic, techniques}
}

@article{Rein2018,
    title = {{The random walk of cars and their collision probabilities with planets}},
    year = {2018},
    author = {Rein, Hanno and Tamayo, Daniel and Vokrouhlicky, David},
    number = {February},
    volume = {000},
    url = {http://arxiv.org/abs/1802.04718},
    isbn = {9625452524},
    arxivId = {1802.04718},
    keywords = {dynamical evolution, gravitation, methods, numerical, planets and satellites}
}

@article{Largo2010,
    title = {{The reaction between NH + and CH 3 COOH : a possible process for the formation of glycine precursors in the interstellar medium}},
    year = {2010},
    journal = {Astronomy {\&} Astrophysics},
    author = {Largo, L. and Redondo, P. and Ray{\'{o}}n, V.M. and Largo, A. and Barrientos, C.},
    pages = {A79},
    volume = {516},
    isbn = {0004-6361{\textbackslash}n1432-0746},
    doi = {10.1051/0004-6361/201014057},
    issn = {0004-6361},
    keywords = {astrobiology, astrochemistry, methods, molecular data, molecular processes, numerical}
}

@article{Schroder2008,
    title = {{The reflectance spectrum of Titan's surface at the Huygens landing site determined by the descent imager/spectral radiometer}},
    year = {2008},
    journal = {Planetary and Space Science},
    author = {Schr{\"{o}}der, S. E. and Keller, H. U.},
    number = {5},
    pages = {753--769},
    volume = {56},
    doi = {10.1016/j.pss.2007.10.011},
    issn = {00320633},
    arxivId = {1702.00653},
    keywords = {Titan}
}

@article{Salvador2017,
    title = {{The relative influence of H2O and CO2 on the primitive surface conditions and evolution of rocky planets}},
    year = {2017},
    journal = {Journal of Geophysical Research: Planets},
    author = {Salvador, A. and Massol, H. and Davaille, A. and Marcq, E. and Sarda, P. and Chassefi{\`{e}}re, E.},
    pages = {1--29},
    url = {http://doi.wiley.com/10.1002/2017JE005286},
    doi = {10.1002/2017JE005286},
    issn = {21699097}
}

@article{Zhong2009,
    title = {{The rheology of cryovolcanic slurries: Motivation and phenomenology of methanol-water slurries with implications for Titan}},
    year = {2009},
    journal = {Icarus},
    author = {Zhong, Fang and Mitchell, Karl L. and Hays, Charles C. and Choukroun, Mathieu and Barmatz, Martin and Kargel, Jeffrey S.},
    number = {2},
    pages = {607--619},
    volume = {202},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.03.015},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.03.015},
    issn = {00191035},
    keywords = {Ices, Satellites, Saturn, Titan, Volcanism, mechanical properties}
}

@article{DUXBURY1997,
    title = {{The Role of an Internal Heat Source for the Eruptive Plumes on Triton}},
    year = {1997},
    journal = {Icarus},
    author = {DUXBURY, N and BROWN, R},
    number = {1},
    pages = {83--93},
    volume = {125},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103596955542},
    isbn = {0019-1035},
    doi = {10.1006/icar.1996.5554},
    issn = {00191035}
}

@article{Yoon2014,
    title = {{The role of benzene photolysis in Titan haze formation}},
    year = {2014},
    journal = {Icarus},
    author = {Yoon, Y. Heidi and H{\"{o}}rst, Sarah M. and Hicks, Raea K. and Li, Rui and de Gouw, Joost A. and Tolbert, Margaret A.},
    pages = {233--241},
    volume = {233},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.02.006},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.02.006},
    issn = {00191035},
    keywords = {Atmospheres, chemistry, Experimental techniques, Photochemistry, Titan, atmosphere}
}

@article{Westlake2014,
    title = {{The role of ion-molecule reactions in the growth of heavy ions in Titan's ionosphere}},
    year = {2014},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Westlake, J. H. and Waite, J. H. and Carrasco, N. and Richard, M. and Cravens, T.},
    number = {7},
    pages = {5951--5963},
    volume = {119},
    isbn = {2169-9402},
    doi = {10.1002/2014JA020208},
    issn = {21699402},
    keywords = {Titan, heavy ion, ion-molecule chemistry, ionosphere}
}

@article{Ferris2005,
    title = {{The role of photochemistry in Titan's atmospheric chemistry}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {Ferris, James and Tran, Buu and Joseph, Jeffrey and Vuitton, Veronique and Briggs, Robert and Force, Michael},
    number = {2},
    pages = {251--257},
    volume = {36},
    doi = {10.1016/j.asr.2005.03.056},
    issn = {02731177},
    keywords = {Huygens probe, Photochemistry, Titan's atmosphere, Titan's atmospheric chemistry, Titan's haze}
}

@article{Khurana2017,
    title = {{The role of plasma slowdown in the generation of Rhea's Alfv{\'{e}}n wings}},
    year = {2017},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Khurana, Krishan K. and Fatemi, Shahab and Lindkvist, Jesper and Roussos, Elias and Krupp, Norbert and Holmstr??m, Mats and Russell, Christopher T. and Dougherty, Michele K.},
    number = {2},
    pages = {1778--1788},
    volume = {122},
    doi = {10.1002/2016JA023595},
    issn = {21699402},
    keywords = {Dione, Enceladus, Rhea, Saturn, Tethys, magnetic field}
}

@article{Smith1979,
    title = {{The role of SO2 in volcanism on Io}},
    year = {1979},
    journal = {Nature},
    author = {Smith, B. A. and Shoemaker, E. M. and Kieffer, S. W. and Cook II, A. F.}
}

@article{Ogi2012,
    title = {{The role of summer surface wind anomalies in the summer Arctic sea ice extent in 2010 and 2011}},
    year = {2012},
    journal = {Geophysical Research Letters},
    author = {Ogi, Masayo and Wallace, John M.},
    number = {9},
    pages = {1--6},
    volume = {39},
    isbn = {0094-8276},
    doi = {10.1029/2012GL051330},
    issn = {00948276},
    keywords = {Arctic sea ice extent, summer in 2010 and 2011, summer wind anomalies}
}

@article{Zhang1999,
    title = {{The Role of Vertical Mixing in the Temporal Evolution of Ground-Level Ozone Concentrations}},
    year = {1999},
    journal = {Journal of Applied Meteorology},
    author = {Zhang, Jian and Rao, S. Trivikrama},
    number = {12},
    pages = {1674--1691},
    volume = {38},
    isbn = {0894-8763},
    doi = {10.1175/1520-0450(1999)038<1674:TROVMI>2.0.CO;2},
    issn = {0894-8763}
}

@misc{Keedy1992,
    title = {{The Rotational Vibrational-Spectra of HCN and DCN - a Physical-Chemistry Experiment}},
    year = {1992},
    booktitle = {Journal of Chemical Education},
    author = {Keedy, C R},
    number = {11},
    pages = {A296-A298},
    volume = {69},
    isbn = {0021-9584}
}

@article{Fortenberry2016,
    title = {{The rovibrational nature of <i>cis</i> - and <i>trans</i> -HNNS: A possible nitrogen molecule progenitor}},
    year = {2016},
    journal = {The Journal of Chemical Physics},
    author = {Fortenberry, Ryan C.},
    number = {20},
    pages = {204302},
    volume = {145},
    url = {http://aip.scitation.org/doi/10.1063/1.4968036},
    doi = {10.1063/1.4968036},
    issn = {0021-9606}
}

@article{Nicholson1920,
    title = {{The satellites in the solar system}},
    year = {1920},
    journal = {Publications of the Astronomical Society of the Pacific},
    author = {Nicholson, S.},
    number = {186},
    pages = {139--144},
    volume = {32}
}

@article{Arridge2014,
    title = {{The science case for an orbital mission to Uranus: Exploring the origins and evolution of ice giant planets}},
    year = {2014},
    journal = {Planetary and Space Science},
    author = {Arridge, C. S. and Achilleos, N. and Agarwal, J. and Agnor, C. B. and Ambrosi, R. and Andr??, N. and Badman, S. V. and Baines, K. and Banfield, D. and Barth??l??my, M. and Bisi, M. M. and Blum, J. and Bocanegra-Bahamon, T. and Bonfond, B. and Bracken, C. and Brandt, P. and Briand, C. and Briois, C. and Brooks, S. and Castillo-Rogez, J. and Cavali??, T. and Christophe, B. and Coates, A. J. and Collinson, G. and Cooper, J. F. and Costa-Sitja, M. and Courtin, R. and Daglis, I. A. and De Pater, I. and Desai, M. and Dirkx, D. and Dougherty, M. K. and Ebert, R. W. and Filacchione, G. and Fletcher, L. N. and Fortney, J. and Gerth, I. and Grassi, D. and Grodent, D. and Gr??n, E. and Gustin, J. and Hedman, M. and Helled, R. and Henri, P. and Hess, S. and Hillier, J. K. and Hofstadter, M. H. and Holme, R. and Horanyi, M. and Hospodarsky, G. and Hsu, S. and Irwin, P. and Jackman, C. M. and Karatekin, O. and Kempf, S. and Khalisi, E. and Konstantinidis, K. and Kr??ger, H. and Kurth, W. S. and Labrianidis, C. and Lainey, V. and Lamy, L. L. and Laneuville, M. and Lucchesi, D. and Luntzer, A. and MacArthur, J. and Maier, A. and Masters, A. and McKenna-Lawlor, S. and Melin, H. and Milillo, A. and Moragas-Klostermeyer, G. and Morschhauser, A. and Moses, J. I. and Mousis, O. and Nettelmann, N. and Neubauer, F. M. and Nordheim, T. and Noyelles, B. and Orton, G. S. and Owens, M. and Peron, R. and Plainaki, C. and Postberg, F. and Rambaux, N. and Retherford, K. and Reynaud, S. and Roussos, E. and Russell, C. T. and Rymer, A. M. and Sallantin, R. and S??nchez-Lavega, A. and Santolik, O. and Saur, J. and Sayanagi, K. M. and Schenk, P. and Schubert, J. and Sergis, N. and Sittler, E. C. and Smith, A. and Spahn, F. and Srama, R. and Stallard, T. and Sterken, V. and Sternovsky, Z. and Tiscareno, M. and Tobie, G. and Tosi, F. and Trieloff, M. and Turrini, D. and Turtle, E. P. and Vinatier, S. and Wilson, R. and Zarka, P.},
    number = {PA},
    pages = {122--140},
    volume = {104},
    doi = {10.1016/j.pss.2014.08.009},
    issn = {00320633},
    keywords = {Atmosphere, Magnetosphere, Natural satellites, Planetary interior, Rings, Uranus}
}

@book{Gudipati2013a,
    title = {{The Science of Solar System Ices}},
    year = {2013},
    booktitle = {The Science of Sjolar System Ices},
    author = {Gudipati, Murthy S. and Castillo-Rogez, JC},
    editor = {{Springer}},
    pages = {47--72},
    volume = {356},
    url = {http://www.springerlink.com/index/10.1007/978-1-4614-3076-6},
    isbn = {978-1-4614-3075-9},
    doi = {10.1007/978-1-4614-3076-6},
    keywords = {ices, science of solar system}
}

@book{McKay1997a,
    title = {{The search for life on Mars}},
    year = {1997},
    booktitle = {Origin of Life and Evolution of the Biosphere},
    author = {McKay, Christopher P},
    pages = {263--289},
    volume = {27},
    url = {http://link.springer.com/chapter/10.1007/978-94-015-8907-9_14},
    isbn = {978-94-015-8907-9},
    doi = {10.1007/978-94-015-8907-9}
}

@article{West2018,
    title = {{The seasonal cycle of Titan's detached haze}},
    year = {2018},
    journal = {Nature Astronomy},
    author = {West, Robert A. and Seignovert, Benoît and Rannou, Pascal and Dumont, Philip and Turtle, Elizabeth P. and Perry, Jason and Roy, Mou and Ovanessian, Aida},
    number = {Figure 1},
    volume = {162},
    url = {http://www.nature.com/articles/s41550-018-0434-z},
    isbn = {1844251411},
    doi = {10.1038/s41550-018-0434-z},
    issn = {2397-3366},
    arxivId = {arXiv:1804.10842v1}
}

@article{DePater1991,
    title = {{The significance of microwave observations for the planets}},
    year = {1991},
    journal = {Physics Reports},
    author = {de Pater, Imke},
    number = {1},
    pages = {1--50},
    volume = {200},
    isbn = {0370-1573},
    doi = {10.1016/0370-1573(91)90103-S},
    issn = {03701573}
}

@article{F.,
    title = {{THE SIMULTANEOUS DISAPPEARANCE OF JUPIter's four moons, with some notes upon the laws that govern their motions}},
    author = {F., Abbott},
    pages = {24--26}
}

@article{Robinson2002,
    title = {{The singlet-triplet spectroscopy of 1,3-butadiene using cavity ring-down spectroscopy}},
    year = {2002},
    journal = {Journal of Chemical Physics},
    author = {Robinson, Allison G. and Winter, Paul R. and Zwier, Timothy S.},
    number = {18},
    pages = {7918--7925},
    volume = {116},
    doi = {10.1063/1.1467903},
    issn = {00219606}
}

@article{Tobiska2000,
    title = {{The SOLAR2000 empirical solar irradiance model and forecast tool}},
    year = {2000},
    journal = {Journal of Atmospheric and Solar-Terrestrial Physics},
    author = {Tobiska, W. Kent and Woods, Tom and Eparvier, Frank and Viereck, Rodney and Floyd, Linton and Bouwer, Dave and Rottman, Gary and White, O. R.},
    number = {14},
    pages = {1233--1250},
    volume = {62},
    isbn = {1364-6826},
    doi = {10.1016/S1364-6826(00)00070-5},
    issn = {13646826},
    keywords = {SOLAR2000, Solar EUV, Solar irradiances, Solar spectrum, Space weather forecasts}
}

@article{Solomonidou2018,
    title = {{The Spectral Nature of Titan's Major Geomorphological Units: Constraints on Surface Composition}},
    year = {2018},
    journal = {Journal of Geophysical Research: Planets},
    author = {Solomonidou, A. and Coustenis, A. and Lopes, R. M. C. and Malaska, M. J. and Rodriguez, S. and Drossart, P. and Elachi, C. and Schmitt, B. and Philippe, S. and Janssen, M. and Hirtzig, M. and Wall, S. and Sotin, C. and Lawrence, K. and Altobelli, N. and Bratsolis, E. and Radebaugh, J. and Stephan, K. and Brown, R. H. and Le Mou{\'{e}}lic, S. and Le Gall, A. and Villanueva, E. V. and Brossier, J. F. and Bloom, A. A. and Witasse, O. and Matsoukas, C. and Schoenfeld, A.},
    url = {http://doi.wiley.com/10.1002/2017JE005477},
    doi = {10.1002/2017JE005477},
    issn = {21699097}
}

@article{Hicks2004,
    title = {{The spectral variability of Triton from 1997-2000}},
    year = {2004},
    journal = {Icarus},
    author = {Hicks, Michael D. and Buratti, Bonnie J.},
    number = {1},
    pages = {210--218},
    volume = {171},
    doi = {10.1016/j.icarus.2004.02.012},
    issn = {00191035},
    keywords = {Photometry, Satellite surfaces, Satellites of Neptune, Spectroscopy, Triton}
}

@article{Anderson2008,
    title = {{The structure of Mercury's magnetic field from MESSENGER's first flyby}},
    year = {2008},
    journal = {Science (New York, N.Y.)},
    author = {Anderson, Brian J. and Acu{\~{n}}a, Mario H. and Korth, Haje and Purucker, Michael E and Johnson, Catherine L. and Slavin, James A. and Solomon, Sean C. and McNutt, Ralph L.},
    number = {i},
    pages = {82--85},
    volume = {321},
    doi = {10.1126/science.1159081},
    issn = {0036-8075},
    pmid = {18599775}
}

@article{Liu2016,
    title = {{The tectonics of Titan: Global structural mapping from Cassini RADAR}},
    year = {2016},
    journal = {Icarus},
    author = {Liu, Zac Yung Chun and Radebaugh, Jani and Harris, Ron A. and Christiansen, Eric H. and Neish, Catherine D. and Kirk, Randolph L. and Lorenz, Ralph D.},
    pages = {14--29},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.11.021},
    doi = {10.1016/j.icarus.2015.11.021},
    issn = {10902643},
    keywords = {Geological processes, Radar observations, Satellites, surfaces, Tectonics, Titan, surface}
}

@article{Fallis2013,
    title = {{The temperature effect on the absorption of 15 microns CO2 band}},
    year = {2013},
    journal = {Journal of Chemical Information and Modeling},
    author = {Sasamori, T.},
    number = {9},
    pages = {1689--1699},
    volume = {53},
    isbn = {9788578110796},
    doi = {10.1017/CBO9781107415324.004},
    issn = {1098-6596},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {icle}
}

@article{Noble2013,
    title = {{The thermal reactivity of HCN and NH3 in interstellar ice analogues}},
    year = {2013},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Noble, J. A. and Theule, P. and Borget, F. and Danger, G. and Chomat, M. and Duvernay, F. and Mispelaer, F. and Chiavassa, T.},
    number = {4},
    pages = {3262--3273},
    volume = {428},
    doi = {10.1093/mnras/sts272},
    issn = {00358711},
    arxivId = {arXiv:1210.7066v1},
    keywords = {Astrochemistry, ISM: molecules, Methods: laboratory, Molecular data, Molecular processes}
}

@article{Noble2013b,
    title = {{The thermal reactivity of HCN and NH3in interstellar ice analogues}},
    year = {2013},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Noble, J. A. and Theule, P. and Borget, F. and Danger, G. and Chomat, M. and Duvernay, F. and Mispelaer, F. and Chiavassa, T.},
    number = {4},
    pages = {3262--3273},
    volume = {428},
    doi = {10.1093/mnras/sts272},
    issn = {00358711},
    arxivId = {1210.7066},
    keywords = {Astrochemistry, ISM: molecules, Methods: laboratory, Molecular data, Molecular processes}
}

@article{McKay1989,
    title = {{The thermal structure of Titan's atmosphere.}},
    year = {1989},
    journal = {Icarus},
    author = {McKay, C P and Pollack, J B and Courtin, R},
    pages = {23--53},
    volume = {80},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(89)90160-7},
    issn = {00191035},
    pmid = {11538676},
    keywords = {NASA Center ARC, NASA Discipline Exobiology, NASA Discipline Number 52-50, NASA Program Exobiology}
}

@article{Snowden2013,
    title = {{The thermal structure of Titan’s upper atmosphere, I: Temperature profiles from Cassini INMS observations}},
    year = {2013},
    journal = {Icarus},
    author = {Snowden, D and Yelle, R V and Cui, J and Wahlund, J and Edberg, N J T and {\AA}gren, K},
    number = {1},
    pages = {552--582},
    volume = {226},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.06.006},
    doi = {10.1016/j.icarus.2013.06.006},
    issn = {0019-1035}
}

@article{Snowden2014,
    title = {{The thermal structure of Titan’s upper atmosphere, II: Energetics}},
    year = {2014},
    journal = {Icarus},
    author = {Snowden, D and Yelle, R V},
    pages = {64--77},
    volume = {228},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.08.027},
    doi = {10.1016/j.icarus.2013.08.027},
    issn = {0019-1035},
    keywords = {"Atmosphere, "Titan, Aeronomy, atmosphere", structure"}
}

@article{Sciamma-OBrien2015,
    title = {{The THS experiment: Simulating Titan's atmospheric chemistry at low temperature (200 K)}},
    year = {2015},
    journal = {Proceedings of the International Astronomical Union},
    author = {Sciamma-O'Brien, Ella and Upton, Kathleen T. and Beauchamp, Jack L. and Salama, Farid},
    number = {A29A},
    pages = {327--328},
    volume = {11},
    url = {https://www.cambridge.org/core/product/identifier/S1743921316003197/type/journal_article},
    doi = {10.1017/S1743921316003197},
    issn = {1743-9213},
    keywords = {astrochemistry, laboratory, methods, molecular processes, planets and, plasmas}
}

@article{Moore2000,
    title = {{The Tidal Response of Europa}},
    year = {2000},
    journal = {Icarus},
    author = {Moore, William B. and Schubert, Gerald},
    number = {1},
    pages = {317--319},
    volume = {147},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103500964601},
    isbn = {0019-1035},
    doi = {10.1006/icar.2000.6460},
    issn = {00191035}
}

@misc{Sagan1982,
    title = {{The tide in the seas of Titan}},
    year = {1982},
    booktitle = {Nature},
    author = {Sagan, Carl and Dermott, S F},
    pages = {731},
    volume = {300},
    doi = {10.1038/300731a0},
    issn = {00280836}
}

@article{Lebreton2012,
    title = {{The Titan Cassini-Huygens Probe}},
    year = {2012},
    author = {Lebreton, J. P.},
    pages = {92195},
    doi = {10.1038/nature04347.}
}

@misc{Sagan,
    title = {{The Titan Haze Revisited - Origin and production rates}},
    author = {Sagan, C.}
}

@article{Sciamma-OBrien2017,
    title = {{The Titan Haze Simulation (THS) experiment on COSmIC. Part II. Ex-situ analysis of aerosols produced at low temperature}},
    year = {2017},
    journal = {Icarus},
    author = {Sciamma-O'Brien, Ella and Upton, Kathleen T. and Salama, Farid},
    pages = {214--226},
    volume = {289},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2017.02.004},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2017.02.004},
    issn = {10902643},
    keywords = {Aeronomy, Atmospheres, Chemistry, Experimental techniques, Spectroscopy, Titan, Atmosphere}
}

@article{Sciamma-OBrien2014,
    title = {{The Titan haze simulation experiment on cOsmic: Probing titan's atmospheric chemistry at low temperature}},
    year = {2014},
    journal = {Icarus},
    author = {Sciamma-O'Brien, Ella and Ricketts, Claire L. and Salama, Farid},
    pages = {325--336},
    volume = {243},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.08.004},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.08.004},
    issn = {10902643},
    keywords = {Atmospheres, Experimental techniques, Organic chemistry, Titan, atmosphere, chemistry}
}

@article{Fortenberry2011,
    title = {{The trans-HOCO radical: Quartic force fields, vibrational frequencies, and spectroscopic constants}},
    year = {2011},
    journal = {Journal of Chemical Physics},
    author = {Fortenberry, Ryan C. and Huang, Xinchuan and Francisco, Joséeph S. and Crawford, T. Daniel and Lee, Timothy J.},
    number = {13},
    pages = {1--8},
    volume = {135},
    isbn = {00219606},
    doi = {10.1063/1.3643336},
    issn = {00219606},
    pmid = {21992299}
}

@article{Bandy1993,
    title = {{The ultraviolet photochemistry of diacetylene : Direct detection products of the metastable C4Hg + C4H2 reaction}},
    year = {1993},
    journal = {J. Chem. Phys.},
    author = {Bandy, Ralph E and Lakshminarayan, Chitra and Frost, Rex K and Zwiera, Timothy S},
    number = {April},
    volume = {98}
}

@article{Bandy1993b,
    title = {{The ultraviolet photochemistry of diacetylene: Direct detection of primary * products of the metastable C4H 2 + C4H2 reaction}},
    year = {1993},
    journal = {The Journal of Chemical Physics},
    author = {Bandy, Ralph E and Lakshminarayan, Chitra and Frost, Rex K and Zwier, Timothy S},
    volume = {5362},
    doi = {10.1063/1.464909}
}

@article{Fleury2015,
    title = {{The upper atmopshere of the early Earth , a source of prebiotic organic compounds}},
    year = {2015},
    author = {Fleury, Benjamin}
}

@article{Nuth1982,
    title = {{The vacuum ultraviolet spectra of HCN, C2N2, and CH3CN}},
    year = {1982},
    journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
    author = {Nuth, Joseph A. and Glicker, Sol},
    number = {3},
    pages = {223--231},
    volume = {28},
    doi = {10.1016/0022-4073(82)90025-5},
    issn = {00224073}
}

@article{Michels1950,
    title = {{The vapour pressure of Ethylene}},
    year = {1950},
    journal = {Physica},
    author = {Michels, A and Wassenaar, T},
    number = {3},
    pages = {2--5}
}

@article{SinozakiH.HaraR.1926,
    title = {{The vapour pressures of Hydrogen Cyanide}},
    year = {1926},
    author = {Sinozaki, H., Hara, R., and Shinroky Mitsukuri},
    number = {1923},
    pages = {1924--1926},
    volume = {26}
}

@article{Yelle2006,
    title = {{The vertical structure of Titan's upper atmosphere from Cassini Ion Neutral Mass Spectrometer measurements}},
    year = {2006},
    journal = {Icarus},
    author = {Yelle, Roger V and Borggren, N and Haye, V De and Kasprzak, W T and Niemann, H B},
    number = {2},
    pages = {567--576},
    volume = {182},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103505004033},
    doi = {10.1016/j.icarus.2005.10.029},
    issn = {00191035},
    keywords = {aeronomy, planets}
}

@article{Gent,
    title = {{The Views of Christiaan Huygens on Astrology The Birth of Christiaan Huygens}},
    author = {Gent, Robert H Van}
}

@article{Jolly2010,
    title = {{THE {$\nu$}8 BENDING MODE OF DIACETYLENE : FROM LABORATORY SPECTROSCOPY TO THE DETECTION OF 13 C ISOTOPOLOGUES IN TITAN’S ATMOSPHERE}},
    year = {2010},
    journal = {The Astrophysical Journal},
    author = {Jolly, A and Fayt, A and Benilan, Y and Jacquemart, D and Nixon, C A and Jennings, D E},
    pages = {852--859},
    doi = {10.1088/0004-637X/714/1/852},
    keywords = {astrochemistry, atmospheres, color figures, detection, molecular data, online-only material, planets and satellites}
}

@article{Palaudoux2012,
    title = {{Theoretical investigations of the N 2 H 2 + cation and of its reactivity Theoretical investigations of the N 2 H 2 ¿ cation and of its reactivity}},
    year = {2012},
    author = {Palaudoux, J and Hochlaf, M},
    number = {2004},
    volume = {1782},
    doi = {10.1063/1.1765097}
}

@article{Vila2000,
    title = {{Theoretical study of the low-lying electronically excited states of diacetylene}},
    year = {2000},
    journal = {Journal of Physical Chemistry A},
    author = {Vila, Fernando and Borowski, Piotr and Jordan, Kenneth D.},
    number = {39},
    pages = {9009--9016},
    volume = {104},
    doi = {10.1021/jp001969c},
    issn = {10895639}
}

@article{Nayak2005,
    title = {{Theoretical study on the excited states of HCN}},
    year = {2005},
    journal = {Journal of Chemical Physics},
    author = {Nayak, Malaya K. and Chaudhuri, Rajat K. and Krishnamachari, S. N L G},
    number = {18},
    pages = {0--4},
    volume = {122},
    doi = {10.1063/1.1895669},
    issn = {00219606},
    pmid = {15918720}
}

@article{He2015,
    title = {{Thermal degradation of organics for pyrolysis in space: Titan's atmospheric aerosol case study}},
    year = {2015},
    journal = {Icarus},
    author = {He, Jing and Buch, Arnaud and Carrasco, Nathalie and Szopa, Cyril},
    pages = {205--212},
    volume = {248},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.10.010},
    doi = {10.1016/j.icarus.2014.10.010},
    issn = {10902643},
    keywords = {Experimental techniques, Instrumentation, Titan, Titan, atmosphere}
}

@article{Hussmann2002,
    title = {{Thermal Equilibrium States of Europa's Ice Shell: Implications for Internal Ocean Thickness and Surface Heat Flow}},
    year = {2002},
    journal = {Icarus},
    author = {Hussmann, H. and Spohn, Tilman and Wieczerkowski, Karin},
    number = {1},
    pages = {143--151},
    volume = {156},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103501967764},
    doi = {10.1006/icar.2001.6776},
    issn = {00191035},
    keywords = {europa, interiors, satellites of jupiter, tides}
}

@article{Samuelson1991,
    title = {{Thermal infrared properties of Titan's stratospheric aerosol}},
    year = {1991},
    author = {Samuelson, Robert E. and Mayo, Louis a.},
    pages = {207--219},
    volume = {219}
}

@article{Ojakangas1989a,
    title = {{Thermal State of an Ice Shell on Europa}},
    year = {1989},
    journal = {Icarus},
    author = {Ojakangas, G. W. and Stevenson, D. J.},
    pages = {220--241},
    volume = {241}
}

@article{Tokano2005,
    title = {{Thermal structure of putative hydrocarbon lakes on Titan}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {Tokano, Tetsuya},
    number = {2},
    pages = {286--294},
    volume = {36},
    isbn = {0273-1177},
    doi = {10.1016/j.asr.2005.03.051},
    issn = {02731177},
    keywords = {Exobiology, Lakes, Thermal structure, Titan}
}

@article{Gall2017,
    title = {{Thermally anomalous features in the subsurface of Enceladus ’ s south polar terrain}},
    year = {2017},
    journal = {Nature Publishing Group},
    author = {Gall, A Le and Leyrat, C and Janssen, M A and Choblet, G and Tobie, G and Bourgeois, O and Lucas, A and Howett, C and Kirk, R and Lorenz, R D and West, R D and Stolzenbach, A and Mass{\'{e}}, M and Hayes, A H},
    number = {March},
    pages = {1--5},
    volume = {1},
    publisher = {Macmillan Publishers Limited, part of Springer Nature.},
    url = {http://dx.doi.org/10.1038/s41550-017-0063},
    doi = {10.1038/s41550-017-0063}
}

@article{Kosower2007,
    title = {{Thin-film infrared spectroscopy of acetonitrile}},
    year = {2007},
    journal = {ChemPhysChem},
    author = {Kosower, Edward M. and Markovich, Gil and Borz, Galina},
    number = {17},
    pages = {2513--2519},
    volume = {8},
    doi = {10.1002/cphc.200700465},
    issn = {14394235},
    pmid = {17957656},
    keywords = {IR spectroscopy, Nanostructures, Nitrites, Thin films, Vicinal region}
}

@article{Pernot2010,
    title = {{Tholinomics—Chemical Analysis of Nitrogen-Rich Polymers}},
    year = {2010},
    journal = {Analytical Chemistry},
    author = {Pernot, Pascal and Carrasco, Nathalie and Thissen, Roland and Schmitz-Afonso, Isabelle},
    number = {4},
    pages = {1371--1380},
    volume = {82},
    url = {http://pubs.acs.org/doi/abs/10.1021/ac902458q},
    isbn = {0003-2700},
    doi = {10.1021/ac902458q},
    issn = {0003-2700},
    pmid = {20102174}
}

@article{Cruikshank2005,
    title = {{Tholins as coloring agents on outer Solar System bodies}},
    year = {2005},
    author = {Cruikshank, Dale P and Imanaka, Hiroshi and Ore, Cristina M Dalle},
    pages = {178--183},
    volume = {36},
    doi = {10.1016/j.asr.2005.07.026},
    keywords = {1, bodies in the outer, color is defined, colors ranging from neutral, exhibit, infrared spectroscopy, organic chemistry, oss, outer solar system, solar system, solid bodies in the, the colors of small, tholin, titan, to very red}
}

@article{Sagan1979,
    title = {{Tholins: organic chemistry of interstellar grains and gas}},
    year = {1979},
    journal = {Nature},
    author = {Sagan, C. and Khare, B. N.},
    number = {5692},
    pages = {102--107},
    volume = {277},
    url = {http://adsabs.harvard.edu/abs/1979Natur.277..102S},
    isbn = {9788578110796},
    doi = {10.1038/277102a0},
    issn = {0028-0836},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {COSMIC GASES, GAS CHROMATOGRAPHY, INFRARED SPECTRA, INTERSTELLAR CHEMISTRY, MASS SPECTROSCOPY, ORGANIC CHEMISTRY, ORGANIC COMPOUNDS, PHOTODISSOCIATION, RADIATION CHEMISTRY, SOLIDS, ULTRAVIOLET RADIATION}
}

@article{Rauscher2013,
    title = {{THREE-DIMENSIONAL ATMOSPHERIC CIRCULATION MODELS OF HD 189733b AND HD 209458b WITH CONSISTENT MAGNETIC DRAG AND OHMIC DISSIPATION}},
    year = {2013},
    journal = {The Astrophysical Journal},
    author = {Rauscher, Emily and Menou, Kristen},
    number = {1},
    pages = {103},
    volume = {764},
    url = {http://stacks.iop.org/0004-637X/764/i=1/a=103?key=crossref.ad7b94496d11a1b888999a0dc62fe00f},
    doi = {10.1088/0004-637X/764/1/103},
    issn = {0004-637X},
    keywords = {color figures, hd 189733b, hd 209458b, hydrodynamics, individual, magnetic fields, methods, numerical, online-only material, planets and satellites}
}

@article{Snowden2007,
    title = {{Three-dimensional multifluid simulation of the plasma interaction at Titan}},
    year = {2007},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Snowden, D. and Winglee, R. and Bertucci, C. and Dougherty, M.},
    number = {12},
    pages = {1--9},
    volume = {112},
    isbn = {0148-0227},
    doi = {10.1029/2007JA012393},
    issn = {21699402},
    keywords = {Titan, doi:10.1029/2007JA012393, http://dx.doi.org/10.1029/2007JA012393, induced magnetosphere, multifluid simulation}
}

@article{Kim2000,
    title = {{Three-Micrometer CH4 Line Emission from Titan's High-Altitude Atmosphere}},
    year = {2000},
    journal = {Icarus},
    author = {Kim, S},
    number = {2},
    pages = {588--591},
    volume = {147},
    url = {http://dx.doi.org/10.1006/icar.2000.6481},
    doi = {10.1006/icar.2000.6481},
    issn = {00191035}
}

@article{Kleuskens2006,
    title = {{Tidal deformation of Europa and Phobos: implications on their structure and history}},
    year = {2006},
    journal = {October},
    author = {Kleuskens, P},
    number = {October}
}

@article{Cassen1980,
    title = {{Tidal dissipation in Europa: a correction}},
    year = {1980},
    journal = {Geophysical Research Letters},
    author = {Cassen, P. and Peale, S. J. and Reynolds, R. T.},
    number = {11},
    pages = {987--988},
    volume = {7}
}

@misc{Sohl1995,
    title = {{Tidal dissipation on Titan}},
    year = {1995},
    booktitle = {Icarus},
    author = {Sohl, F and Sears, W D and Lorenz, R D},
    pages = {278--294},
    volume = {115},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-data_query?bibcode=1995Icar..115..278S&link_type=EJOURNAL%5Cnpapers2://publication/doi/10.1006/icar.1995.1097},
    doi = {10.1006/icar.1995.1097},
    issn = {00191035}
}

@article{Tobie2005,
    title = {{Tidal dissipation within large icy satellites: Applications to Europa and Titan}},
    year = {2005},
    journal = {Icarus},
    author = {Tobie, G. and Mocquet, A. and Sotin, C.},
    number = {2},
    pages = {534--549},
    volume = {177},
    isbn = {00191035},
    doi = {10.1016/j.icarus.2005.04.006},
    issn = {00191035},
    keywords = {Europa, Ice, Large icy satellites, Silicate, Tidal dissipation, Titan, Viscoelasticity}
}

@article{Peale1980,
    title = {{Tidal dissipation, orbital evolution, and the nature of Saturn's inner satellites}},
    year = {1980},
    journal = {Icarus},
    author = {Peale, S. J. and Cassen, P and Reynolds, RT},
    pages = {1196--1205},
    volume = {72},
    url = {http://www.sciencedirect.com/science/article/pii/0019103580900883},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(80)90088-3},
    issn = {00191035}
}

@article{Segatz1988,
    title = {{Tidal dissipation, surface heat flow, and figure of viscoelastic models of Io}},
    year = {1988},
    journal = {Icarus},
    author = {Segatz, M. and Spohn, T. and Ross, M. N. and Schubert, G.},
    number = {2},
    pages = {187--206},
    volume = {75},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(88)90001-2},
    issn = {10902643}
}

@article{Chyba1989,
    title = {{Tidal evolution in the Neptune-Triton system}},
    year = {1989},
    journal = {Astronomy {\&} Astrophysics},
    author = {Chyba, C. F. and Jankowski, D. G. and Nicholson, P. D.}
}

@article{Cuk2016,
    title = {{Tidal evolution of the Moon from a high-obliquity, high-angular-momentum Earth}},
    year = {2016},
    journal = {Nature},
    author = {{\'{C}}uk, Matija and Hamilton, Douglas P. and Lock, Simon J. and Stewart, Sarah T.},
    number = {7629},
    pages = {402--406},
    volume = {539},
    publisher = {Nature Publishing Group},
    url = {http://www.nature.com/doifinder/10.1038/nature19846},
    isbn = {9788578110796},
    doi = {10.1038/nature19846},
    issn = {0028-0836}
}

@article{Moore2003,
    title = {{Tidal heating and convection in Io}},
    year = {2003},
    journal = {Journal of Geophysical Research},
    author = {Moore, W. B.},
    number = {E8},
    pages = {1--6},
    volume = {108},
    isbn = {0148-0227},
    doi = {10.1029/2002JE001943},
    issn = {0148-0227},
    keywords = {http://dx.doi.org/10.1029/2002JE001943, doi:10.102}
}

@article{Driscoll2015,
    title = {{Tidal Heating of Earth-like Exoplanets around M Stars: Thermal, Magnetic, and Orbital Evolutions}},
    year = {2015},
    journal = {Astrobiology},
    author = {Driscoll, P.E. and Barnes, R.},
    number = {9},
    pages = {739--760},
    volume = {15},
    url = {http://online.liebertpub.com/doi/10.1089/ast.2015.1325},
    isbn = {10.1089/ast.2015.1325},
    doi = {10.1089/ast.2015.1325},
    issn = {1531-1074},
    pmid = {26393398},
    arxivId = {1509.07452}
}

@article{Jackson2008,
    title = {{Tidal heating of terrestrial extrasolar planets and implications for their habitability}},
    year = {2008},
    journal = {Monthly Notices of the Royal Astronomical Society},
    author = {Jackson, Brian and Barnes, Rory and Greenberg, Richard},
    number = {1},
    pages = {237--245},
    volume = {391},
    doi = {10.1111/j.1365-2966.2008.13868.x},
    issn = {00358711},
    arxivId = {0808.2770},
    keywords = {Astrobiology, Celestial mechanics, Planetary systems}
}

@article{Greenberga,
    title = {{Tidal stress on Europa: Non-synchronous Rotation and Diurnal Variations}},
    author = {Greenberg, Richard and Hoppa, Gregory and Geissler, Paul and Tufts, B R and Durda, Daniel},
    pages = {4--5}
}

@article{Greenberg2003,
    title = {{Tidal stress patterns on Europa's crust}},
    year = {2003},
    journal = {Celestial Mechanics and Dynamical Astronomy},
    author = {Greenberg, Richard and Hoppa, Gregory V. and Bart, Gwen and Hurford, Terry},
    number = {1-2},
    pages = {171--188},
    volume = {87},
    doi = {10.1023/A:1026169424511},
    issn = {09232958},
    keywords = {Europa, Stress, Tides}
}

@article{Patthoff2017,
    title = {{Tidal Stresses and Volcanism on Io}},
    year = {2017},
    journal = {LPSC},
    author = {Patthoff, D. A. and Davies, A. G.},
    pages = {1--2},
    volume = {1748}
}

@article{Folonier2017,
    title = {{Tidal synchronization of an anelastic multi-layered body. Titan’s synchronous rotation.}},
    year = {2017},
    author = {Folonier, Hugo and Ferraz-mello, Sylvio},
    arxivId = {arXiv:1706.08603v1},
    keywords = {atmospheric torque, creep, differentiated body, gravitational coupling, satellites, stationary rotation, synchronous rotation, tidal friction, tide, titan}
}

@article{Tokano2002,
    title = {{Tidal Winds on Titan Caused by Saturn}},
    year = {2002},
    journal = {International Journal of Solar System Studies},
    author = {Tokano, T},
    number = {2},
    pages = {499--515},
    volume = {158},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103502968831},
    isbn = {0019-1035},
    doi = {10.1006/icar.2002.6883},
    issn = {00191035},
    keywords = {atmos, atmospheric structure, meteorology, pheric, satellites saturn, tides, titan}
}

@article{Tokano2002b,
    title = {{Tidal winds on Titan caused by Saturn}},
    year = {2002},
    journal = {Icarus},
    author = {Tokano, Tetsuya and Neubauer, Fritz M.},
    number = {2},
    pages = {499--515},
    volume = {158},
    isbn = {0019-1035},
    doi = {10.1006/icar.2002.6883},
    issn = {00191035},
    keywords = {Atmospheric, Atmospheric structure, Meteorology, Satellites of Saturn, Tides, Titan}
}

@article{Tobie2003,
    title = {{Tidally heated convection: Constraints on Europa's ice shell thickness}},
    year = {2003},
    journal = {Journal of Geophysical Research},
    author = {Tobie, Gabriel and Choblet, Gael and Sotin, Christophe},
    number = {E11},
    pages = {5124},
    volume = {108},
    url = {http://doi.wiley.com/10.1029/2003JE002099},
    doi = {10.1029/2003JE002099},
    issn = {0148-0227}
}

@article{Cameron2012,
    title = {{Tidally-Driven Strike-Slip Failure Mechanics on Ganymede}},
    year = {2012},
    author = {Cameron, Marissa E and Smith-Konter, Bridget and Pappalardo, Robert T. and Collins, Geoffrey C. and Nimmo, Francis},
    number = {2008},
    pages = {2008}
}

@article{Wunsch2016,
    title = {{Tides of global ice-covered oceans}},
    year = {2016},
    journal = {Icarus},
    author = {Wunsch, Carl},
    pages = {122--130},
    volume = {274},
    publisher = {Elsevier Inc.},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103516300227},
    doi = {http://dx.doi.org/10.1016/j.icarus.2016.03.026},
    issn = {0019-1035},
    keywords = {Ice-covered satellites, Neoproterozoic Earth, Tides}
}

@article{Wahr2006,
    title = {{Tides on Europa, and the thickness of Europa's icy shell}},
    year = {2006},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Wahr, J. M. and Zuber, M. T. and Smith, David E. and Lunine, J. I.},
    number = {12},
    pages = {1--10},
    volume = {111},
    isbn = {9789401152525},
    doi = {10.1029/2006JE002729},
    issn = {01480227}
}

@article{Beuthe2015a,
    title = {{Tides on Europa: The membrane paradigm}},
    year = {2015},
    journal = {Icarus},
    author = {Beuthe, Mikael},
    pages = {109--134},
    volume = {248},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.10.027},
    doi = {10.1016/j.icarus.2014.10.027},
    issn = {10902643},
    arxivId = {1410.4735},
    keywords = {Europa, Planetary dynamics, Tectonics, Tides}
}

@article{Beuthe2015,
    title = {{Tides on Europa: The membrane paradigm}},
    year = {2015},
    journal = {Icarus},
    author = {Beuthe, Mikael},
    pages = {109--134},
    volume = {248},
    doi = {10.1016/j.icarus.2014.10.027},
    issn = {10902643},
    arxivId = {1410.4735},
    keywords = {Europa, Planetary dynamics, Tectonics, Tides}
}

@article{Jara-Orue2016,
    title = {{Tides on Jupiter's moon Ganymede and their relation to its internal structure}},
    year = {2016},
    journal = {Netherlands Journal of Geosciences},
    author = {Jara-Oru{\'{e}}, H.M. and Vermeersen, B.L.A.},
    number = {02},
    pages = {191--201},
    volume = {95},
    url = {http://www.journals.cambridge.org/abstract_S0016774615000232},
    doi = {10.1017/njg.2015.23},
    issn = {0016-7746},
    keywords = {Ganymede, interior, solid body, tides}
}

@article{Ma2009,
    title = {{Time-dependent global MHD simulations of Cassini T32 flyby: From magnetosphere to magnetosheath}},
    year = {2009},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Ma, Y. J. and Russell, C. T. and Nagy, A. F. and Toth, G. and Bertucci, C. and Dougherty, M. K. and Neubauer, F. M. and Wellbrock, A. and Coates, A. J. and Garnier, P. and Wahlund, J. E. and Cravens, T. E. and Crary, F. J.},
    number = {3},
    pages = {1--13},
    volume = {114},
    isbn = {0148-0227},
    doi = {10.1029/2008JA013676},
    issn = {21699402}
}

@article{Howling1994,
    title = {{Time-resolved measurements of highly polymerized negative ions in radio frequency silane plasma deposition experiments}},
    year = {1994},
    journal = {Journal of Applied Physics},
    author = {Howling, A. A. and Sansonnens, L. and Dorier, J. L. and Hollenstein, Ch},
    number = {3},
    pages = {1340--1353},
    volume = {75},
    isbn = {doi:10.1063/1.356413},
    doi = {10.1063/1.356413},
    issn = {00218979}
}

@article{Sebree2014,
    title = {{Titan aerosol analog absorption features produced from aromatics in the far infrared}},
    year = {2014},
    journal = {Icarus},
    author = {Sebree, Joshua A. and Trainer, Melissa G. and Loeffler, Mark J. and Anderson, Carrie M.},
    pages = {146--152},
    volume = {236},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.03.039},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2014.03.039},
    issn = {10902643},
    keywords = {Atmospheres, chemistry, Spectroscopy, Titan, atmosphere}
}

@article{Rages1980,
    title = {{Titan aerosols: Optical properties and vertical distribution}},
    year = {1980},
    journal = {Icarus},
    author = {Rages, Kathy and Pollack, James B.},
    number = {1},
    pages = {119--130},
    volume = {41},
    isbn = {0019-1035},
    doi = {10.1016/0019-1035(80)90164-5},
    issn = {10902643}
}

@article{Navarro-Gonzalez2005,
    title = {{Titan before Cassini/Huygens: Exo/astrobiology aspects}},
    year = {2005},
    journal = {Advances in Space Research},
    author = {Navarro-Gonz{\'{a}}lez, Rafael and Raulin, Francois},
    number = {2},
    pages = {237--240},
    volume = {36},
    doi = {10.1016/j.asr.2005.10.001},
    issn = {02731177}
}

@book{Brown2009a,
    title = {{Titan from Cassini-Huygens}},
    year = {2009},
    author = {Brown, R. H. and Lebreton, J. P. and Waite, J. H.},
    edition = {Springer},
    pages = {412},
    publisher = {Springer}
}

@article{Brown2009,
    title = {{TItan from Cassini-Huygens}},
    year = {2009},
    author = {Brown, R. H. and Lebreton, J. P. and Waite, J.H.}
}

@article{Lebonnois2012,
    title = {{Titan global climate model: A new 3-dimensional version of the IPSL Titan GCM}},
    year = {2012},
    journal = {Icarus},
    author = {Lebonnois, S. and Burgalat, J. and Rannou, P. and Charnay, B.},
    number = {1},
    pages = {707--722},
    volume = {218},
    doi = {10.1016/j.icarus.2011.11.032},
    issn = {00191035},
    keywords = {Atmospheres, Dynamics, Titan}
}

@article{Modolo2009,
    title = {{Titan ionospheric conductivities from Cassini measurements}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Modolo, R and Opgenoorth, H J and Strobel, D and Garnier, P and Mu, I},
    pages = {1828--1833},
    volume = {57},
    doi = {10.1016/j.pss.2009.01.007}
}

@article{Nixon2016,
    title = {{Titan Science with the James Webb Space Telescope}},
    year = {2016},
    journal = {Astronomical Society of the Pacific},
    author = {Nixon, Conor A. and Achterberg, R. K. and {\'{A}}d{\'{a}}mkovics, Mátá and B{\'{e}}zard, Bruno and Bjoraker, Gordon L. and Cornet, Thmas and Hayes, Alexander G. and Lellouch, Emmanuel and Lemmon, Mark T. and L{\'{o}}pez-Puertas, Manuel and Rodriguez, Sébastien and Sotin, Christophe and Teanby, Nicholas A. and Turtle, Elizabeth P. and West, Robert A.},
    number = {959},
    pages = {1--28},
    volume = {128},
    publisher = {IOP Publishing},
    url = {http://dx.doi.org/10.1088/1538-3873/128/959/018009},
    doi = {10.1088/1538-3873/128/959/018009},
    issn = {0004-6280},
    arxivId = {arXiv:1510.05878v1},
    keywords = {color fi gures, comets, comets: general, general, methods, methods: observational, observational, online material}
}

@article{Robinson2014,
    title = {{Titan solar occultation observations reveal transit spectra of a hazy world.}},
    year = {2014},
    journal = {Proceedings of the National Academy of Sciences of the United States of America},
    author = {Robinson, Tyler D and Maltagliati, Luca and Marley, Mark S and Fortney, Jonathan J},
    number = {25},
    pages = {9042--7},
    volume = {111},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/24876272},
    doi = {10.1073/pnas.1403473111},
    issn = {1091-6490},
    pmid = {24876272},
    arxivId = {arXiv:1406.3314v1}
}

@article{Bellucci2009,
    title = {{Titan solar occultation observed by Cassini/VIMS: Gas absorption and constraints on aerosol composition}},
    year = {2009},
    journal = {Icarus},
    author = {Bellucci, A. and Sicardy, B. and Drossart, P. and Rannou, P. and Nicholson, P. D. and Hedman, M. and Baines, K. H. and Burrati, B.},
    number = {1},
    pages = {198--216},
    volume = {201},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2008.12.024},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2008.12.024},
    issn = {00191035},
    keywords = {Atmospheres, Occultations, Titan, composition}
}

@article{Cable2012,
    title = {{Titan tholins: Simulating Titan organic chemistry in the Cassini-Huygens era}},
    year = {2012},
    journal = {Chemical Reviews},
    author = {Cable, Morgan L. and H{\"{o}}rst, Sarah M. and Hodyss, Robert and Beauchamp, Patricia M. and Smith, Mark A. and Willis, Peter A.},
    number = {3},
    pages = {1882--1909},
    volume = {112},
    doi = {10.1021/cr200221x},
    issn = {00092665},
    pmid = {22091924}
}

@article{Coustenis2010,
    title = {{Titan trace gaseous composition from CIRS at the end of the Cassini-Huygens prime mission}},
    year = {2010},
    journal = {Icarus},
    author = {Coustenis, A. and Jennings, D. E. and Nixon, C. A. and Achterberg, R. K. and Lavvas, P. and Vinatier, S. and Teanby, N. A. and Bjoraker, G. L. and Carlson, R. C. and Piani, L. and Bampasidis, G. and Flasar, F. M. and Romani, P. N.},
    number = {1},
    pages = {461--476},
    volume = {207},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.11.027},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.11.027},
    issn = {00191035},
    keywords = {Abundances, atmospheres, Atmospheres, chemistry, Atmospheres, composition, Organic chemistry, Satellites, atmospheres, Satellites, composition, Spectroscopy, Titan}
}

@article{Gilliam2011,
    title = {{Titan under a red dwarf star and as a rogue planet: Requirements for liquid methane}},
    year = {2011},
    journal = {Planetary and Space Science},
    author = {Gilliam, Ashley E. and McKay, Christopher P.},
    number = {9},
    pages = {835--839},
    volume = {59},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2011.03.012},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2011.03.012},
    issn = {00320633},
    keywords = {Gliese 581, Habitability, Liquid methane, Red dwarf stars, Titan}
}

@book{Lorenz2008,
    title = {{Titan unveiled : Saturn's mysterious moon explored}},
    year = {2008},
    author = {Lorenz, Ralph and Mitton, Jacqueline.},
    pages = {265},
    isbn = {9781400834754},
    issn = {0717-6163},
    pmid = {15003161},
    arxivId = {arXiv:1011.1669v3}
}

@book{Lorenz2008a,
    title = {{Titan Unveiled: Saturn's Mysterious Moon Explored}},
    year = {2008},
    author = {Lorenz, Ralph and Mitton, Jacqueline},
    pages = {246},
    isbn = {9780691125879}
}

@article{Huygens2001,
    title = {{Titan Winds Derived from Probe Radio Frequency Measurements}},
    year = {2001},
    author = {Huygens, T.H.E and Wind, Doppler},
    pages = {613--640}
}

@article{Simon2015,
    title = {{Titan ’ s induced magnetosphere under non-ideal upstream conditions : 3D multi-species hybrid simulations}},
    year = {2015},
    journal = {Planetary and Space Science},
    author = {Simon, Sven and Motschmann, Uwe},
    number = {14-15},
    pages = {2001--2015},
    volume = {57},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.pss.2009.08.010},
    doi = {10.1016/j.pss.2009.08.010},
    issn = {0032-0633},
    keywords = {Hybrid model, Plasma interaction with moons, Real-time simulations, Saturn's magnetosphere, Titan}
}

@article{Anderson2011,
    title = {{Titan's aerosol and stratospheric ice opacities between 18 and 500 um: Vertical and spectral characteristics from Cassini CIRS}},
    year = {2011},
    journal = {Icarus},
    author = {Anderson, C. M. and Samuelson, R. E.},
    number = {2},
    pages = {762--778},
    volume = {212},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.01.024},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2011.01.024},
    issn = {00191035},
    keywords = {Ices, Radiative transfer, Titan}
}

@article{Horst2017,
    title = {{Titan's Atmosphere and Climate}},
    year = {2017},
    journal = {Journal of Geophysical Research: Planets},
    author = {H{\"{o}}rst, Sarah M.},
    pages = {432--482},
    url = {http://arxiv.org/abs/1702.08611},
    doi = {10.1002/2016JE005240},
    issn = {21699097},
    arxivId = {1702.08611}
}

@article{Maltagliati2015,
    title = {{Titan's atmosphere as observed by Cassini/VIMS solar occultations: CH4, CO and evidence for C2H6 absorption}},
    year = {2015},
    journal = {Icarus},
    author = {Maltagliati, Luca and Bezard, Bruno and Vinatier, Sandrine and Hedman, Matthew M. and Lellouch, Emmanuel and Nicholson, Philip D. and Sotin, Christophe and de Kok, Remco J. and Sicardy, Bruno},
    pages = {1--24},
    volume = {248},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2014.10.004},
    doi = {10.1016/j.icarus.2014.10.004},
    issn = {10902643},
    keywords = {Atmospheres, Infrared observations, Occultations, Spectroscopy, Titan, atmosphere, composition}
}

@article{Coustenis2003a,
    title = {{Titan's atmosphere from ISO mid-infrared spectroscopy}},
    year = {2003},
    journal = {Icarus},
    author = {Coustenis, A. and Salama, A. and Schulz, B. and Ott, S. and Lellouch, E. and Encrenaz, Th and Gautier, D. and Feuchtgruber, H.},
    number = {2},
    pages = {383--403},
    volume = {161},
    doi = {10.1016/S0019-1035(02)00028-3},
    issn = {00191035},
    keywords = {Atmosphere, ISO, Infrared observations, Satellites, Titan}
}

@article{Peng2013,
    title = {{Titan's atmosphere simulation experiment using continuum UV-VUV synchrotron radiation}},
    year = {2013},
    journal = {Journal of Geophysical Research: Planets},
    author = {Peng, Z and Gautier, T and Carrasco, N and Pernot, P and Giuliani, A and Mahjoub, A and Correia, J.-J. and Buch, A and B{\'{e}}nilan, Y and Szopa, C and Cernogora, G},
    number = {4},
    pages = {778--788},
    volume = {118},
    url = {http://dx.doi.org/10.1002/jgre.20064},
    doi = {10.1002/jgre.20064},
    issn = {2169-9100},
    keywords = {0317 Chemical kinetic and photochemical properties, 0343 Planetary atmospheres, 0394 Instruments and techniques, 2459 Planetary ionospheres, 6281 Titan, Plasmas, Titan, laboratory simulation, photochemistry, planetary atmospheres}
}

@article{Samuelson2003,
    title = {{Titan's atmospheric engine: An overview}},
    year = {2003},
    journal = {Planetary and Space Science},
    author = {Samuelson, Robert E.},
    number = {2},
    pages = {127--145},
    volume = {51},
    isbn = {0032-0633},
    doi = {10.1016/S0032-0633(02)00143-5},
    issn = {00320633},
    keywords = {Atmosphere, Engine, Overview, Titan}
}

@article{Flasar2005,
    title = {{Titan's Atmospheric Temperatures, Winds, and Composition}},
    year = {2005},
    journal = {Science},
    author = {Flasar, F M and Achterberg, R K and Conrath, B J and Gierasch, P J and Kunde, V G and Nixon, C A and Bjoraker, G L and Jennings, D E and Romani, P N and Simon-Miller, A A and Bezard, B and Coustenis, A and Irwin, P G J and Teanby, N A and Brasunas, J and Pearl, J C and Segura, M E and Carlson, R C and Mamoutkine, A and Schinder, P J and Barucci, A and Courtin, R and Fouchet, T and Gautier, D and Lellouch, E and Marten, A and Prange, R and Vinatier, S and Strobel, D F and Calcutt, S B and Read, P L and Taylor, F W and Bowles, N and Samuelson, R E and Orton, G S and Spilker, L J and Owen, T C and Spencer, J R and Showalter, M R and Ferrari, C and Abbas, M M and Raulin, F and Edgington, S and Ade, P and Wishnow, E H},
    number = {5724},
    pages = {975--978},
    volume = {308},
    url = {http://www.sciencemag.org/cgi/content/abstract/308/5724/975},
    isbn = {1095-9203 (Electronic){\textbackslash}n0036-8075 (Linking)},
    doi = {10.1126/science.1111150},
    issn = {0036-8075},
    pmid = {15894528}
}

@article{Smith2004,
    title = {{Titan's atomic and molecular nitrogen tori}},
    year = {2004},
    journal = {Geophysical Research Letters},
    author = {Smith, H. T. and Johnson, R. E. and Shematovich, V. I.},
    number = {16},
    pages = {2--5},
    volume = {31},
    doi = {10.1029/2004GL020580},
    issn = {00948276},
    keywords = {doi:10.1029/2004GL020580, http://dx.doi.org/10.1029/2004GL020580}
}

@article{Rodriguez2011,
    title = {{Titan's cloud seasonal activity from winter to spring with Cassini/VIMS}},
    year = {2011},
    journal = {Icarus},
    author = {Rodriguez, S. and Le Mou{\'{e}}lic, S. and Rannou, P. and Sotin, C. and Brown, R. H. and Barnes, J. W. and Griffith, C. A. and Burgalat, J. and Baines, K. H. and Buratti, B. J. and Clark, R. N. and Nicholson, P. D.},
    number = {1},
    pages = {89--110},
    volume = {216},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.07.031},
    doi = {10.1016/j.icarus.2011.07.031},
    issn = {00191035},
    keywords = {Meteorology, Satellites, Atmospheres, Titan}
}

@article{Nixon2018,
    title = {{Titan's cold case files - Outstanding questions after Cassini-Huygens}},
    year = {2018},
    journal = {Planetary and Space Science},
    author = {Nixon, C. A. and Lorenz, R. D. and Achterberg, R. K. and Buch, A. and Coll, P. and Clark, R. N. and Courtin, R. and Hayes, A. and Iess, L. and Johnson, R. E. and Lopes, R. M.C. and Mastrogiuseppe, M. and Mandt, K. and Mitchell, D. G. and Raulin, F. and Rymer, A. M. and Todd Smith, H. and Solomonidou, A. and Sotin, C. and Strobel, D. and Turtle, E. P. and Vuitton, V. and West, R. A. and Yelle, R. V.},
    number = {January},
    pages = {50--72},
    volume = {155},
    publisher = {Elsevier Ltd},
    url = {https://doi.org/10.1016/j.pss.2018.02.009},
    doi = {10.1016/j.pss.2018.02.009},
    issn = {00320633}
}

@article{West2018a,
    title = {{Titan's Detached Haze Seasonal Cycle}},
    year = {2018},
    journal = {Nature Astronomy},
    author = {West, Robert A. and Seignovert, Benoît and Rannou, Pascal and Dumont, Philip and Turtle, Elizabeth P. and Perry, Jason and Roy, Mou and Ovanessian, Aida},
    number = {in press},
    isbn = {1844251411},
    doi = {10.1038/s41550-018-0434-z},
    issn = {2397-3366}
}

@article{Strobel2009,
    title = {{Titan's hydrodynamically escaping atmosphere: Escape rates and the structure of the exobase region}},
    year = {2008},
    journal = {Icarus},
    author = {Strobel, Darrell F.},
    number = {2},
    pages = {632--641},
    volume = {202},
    doi = {10.1016/j.icarus.2009.03.007},
    issn = {00191035},
    keywords = {Aeronomy, Atmospheres, Titan, dynamics, evolution, structure}
}

@article{Strobel2009b,
    title = {{Titan's hydrodynamically escaping atmosphere: Escape rates and the structure of the exobase region}},
    year = {2009},
    journal = {Icarus},
    author = {Strobel, Darrell F.},
    number = {2},
    pages = {632--641},
    volume = {202},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.03.007},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.03.007},
    issn = {00191035},
    keywords = {Aeronomy, Atmospheres, Titan, dynamics, evolution, structure}
}

@article{Bertucci2015,
    title = {{Titan's interaction with the supersonic solar wind}},
    year = {2015},
    journal = {Geophysical Research Letters},
    author = {Bertucci, C. and Hamilton, D. C. and Kurth, W. S. and Hospodarsky, G. and Mitchell, D. and Sergis, N. and Edberg, N. J T and Dougherty, M. K.},
    number = {2},
    pages = {193--200},
    volume = {42},
    doi = {10.1002/2014GL062106},
    issn = {19448007},
    arxivId = {astro-ph.EP/1410.4159},
    keywords = {Mars, Titan, Venus, solar wind}
}

@article{Lorenz2008b,
    title = {{Titan's inventory of organic surface materials}},
    year = {2008},
    journal = {Geophysical Research Letters},
    author = {Lorenz, Ralph D. and Mitchell, Karl L. and Kirk, Randolph L. and Hayes, Alexander G. and Aharonson, Oded and Zebker, Howard A. and Paillou, Phillipe and Radebaugh, Jani and Lunine, Jonathan I. and Janssen, Michael A. and Wall, Stephen D. and Lopes, Rosaly M. and Stiles, Bryan and Ostro, Steve and Mitri, Giuseppe and Stofan, Ellen R.},
    number = {2},
    pages = {4--9},
    volume = {35},
    doi = {10.1029/2007GL032118},
    issn = {00948276},
    keywords = {http://dx.doi.org/10.1029/2007GL032118, doi:10.102}
}

@article{McEwan2007,
    title = {{Titan's ion chemistry: A laboratory perspective}},
    year = {2007},
    journal = {Mass Spectrometry Reviews},
    author = {McEwan, Murray J. and Anicich, Vincent G.},
    number = {2},
    pages = {281--319},
    volume = {26},
    doi = {10.1002/mas.20117},
    issn = {02777037},
    pmid = {17216629},
    keywords = {Chemical processing, Ion-molecule, Ionosphere, Titan}
}

@article{Nagy1998,
    title = {{Titan's ionosphere: A review}},
    year = {1998},
    author = {Nagy, Andrew F and Cravens, Thomas E},
    pages = {38--44}
}

@article{Shebanits2017,
    title = {{Titan's ionosphere: A survey of solar EUV influences}},
    year = {2017},
    journal = {Journal of Geophysical Research: Space Physics},
    author = {Shebanits, O. and Vigren, E. and Wahlund, J. E. and Holmberg, M. K.G. and Morooka, M. and Edberg, N. J.T. and Mandt, K. E. and Waite, J. H.},
    number = {7},
    pages = {7491--7503},
    volume = {122},
    doi = {10.1002/2017JA023987},
    issn = {21699402},
    keywords = {Titan, correllations, ionosphere, ions, solar EUV}
}

@article{Cravens2005,
    title = {{Titan's ionosphere: Model comparisons with Cassini Ta data}},
    year = {2005},
    journal = {Geophysical Research Letters},
    author = {Cravens, T. E. and Robertson, I. P. and Clark, J. and Wahlund, J. E. and Waite, Jr H. and Ledvina, S. A. and Niemann, H. B. and Yelle, R. V. and Kasprzak, W. T. and Luhmann, J. G. and McNutt, R. L. and Ip, W. H. and De La Haye, V. and M??ller-Wodarg, I. and Young, D. T. and Coates, A. J.},
    number = {12},
    pages = {1--5},
    volume = {32},
    doi = {10.1029/2005GL023249},
    issn = {00948276}
}

@article{Westlake2012,
    title = {{Titan's ionospheric composition and structure: Photochemical modeling of Cassini INMS data}},
    year = {2012},
    journal = {Journal of Geophysical Research E: Planets},
    author = {Westlake, J. H. and Waite, J. H. and Mandt, K. E. and Carrasco, N. and Bell, J. M. and Magee, B. A. and Wahlund, J. E.},
    number = {1},
    pages = {1--21},
    volume = {117},
    isbn = {0148-0227},
    doi = {10.1029/2011JE003883},
    issn = {01480227}
}

@article{Turtle2018,
    title = {{Titan's Meteorology Over the Cassini Mission: Evidence for Extensive Subsurface Methane Reservoirs}},
    year = {2018},
    journal = {Geophysical Research Letters},
    author = {Turtle, E. P. and Perry, J. E. and Barbara, J. M. and Del Genio, A. D. and Rodriguez, S. and Le Mou{\'{e}}lic, S. and Sotin, C. and Lora, J. M. and Faulk, S. and Corlies, P. and Kelland, J. and MacKenzie, S. M. and West, R. A. and McEwen, A. S. and Lunine, J. I. and Pitesky, J. and Ray, T. L. and Roy, M.},
    number = {11},
    pages = {5320--5328},
    volume = {45},
    doi = {10.1029/2018GL078170},
    issn = {19448007},
    keywords = {Cassini, Titan, atmospheric modeling, clouds, methane cycle, seasonal change}
}

@article{Atreya2006,
    title = {{Titan's methane cycle}},
    year = {2006},
    journal = {Planetary and Space Science},
    author = {Atreya, Sushil K. and Adams, Elena Y. and Niemann, Hasso B. and Demick-Montelara, Jaime E. and Owen, Tobias C. and Fulchignoni, Marcello and Ferri, Francesca and Wilson, Eric H.},
    number = {12},
    pages = {1177--1187},
    volume = {54},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2006.05.028},
    issn = {00320633},
    keywords = {Meteorology, Methalogical cycle, Methane, Origin, Serpentinization, Titan}
}

@article{Gilliam2016,
    title = {{Titan's missing ethane: From the atmosphere to the subsurface}},
    year = {2016},
    journal = {Icarus},
    author = {Gilliam, Ashley E. and Lerman, Abraham},
    pages = {252--258},
    volume = {275},
    publisher = {Elsevier B.V.},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2016.04.025},
    issn = {10902643},
    keywords = {Atmospheres, chemistry, Prebiotic chemistry, Titan, atmosphere, Titan, surface}
}

@article{Morisson2016,
    title = {{Titan's organic aerosols: Molecular composition and structure of laboratory analogues inferred from pyrolysis gas chromatography mass spectrometry analysis}},
    year = {2016},
    journal = {Icarus},
    author = {Morisson, Marietta and Szopa, Cyril and Carrasco, Nathalie and Buch, Arnaud and Gautier, Thomas},
    pages = {442--454},
    volume = {277},
    publisher = {Elsevier Inc.},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103516302494},
    doi = {10.1016/j.icarus.2016.05.038},
    issn = {00191035},
    keywords = {"Atmospheres, composition", "Saturn, satellites", Experimental techniques, Prebiotic chemistry, Titan}
}

@misc{Scattergood1988,
    title = {{Titan's organic haze over the last four billion years}},
    year = {1988},
    author = {Scattergood, T W and Mckay, C P and Pollack, J. B. and Giver, C. R.}
}

@article{Nixon2009,
    title = {{Titan's prolific propane: The Cassini CIRS perspective}},
    year = {2009},
    journal = {Planetary and Space Science},
    author = {Nixon, C. A. and Jennings, D. E. and Flaud, J. M. and B{\'{e}}zard, B. and Teanby, N. A. and Irwin, P. G J and Ansty, T. M. and Coustenis, A. and Vinatier, S. and Flasar, F. M.},
    number = {13},
    pages = {1573--1585},
    volume = {57},
    isbn = {0032-0633},
    doi = {10.1016/j.pss.2009.06.021},
    issn = {00320633},
    arxivId = {0909.1794},
    keywords = {Abundance retrieval, Atmospheric abundances, outer planets, Infrared spectroscopy, Propane, Titan atmosphere}
}

@misc{Lemmon1993,
    title = {{Titan's Rotation: Surface Feature Observed}},
    year = {1993},
    author = {Lemmon, M. and Karkoschka, E. and Tomasko, M. G.}
}

@article{Teanby2009,
    title = {{Titan's stratospheric C2N2, C3H4, and C4H2 abundances from Cassini/CIRS far-infrared spectra}},
    year = {2009},
    journal = {Icarus},
    author = {Teanby, N. A. and Irwin, P. G J and de Kok, R. and Jolly, A. and B{\'{e}}zard, B. and Nixon, C. A. and Calcutt, S. B.},
    number = {2},
    pages = {620--631},
    volume = {202},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2009.03.022},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2009.03.022},
    issn = {00191035},
    keywords = {Atmospheres, Titan, composition}
}

@article{Hayes2016,
    title = {{Titan's surface and atmosphere}},
    year = {2016},
    journal = {Icarus},
    author = {Hayes, Alexander G. and Soderblom, Jason M. and {\'{A}}d{\'{a}}mkovics, Máté},
    pages = {1},
    volume = {270},
    doi = {10.1016/j.icarus.2016.02.029},
    issn = {10902643}
}

@article{Richardson2004,
    title = {{Titan's surface and rotation: New results from Voyager 1 images}},
    year = {2004},
    journal = {Icarus},
    author = {Richardson, James and Lorenz, Ralph D. and McEwen, Alfred},
    number = {1},
    pages = {113--124},
    volume = {170},
    doi = {10.1016/j.icarus.2004.03.010},
    issn = {00191035},
    keywords = {Atmosphere, Image processing, Satellites, Surface, Titan}
}

@article{Janssen2015,
    title = {{Titan's surface at 2.18-cm wavelength imaged by the Cassini RADAR radiometer: Results and interpretations through the first ten years of observation}},
    year = {2015},
    journal = {Icarus},
    author = {Janssen, M. A. and Le Gall, A. and Lopes, R. M. and Lorenz, R. D. and Malaska, M. J. and Hayes, A. G. and Neish, C. D. and Solomonidou, A. and Mitchell, K. L. and Radebaugh, J. and Keihm, S. J. and Choukroun, M. and Leyrat, C. and Encrenaz, P. J. and Mastrogiuseppe, M.},
    pages = {443--459},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.09.027},
    doi = {10.1016/j.icarus.2015.09.027},
    issn = {10902643},
    keywords = {Radio observations, Satellites, composition, Satellites, surfaces, Titan, surface}
}

@article{Janssen2009,
    title = {{Titan's surface at 2.2-cm wavelength imaged by the Cassini RADAR radiometer: Calibration and first results}},
    year = {2009},
    journal = {Icarus},
    author = {Janssen, M. A. and Lorenz, R. D. and West, R. and Paganelli, F. and Lopes, R. M. and Kirk, R. L. and Elachi, C. and Wall, S. D. and Johnson, W. T K and Anderson, Y. and Boehmer, R. A. and Callahan, P. and Gim, Y. and Hamilton, G. A. and Kelleher, K. D. and Roth, L. and Stiles, B. and Le Gall, A.},
    number = {1},
    pages = {222--239},
    volume = {200},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2008.10.017},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2008.10.017},
    issn = {00191035},
    keywords = {Instrumentation, Radio observations, Satellites, Titan, composition, surfaces}
}

@article{Aharonson2014,
    title = {{Titan's surface geology}},
    year = {2014},
    journal = {Titan: Interior, Surface, Atmosphere, and Space Environment},
    author = {Aharonson, O and Hayes, A G and Hayne, P O and Lopes, R M and Lucas, A and Perron, J T},
    pages = {63--101},
    doi = {10.1017/CBO9780511667398}
}

@article{Coustenis2016,
    title = {{Titan's temporal evolution in stratospheric trace gases near the poles}},
    year = {2016},
    journal = {Icarus},
    author = {Coustenis, Athena and Jennings, Donald E. and Achterberg, Richard K. and Bampasidis, Georgios and Lavvas, Panayiotis and Nixon, Conor A. and Teanby, Nicholas A. and Anderson, Carrie M. and Cottini, Valeria and Flasar, F. Michael},
    pages = {409--420},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.08.027},
    doi = {10.1016/j.icarus.2015.08.027},
    issn = {10902643},
    keywords = {Atmospheres, composition, Atmospheres, evolution, Atmospheres, structure, Satellites, composition, Titan, atmosphere}
}

@article{Corlies2017,
    title = {{Titan's topography and shape at the end of the Cassini mission}},
    year = {2017},
    journal = {Geophysical Research Letters},
    author = {Corlies, P. and Hayes, A. G. and Birch, S. P. D. and Lorenz, R. and Stiles, B. W. and Kirk, R. and Poggiali, V. and Zebker, H. and Iess, L.},
    pages = {754--761},
    url = {http://doi.wiley.com/10.1002/2017GL075518},
    doi = {10.1002/2017GL075518},
    issn = {00948276}
}

@article{Strobel1992,
    title = {{Titan's upper atmosphere: Structure and ultraviolet emissions}},
    year = {1992},
    journal = {Icarus},
    author = {Strobel, Darrell F. and Summers, Michael E. and Zhu, Xun},
    number = {2},
    pages = {512--526},
    volume = {100},
    doi = {10.1016/0019-1035(92)90114-M},
    issn = {10902643}
}

@article{Ip1990a,
    title = {{Titan's upper ionosphere}},
    year = {1990},
    journal = {The Astrophysical journal},
    author = {Ip, W. H.},
    pages = {354--363}
}

@article{Lavvas2010,
    title = {{Titan's vertical aerosol structure at the Huygens landing site: Constraints on particle size, density, charge, and refractive index}},
    year = {2010},
    journal = {Icarus},
    author = {Lavvas, P. and Yelle, R. V. and Griffith, C. A.},
    number = {2},
    pages = {832--842},
    volume = {210},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2010.07.025},
    doi = {10.1016/j.icarus.2010.07.025},
    issn = {00191035},
    keywords = {Atmospheres, Titan}
}

@article{Lorenz2001,
    title = {{Titan, Mars and Earth: Entropy production by latitudinal heat transport}},
    year = {2001},
    journal = {Geophysical Research Letters},
    author = {Lorenz, R. D. and Lunine, J. I. and Withers, P.},
    number = {16},
    pages = {3169},
    volume = {28},
    isbn = {0094-8276},
    doi = {10.1029/2001GL013455},
    issn = {00948276}
}

@article{Cuk2013,
    title = {{Titan-Hyperion Resonance and the Tidal Q of Saturn}},
    year = {2013},
    journal = {arXiv:1311.6780},
    author = {{\'{C}}uk, M and Dones, L and Nesvorn{\'{y}}, D},
    url = {http://arxiv.org/abs/1311.6780},
    arxivId = {1311.6780}
}

@article{Kuiper1944,
    title = {{Titan: a Satellite with an Atmosphere}},
    year = {1944},
    journal = {Astrophys. J.},
    author = {Kuiper, G P},
    pages = {378--383},
    volume = {100},
    isbn = {0004-637X},
    doi = {10.1086/144679},
    issn = {0004-637X},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3}
}

@article{Moore2011,
    title = {{Titan: An exogenic world?}},
    year = {2011},
    journal = {Icarus},
    author = {Moore, Jeffrey M. and Pappalardo, Robert T.},
    number = {2},
    pages = {790--806},
    volume = {212},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2011.01.019},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2011.01.019},
    issn = {00191035},
    keywords = {Saturn, satellites, Titan, Titan, atmosphere, Titan, hydrology, Titan, surface}
}

@article{ReidThompson1984,
    title = {{Titan: Far-infrared and microwave remote sensing of methane clouds and organic haze}},
    year = {1984},
    journal = {Icarus},
    author = {Thompson, W. R. and Sagan, Carl},
    number = {2},
    month = {11},
    pages = {236--259},
    volume = {60},
    url = {http://www.sciencedirect.com/science/article/pii/0019103584901878},
    doi = {10.1016/0019-1035(84)90187-8},
    issn = {00191035}
}

@book{Environment,
    title = {{Titan: Interior, Surface, Atmosphere, and Space Enviroment}},
    author = {Environment, Space and Union, Geophysical and Spectrometer, Neutral Mass},
    isbn = {9780521035453}
}

@article{Muller-Wodarg2014,
    title = {{Titan: Interior, Surface, Atmosphere, and Space Environment}},
    year = {2014},
    author = {{Muller-Wodarg} and Griffith, C. A. and Lellouch, E. and Cravens, T.E.},
    pages = {1--287},
    isbn = {9780521035453}
}

@article{Trafton1974,
    title = {{Titan: Unidentified strong absorptions in the photometric infrared}},
    year = {1974},
    journal = {Icarus},
    author = {Trafton, L.},
    number = {2},
    pages = {175--187},
    volume = {21},
    doi = {10.1016/0019-1035(74)90134-1},
    issn = {10902643}
}

@article{Maltagliati,
    title = {{Titan’s atmosphere as observed by Cassini / VIMS solar occultations : CH 4 , CO and evidence for C 2 H 6 absorption}},
    author = {Maltagliati, Luca and B{\'{e}}zard, Bruno and Vinatier, Sandrine and Hedman, Matthew M and Paris, Lesia-observatoire De and Janssen, Jules}
}

@article{Sciamma-OBrien2010,
    title = {{Titan’s atmosphere: An optimal gas mixture for aerosol production?}},
    year = {2010},
    journal = {Icarus},
    author = {Sciamma-O’Brien, E. and Carrasco, N. and Szopa, C. and Buch, A. and Cernogora, G.},
    number = {2},
    month = {10},
    pages = {704--714},
    volume = {209},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103510001570},
    doi = {10.1016/j.icarus.2010.04.009},
    issn = {00191035},
    keywords = {Atmospheres, Chemistry, Experimental techniques, Satellites, Atmospheres, Saturn, Satellites, Titan}
}

@article{Lavvas2014,
    title = {{Titan’s emission processes during eclipse}},
    year = {2014},
    journal = {Icarus},
    author = {Lavvas, P. and West, R.A. and Gronoff, G. and Rannou, P.},
    month = {10},
    pages = {397--408},
    volume = {241},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103514003637},
    doi = {10.1016/j.icarus.2014.07.008},
    issn = {00191035},
    keywords = {Aurorae, Eclipses, Titan}
}

@article{Rannou2016,
    title = {{Titan’s surface spectra at the Huygens landing site and Shangri-La}},
    year = {2016},
    journal = {Icarus},
    author = {Rannou, P. and Toledo, D. and Lavvas, P. and D’Aversa, E. and Moriconi, M.L. and Adriani, A. and Le Mou{\'{e}}lic, S. and Sotin, C. and Brown, R.},
    month = {5},
    pages = {291--306},
    volume = {270},
    url = {http://www.sciencedirect.com/science/article/pii/S0019103515004212},
    doi = {10.1016/j.icarus.2015.09.016},
    issn = {00191035},
    keywords = {Photometry, Titan, surface}
}

@article{Westlake2011,
    title = {{Titan’s thermospheric response to various plasma environments}},
    year = {2011},
    author = {Westlake, J H and Bell, J M and Jr, J H Waite and Johnson, R E and Luhmann, J G and Mandt, K E and Magee, B A and Rymer, A M},
    number = {December 2010},
    pages = {1--12},
    volume = {116},
    doi = {10.1029/2010JA016251},
    keywords = {doi:10.102, http://dx.doi.org/10.1029/2010JA016251}
}

@article{Hayes2017,
    title = {{Topographic Constraints on the Evolution and Connectivity of Titan's Lacustrine Basins}},
    year = {2017},
    journal = {Geophysical Research Letters},
    author = {Hayes, A. G. and Birch, S. P. D. and Dietrich, W. E. and Howard, A. D. and Kirk, R. L. and Poggiali, V. and Mastrogiuseppe, M. and Michaelides, R. J. and Corlies, P. M. and Moore, J. M. and Malaska, M. J. and Mitchell, K. L. and Lorenz, R. D. and Wood, C. A.},
    pages = {745--753},
    url = {http://doi.wiley.com/10.1002/2017GL075468},
    doi = {10.1002/2017GL075468},
    issn = {00948276}
}

@article{Johnson2006,
    title = {{Toroidal Atmospheres around Extrasolar Planets}},
    year = {2006},
    journal = {The Publications of the Astronomical Society of the Pacific},
    author = {Johnson, R E and Huggins, P J},
    pages = {1136},
    volume = {118},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-data_query?bibcode=2006PASP..118.1136J&link_type=ABSTRACT%5Cnpapers://0be24a46-325a-4116-a3c6-fd8a3b614472/Paper/p10272},
    doi = {10.1086/506183},
    issn = {0004-6280},
    keywords = {Planets and Satellites: General, Stars: Planetary Systems}
}

@article{Fortenberrya,
    title = {{Toward the Laboratory Identification of the Not-So-Simple NS 2 Neutral and Anion Isomers}},
    author = {Fortenberry, Ryan C and Thackston, Russell and Francisco, Joseph S and Lee, J},
    pages = {1--4}
}

@article{Fortenberry2017,
    title = {{Toward the laboratory identification of the not-so-simple NS2 neutral and anion isomers}},
    year = {2017},
    journal = {The Journal of Chemical Physics},
    author = {Fortenberry, R. C. and Thackston, Russell and Francisco, Joseph S and Lee, T.},
    doi = {10.1063/1.4948235}
}

@article{Carrasco2008a,
    title = {{Towards a reduction of the bimolecular reaction model for Titan ionosphere}},
    year = {2008},
    journal = {International Journal of Chemical Kinetics},
    author = {Carrasco, N. and Plessis, S. and Pernot, P.},
    number = {11},
    pages = {699--709},
    volume = {40},
    url = {http://dx.doi.org/10.1002/kin.20374},
    doi = {10.1002/kin}
}

@article{Walter2005,
    title = {{Towards linearization of atmospheric radiative transfer in spherical geometry}},
    year = {2005},
    journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
    author = {Walter, Holger H. and Landgraf, Jochen},
    number = {2},
    pages = {175--200},
    volume = {95},
    doi = {10.1016/j.jqsrt.2004.08.043},
    issn = {00224073},
    keywords = {Adjoint formulation, Linearization, Perturbation theory, Radiative transfer, Spherical geometry}
}

@article{Nimmo2018,
    title = {{Transforming Dust to Planets}},
    year = {2018},
    journal = {Space Science Reviews},
    author = {Nimmo, Francis and Kretke, Katherine and Ida, Shigeru and Matsumura, Soko and Kleine, Thorsten},
    number = {5},
    pages = {101},
    volume = {214},
    publisher = {Springer Nature B.V.},
    url = {http://link.springer.com/10.1007/s11214-018-0533-2},
    isbn = {1121401805},
    doi = {10.1007/s11214-018-0533-2},
    issn = {0038-6308},
    keywords = {accretion, carlson, edited by stephen j, isotope cosmochemistry, mojzsis, moon, orbital migration, planetary interiors, ramon brasser and richard, s evolution before the, the solar system, w}
}

@article{Zahnle2014,
    title = {{Transient climate effects of large impacts on Titan}},
    year = {2014},
    journal = {Icarus},
    author = {Zahnle, Kevin J. and Korycansky, Donald G. and Nixon, Conor A.},
    pages = {378--391},
    volume = {229},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.11.006},
    doi = {10.1016/j.icarus.2013.11.006},
    issn = {00191035},
    keywords = {Impact processes, Titan, Titan, atmosphere, Titan, hydrology}
}

@article{Wattieaux2015,
    title = {{Transient phenomena during dust formation in a N <sub>2</sub> –CH <sub>4</sub> capacitively coupled plasma}},
    year = {2015},
    journal = {Plasma Sources Science and Technology},
    author = {Wattieaux, G and Carrasco, N and Henault, M and Boufendi, L and Cernogora, G},
    number = {1},
    pages = {015028},
    volume = {24},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0963-0252/24/i=1/a=015028?key=crossref.c0350fef26eea5c69b4714e0fbc95b20},
    doi = {10.1088/0963-0252/24/1/015028},
    issn = {0963-0252}
}

@article{Carr2013,
    title = {{Transient Water Vapor at Europa's South Pole}},
    year = {2013},
    journal = {Science},
    author = {Carr, M H and Belton, M J and Chapman, C R and Davies, M E and Geissler, P and Greenberg, R and McEwen, a S and Tufts, B R and Greeley, R and Sullivan, R and Head, J W and Pappalardo, R T and Klaasen, K P and Johnson, T V and Kaufman, J and Senske, D and Moore, J and Neukum, G and Schubert, G and Burns, J a and Thomas, P and Veverka, J},
    number = {December},
    pages = {363--365},
    volume = {391},
    isbn = {0028-0836 (Print)},
    doi = {10.1038/34857},
    issn = {0028-0836},
    pmid = {9450749}
}

@article{Poppenhaeger2013,
    title = {{Transit observations of the Hot Jupiter HD 189733b at X-ray wavelengths}},
    year = {2013},
    journal = {arXiv preprint arXiv:1306.2311},
    author = {Poppenhaeger, K and Schmitt, J. H. M. M. and Wolk, S. J.},
    number = {September 2011},
    pages = {15},
    volume = {016},
    url = {http://arxiv.org/abs/1306.2311},
    doi = {10.1088/0004-637X/773/1/62},
    issn = {0004-637X},
    arxivId = {1306.2311},
    keywords = {activity, binaries, color figures, coronae, general, hd 189733, individual, online-only material, planetary systems, stars, supplemental data, x-rays}
}

@article{Ben-Jaffel2014,
    title = {{Transit of Exomoon Plasma Tori: New Diagnosis}},
    year = {2014},
    journal = {The Astrophysical Journal},
    author = {Ben-Jaffel, Lotfi and Ballester, Gilda E.},
    number = {2},
    pages = {L30},
    volume = {785},
    url = {http://stacks.iop.org/2041-8205/785/i=2/a=L30?key=crossref.a63a0a469566af842f079615af59d123},
    doi = {10.1088/2041-8205/785/2/L30},
    issn = {2041-8205},
    arxivId = {arXiv:1404.1084v1},
    keywords = {atmospheres, be, been rarely cited, color figures, composition, detection, online-only material, opacity, planetary systems, planets and satellites, plasma torus that may, plasmas, the occurrence of a, ultraviolet}
}

@article{Kostogryz2014,
    title = {{Transit polarimetry of exoplanetary system HD189733}},
    year = {2014},
    author = {Kostogryz, N. M. and Berdyugina, S. V. and Yakobchuk, T. M},
    number = {June},
    pages = {5},
    volume = {189733},
    url = {http://arxiv.org/abs/1408.5023},
    arxivId = {1408.5023}
}

@article{Sing2008,
    title = {{Transit spectrophotometry of the exoplanet HD189733b. I. Searching for water but finding haze with HST NICMOS}},
    year = {2008},
    journal = {arXiv.org},
    author = {Sing, David K and Desert, J M and des Etangs, A Lecavelier and Ballester, G E and Vidal-Madjar, A and Parmentier, V and Hebrard, G and Henry, G W},
    pages = {2008},
    volume = {astro-ph.E},
    url = {http://arxiv.org/abs/0907.4991v1%5Cnpapers3://publication/uuid/2E560D9E-CF3E-44A1-B205-25C2C919A5F8},
    doi = {10.1051/0004-6361/200912776},
    issn = {0004-6361},
    arxivId = {0907.4991},
    keywords = {binaries, eclipsing, hd 189733, individual, photometric, planetary systems, stars, techniques}
}

@article{Lebonnois2002,
    title = {{Transition from Gaseous Compounds to Aerosols in Titan's Atmosphere}},
    year = {2002},
    journal = {Icarus},
    author = {Lebonnois, Sébastien and Bakes, E L O and Mckay, Christopher P},
    pages = {505--517},
    volume = {159},
    isbn = {0019-1035},
    doi = {10.1006/icar.2002.6943},
    issn = {00191035},
    keywords = {Titan, atmosp-heric, composition, organic chemistry, photochemistry}
}

@article{McKinnon2007,
    title = {{Triton}},
    year = {2007},
    journal = {Encyclopedia of the Solar System},
    author = {McKinnon, W and Kirk, R},
    pages = {483--502},
    url = {http://dx.doi.org/10.1016/B978-012088589-3/50030-X%5Cnhttp://www.sciencedirect.com/science/article/pii/B9780120885893500001%5Cnhttp://linkinghub.elsevier.com/retrieve/pii/B978012088589350030X},
    doi = {10.1016/B978-012088589-3/50030-X}
}

@article{Cheng1990,
    title = {{Triton Torus and Neptune Aurora}},
    year = {1990},
    author = {Cheng, Andrew F},
    number = {September},
    pages = {1669--1672}
}

@article{Rufu2017,
    title = {{Triton's Evolution with a Primordial Neptunian Satellite System}},
    year = {2017},
    journal = {The Astronomical Journal},
    author = {Rufu, Raluca and Canup, Robin M.},
    number = {5},
    pages = {208},
    volume = {154},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/1538-3881/154/i=5/a=208?key=crossref.a47e49165884dfddb01d150c8c757f1c},
    doi = {10.3847/1538-3881/aa9184},
    issn = {1538-3881},
    arxivId = {1711.01581},
    keywords = {dynamical evolution and stability, methods, numerical, planets and satellites, planets and satellites: dynamical evolution and st}
}

@article{Hurford2017,
    title = {{Triton's Fractures As Evidence for a Subsurface Ocean}},
    year = {2017},
    author = {Hurford, T A and Henning, W G and Spitale, J N and Rhoden, A R and Kattenhorn, S A and Hamilton, D P and Hansen, C J and Kirk, R L and Quick, L C and Bleacher, J},
    number = {November},
    url = {http://www.hou.usra.edu/meetings/lpsc2017/pdf/2376.pdf}
}

@article{Merlin2018,
    title = {{Triton’s surface ices : Distribution , temperature and mixing state from VLT /}},
    year = {2018},
    journal = {Icarus},
    author = {Merlin, F and Lellouch, E and Quirico, E and Schmitt, B},
    number = {February},
    pages = {274--293},
    volume = {314},
    publisher = {Elsevier},
    url = {https://doi.org/10.1016/j.icarus.2018.06.003},
    doi = {10.1016/j.icarus.2018.06.003},
    issn = {0019-1035},
    keywords = {IR spectroscopy, Ices, Radiative transfer, Satellite{\_} surface and composition, Triton}
}

@article{Rodriguez2016,
    title = {{Tsunami Waves Extensively Resurfaced the Shorelines of an Early Martian Ocean}},
    year = {2016},
    journal = {47th Lunar and Planetary Science Conference},
    author = {Rodriguez, J.A.P. and Fair{\'{e}}n, A.G. and Linares, R. and Zarroca, M. and Platz, T. and Komatsu, G. and Kargel, J. S. and Gulick, V. and Jianguo, Y. and Higuchi, K. and Miyamoto, H. and Baker, V.R. and Glines, N.},
    number = {April},
    pages = {47--48},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/srep25106},
    doi = {10.1038/srep25106}
}

@article{F.1926,
    title = {{{\"{U}}ber Diacetylen}},
    year = {1926},
    author = {F., Straus and L., Kollek},
    pages = {1664--1681}
}

@article{Herzberg1957,
    title = {{ULTRAVIOLET ABSORPTION SPECTRA OF HCN AND DCN 1. The Alpha-X and Beta-X Systems}},
    year = {1957},
    journal = {Canadian Journal of Physics},
    author = {Herzberb, G. and Innes, K. K.}
}

@article{Frost1996,
    title = {{Ultraviolet photochemistry of diacetylene: The metastable C4H2* reaction with ethene, propene, and propyne}},
    year = {1996},
    journal = {Journal of the American Chemical Society},
    author = {Frost, Rex K. and Arlington, Caleb A. and Ramos, Christopher and Zwier, Timothy S.},
    number = {18},
    pages = {4451--4461},
    volume = {118},
    doi = {10.1021/ja953757c},
    issn = {00027863}
}

@article{Gerakines2004,
    title = {{Ultraviolet photolysis and proton irradiation of astrophysical ice analogs containing hydrogen cyanide}},
    year = {2004},
    journal = {Icarus},
    author = {Gerakines, P. A. and Moore, M. H. and Hudson, R. L.},
    number = {1},
    pages = {202--213},
    volume = {170},
    doi = {10.1016/j.icarus.2004.02.005},
    issn = {00191035},
    keywords = {Comers, composition, Lees, Photochemistry, Radiation chemistry, Spectroscopy}
}

@article{Carrasco2007a,
    title = {{Uncertainty analysis of bimolecular reactions in Titan ionosphere chemistry model}},
    year = {2007},
    journal = {Planetary and Space Science},
    author = {Carrasco, N. and Dutuit, O. and Thissen, R. and Banaszkiewicz, M. and Pernot, P.},
    number = {1-2},
    pages = {141--157},
    volume = {55},
    isbn = {00320633 (ISSN)},
    doi = {10.1016/j.pss.2006.06.004},
    issn = {00320633},
    keywords = {Branching ratio, Chemical rate constant, Elicitation, Ionospheric chemistry, Mass spectrum, Monte Carlo uncertainty propagation, Titan}
}

@article{Kliore2011,
    title = {{Unusual electron density profiles observed by Cassini radio occultations in Titan ’ s ionosphere : Effects of enhanced magnetospheric electron precipitation ?}},
    year = {2011},
    author = {Kliore, A J and Nagy, A F and Cravens, T E and Richard, M S and Rymer, A M},
    pages = {1--7},
    volume = {116},
    doi = {10.1029/2011JA016694},
    keywords = {http://dx.doi.org/10.1029/2011JA016694, doi:10.102}
}

@misc{Strobel1993,
    title = {{Upper Limit on Titan's Atmospheric Argon Abundance}},
    year = {1993},
    author = {Strobel, D. F. and Hall, D. T. and Zhu, X. and Summers, M. E.}
}

@article{Nixon2013,
    title = {{Upper limits for PH3 and H2S in Titan's atmosphere from Cassini CIRS}},
    year = {2013},
    journal = {Icarus},
    author = {Nixon, Conor A. and Teanby, Nicholas A. and Irwin, Patrick G J and H{\"{o}}rst, Sarah M.},
    number = {1},
    pages = {253--256},
    volume = {224},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2013.02.024},
    doi = {10.1016/j.icarus.2013.02.024},
    issn = {00191035},
    keywords = {Abundances, Atmospheres, Atmospheres, Composition, Saturn, Satellites, Titan}
}

@article{Nixon2010,
    title = {{Upper limits for undetected trace species in the stratosphere of Titan}},
    year = {2010},
    journal = {Jet Propulsion},
    author = {Nixon, Conor A and Achterberg, R. K. and Teanby, Nicholas A and Irwin, Patrick G J and Flaud, Jean-marie and Kleiner, Isabelle and Dehayem-kamadjeu, Alix and Brown, De Linda R and Sams, Robert L and Mamoutkine, Andrei and Vinatier, Sandrine and Bjoraker, Gordon L and Jennings, Donald E and Romani, N and Flasar, F Michael},
    pages = {1--17},
    isbn = {10.1039/C003771K},
    doi = {10.1039/c003771k},
    issn = {1359-6640},
    pmid = {21302543}
}

@article{Frankland2016,
    title = {{Uptake of acetylene on cosmic dust and production of benzene in Titan's atmosphere}},
    year = {2016},
    journal = {Icarus},
    author = {Frankland, Victoria L. and James, Alexander D. and S{\'{a}}nchez, Juan Diego Carrillo and Mangan, Thomas P. and Willacy, Karen and Poppe, Andrew R. and Plane, John M.C.},
    pages = {88--99},
    volume = {278},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2016.06.007},
    doi = {10.1016/j.icarus.2016.06.007},
    issn = {10902643},
    keywords = {Interplanetary dust, Kuiper belt, Titan, atmosphere}
}

@article{Khurana2002,
    title = {{Using Surface Observatories}},
    year = {2002},
    journal = {Astrobiology},
    author = {Khurana, Krishan K and Kivelson, Margaret G and Russell, Christopher T},
    number = {1},
    pages = {93--103},
    volume = {2}
}

@article{Bonfond2008,
    title = {{UV Io footprint leading spot: A key feature for understanding the UV Io footprint multiplicity?}},
    year = {2008},
    journal = {Geophysical Research Letters},
    author = {Bonfond, B. and Grodent, D. and G{\'{e}}rard, J. C. and Radioti, A. and Saur, J. and Jacobsen, S.},
    number = {5},
    pages = {1--5},
    volume = {35},
    isbn = {1944-8007},
    doi = {10.1029/2007GL032418},
    issn = {00948276}
}

@article{Couturier-Tamburelli2018,
    title = {{UV–Vis Light-induced Aging of Titan’s Haze and Ice}},
    year = {2018},
    journal = {The Astrophysical Journal},
    author = {Couturier-Tamburelli, I. and Pi{\'{e}}tri, Nathalie and Letty, Vincent Le and Chiavassa, Thierry and Gudipati, Murthy},
    number = {2},
    pages = {117},
    volume = {852},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/852/i=2/a=117?key=crossref.abe561613a5ab2e74417801d20fd9c92},
    doi = {10.3847/1538-4357/aa9e8d},
    issn = {1538-4357},
    keywords = {astrochemistry, atmospheres, laboratory, methods, methods: la, planetary system, planets and satellites, refractory, solid state, solid state: refractory, spectroscopic, techniques, ultraviolet}
}

@article{Carruth1973,
    title = {{Vapor Pressure of Normal Paraffins Ethane Through n-Decane from Their Triple Points to About 10Mm Hg}},
    year = {1973},
    journal = {Journal of Chemical and Engineering},
    author = {Carruth, G. and Kobayashi, R},
    number = {2},
    pages = {115--126},
    volume = {18},
    url = {http://pubs.acs.org/doi/abs/10.1021/je60057a009},
    doi = {10.1021/je60057a009},
    issn = {0021-9568}
}

@article{Ambrose1964,
    title = {{Vapour Pressure of Acetylene}},
    year = {1964},
    journal = {Faraday Society},
    author = {Ambrose, D and Townsend, R},
    pages = {603}
}

@article{Cauley2016,
    title = {{Variation in the Pre-Transit Balmer Line Signal Around the Hot Jupiter Hd 189733B}},
    year = {2016},
    journal = {The Astronomical Journal},
    author = {Cauley, P. Wilson and Redfield, Seth and Jensen, Adam G. and Barman, Travis},
    number = {1},
    pages = {20},
    volume = {152},
    url = {http://stacks.iop.org/1538-3881/152/i=1/a=20?key=crossref.e5d37a31769e619e917d270c1d029f6a},
    doi = {10.3847/0004-6256/152/1/20},
    issn = {1538-3881},
    keywords = {activity, atmospheres, gaseous planets, magnetic fi elds, planets and satellites, stars}
}

@article{Vinatier2007,
    title = {{Vertical abundance profiles of hydrocarbons in Titan's atmosphere at 15{\textordmasculine} S and 80{\textordmasculine} N retrieved from Cassini/CIRS spectra}},
    year = {2007},
    journal = {Icarus},
    author = {Vinatier, Sandrine and B{\'{e}}zard, Bruno and Fouchet, Thierry and Teanby, Nick A. and de Kok, Remco and Irwin, Patrick G J and Conrath, Barney J. and Nixon, Conor A. and Romani, Paul N. and Flasar, F. Michael and Coustenis, Athena},
    number = {1},
    pages = {120--138},
    volume = {188},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2006.10.031},
    issn = {00191035},
    keywords = {Abundances, Infrared observations, Titan, atmosphere}
}

@article{Lara1996,
    title = {{Vertical distribution of Titan's atmospheric neutral constituents}},
    year = {1996},
    journal = {Journal of Geophysical Research},
    author = {Lara, L. M. and Lellouch, E. and L{\'{o}}pez-Moreno, J. J. and Rodrigo, R.},
    number = {E10},
    pages = {23261},
    volume = {101},
    url = {http://adsabs.harvard.edu/abs/1996JGR...10123261L},
    doi = {10.1029/96JE02036},
    issn = {0148-0227},
    keywords = {Oceanography: Biological and Chemical: Photochemis}
}

@article{Teanby2007,
    title = {{Vertical profiles of HCN, HC3N, and C2H2 in Titan's atmosphere derived from Cassini/CIRS data}},
    year = {2007},
    journal = {Icarus},
    author = {Teanby, N. A. and Irwin, P. G J and de Kok, R. and Vinatier, S. and B{\'{e}}zard, B. and Nixon, C. A. and Flasar, F. M. and Calcutt, S. B. and Bowles, N. E. and Fletcher, L. and Howett, C. and Taylor, F. W.},
    number = {2},
    pages = {364--384},
    volume = {186},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2006.09.024},
    issn = {00191035},
    keywords = {Atmospheres, Titan, composition}
}

@article{Doose2016,
    title = {{Vertical structure and optical properties of Titan's aerosols from radiance measurements made inside and outside the atmosphere}},
    year = {2016},
    journal = {Icarus},
    author = {Doose, Lyn R. and Karkoschka, Erich and Tomasko, Martin G. and Anderson, Carrie M.},
    pages = {355--375},
    volume = {270},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2015.09.039},
    doi = {10.1016/j.icarus.2015.09.039},
    issn = {10902643},
    keywords = {Atmospheres, Radiative transfer, Titan, atmosphere, structure}
}

@article{Roy2010,
    title = {{Very high resolution mass spectrometry of HCN polymers and tholins}},
    year = {2010},
    author = {Roy, Le and Fray, Nicolas and Brien, Ella Sciamma-o and Carrasco, Nathalie and Szopa, Cyril},
    pages = {495--508},
    doi = {10.1039/c003758c}
}

@article{Bak1975,
    title = {{Vibrational Spectra of Aminoacetonitrile}},
    year = {1975},
    journal = {Canadian Journal of Physics},
    author = {Bak, B. and Hansen, E. L. and Nicolaisen, F. M. and Nielsen, O. F.},
    number = {Table 1},
    pages = {2183},
    volume = {53}
}

@article{Esposti2005,
    title = {{Vibrationally excited states of HC5N: Millimeter-wave spectroscopy and coupled cluster calculations}},
    year = {2005},
    journal = {Journal of Molecular Spectroscopy},
    author = {Degli Esposti, C. and Bizzocchi, L. and Botschwina, P. and Yamada, K. M.T. and Winnewisser, G. and Thorwirth, S. and F{\"{o}}rster, P.},
    number = {2},
    pages = {185--195},
    volume = {230},
    doi = {10.1016/j.jms.2004.11.010},
    issn = {00222852},
    keywords = {CCSD(T) calculations, HC5N, Resonances, Rotational spectroscopy, Vibrationally excited states}
}

@article{Asphaug2016a,
    title = {{Viscoelastic modeling of tidal stresses on satellites with an enhanced SatStressGUI}},
    year = {2016},
    author = {Patthoff, D. A. and Pappalardo, Robert T. and Li, J. B. and Ayton, B. J. and Dubois, D. and Kay, J. P. and Kattenhorn, Simon A.},
    pages = {9--10},
    isbn = {1189985144},
    doi = {10.1016/j.icarus.2007.12.027.}
}

@article{Dobos2015,
    title = {{Viscoelastic Models of Tidally Heated Exomoons}},
    year = {2015},
    journal = {ApJ},
    author = {Dobos, Vera and Turner, Edwin L.},
    number = {1},
    pages = {41},
    volume = {804},
    url = {http://adsabs.harvard.edu/abs/2015arXiv150207090D%5Cnhttp://stacks.iop.org/0004-637X/804/i=1/a=41?key=crossref.e52345e0686400d93c558b93d0b0a087},
    doi = {10.1088/0004-637X/804/1/41},
    issn = {1538-4357},
    arxivId = {1502.07090},
    keywords = {Astrophysics - Earth and Planetary Astrophysics}
}

@article{Trifonov2011,
    title = {{Vocabulary of Definitions of Life Suggests a Definition}},
    year = {2011},
    journal = {Journal of Biomolecular Structure and Dynamics},
    author = {Trifonov, Edward N.},
    number = {2},
    pages = {259--266},
    volume = {29},
    url = {http://www.tandfonline.com/doi/abs/10.1080/073911011010524992},
    isbn = {1538-0254 (Electronic){\textbackslash}r0739-1102 (Linking)},
    doi = {10.1080/073911011010524992},
    issn = {0739-1102},
    pmid = {21875147},
    keywords = {consensus, definientia, evolution, origin of life, self-reproduction, variations}
}

@article{Johnson2015,
    title = {{Volatile Loss and Classification of Kuiper Belt Objects}},
    year = {2015},
    journal = {The Astrophysical Journal},
    author = {Johnson, R. E. and Oza, A. and Young, L. A. and Volkov, A. N. and Schmidt, C.},
    number = {1},
    pages = {43},
    volume = {809},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/0004-637X/809/i=1/a=43?key=crossref.2df71f738c24327b39a770fb752e1d04},
    doi = {10.1088/0004-637X/809/1/43},
    issn = {1538-4357},
    keywords = {Kuiper belt objects: individual, atmospheres, individual, kuiper belt objects, planets and satellites, planets and satellites: atmospheres}
}

@article{Lunine1992,
    title = {{VOLATILE PROCESSES IN TRITON’S ATMOSPHERE AND SURFACE A Simple , Constant Albedo Model of Global Nitrogen Transport}},
    year = {1992},
    author = {Lunine, J I},
    number = {11},
    volume = {12}
}

@article{Carrasco2012,
    title = {{Volatile products controlling Titan's tholins production}},
    year = {2012},
    journal = {Icarus},
    author = {Carrasco, N. and Gautier, Thomas and Es-sebbar, Et touhami and Pernot, Pascal and Cernogora, Guy},
    number = {1},
    pages = {230--240},
    volume = {219},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.02.034},
    isbn = {0019-1035},
    doi = {10.1016/j.icarus.2012.02.034},
    issn = {00191035},
    keywords = {Astrobiology, Atmospheres, Chemistry, Ionospheres, Titan}
}

@misc{CookII1982,
    title = {{Volcanism in Ice on Europa}},
    year = {1982},
    author = {Cook II, A. F.}
}

@article{Tyler1989,
    title = {{Voyager Radio Science Observations of Neptune and Triton}},
    year = {1989},
    author = {Tyler, G Leonard and Sweetnam, D. N. and Anderson, J. D. and Borutzki, S. E. and Campbell, J. K. and Eshleman, V. R. and Gresh, D. L. and Gurrola, E. M. and Hinson, D. P. and Kawashima, N. and Kursinski, E. R. and Levy, G. S. and Lindal, G. F. and Lyons, J. R. and Marouf, E. A. and Rosen, P. A. and Simpson, R. A. and Wood, G. E.},
    number = {5287},
    pages = {1187--1191},
    volume = {274}
}

@article{Carrasco2013,
    title = {{VUV photochemistry simulation of planetary upper atmosphere using synchrotron radiation}},
    year = {2013},
    journal = {Journal of Synchrotron Radiation},
    author = {Carrasco, N. and Giuliani, Alexandre and Correia, Jean Jacques and Cernogora, Guy},
    number = {4},
    pages = {587--589},
    volume = {20},
    isbn = {0909049513},
    doi = {10.1107/S0909049513013538},
    issn = {09090495},
    pmid = {23765300},
    keywords = {Titan, VUV photochemistry, atmosphere, planets, reactivity}
}

@article{Pesnell2004,
    title = {{Watching meteors on Triton}},
    year = {2004},
    journal = {Icarus},
    author = {Pesnell, W. Dean and Grebowsky, J. M. and Weisman, Andrew L.},
    number = {2},
    pages = {482--491},
    volume = {169},
    doi = {10.1016/j.icarus.2004.01.011},
    issn = {00191035},
    keywords = {Atmosphere, composition, Ionosphere, Meteoroids}
}

@article{Fleury2015a,
    title = {{Water Formation in the Upper Atmosphere of the Early Earth}},
    year = {2015},
    journal = {The Astrophysical Journal},
    author = {Fleury, Benjamin and Carrasco, Nathalie and Marcq, Emmanuel and Vettier, Ludovic and M{\"{a}}{\"{a}}tt{\"{a}}nen, Anni},
    number = {2},
    pages = {L29},
    volume = {807},
    publisher = {IOP Publishing},
    url = {http://stacks.iop.org/2041-8205/807/i=2/a=L29?key=crossref.28b314bf53635235f7d2ca5fda4505c1},
    doi = {10.1088/2041-8205/807/2/L29},
    issn = {2041-8213},
    keywords = {Earth, astrochemistry, atmospheres, earth, planets and satellites, planets and satellites: atmospheres}
}

@article{Cruikshank2000,
    title = {{Water Ice on Triton}},
    year = {2000},
    journal = {Icarus},
    author = {Cruikshank, D},
    number = {1},
    pages = {309--316},
    volume = {147},
    url = {http://linkinghub.elsevier.com/retrieve/pii/S0019103500964510},
    doi = {10.1006/icar.2000.6451},
    issn = {00191035},
    keywords = {ices, infrared observations, satellite, satellites of neptune, spectroscopy, surfaces, triton}
}

@article{Cottini2012,
    title = {{Water vapor in Titan's stratosphere from Cassini CIRS far-infrared spectra}},
    year = {2012},
    journal = {Icarus},
    author = {Cottini, V. and Nixon, C. A. and Jennings, D. E. and Anderson, C. M. and Gorius, N. and Bjoraker, G. L. and Coustenis, A. and Teanby, N. A. and Achterberg, R. K. and B{\'{e}}zard, B. and de Kok, R. and Lellouch, E. and Irwin, P. G.J. and Flasar, F. M. and Bampasidis, G.},
    number = {2},
    pages = {855--862},
    volume = {220},
    publisher = {Elsevier Inc.},
    url = {http://dx.doi.org/10.1016/j.icarus.2012.06.014},
    doi = {10.1016/j.icarus.2012.06.014},
    issn = {00191035},
    keywords = {Atmospheres, Composition, Satellites, Atmospheres, Spectroscopy, Titan}
}

@article{Swain2009,
    title = {{WATER, METHANE, AND CARBON DIOXIDE PRESENT IN THE DAYSIDE SPECTRUM OF THE EXOPLANET HD 209458b}},
    year = {2009},
    journal = {The Astrophysical Journal},
    author = {Swain, M. R. and Tinetti, G. and Vasisht, G. and Deroo, P. and Griffith, C. and Bouwman, J. and Chen, Pin and Yung, Y. and Burrows, A. and Brown, L. R. and Matthews, J. and Rowe, J. F. and Kuschnig, R. and Angerhausen, D.},
    number = {2},
    pages = {1616--1621},
    volume = {704},
    url = {http://stacks.iop.org/0004-637X/704/i=2/a=1616?key=crossref.dc6d48780b3cef704f2b687aaac22f70},
    doi = {10.1088/0004-637X/704/2/1616},
    issn = {0004-637X},
    keywords = {planetary systems, spectroscopic, techniques}
}

@article{Lecture2007,
    title = {{What Cassini-Huygens has revealed about Titan}},
    year = {2007},
    author = {Lecture, Harold Jeffreys and Society, Royal Astronomical and Coustenis, Athena and Huygens, Cassini-},
    number = {April},
    volume = {48}
}

@article{Pappalardo2011,
    title = {{What we don't know about Europa}},
    year = {2011},
    journal = {LPSC 42},
    author = {Pappalardo, R. T.},
    pages = {1--2}
}

@article{Yu2018,
    title = {{Where does Titan Sand Come From: Insight from Mechanical Properties of Titan Sand Candidates}},
    year = {2018},
    journal = {Journal of Geophysical Research: Planets},
    author = {Yu, Xinting and H{\"{o}}rst, Sarah M and He, Chao and Mcguiggan, Patricia and Crawford, Bryan},
    number = {July},
    url = {https://arxiv.org/pdf/1806.08056.pdf},
    arxivId = {arXiv:1806.08056v1}
}

@article{Hofstadter2013,
    title = {{White Paper for the Planetary Science Decadal Survey the Atmospheres of the Ice Giants, Uranus and Neptune}},
    year = {2013},
    author = {Hofstadter, Mark and Fletcher, Leigh and Irwin, Patrick and Orton, Glenn and Rages, Kathy}
}

@article{Li2012,
    title = {{Why isn't the solar constant a constant?}},
    year = {2012},
    author = {Li, K. J. and Feng, W. and Xu, J. C. and Gao, P. X. and Yang, L. H. and Liang, H. F. and Zhan, L. S.},
    pages = {1--17},
    volume = {2},
    url = {http://arxiv.org/abs/1201.0819 http://dx.doi.org/10.1088/0004-637X/747/2/135},
    doi = {10.1088/0004-637X/747/2/135},
    arxivId = {1201.0819},
    keywords = {activity, general, sun, sunspots}
}
